PHENIX Results on Jet Correlations versus Reaction Plane

In relativistic heavy-ion collisions, studying jet correlations and their dependence on the angle of emission with respect to the reaction plane can be used to shed light on the path length dependence of the energy lost by the jet. In this paper, we present recent PHENIX results on jet correlations versus reaction plane, as a function of centrality and transverse momentum.

==> configure <==
#! /bin/sh
# Guess values for system-dependent variables and create Makefiles.
# Generated by GNU Autoconf 2.61 for WWND2008_Winter 1.0.
#
# Report bugs to <winter@alum.mit.edu>.
#
# Copyright (C) 1992, 1993, 1994, 1995, 1996, 1998, 1999, 2000, 2001,
# 2002, 2003, 2004, 2005, 2006 Free Software Foundation, Inc.
# This configure script is free software; the Free Software Foundation
# gives unlimited permission to copy, distribute and modify it.
## --------------------- ##
## M4sh Initialization.  ##
## --------------------- ##

# Be more Bourne compatible
DUALCASE=1; export DUALCASE # for MKS sh
if test -n "${ZSH_VERSION+set}" && (emulate sh) >/dev/null 2>&1; then
  emulate sh
  NULLCMD=:
  # Zsh 3.x and 4.x performs word splitting on ${1+"$@"}, which
  # is contrary to our usage.  Disable this feature.
  alias -g '${1+"$@"}'='"$@"'
  setopt NO_GLOB_SUBST
else
  case `(set -o) 2>/dev/null` in
  *posix*) set -o posix ;;
esac

fi




# PATH needs CR
# Avoid depending upon Character Ranges.
as_cr_letters='abcdefghijklmnopqrstuvwxyz'
as_cr_LETTERS='ABCDEFGHIJKLMNOPQRSTUVWXYZ'
as_cr_Letters=$as_cr_letters$as_cr_LETTERS
as_cr_digits='0123456789'
as_cr_alnum=$as_cr_Letters$as_cr_digits

# The user is always right.
if test "${PATH_SEPARATOR+set}" != set; then
  echo "#! /bin/sh" >conf$$.sh
  echo  "exit 0"   >>conf$$.sh
  chmod +x conf$$.sh
  if (PATH="/nonexistent;."; conf$$.sh) >/dev/null 2>&1; then
    PATH_SEPARATOR=';'
  else
    PATH_SEPARATOR=:
  fi
  rm -f conf$$.sh
fi

# Support unset when possible.
if ( (MAIL=60; unset MAIL) || exit) >/dev/null 2>&1; then
  as_unset=unset
else
  as_unset=false
fi


# IFS
# We need space, tab and new line, in precisely that order.  Quoting is
# there to prevent editors from complaining about space-tab.
# (If _AS_PATH_WALK were called with IFS unset, it would disable word
# splitting by setting IFS to empty value.)
as_nl='
'
IFS=" ""	$as_nl"

# Find who we are.  Look in the path if we contain no directory separator.
case $0 in
  *[\\/]* ) as_myself=$0 ;;
  *) as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  test -r "$as_dir/$0" && as_myself=$as_dir/$0 && break
done
IFS=$as_save_IFS

     ;;
esac
# We did not find ourselves, most probably we were run as `sh COMMAND'
# in which case we are not to be found in the path.
if test "x$as_myself" = x; then
  as_myself=$0
fi
if test ! -f "$as_myself"; then
  echo "$as_myself: error: cannot find myself; rerun with an absolute file name" >&2
  { (exit 1); exit 1; }
fi

# Work around bugs in pre-3.0 UWIN ksh.
for as_var in ENV MAIL MAILPATH
do ($as_unset $as_var) >/dev/null 2>&1 && $as_unset $as_var
done
PS1='$ '
PS2='> '
PS4='+ '

# NLS nuisances.
for as_var in \
  LANG LANGUAGE LC_ADDRESS LC_ALL LC_COLLATE LC_CTYPE LC_IDENTIFICATION \
  LC_MEASUREMENT LC_MESSAGES LC_MONETARY LC_NAME LC_NUMERIC LC_PAPER \
  LC_TELEPHONE LC_TIME
do
  if (set +x; test -z "`(eval $as_var=C; export $as_var) 2>&1`"); then
    eval $as_var=C; export $as_var
  else
    ($as_unset $as_var) >/dev/null 2>&1 && $as_unset $as_var
  fi
done

# Required to use basename.
if expr a : '\(a\)' >/dev/null 2>&1 &&
   test "X`expr 00001 : '.*\(...\)'`" = X001; then
  as_expr=expr
else
  as_expr=false
fi

if (basename -- /) >/dev/null 2>&1 && test "X`basename -- / 2>&1`" = "X/"; then
  as_basename=basename
else
  as_basename=false
fi


# Name of the executable.
as_me=`$as_basename -- "$0" ||
$as_expr X/"$0" : '.*/\([^/][^/]*\)/*$' \| \
	 X"$0" : 'X\(//\)$' \| \
	 X"$0" : 'X\(/\)' \| . 2>/dev/null ||
echo X/"$0" |
    sed '/^.*\/\([^/][^/]*\)\/*$/{
	    s//\1/
	    q
	  }
	  /^X\/\(\/\/\)$/{
	    s//\1/
	    q
	  }
	  /^X\/\(\/\).*/{
	    s//\1/
	    q
	  }
	  s/.*/./; q'`

# CDPATH.
$as_unset CDPATH


if test "x$CONFIG_SHELL" = x; then
  if (eval ":") 2>/dev/null; then
  as_have_required=yes
else
  as_have_required=no
fi

  if test $as_have_required = yes && 	 (eval ":
(as_func_return () {
  (exit \$1)
}
as_func_success () {
  as_func_return 0
}
as_func_failure () {
  as_func_return 1
}
as_func_ret_success () {
  return 0
}
as_func_ret_failure () {
  return 1
}

exitcode=0
if as_func_success; then
  :
else
  exitcode=1
  echo as_func_success failed.
fi

if as_func_failure; then
  exitcode=1
  echo as_func_failure succeeded.
fi

if as_func_ret_success; then
  :
else
  exitcode=1
  echo as_func_ret_success failed.
fi

if as_func_ret_failure; then
  exitcode=1
  echo as_func_ret_failure succeeded.
fi

if ( set x; as_func_ret_success y && test x = \"\$1\" ); then
  :
else
  exitcode=1
  echo positional parameters were not saved.
fi

test \$exitcode = 0) || { (exit 1); exit 1; }

(
  as_lineno_1=\$LINENO
  as_lineno_2=\$LINENO
  test \"x\$as_lineno_1\" != \"x\$as_lineno_2\" &&
  test \"x\`expr \$as_lineno_1 + 1\`\" = \"x\$as_lineno_2\") || { (exit 1); exit 1; }
") 2> /dev/null; then
  :
else
  as_candidate_shells=
    as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in /bin$PATH_SEPARATOR/usr/bin$PATH_SEPARATOR$PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  case $as_dir in
	 /*)
	   for as_base in sh bash ksh sh5; do
	     as_candidate_shells="$as_candidate_shells $as_dir/$as_base"
	   done;;
       esac
done
IFS=$as_save_IFS


      for as_shell in $as_candidate_shells $SHELL; do
	 # Try only shells that exist, to save several forks.
	 if { test -f "$as_shell" || test -f "$as_shell.exe"; } &&
		{ ("$as_shell") 2> /dev/null <<\_ASEOF
if test -n "${ZSH_VERSION+set}" && (emulate sh) >/dev/null 2>&1; then
  emulate sh
  NULLCMD=:
  # Zsh 3.x and 4.x performs word splitting on ${1+"$@"}, which
  # is contrary to our usage.  Disable this feature.
  alias -g '${1+"$@"}'='"$@"'
  setopt NO_GLOB_SUBST
else
  case `(set -o) 2>/dev/null` in
  *posix*) set -o posix ;;
esac

fi


:
_ASEOF
}; then
  CONFIG_SHELL=$as_shell
	       as_have_required=yes
	       if { "$as_shell" 2> /dev/null <<\_ASEOF
if test -n "${ZSH_VERSION+set}" && (emulate sh) >/dev/null 2>&1; then
  emulate sh
  NULLCMD=:
  # Zsh 3.x and 4.x performs word splitting on ${1+"$@"}, which
  # is contrary to our usage.  Disable this feature.
  alias -g '${1+"$@"}'='"$@"'
  setopt NO_GLOB_SUBST
else
  case `(set -o) 2>/dev/null` in
  *posix*) set -o posix ;;
esac

fi


:
(as_func_return () {
  (exit $1)
}
as_func_success () {
  as_func_return 0
}
as_func_failure () {
  as_func_return 1
}
as_func_ret_success () {
  return 0
}
as_func_ret_failure () {
  return 1
}

exitcode=0
if as_func_success; then
  :
else
  exitcode=1
  echo as_func_success failed.
fi

if as_func_failure; then
  exitcode=1
  echo as_func_failure succeeded.
fi

if as_func_ret_success; then
  :
else
  exitcode=1
  echo as_func_ret_success failed.
fi

if as_func_ret_failure; then
  exitcode=1
  echo as_func_ret_failure succeeded.
fi

if ( set x; as_func_ret_success y && test x = "$1" ); then
  :
else
  exitcode=1
  echo positional parameters were not saved.
fi

test $exitcode = 0) || { (exit 1); exit 1; }

(
  as_lineno_1=$LINENO
  as_lineno_2=$LINENO
  test "x$as_lineno_1" != "x$as_lineno_2" &&
  test "x`expr $as_lineno_1 + 1`" = "x$as_lineno_2") || { (exit 1); exit 1; }

_ASEOF
}; then
  break
fi

fi

      done

      if test "x$CONFIG_SHELL" != x; then
  for as_var in BASH_ENV ENV
        do ($as_unset $as_var) >/dev/null 2>&1 && $as_unset $as_var
        done
        export CONFIG_SHELL
        exec "$CONFIG_SHELL" "$as_myself" ${1+"$@"}
fi


    if test $as_have_required = no; then
  echo This script requires a shell more modern than all the
      echo shells that I found on your system.  Please install a
      echo modern shell, or manually run the script under such a
      echo shell if you do have one.
      { (exit 1); exit 1; }
fi


fi

fi



(eval "as_func_return () {
  (exit \$1)
}
as_func_success () {
  as_func_return 0
}
as_func_failure () {
  as_func_return 1
}
as_func_ret_success () {
  return 0
}
as_func_ret_failure () {
  return 1
}

exitcode=0
if as_func_success; then
  :
else
  exitcode=1
  echo as_func_success failed.
fi

if as_func_failure; then
  exitcode=1
  echo as_func_failure succeeded.
fi

if as_func_ret_success; then
  :
else
  exitcode=1
  echo as_func_ret_success failed.
fi

if as_func_ret_failure; then
  exitcode=1
  echo as_func_ret_failure succeeded.
fi

if ( set x; as_func_ret_success y && test x = \"\$1\" ); then
  :
else
  exitcode=1
  echo positional parameters were not saved.
fi

test \$exitcode = 0") || {
  echo No shell found that supports shell functions.
  echo Please tell autoconf@gnu.org about your system,
  echo including any error possibly output before this
  echo message
}



  as_lineno_1=$LINENO
  as_lineno_2=$LINENO
  test "x$as_lineno_1" != "x$as_lineno_2" &&
  test "x`expr $as_lineno_1 + 1`" = "x$as_lineno_2" || {

  # Create $as_me.lineno as a copy of $as_myself, but with $LINENO
  # uniformly replaced by the line number.  The first 'sed' inserts a
  # line-number line after each line using $LINENO; the second 'sed'
  # does the real work.  The second script uses 'N' to pair each
  # line-number line with the line containing $LINENO, and appends
  # trailing '-' during substitution so that $LINENO is not a special
  # case at line end.
  # (Raja R Harinath suggested sed '=', and Paul Eggert wrote the
  # scripts with optimization help from Paolo Bonzini.  Blame Lee
  # E. McMahon (1931-1989) for sed's syntax.  :-)
  sed -n '
    p
    /[$]LINENO/=
  ' <$as_myself |
    sed '
      s/[$]LINENO.*/&-/
      t lineno
      b
      :lineno
      N
      :loop
      s/[$]LINENO\([^'$as_cr_alnum'_].*\n\)\(.*\)/\2\1\2/
      t loop
      s/-\n.*//
    ' >$as_me.lineno &&
  chmod +x "$as_me.lineno" ||
    { echo "$as_me: error: cannot create $as_me.lineno; rerun with a POSIX shell" >&2
   { (exit 1); exit 1; }; }

  # Don't try to exec as it changes $[0], causing all sort of problems
  # (the dirname of $[0] is not the place where we might find the
  # original and so on.  Autoconf is especially sensitive to this).
  . "./$as_me.lineno"
  # Exit status is that of the last command.
  exit
}


if (as_dir=`dirname -- /` && test "X$as_dir" = X/) >/dev/null 2>&1; then
  as_dirname=dirname
else
  as_dirname=false
fi

ECHO_C= ECHO_N= ECHO_T=
case `echo -n x` in
-n*)
  case `echo 'x\c'` in
  *c*) ECHO_T='	';;	# ECHO_T is single tab character.
  *)   ECHO_C='\c';;
  esac;;
*)
  ECHO_N='-n';;
esac

if expr a : '\(a\)' >/dev/null 2>&1 &&
   test "X`expr 00001 : '.*\(...\)'`" = X001; then
  as_expr=expr
else
  as_expr=false
fi

rm -f conf$$ conf$$.exe conf$$.file
if test -d conf$$.dir; then
  rm -f conf$$.dir/conf$$.file
else
  rm -f conf$$.dir
  mkdir conf$$.dir
fi
echo >conf$$.file
if ln -s conf$$.file conf$$ 2>/dev/null; then
  as_ln_s='ln -s'
  # ... but there are two gotchas:
  # 1) On MSYS, both `ln -s file dir' and `ln file dir' fail.
  # 2) DJGPP < 2.04 has no symlinks; `ln -s' creates a wrapper executable.
  # In both cases, we have to default to `cp -p'.
  ln -s conf$$.file conf$$.dir 2>/dev/null && test ! -f conf$$.exe ||
    as_ln_s='cp -p'
elif ln conf$$.file conf$$ 2>/dev/null; then
  as_ln_s=ln
else
  as_ln_s='cp -p'
fi
rm -f conf$$ conf$$.exe conf$$.dir/conf$$.file conf$$.file
rmdir conf$$.dir 2>/dev/null

if mkdir -p . 2>/dev/null; then
  as_mkdir_p=:
else
  test -d ./-p && rmdir ./-p
  as_mkdir_p=false
fi

if test -x / >/dev/null 2>&1; then
  as_test_x='test -x'
else
  if ls -dL / >/dev/null 2>&1; then
    as_ls_L_option=L
  else
    as_ls_L_option=
  fi
  as_test_x='
    eval sh -c '\''
      if test -d "$1"; then
        test -d "$1/.";
      else
	case $1 in
        -*)set "./$1";;
	esac;
	case `ls -ld'$as_ls_L_option' "$1" 2>/dev/null` in
	???[sx]*):;;*)false;;esac;fi
    '\'' sh
  '
fi
as_executable_p=$as_test_x

# Sed expression to map a string onto a valid CPP name.
as_tr_cpp="eval sed 'y%*$as_cr_letters%P$as_cr_LETTERS%;s%[^_$as_cr_alnum]%_%g'"

# Sed expression to map a string onto a valid variable name.
as_tr_sh="eval sed 'y%*+%pp%;s%[^_$as_cr_alnum]%_%g'"




# Check that we are running under the correct shell.
SHELL=${CONFIG_SHELL-/bin/sh}

case X$ECHO in
X*--fallback-echo)
  # Remove one level of quotation (which was required for Make).
  ECHO=`echo "$ECHO" | sed 's,\\\\\$\\$0,'$0','`
  ;;
esac

echo=${ECHO-echo}
if test "X$1" = X--no-reexec; then
  # Discard the --no-reexec flag, and continue.
  shift
elif test "X$1" = X--fallback-echo; then
  # Avoid inline document here, it may be left over
  :
elif test "X`($echo '\t') 2>/dev/null`" = 'X\t' ; then
  # Yippee, $echo works!
  :
else
  # Restart under the correct shell.
  exec $SHELL "$0" --no-reexec ${1+"$@"}
fi

if test "X$1" = X--fallback-echo; then
  # used as fallback echo
  shift
  cat <<EOF
$*
EOF
  exit 0
fi

# The HP-UX ksh and POSIX shell print the target directory to stdout
# if CDPATH is set.
(unset CDPATH) >/dev/null 2>&1 && unset CDPATH

if test -z "$ECHO"; then
if test "X${echo_test_string+set}" != Xset; then
# find a string as large as possible, as long as the shell can cope with it
  for cmd in 'sed 50q "$0"' 'sed 20q "$0"' 'sed 10q "$0"' 'sed 2q "$0"' 'echo test'; do
    # expected sizes: less than 2Kb, 1Kb, 512 bytes, 16 bytes, ...
    if (echo_test_string=`eval $cmd`) 2>/dev/null &&
       echo_test_string=`eval $cmd` &&
       (test "X$echo_test_string" = "X$echo_test_string") 2>/dev/null
    then
      break
    fi
  done
fi

if test "X`($echo '\t') 2>/dev/null`" = 'X\t' &&
   echo_testing_string=`($echo "$echo_test_string") 2>/dev/null` &&
   test "X$echo_testing_string" = "X$echo_test_string"; then
  :
else
  # The Solaris, AIX, and Digital Unix default echo programs unquote
  # backslashes.  This makes it impossible to quote backslashes using
  #   echo "$something" | sed 's/\\/\\\\/g'
  #
  # So, first we look for a working echo in the user's PATH.

  lt_save_ifs="$IFS"; IFS=$PATH_SEPARATOR
  for dir in $PATH /usr/ucb; do
    IFS="$lt_save_ifs"
    if (test -f $dir/echo || test -f $dir/echo$ac_exeext) &&
       test "X`($dir/echo '\t') 2>/dev/null`" = 'X\t' &&
       echo_testing_string=`($dir/echo "$echo_test_string") 2>/dev/null` &&
       test "X$echo_testing_string" = "X$echo_test_string"; then
      echo="$dir/echo"
      break
    fi
  done
  IFS="$lt_save_ifs"

  if test "X$echo" = Xecho; then
    # We didn't find a better echo, so look for alternatives.
    if test "X`(print -r '\t') 2>/dev/null`" = 'X\t' &&
       echo_testing_string=`(print -r "$echo_test_string") 2>/dev/null` &&
       test "X$echo_testing_string" = "X$echo_test_string"; then
      # This shell has a builtin print -r that does the trick.
      echo='print -r'
    elif (test -f /bin/ksh || test -f /bin/ksh$ac_exeext) &&
	 test "X$CONFIG_SHELL" != X/bin/ksh; then
      # If we have ksh, try running configure again with it.
      ORIGINAL_CONFIG_SHELL=${CONFIG_SHELL-/bin/sh}
      export ORIGINAL_CONFIG_SHELL
      CONFIG_SHELL=/bin/ksh
      export CONFIG_SHELL
      exec $CONFIG_SHELL "$0" --no-reexec ${1+"$@"}
    else
      # Try using printf.
      echo='printf %s\n'
      if test "X`($echo '\t') 2>/dev/null`" = 'X\t' &&
	 echo_testing_string=`($echo "$echo_test_string") 2>/dev/null` &&
	 test "X$echo_testing_string" = "X$echo_test_string"; then
	# Cool, printf works
	:
      elif echo_testing_string=`($ORIGINAL_CONFIG_SHELL "$0" --fallback-echo '\t') 2>/dev/null` &&
	   test "X$echo_testing_string" = 'X\t' &&
	   echo_testing_string=`($ORIGINAL_CONFIG_SHELL "$0" --fallback-echo "$echo_test_string") 2>/dev/null` &&
	   test "X$echo_testing_string" = "X$echo_test_string"; then
	CONFIG_SHELL=$ORIGINAL_CONFIG_SHELL
	export CONFIG_SHELL
	SHELL="$CONFIG_SHELL"
	export SHELL
	echo="$CONFIG_SHELL $0 --fallback-echo"
      elif echo_testing_string=`($CONFIG_SHELL "$0" --fallback-echo '\t') 2>/dev/null` &&
	   test "X$echo_testing_string" = 'X\t' &&
	   echo_testing_string=`($CONFIG_SHELL "$0" --fallback-echo "$echo_test_string") 2>/dev/null` &&
	   test "X$echo_testing_string" = "X$echo_test_string"; then
	echo="$CONFIG_SHELL $0 --fallback-echo"
      else
	# maybe with a smaller string...
	prev=:

	for cmd in 'echo test' 'sed 2q "$0"' 'sed 10q "$0"' 'sed 20q "$0"' 'sed 50q "$0"'; do
	  if (test "X$echo_test_string" = "X`eval $cmd`") 2>/dev/null
	  then
	    break
	  fi
	  prev="$cmd"
	done

	if test "$prev" != 'sed 50q "$0"'; then
	  echo_test_string=`eval $prev`
	  export echo_test_string
	  exec ${ORIGINAL_CONFIG_SHELL-${CONFIG_SHELL-/bin/sh}} "$0" ${1+"$@"}
	else
	  # Oops.  We lost completely, so just stick with echo.
	  echo=echo
	fi
      fi
    fi
  fi
fi
fi

# Copy echo and quote the copy suitably for passing to libtool from
# the Makefile, instead of quoting the original, which is used later.
ECHO=$echo
if test "X$ECHO" = "X$CONFIG_SHELL $0 --fallback-echo"; then
   ECHO="$CONFIG_SHELL \\\$\$0 --fallback-echo"
fi




tagnames=${tagnames+${tagnames},}CXX

tagnames=${tagnames+${tagnames},}F77

exec 7<&0 </dev/null 6>&1

# Name of the host.
# hostname on some systems (SVR3.2, Linux) returns a bogus exit status,
# so uname gets run too.
ac_hostname=`(hostname || uname -n) 2>/dev/null | sed 1q`

#
# Initializations.
#
ac_default_prefix=/usr/local
ac_clean_files=
ac_config_libobj_dir=.
LIBOBJS=
cross_compiling=no
subdirs=
MFLAGS=
MAKEFLAGS=
SHELL=${CONFIG_SHELL-/bin/sh}

# Identity of this package.
PACKAGE_NAME='WWND2008_Winter'
PACKAGE_TARNAME='wwnd2008_winter'
PACKAGE_VERSION='1.0'
PACKAGE_STRING='WWND2008_Winter 1.0'
PACKAGE_BUGREPORT='winter@alum.mit.edu'

# Factoring default headers for most tests.
ac_includes_default="\
#include <stdio.h>
#ifdef HAVE_SYS_TYPES_H
# include <sys/types.h>
#endif
#ifdef HAVE_SYS_STAT_H
# include <sys/stat.h>
#endif
#ifdef STDC_HEADERS
# include <stdlib.h>
# include <stddef.h>
#else
# ifdef HAVE_STDLIB_H
#  include <stdlib.h>
# endif
#endif
#ifdef HAVE_STRING_H
# if !defined STDC_HEADERS && defined HAVE_MEMORY_H
#  include <memory.h>
# endif
# include <string.h>
#endif
#ifdef HAVE_STRINGS_H
# include <strings.h>
#endif
#ifdef HAVE_INTTYPES_H
# include <inttypes.h>
#endif
#ifdef HAVE_STDINT_H
# include <stdint.h>
#endif
#ifdef HAVE_UNISTD_H
# include <unistd.h>
#endif"

ac_subst_vars='SHELL
PATH_SEPARATOR
PACKAGE_NAME
PACKAGE_TARNAME
PACKAGE_VERSION
PACKAGE_STRING
PACKAGE_BUGREPORT
exec_prefix
prefix
program_transform_name
bindir
sbindir
libexecdir
datarootdir
datadir
sysconfdir
sharedstatedir
localstatedir
includedir
oldincludedir
docdir
infodir
htmldir
dvidir
pdfdir
psdir
libdir
localedir
mandir
DEFS
ECHO_C
ECHO_N
ECHO_T
LIBS
build_alias
host_alias
target_alias
INSTALL_PROGRAM
INSTALL_SCRIPT
INSTALL_DATA
am__isrc
CYGPATH_W
PACKAGE
VERSION
ACLOCAL
AUTOCONF
AUTOMAKE
AUTOHEADER
MAKEINFO
install_sh
STRIP
INSTALL_STRIP_PROGRAM
mkdir_p
AWK
SET_MAKE
am__leading_dot
AMTAR
am__tar
am__untar
CC
CFLAGS
LDFLAGS
CPPFLAGS
ac_ct_CC
EXEEXT
OBJEXT
DEPDIR
am__include
am__quote
AMDEP_TRUE
AMDEP_FALSE
AMDEPBACKSLASH
CCDEPMODE
am__fastdepCC_TRUE
am__fastdepCC_FALSE
CXX
CXXFLAGS
ac_ct_CXX
CXXDEPMODE
am__fastdepCXX_TRUE
am__fastdepCXX_FALSE
build
build_cpu
build_vendor
build_os
host
host_cpu
host_vendor
host_os
SED
GREP
EGREP
LN_S
ECHO
AR
RANLIB
CPP
CXXCPP
F77
FFLAGS
ac_ct_F77
LIBTOOL
LATEX
PDFLATEX
BIBTEX
DVIPS
PS2PDF
LIBOBJS
LTLIBOBJS'
ac_subst_files=''
      ac_precious_vars='build_alias
host_alias
target_alias
CC
CFLAGS
LDFLAGS
LIBS
CPPFLAGS
CXX
CXXFLAGS
CCC
CPP
CXXCPP
F77
FFLAGS'


# Initialize some variables set by options.
ac_init_help=
ac_init_version=false
# The variables have the same names as the options, with
# dashes changed to underlines.
cache_file=/dev/null
exec_prefix=NONE
no_create=
no_recursion=
prefix=NONE
program_prefix=NONE
program_suffix=NONE
program_transform_name=s,x,x,
silent=
site=
srcdir=
verbose=
x_includes=NONE
x_libraries=NONE

# Installation directory options.
# These are left unexpanded so users can "make install exec_prefix=/foo"
# and all the variables that are supposed to be based on exec_prefix
# by default will actually change.
# Use braces instead of parens because sh, perl, etc. also accept them.
# (The list follows the same order as the GNU Coding Standards.)
bindir='${exec_prefix}/bin'
sbindir='${exec_prefix}/sbin'
libexecdir='${exec_prefix}/libexec'
datarootdir='${prefix}/share'
datadir='${datarootdir}'
sysconfdir='${prefix}/etc'
sharedstatedir='${prefix}/com'
localstatedir='${prefix}/var'
includedir='${prefix}/include'
oldincludedir='/usr/include'
docdir='${datarootdir}/doc/${PACKAGE_TARNAME}'
infodir='${datarootdir}/info'
htmldir='${docdir}'
dvidir='${docdir}'
pdfdir='${docdir}'
psdir='${docdir}'
libdir='${exec_prefix}/lib'
localedir='${datarootdir}/locale'
mandir='${datarootdir}/man'

ac_prev=
ac_dashdash=
for ac_option
do
  # If the previous option needs an argument, assign it.
  if test -n "$ac_prev"; then
    eval $ac_prev=\$ac_option
    ac_prev=
    continue
  fi

  case $ac_option in
  *=*)	ac_optarg=`expr "X$ac_option" : '[^=]*=\(.*\)'` ;;
  *)	ac_optarg=yes ;;
  esac

  # Accept the important Cygnus configure options, so we can diagnose typos.

  case $ac_dashdash$ac_option in
  --)
    ac_dashdash=yes ;;

  -bindir | --bindir | --bindi | --bind | --bin | --bi)
    ac_prev=bindir ;;
  -bindir=* | --bindir=* | --bindi=* | --bind=* | --bin=* | --bi=*)
    bindir=$ac_optarg ;;

  -build | --build | --buil | --bui | --bu)
    ac_prev=build_alias ;;
  -build=* | --build=* | --buil=* | --bui=* | --bu=*)
    build_alias=$ac_optarg ;;

  -cache-file | --cache-file | --cache-fil | --cache-fi \
  | --cache-f | --cache- | --cache | --cach | --cac | --ca | --c)
    ac_prev=cache_file ;;
  -cache-file=* | --cache-file=* | --cache-fil=* | --cache-fi=* \
  | --cache-f=* | --cache-=* | --cache=* | --cach=* | --cac=* | --ca=* | --c=*)
    cache_file=$ac_optarg ;;

  --config-cache | -C)
    cache_file=config.cache ;;

  -datadir | --datadir | --datadi | --datad)
    ac_prev=datadir ;;
  -datadir=* | --datadir=* | --datadi=* | --datad=*)
    datadir=$ac_optarg ;;

  -datarootdir | --datarootdir | --datarootdi | --datarootd | --dataroot \
  | --dataroo | --dataro | --datar)
    ac_prev=datarootdir ;;
  -datarootdir=* | --datarootdir=* | --datarootdi=* | --datarootd=* \
  | --dataroot=* | --dataroo=* | --dataro=* | --datar=*)
    datarootdir=$ac_optarg ;;

  -disable-* | --disable-*)
    ac_feature=`expr "x$ac_option" : 'x-*disable-\(.*\)'`
    # Reject names that are not valid shell variable names.
    expr "x$ac_feature" : ".*[^-._$as_cr_alnum]" >/dev/null &&
      { echo "$as_me: error: invalid feature name: $ac_feature" >&2
   { (exit 1); exit 1; }; }
    ac_feature=`echo $ac_feature | sed 's/[-.]/_/g'`
    eval enable_$ac_feature=no ;;

  -docdir | --docdir | --docdi | --doc | --do)
    ac_prev=docdir ;;
  -docdir=* | --docdir=* | --docdi=* | --doc=* | --do=*)
    docdir=$ac_optarg ;;

  -dvidir | --dvidir | --dvidi | --dvid | --dvi | --dv)
    ac_prev=dvidir ;;
  -dvidir=* | --dvidir=* | --dvidi=* | --dvid=* | --dvi=* | --dv=*)
    dvidir=$ac_optarg ;;

  -enable-* | --enable-*)
    ac_feature=`expr "x$ac_option" : 'x-*enable-\([^=]*\)'`
    # Reject names that are not valid shell variable names.
    expr "x$ac_feature" : ".*[^-._$as_cr_alnum]" >/dev/null &&
      { echo "$as_me: error: invalid feature name: $ac_feature" >&2
   { (exit 1); exit 1; }; }
    ac_feature=`echo $ac_feature | sed 's/[-.]/_/g'`
    eval enable_$ac_feature=\$ac_optarg ;;

  -exec-prefix | --exec_prefix | --exec-prefix | --exec-prefi \
  | --exec-pref | --exec-pre | --exec-pr | --exec-p | --exec- \
  | --exec | --exe | --ex)
    ac_prev=exec_prefix ;;
  -exec-prefix=* | --exec_prefix=* | --exec-prefix=* | --exec-prefi=* \
  | --exec-pref=* | --exec-pre=* | --exec-pr=* | --exec-p=* | --exec-=* \
  | --exec=* | --exe=* | --ex=*)
    exec_prefix=$ac_optarg ;;

  -gas | --gas | --ga | --g)
    # Obsolete; use --with-gas.
    with_gas=yes ;;

  -help | --help | --hel | --he | -h)
    ac_init_help=long ;;
  -help=r* | --help=r* | --hel=r* | --he=r* | -hr*)
    ac_init_help=recursive ;;
  -help=s* | --help=s* | --hel=s* | --he=s* | -hs*)
    ac_init_help=short ;;

  -host | --host | --hos | --ho)
    ac_prev=host_alias ;;
  -host=* | --host=* | --hos=* | --ho=*)
    host_alias=$ac_optarg ;;

  -htmldir | --htmldir | --htmldi | --htmld | --html | --htm | --ht)
    ac_prev=htmldir ;;
  -htmldir=* | --htmldir=* | --htmldi=* | --htmld=* | --html=* | --htm=* \
  | --ht=*)
    htmldir=$ac_optarg ;;

  -includedir | --includedir | --includedi | --included | --include \
  | --includ | --inclu | --incl | --inc)
    ac_prev=includedir ;;
  -includedir=* | --includedir=* | --includedi=* | --included=* | --include=* \
  | --includ=* | --inclu=* | --incl=* | --inc=*)
    includedir=$ac_optarg ;;

  -infodir | --infodir | --infodi | --infod | --info | --inf)
    ac_prev=infodir ;;
  -infodir=* | --infodir=* | --infodi=* | --infod=* | --info=* | --inf=*)
    infodir=$ac_optarg ;;

  -libdir | --libdir | --libdi | --libd)
    ac_prev=libdir ;;
  -libdir=* | --libdir=* | --libdi=* | --libd=*)
    libdir=$ac_optarg ;;

  -libexecdir | --libexecdir | --libexecdi | --libexecd | --libexec \
  | --libexe | --libex | --libe)
    ac_prev=libexecdir ;;
  -libexecdir=* | --libexecdir=* | --libexecdi=* | --libexecd=* | --libexec=* \
  | --libexe=* | --libex=* | --libe=*)
    libexecdir=$ac_optarg ;;

  -localedir | --localedir | --localedi | --localed | --locale)
    ac_prev=localedir ;;
  -localedir=* | --localedir=* | --localedi=* | --localed=* | --locale=*)
    localedir=$ac_optarg ;;

  -localstatedir | --localstatedir | --localstatedi | --localstated \
  | --localstate | --localstat | --localsta | --localst | --locals)
    ac_prev=localstatedir ;;
  -localstatedir=* | --localstatedir=* | --localstatedi=* | --localstated=* \
  | --localstate=* | --localstat=* | --localsta=* | --localst=* | --locals=*)
    localstatedir=$ac_optarg ;;

  -mandir | --mandir | --mandi | --mand | --man | --ma | --m)
    ac_prev=mandir ;;
  -mandir=* | --mandir=* | --mandi=* | --mand=* | --man=* | --ma=* | --m=*)
    mandir=$ac_optarg ;;

  -nfp | --nfp | --nf)
    # Obsolete; use --without-fp.
    with_fp=no ;;

  -no-create | --no-create | --no-creat | --no-crea | --no-cre \
  | --no-cr | --no-c | -n)
    no_create=yes ;;

  -no-recursion | --no-recursion | --no-recursio | --no-recursi \
  | --no-recurs | --no-recur | --no-recu | --no-rec | --no-re | --no-r)
    no_recursion=yes ;;

  -oldincludedir | --oldincludedir | --oldincludedi | --oldincluded \
  | --oldinclude | --oldinclud | --oldinclu | --oldincl | --oldinc \
  | --oldin | --oldi | --old | --ol | --o)
    ac_prev=oldincludedir ;;
  -oldincludedir=* | --oldincludedir=* | --oldincludedi=* | --oldincluded=* \
  | --oldinclude=* | --oldinclud=* | --oldinclu=* | --oldincl=* | --oldinc=* \
  | --oldin=* | --oldi=* | --old=* | --ol=* | --o=*)
    oldincludedir=$ac_optarg ;;

  -prefix | --prefix | --prefi | --pref | --pre | --pr | --p)
    ac_prev=prefix ;;
  -prefix=* | --prefix=* | --prefi=* | --pref=* | --pre=* | --pr=* | --p=*)
    prefix=$ac_optarg ;;

  -program-prefix | --program-prefix | --program-prefi | --program-pref \
  | --program-pre | --program-pr | --program-p)
    ac_prev=program_prefix ;;
  -program-prefix=* | --program-prefix=* | --program-prefi=* \
  | --program-pref=* | --program-pre=* | --program-pr=* | --program-p=*)
    program_prefix=$ac_optarg ;;

  -program-suffix | --program-suffix | --program-suffi | --program-suff \
  | --program-suf | --program-su | --program-s)
    ac_prev=program_suffix ;;
  -program-suffix=* | --program-suffix=* | --program-suffi=* \
  | --program-suff=* | --program-suf=* | --program-su=* | --program-s=*)
    program_suffix=$ac_optarg ;;

  -program-transform-name | --program-transform-name \
  | --program-transform-nam | --program-transform-na \
  | --program-transform-n | --program-transform- \
  | --program-transform | --program-transfor \
  | --program-transfo | --program-transf \
  | --program-trans | --program-tran \
  | --progr-tra | --program-tr | --program-t)
    ac_prev=program_transform_name ;;
  -program-transform-name=* | --program-transform-name=* \
  | --program-transform-nam=* | --program-transform-na=* \
  | --program-transform-n=* | --program-transform-=* \
  | --program-transform=* | --program-transfor=* \
  | --program-transfo=* | --program-transf=* \
  | --program-trans=* | --program-tran=* \
  | --progr-tra=* | --program-tr=* | --program-t=*)
    program_transform_name=$ac_optarg ;;

  -pdfdir | --pdfdir | --pdfdi | --pdfd | --pdf | --pd)
    ac_prev=pdfdir ;;
  -pdfdir=* | --pdfdir=* | --pdfdi=* | --pdfd=* | --pdf=* | --pd=*)
    pdfdir=$ac_optarg ;;

  -psdir | --psdir | --psdi | --psd | --ps)
    ac_prev=psdir ;;
  -psdir=* | --psdir=* | --psdi=* | --psd=* | --ps=*)
    psdir=$ac_optarg ;;

  -q | -quiet | --quiet | --quie | --qui | --qu | --q \
  | -silent | --silent | --silen | --sile | --sil)
    silent=yes ;;

  -sbindir | --sbindir | --sbindi | --sbind | --sbin | --sbi | --sb)
    ac_prev=sbindir ;;
  -sbindir=* | --sbindir=* | --sbindi=* | --sbind=* | --sbin=* \
  | --sbi=* | --sb=*)
    sbindir=$ac_optarg ;;

  -sharedstatedir | --sharedstatedir | --sharedstatedi \
  | --sharedstated | --sharedstate | --sharedstat | --sharedsta \
  | --sharedst | --shareds | --shared | --share | --shar \
  | --sha | --sh)
    ac_prev=sharedstatedir ;;
  -sharedstatedir=* | --sharedstatedir=* | --sharedstatedi=* \
  | --sharedstated=* | --sharedstate=* | --sharedstat=* | --sharedsta=* \
  | --sharedst=* | --shareds=* | --shared=* | --share=* | --shar=* \
  | --sha=* | --sh=*)
    sharedstatedir=$ac_optarg ;;

  -site | --site | --sit)
    ac_prev=site ;;
  -site=* | --site=* | --sit=*)
    site=$ac_optarg ;;

  -srcdir | --srcdir | --srcdi | --srcd | --src | --sr)
    ac_prev=srcdir ;;
  -srcdir=* | --srcdir=* | --srcdi=* | --srcd=* | --src=* | --sr=*)
    srcdir=$ac_optarg ;;

  -sysconfdir | --sysconfdir | --sysconfdi | --sysconfd | --sysconf \
  | --syscon | --sysco | --sysc | --sys | --sy)
    ac_prev=sysconfdir ;;
  -sysconfdir=* | --sysconfdir=* | --sysconfdi=* | --sysconfd=* | --sysconf=* \
  | --syscon=* | --sysco=* | --sysc=* | --sys=* | --sy=*)
    sysconfdir=$ac_optarg ;;

  -target | --target | --targe | --targ | --tar | --ta | --t)
    ac_prev=target_alias ;;
  -target=* | --target=* | --targe=* | --targ=* | --tar=* | --ta=* | --t=*)
    target_alias=$ac_optarg ;;

  -v | -verbose | --verbose | --verbos | --verbo | --verb)
    verbose=yes ;;

  -version | --version | --versio | --versi | --vers | -V)
    ac_init_version=: ;;

  -with-* | --with-*)
    ac_package=`expr "x$ac_option" : 'x-*with-\([^=]*\)'`
    # Reject names that are not valid shell variable names.
    expr "x$ac_package" : ".*[^-._$as_cr_alnum]" >/dev/null &&
      { echo "$as_me: error: invalid package name: $ac_package" >&2
   { (exit 1); exit 1; }; }
    ac_package=`echo $ac_package | sed 's/[-.]/_/g'`
    eval with_$ac_package=\$ac_optarg ;;

  -without-* | --without-*)
    ac_package=`expr "x$ac_option" : 'x-*without-\(.*\)'`
    # Reject names that are not valid shell variable names.
    expr "x$ac_package" : ".*[^-._$as_cr_alnum]" >/dev/null &&
      { echo "$as_me: error: invalid package name: $ac_package" >&2
   { (exit 1); exit 1; }; }
    ac_package=`echo $ac_package | sed 's/[-.]/_/g'`
    eval with_$ac_package=no ;;

  --x)
    # Obsolete; use --with-x.
    with_x=yes ;;

  -x-includes | --x-includes | --x-include | --x-includ | --x-inclu \
  | --x-incl | --x-inc | --x-in | --x-i)
    ac_prev=x_includes ;;
  -x-includes=* | --x-includes=* | --x-include=* | --x-includ=* | --x-inclu=* \
  | --x-incl=* | --x-inc=* | --x-in=* | --x-i=*)
    x_includes=$ac_optarg ;;

  -x-libraries | --x-libraries | --x-librarie | --x-librari \
  | --x-librar | --x-libra | --x-libr | --x-lib | --x-li | --x-l)
    ac_prev=x_libraries ;;
  -x-libraries=* | --x-libraries=* | --x-librarie=* | --x-librari=* \
  | --x-librar=* | --x-libra=* | --x-libr=* | --x-lib=* | --x-li=* | --x-l=*)
    x_libraries=$ac_optarg ;;

  -*) { echo "$as_me: error: unrecognized option: $ac_option
Try \`$0 --help' for more information." >&2
   { (exit 1); exit 1; }; }
    ;;

  *=*)
    ac_envvar=`expr "x$ac_option" : 'x\([^=]*\)='`
    # Reject names that are not valid shell variable names.
    expr "x$ac_envvar" : ".*[^_$as_cr_alnum]" >/dev/null &&
      { echo "$as_me: error: invalid variable name: $ac_envvar" >&2
   { (exit 1); exit 1; }; }
    eval $ac_envvar=\$ac_optarg
    export $ac_envvar ;;

  *)
    # FIXME: should be removed in autoconf 3.0.
    echo "$as_me: WARNING: you should use --build, --host, --target" >&2
    expr "x$ac_option" : ".*[^-._$as_cr_alnum]" >/dev/null &&
      echo "$as_me: WARNING: invalid host type: $ac_option" >&2
    : ${build_alias=$ac_option} ${host_alias=$ac_option} ${target_alias=$ac_option}
    ;;

  esac
done

if test -n "$ac_prev"; then
  ac_option=--`echo $ac_prev | sed 's/_/-/g'`
  { echo "$as_me: error: missing argument to $ac_option" >&2
   { (exit 1); exit 1; }; }
fi

# Be sure to have absolute directory names.
for ac_var in	exec_prefix prefix bindir sbindir libexecdir datarootdir \
		datadir sysconfdir sharedstatedir localstatedir includedir \
		oldincludedir docdir infodir htmldir dvidir pdfdir psdir \
		libdir localedir mandir
do
  eval ac_val=\$$ac_var
  case $ac_val in
    [\\/$]* | ?:[\\/]* )  continue;;
    NONE | '' ) case $ac_var in *prefix ) continue;; esac;;
  esac
  { echo "$as_me: error: expected an absolute directory name for --$ac_var: $ac_val" >&2
   { (exit 1); exit 1; }; }
done

# There might be people who depend on the old broken behavior: `$host'
# used to hold the argument of --host etc.
# FIXME: To remove some day.
build=$build_alias
host=$host_alias
target=$target_alias

# FIXME: To remove some day.
if test "x$host_alias" != x; then
  if test "x$build_alias" = x; then
    cross_compiling=maybe
    echo "$as_me: WARNING: If you wanted to set the --build type, don't use --host.
    If a cross compiler is detected then cross compile mode will be used." >&2
  elif test "x$build_alias" != "x$host_alias"; then
    cross_compiling=yes
  fi
fi

ac_tool_prefix=
test -n "$host_alias" && ac_tool_prefix=$host_alias-

test "$silent" = yes && exec 6>/dev/null


ac_pwd=`pwd` && test -n "$ac_pwd" &&
ac_ls_di=`ls -di .` &&
ac_pwd_ls_di=`cd "$ac_pwd" && ls -di .` ||
  { echo "$as_me: error: Working directory cannot be determined" >&2
   { (exit 1); exit 1; }; }
test "X$ac_ls_di" = "X$ac_pwd_ls_di" ||
  { echo "$as_me: error: pwd does not report name of working directory" >&2
   { (exit 1); exit 1; }; }


# Find the source files, if location was not specified.
if test -z "$srcdir"; then
  ac_srcdir_defaulted=yes
  # Try the directory containing this script, then the parent directory.
  ac_confdir=`$as_dirname -- "$0" ||
$as_expr X"$0" : 'X\(.*[^/]\)//*[^/][^/]*/*$' \| \
	 X"$0" : 'X\(//\)[^/]' \| \
	 X"$0" : 'X\(//\)$' \| \
	 X"$0" : 'X\(/\)' \| . 2>/dev/null ||
echo X"$0" |
    sed '/^X\(.*[^/]\)\/\/*[^/][^/]*\/*$/{
	    s//\1/
	    q
	  }
	  /^X\(\/\/\)[^/].*/{
	    s//\1/
	    q
	  }
	  /^X\(\/\/\)$/{
	    s//\1/
	    q
	  }
	  /^X\(\/\).*/{
	    s//\1/
	    q
	  }
	  s/.*/./; q'`
  srcdir=$ac_confdir
  if test ! -r "$srcdir/$ac_unique_file"; then
    srcdir=..
  fi
else
  ac_srcdir_defaulted=no
fi
if test ! -r "$srcdir/$ac_unique_file"; then
  test "$ac_srcdir_defaulted" = yes && srcdir="$ac_confdir or .."
  { echo "$as_me: error: cannot find sources ($ac_unique_file) in $srcdir" >&2
   { (exit 1); exit 1; }; }
fi
ac_msg="sources are in $srcdir, but \`cd $srcdir' does not work"
ac_abs_confdir=`(
	cd "$srcdir" && test -r "./$ac_unique_file" || { echo "$as_me: error: $ac_msg" >&2
   { (exit 1); exit 1; }; }
	pwd)`
# When building in place, set srcdir=.
if test "$ac_abs_confdir" = "$ac_pwd"; then
  srcdir=.
fi
# Remove unnecessary trailing slashes from srcdir.
# Double slashes in file names in object file debugging info
# mess up M-x gdb in Emacs.
case $srcdir in
*/) srcdir=`expr "X$srcdir" : 'X\(.*[^/]\)' \| "X$srcdir" : 'X\(.*\)'`;;
esac
for ac_var in $ac_precious_vars; do
  eval ac_env_${ac_var}_set=\${${ac_var}+set}
  eval ac_env_${ac_var}_value=\$${ac_var}
  eval ac_cv_env_${ac_var}_set=\${${ac_var}+set}
  eval ac_cv_env_${ac_var}_value=\$${ac_var}
done

#
# Report the --help message.
#
if test "$ac_init_help" = "long"; then
  # Omit some internal or obsolete options to make the list less imposing.
  # This message is too long to be a string in the A/UX 3.1 sh.
  cat <<_ACEOF
\`configure' configures WWND2008_Winter 1.0 to adapt to many kinds of systems.

Usage: $0 [OPTION]... [VAR=VALUE]...

To assign environment variables (e.g., CC, CFLAGS...), specify them as
VAR=VALUE.  See below for descriptions of some of the useful variables.

Defaults for the options are specified in brackets.

Configuration:
  -h, --help              display this help and exit
      --help=short        display options specific to this package
      --help=recursive    display the short help of all the included packages
  -V, --version           display version information and exit
  -q, --quiet, --silent   do not print \`checking...' messages
      --cache-file=FILE   cache test results in FILE [disabled]
  -C, --config-cache      alias for \`--cache-file=config.cache'
  -n, --no-create         do not create output files
      --srcdir=DIR        find the sources in DIR [configure dir or \`..']

Installation directories:
  --prefix=PREFIX         install architecture-independent files in PREFIX
			  [$ac_default_prefix]
  --exec-prefix=EPREFIX   install architecture-dependent files in EPREFIX
			  [PREFIX]

By default, \`make install' will install all the files in
\`$ac_default_prefix/bin', \`$ac_default_prefix/lib' etc.  You can specify
an installation prefix other than \`$ac_default_prefix' using \`--prefix',
for instance \`--prefix=\$HOME'.

For better control, use the options below.

Fine tuning of the installation directories:
  --bindir=DIR           user executables [EPREFIX/bin]
  --sbindir=DIR          system admin executables [EPREFIX/sbin]
  --libexecdir=DIR       program executables [EPREFIX/libexec]
  --sysconfdir=DIR       read-only single-machine data [PREFIX/etc]
  --sharedstatedir=DIR   modifiable architecture-independent data [PREFIX/com]
  --localstatedir=DIR    modifiable single-machine data [PREFIX/var]
  --libdir=DIR           object code libraries [EPREFIX/lib]
  --includedir=DIR       C header files [PREFIX/include]
  --oldincludedir=DIR    C header files for non-gcc [/usr/include]
  --datarootdir=DIR      read-only arch.-independent data root [PREFIX/share]
  --datadir=DIR          read-only architecture-independent data [DATAROOTDIR]
  --infodir=DIR          info documentation [DATAROOTDIR/info]
  --localedir=DIR        locale-dependent data [DATAROOTDIR/locale]
  --mandir=DIR           man documentation [DATAROOTDIR/man]
  --docdir=DIR           documentation root [DATAROOTDIR/doc/wwnd2008_winter]
  --htmldir=DIR          html documentation [DOCDIR]
  --dvidir=DIR           dvi documentation [DOCDIR]
  --pdfdir=DIR           pdf documentation [DOCDIR]
  --psdir=DIR            ps documentation [DOCDIR]
_ACEOF

  cat <<\_ACEOF

Program names:
  --program-prefix=PREFIX            prepend PREFIX to installed program names
  --program-suffix=SUFFIX            append SUFFIX to installed program names
  --program-transform-name=PROGRAM   run sed PROGRAM on installed program names

System types:
  --build=BUILD     configure for building on BUILD [guessed]
  --host=HOST       cross-compile to build programs to run on HOST [BUILD]
_ACEOF
fi

if test -n "$ac_init_help"; then
  case $ac_init_help in
     short | recursive ) echo "Configuration of WWND2008_Winter 1.0:";;
   esac
  cat <<\_ACEOF

Optional Features:
  --disable-FEATURE       do not include FEATURE (same as --enable-FEATURE=no)
  --enable-FEATURE[=ARG]  include FEATURE [ARG=yes]
  --disable-dependency-tracking  speeds up one-time build
  --enable-dependency-tracking   do not reject slow dependency extractors
  --enable-static[=PKGS]  build static libraries [default=no]
  --enable-shared[=PKGS]  build shared libraries [default=yes]
  --enable-fast-install[=PKGS]
                          optimize for fast installation [default=yes]
  --disable-libtool-lock  avoid locking (might break parallel builds)

Optional Packages:
  --with-PACKAGE[=ARG]    use PACKAGE [ARG=yes]
  --without-PACKAGE       do not use PACKAGE (same as --with-PACKAGE=no)
  --with-gnu-ld           assume the C compiler uses GNU ld [default=no]
  --with-pic              try to use only PIC/non-PIC objects [default=use
                          both]
  --with-tags[=TAGS]      include additional configurations [automatic]

Some influential environment variables:
  CC          C compiler command
  CFLAGS      C compiler flags
  LDFLAGS     linker flags, e.g. -L<lib dir> if you have libraries in a
              nonstandard directory <lib dir>
  LIBS        libraries to pass to the linker, e.g. -l<library>
  CPPFLAGS    C/C++/Objective C preprocessor flags, e.g. -I<include dir> if
              you have headers in a nonstandard directory <include dir>
  CXX         C++ compiler command
  CXXFLAGS    C++ compiler flags
  CPP         C preprocessor
  CXXCPP      C++ preprocessor
  F77         Fortran 77 compiler command
  FFLAGS      Fortran 77 compiler flags

Use these variables to override the choices made by `configure' or to help
it to find libraries and programs with nonstandard names/locations.

Report bugs to <winter@alum.mit.edu>.
_ACEOF
ac_status=$?
fi

if test "$ac_init_help" = "recursive"; then
  # If there are subdirs, report their specific --help.
  for ac_dir in : $ac_subdirs_all; do test "x$ac_dir" = x: && continue
    test -d "$ac_dir" || continue
    ac_builddir=.

case "$ac_dir" in
.) ac_dir_suffix= ac_top_builddir_sub=. ac_top_build_prefix= ;;
*)
  ac_dir_suffix=/`echo "$ac_dir" | sed 's,^\.[\\/],,'`
  # A ".." for each directory in $ac_dir_suffix.
  ac_top_builddir_sub=`echo "$ac_dir_suffix" | sed 's,/[^\\/]*,/..,g;s,/,,'`
  case $ac_top_builddir_sub in
  "") ac_top_builddir_sub=. ac_top_build_prefix= ;;
  *)  ac_top_build_prefix=$ac_top_builddir_sub/ ;;
  esac ;;
esac
ac_abs_top_builddir=$ac_pwd
ac_abs_builddir=$ac_pwd$ac_dir_suffix
# for backward compatibility:
ac_top_builddir=$ac_top_build_prefix

case $srcdir in
  .)  # We are building in place.
    ac_srcdir=.
    ac_top_srcdir=$ac_top_builddir_sub
    ac_abs_top_srcdir=$ac_pwd ;;
  [\\/]* | ?:[\\/]* )  # Absolute name.
    ac_srcdir=$srcdir$ac_dir_suffix;
    ac_top_srcdir=$srcdir
    ac_abs_top_srcdir=$srcdir ;;
  *) # Relative name.
    ac_srcdir=$ac_top_build_prefix$srcdir$ac_dir_suffix
    ac_top_srcdir=$ac_top_build_prefix$srcdir
    ac_abs_top_srcdir=$ac_pwd/$srcdir ;;
esac
ac_abs_srcdir=$ac_abs_top_srcdir$ac_dir_suffix

    cd "$ac_dir" || { ac_status=$?; continue; }
    # Check for guested configure.
    if test -f "$ac_srcdir/configure.gnu"; then
      echo &&
      $SHELL "$ac_srcdir/configure.gnu" --help=recursive
    elif test -f "$ac_srcdir/configure"; then
      echo &&
      $SHELL "$ac_srcdir/configure" --help=recursive
    else
      echo "$as_me: WARNING: no configuration information is in $ac_dir" >&2
    fi || ac_status=$?
    cd "$ac_pwd" || { ac_status=$?; break; }
  done
fi

test -n "$ac_init_help" && exit $ac_status
if $ac_init_version; then
  cat <<\_ACEOF
WWND2008_Winter configure 1.0
generated by GNU Autoconf 2.61

Copyright (C) 1992, 1993, 1994, 1995, 1996, 1998, 1999, 2000, 2001,
2002, 2003, 2004, 2005, 2006 Free Software Foundation, Inc.
This configure script is free software; the Free Software Foundation
gives unlimited permission to copy, distribute and modify it.
_ACEOF
  exit
fi
cat >config.log <<_ACEOF
This file contains any messages produced by compilers while
running configure, to aid debugging if configure makes a mistake.

It was created by WWND2008_Winter $as_me 1.0, which was
generated by GNU Autoconf 2.61.  Invocation command line was

  $ $0 $@

_ACEOF
exec 5>>config.log
{
cat <<_ASUNAME
## --------- ##
## Platform. ##
## --------- ##

hostname = `(hostname || uname -n) 2>/dev/null | sed 1q`
uname -m = `(uname -m) 2>/dev/null || echo unknown`
uname -r = `(uname -r) 2>/dev/null || echo unknown`
uname -s = `(uname -s) 2>/dev/null || echo unknown`
uname -v = `(uname -v) 2>/dev/null || echo unknown`

/usr/bin/uname -p = `(/usr/bin/uname -p) 2>/dev/null || echo unknown`
/bin/uname -X     = `(/bin/uname -X) 2>/dev/null     || echo unknown`

/bin/arch              = `(/bin/arch) 2>/dev/null              || echo unknown`
/usr/bin/arch -k       = `(/usr/bin/arch -k) 2>/dev/null       || echo unknown`
/usr/convex/getsysinfo = `(/usr/convex/getsysinfo) 2>/dev/null || echo unknown`
/usr/bin/hostinfo      = `(/usr/bin/hostinfo) 2>/dev/null      || echo unknown`
/bin/machine           = `(/bin/machine) 2>/dev/null           || echo unknown`
/usr/bin/oslevel       = `(/usr/bin/oslevel) 2>/dev/null       || echo unknown`
/bin/universe          = `(/bin/universe) 2>/dev/null          || echo unknown`

_ASUNAME

as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  echo "PATH: $as_dir"
done
IFS=$as_save_IFS

} >&5

cat >&5 <<_ACEOF


## ----------- ##
## Core tests. ##
## ----------- ##

_ACEOF


# Keep a trace of the command line.
# Strip out --no-create and --no-recursion so they do not pile up.
# Strip out --silent because we don't want to record it for future runs.
# Also quote any args containing shell meta-characters.
# Make two passes to allow for proper duplicate-argument suppression.
ac_configure_args=
ac_configure_args0=
ac_configure_args1=
ac_must_keep_next=false
for ac_pass in 1 2
do
  for ac_arg
  do
    case $ac_arg in
    -no-create | --no-c* | -n | -no-recursion | --no-r*) continue ;;
    -q | -quiet | --quiet | --quie | --qui | --qu | --q \
    | -silent | --silent | --silen | --sile | --sil)
      continue ;;
    *\'*)
      ac_arg=`echo "$ac_arg" | sed "s/'/'\\\\\\\\''/g"` ;;
    esac
    case $ac_pass in
    1) ac_configure_args0="$ac_configure_args0 '$ac_arg'" ;;
    2)
      ac_configure_args1="$ac_configure_args1 '$ac_arg'"
      if test $ac_must_keep_next = true; then
	ac_must_keep_next=false # Got value, back to normal.
      else
	case $ac_arg in
	  *=* | --config-cache | -C | -disable-* | --disable-* \
	  | -enable-* | --enable-* | -gas | --g* | -nfp | --nf* \
	  | -q | -quiet | --q* | -silent | --sil* | -v | -verb* \
	  | -with-* | --with-* | -without-* | --without-* | --x)
	    case "$ac_configure_args0 " in
	      "$ac_configure_args1"*" '$ac_arg' "* ) continue ;;
	    esac
	    ;;
	  -* ) ac_must_keep_next=true ;;
	esac
      fi
      ac_configure_args="$ac_configure_args '$ac_arg'"
      ;;
    esac
  done
done
$as_unset ac_configure_args0 || test "${ac_configure_args0+set}" != set || { ac_configure_args0=; export ac_configure_args0; }
$as_unset ac_configure_args1 || test "${ac_configure_args1+set}" != set || { ac_configure_args1=; export ac_configure_args1; }

# When interrupted or exit'd, cleanup temporary files, and complete
# config.log.  We remove comments because anyway the quotes in there
# would cause problems or look ugly.
# WARNING: Use '\'' to represent an apostrophe within the trap.
# WARNING: Do not start the trap code with a newline, due to a FreeBSD 4.0 bug.
trap 'exit_status=$?
  # Save into config.log some information that might help in debugging.
  {
    echo

    cat <<\_ASBOX
## ---------------- ##
## Cache variables. ##
## ---------------- ##
_ASBOX
    echo
    # The following way of writing the cache mishandles newlines in values,
(
  for ac_var in `(set) 2>&1 | sed -n '\''s/^\([a-zA-Z_][a-zA-Z0-9_]*\)=.*/\1/p'\''`; do
    eval ac_val=\$$ac_var
    case $ac_val in #(
    *${as_nl}*)
      case $ac_var in #(
      *_cv_*) { echo "$as_me:$LINENO: WARNING: Cache variable $ac_var contains a newline." >&5
echo "$as_me: WARNING: Cache variable $ac_var contains a newline." >&2;} ;;
      esac
      case $ac_var in #(
      _ | IFS | as_nl) ;; #(
      *) $as_unset $ac_var ;;
      esac ;;
    esac
  done
  (set) 2>&1 |
    case $as_nl`(ac_space='\'' '\''; set) 2>&1` in #(
    *${as_nl}ac_space=\ *)
      sed -n \
	"s/'\''/'\''\\\\'\'''\''/g;
	  s/^\\([_$as_cr_alnum]*_cv_[_$as_cr_alnum]*\\)=\\(.*\\)/\\1='\''\\2'\''/p"
      ;; #(
    *)
      sed -n "/^[_$as_cr_alnum]*_cv_[_$as_cr_alnum]*=/p"
      ;;
    esac |
    sort
)
    echo

    cat <<\_ASBOX
## ----------------- ##
## Output variables. ##
## ----------------- ##
_ASBOX
    echo
    for ac_var in $ac_subst_vars
    do
      eval ac_val=\$$ac_var
      case $ac_val in
      *\'\''*) ac_val=`echo "$ac_val" | sed "s/'\''/'\''\\\\\\\\'\'''\''/g"`;;
      esac
      echo "$ac_var='\''$ac_val'\''"
    done | sort
    echo

    if test -n "$ac_subst_files"; then
      cat <<\_ASBOX
## ------------------- ##
## File substitutions. ##
## ------------------- ##
_ASBOX
      echo
      for ac_var in $ac_subst_files
      do
	eval ac_val=\$$ac_var
	case $ac_val in
	*\'\''*) ac_val=`echo "$ac_val" | sed "s/'\''/'\''\\\\\\\\'\'''\''/g"`;;
	esac
	echo "$ac_var='\''$ac_val'\''"
      done | sort
      echo
    fi

    if test -s confdefs.h; then
      cat <<\_ASBOX
## ----------- ##
## confdefs.h. ##
## ----------- ##
_ASBOX
      echo
      cat confdefs.h
      echo
    fi
    test "$ac_signal" != 0 &&
      echo "$as_me: caught signal $ac_signal"
    echo "$as_me: exit $exit_status"
  } >&5
  rm -f core *.core core.conftest.* &&
    rm -f -r conftest* confdefs* conf$$* $ac_clean_files &&
    exit $exit_status
' 0
for ac_signal in 1 2 13 15; do
  trap 'ac_signal='$ac_signal'; { (exit 1); exit 1; }' $ac_signal
done
ac_signal=0

# confdefs.h avoids OS command line length limits that DEFS can exceed.
rm -f -r conftest* confdefs.h

# Predefined preprocessor variables.

cat >>confdefs.h <<_ACEOF
#define PACKAGE_NAME "$PACKAGE_NAME"
_ACEOF


cat >>confdefs.h <<_ACEOF
#define PACKAGE_TARNAME "$PACKAGE_TARNAME"
_ACEOF


cat >>confdefs.h <<_ACEOF
#define PACKAGE_VERSION "$PACKAGE_VERSION"
_ACEOF


cat >>confdefs.h <<_ACEOF
#define PACKAGE_STRING "$PACKAGE_STRING"
_ACEOF


cat >>confdefs.h <<_ACEOF
#define PACKAGE_BUGREPORT "$PACKAGE_BUGREPORT"
_ACEOF


# Let the site file select an alternate cache file if it wants to.
# Prefer explicitly selected file to automatically selected ones.
if test -n "$CONFIG_SITE"; then
  set x "$CONFIG_SITE"
elif test "x$prefix" != xNONE; then
  set x "$prefix/share/config.site" "$prefix/etc/config.site"
else
  set x "$ac_default_prefix/share/config.site" \
	"$ac_default_prefix/etc/config.site"
fi
shift
for ac_site_file
do
  if test -r "$ac_site_file"; then
    { echo "$as_me:$LINENO: loading site script $ac_site_file" >&5
echo "$as_me: loading site script $ac_site_file" >&6;}
    sed 's/^/| /' "$ac_site_file" >&5
    . "$ac_site_file"
  fi
done

if test -r "$cache_file"; then
  # Some versions of bash will fail to source /dev/null (special
  # files actually), so we avoid doing that.
  if test -f "$cache_file"; then
    { echo "$as_me:$LINENO: loading cache $cache_file" >&5
echo "$as_me: loading cache $cache_file" >&6;}
    case $cache_file in
      [\\/]* | ?:[\\/]* ) . "$cache_file";;
      *)                      . "./$cache_file";;
    esac
  fi
else
  { echo "$as_me:$LINENO: creating cache $cache_file" >&5
echo "$as_me: creating cache $cache_file" >&6;}
  >$cache_file
fi

# Check that the precious variables saved in the cache have kept the same
# value.
ac_cache_corrupted=false
for ac_var in $ac_precious_vars; do
  eval ac_old_set=\$ac_cv_env_${ac_var}_set
  eval ac_new_set=\$ac_env_${ac_var}_set
  eval ac_old_val=\$ac_cv_env_${ac_var}_value
  eval ac_new_val=\$ac_env_${ac_var}_value
  case $ac_old_set,$ac_new_set in
    set,)
      { echo "$as_me:$LINENO: error: \`$ac_var' was set to \`$ac_old_val' in the previous run" >&5
echo "$as_me: error: \`$ac_var' was set to \`$ac_old_val' in the previous run" >&2;}
      ac_cache_corrupted=: ;;
    ,set)
      { echo "$as_me:$LINENO: error: \`$ac_var' was not set in the previous run" >&5
echo "$as_me: error: \`$ac_var' was not set in the previous run" >&2;}
      ac_cache_corrupted=: ;;
    ,);;
    *)
      if test "x$ac_old_val" != "x$ac_new_val"; then
	{ echo "$as_me:$LINENO: error: \`$ac_var' has changed since the previous run:" >&5
echo "$as_me: error: \`$ac_var' has changed since the previous run:" >&2;}
	{ echo "$as_me:$LINENO:   former value:  $ac_old_val" >&5
echo "$as_me:   former value:  $ac_old_val" >&2;}
	{ echo "$as_me:$LINENO:   current value: $ac_new_val" >&5
echo "$as_me:   current value: $ac_new_val" >&2;}
	ac_cache_corrupted=:
      fi;;
  esac
  # Pass precious variables to config.status.
  if test "$ac_new_set" = set; then
    case $ac_new_val in
    *\'*) ac_arg=$ac_var=`echo "$ac_new_val" | sed "s/'/'\\\\\\\\''/g"` ;;
    *) ac_arg=$ac_var=$ac_new_val ;;
    esac
    case " $ac_configure_args " in
      *" '$ac_arg' "*) ;; # Avoid dups.  Use of quotes ensures accuracy.
      *) ac_configure_args="$ac_configure_args '$ac_arg'" ;;
    esac
  fi
done
if $ac_cache_corrupted; then
  { echo "$as_me:$LINENO: error: changes in the environment can compromise the build" >&5
echo "$as_me: error: changes in the environment can compromise the build" >&2;}
  { { echo "$as_me:$LINENO: error: run \`make distclean' and/or \`rm $cache_file' and start over" >&5
echo "$as_me: error: run \`make distclean' and/or \`rm $cache_file' and start over" >&2;}
   { (exit 1); exit 1; }; }
fi

























ac_ext=c
ac_cpp='$CPP $CPPFLAGS'
ac_compile='$CC -c $CFLAGS $CPPFLAGS conftest.$ac_ext >&5'
ac_link='$CC -o conftest$ac_exeext $CFLAGS $CPPFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_c_compiler_gnu


am__api_version='1.10'

ac_aux_dir=
for ac_dir in "$srcdir" "$srcdir/.." "$srcdir/../.."; do
  if test -f "$ac_dir/install-sh"; then
    ac_aux_dir=$ac_dir
    ac_install_sh="$ac_aux_dir/install-sh -c"
    break
  elif test -f "$ac_dir/install.sh"; then
    ac_aux_dir=$ac_dir
    ac_install_sh="$ac_aux_dir/install.sh -c"
    break
  elif test -f "$ac_dir/shtool"; then
    ac_aux_dir=$ac_dir
    ac_install_sh="$ac_aux_dir/shtool install -c"
    break
  fi
done
if test -z "$ac_aux_dir"; then
  { { echo "$as_me:$LINENO: error: cannot find install-sh or install.sh in \"$srcdir\" \"$srcdir/..\" \"$srcdir/../..\"" >&5
echo "$as_me: error: cannot find install-sh or install.sh in \"$srcdir\" \"$srcdir/..\" \"$srcdir/../..\"" >&2;}
   { (exit 1); exit 1; }; }
fi

# These three variables are undocumented and unsupported,
# and are intended to be withdrawn in a future Autoconf release.
# They can cause serious problems if a builder's source tree is in a directory
# whose full name contains unusual characters.
ac_config_guess="$SHELL $ac_aux_dir/config.guess"  # Please don't use this var.
ac_config_sub="$SHELL $ac_aux_dir/config.sub"  # Please don't use this var.
ac_configure="$SHELL $ac_aux_dir/configure"  # Please don't use this var.


# Find a good install program.  We prefer a C program (faster),
# so one script is as good as another.  But avoid the broken or
# incompatible versions:
# SysV /etc/install, /usr/sbin/install
# SunOS /usr/etc/install
# IRIX /sbin/install
# AIX /bin/install
# AmigaOS /C/install, which installs bootblocks on floppy discs
# AIX 4 /usr/bin/installbsd, which doesn't work without a -g flag
# AFS /usr/afsws/bin/install, which mishandles nonexistent args
# SVR4 /usr/ucb/install, which tries to use the nonexistent group "staff"
# OS/2's system install, which has a completely different semantic
# ./install, which can be erroneously created by make from ./install.sh.
{ echo "$as_me:$LINENO: checking for a BSD-compatible install" >&5
echo $ECHO_N "checking for a BSD-compatible install... $ECHO_C" >&6; }
if test -z "$INSTALL"; then
if test "${ac_cv_path_install+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  # Account for people who put trailing slashes in PATH elements.
case $as_dir/ in
  ./ | .// | /cC/* | \
  /etc/* | /usr/sbin/* | /usr/etc/* | /sbin/* | /usr/afsws/bin/* | \
  ?:\\/os2\\/install\\/* | ?:\\/OS2\\/INSTALL\\/* | \
  /usr/ucb/* ) ;;
  *)
    # OSF1 and SCO ODT 3.0 have their own names for install.
    # Don't use installbsd from OSF since it installs stuff as root
    # by default.
    for ac_prog in ginstall scoinst install; do
      for ac_exec_ext in '' $ac_executable_extensions; do
	if { test -f "$as_dir/$ac_prog$ac_exec_ext" && $as_test_x "$as_dir/$ac_prog$ac_exec_ext"; }; then
	  if test $ac_prog = install &&
	    grep dspmsg "$as_dir/$ac_prog$ac_exec_ext" >/dev/null 2>&1; then
	    # AIX install.  It has an incompatible calling convention.
	    :
	  elif test $ac_prog = install &&
	    grep pwplus "$as_dir/$ac_prog$ac_exec_ext" >/dev/null 2>&1; then
	    # program-specific install script used by HP pwplus--don't use.
	    :
	  else
	    ac_cv_path_install="$as_dir/$ac_prog$ac_exec_ext -c"
	    break 3
	  fi
	fi
      done
    done
    ;;
esac
done
IFS=$as_save_IFS


fi
  if test "${ac_cv_path_install+set}" = set; then
    INSTALL=$ac_cv_path_install
  else
    # As a last resort, use the slow shell script.  Don't cache a
    # value for INSTALL within a source directory, because that will
    # break other packages using the cache if that directory is
    # removed, or if the value is a relative name.
    INSTALL=$ac_install_sh
  fi
fi
{ echo "$as_me:$LINENO: result: $INSTALL" >&5
echo "${ECHO_T}$INSTALL" >&6; }

# Use test -z because SunOS4 sh mishandles braces in ${var-val}.
# It thinks the first close brace ends the variable substitution.
test -z "$INSTALL_PROGRAM" && INSTALL_PROGRAM='${INSTALL}'

test -z "$INSTALL_SCRIPT" && INSTALL_SCRIPT='${INSTALL}'

test -z "$INSTALL_DATA" && INSTALL_DATA='${INSTALL} -m 644'

{ echo "$as_me:$LINENO: checking whether build environment is sane" >&5
echo $ECHO_N "checking whether build environment is sane... $ECHO_C" >&6; }
# Just in case
sleep 1
echo timestamp > conftest.file
# Do `set' in a subshell so we don't clobber the current shell's
# arguments.  Must try -L first in case configure is actually a
# symlink; some systems play weird games with the mod time of symlinks
# (eg FreeBSD returns the mod time of the symlink's containing
# directory).
if (
   set X `ls -Lt $srcdir/configure conftest.file 2> /dev/null`
   if test "$*" = "X"; then
      # -L didn't work.
      set X `ls -t $srcdir/configure conftest.file`
   fi
   rm -f conftest.file
   if test "$*" != "X $srcdir/configure conftest.file" \
      && test "$*" != "X conftest.file $srcdir/configure"; then

      # If neither matched, then we have a broken ls.  This can happen
      # if, for instance, CONFIG_SHELL is bash and it inherits a
      # broken ls alias from the environment.  This has actually
      # happened.  Such a system could not be considered "sane".
      { { echo "$as_me:$LINENO: error: ls -t appears to fail.  Make sure there is not a broken
alias in your environment" >&5
echo "$as_me: error: ls -t appears to fail.  Make sure there is not a broken
alias in your environment" >&2;}
   { (exit 1); exit 1; }; }
   fi

   test "$2" = conftest.file
   )
then
   # Ok.
   :
else
   { { echo "$as_me:$LINENO: error: newly created file is older than distributed files!
Check your system clock" >&5
echo "$as_me: error: newly created file is older than distributed files!
Check your system clock" >&2;}
   { (exit 1); exit 1; }; }
fi
{ echo "$as_me:$LINENO: result: yes" >&5
echo "${ECHO_T}yes" >&6; }
test "$program_prefix" != NONE &&
  program_transform_name="s&^&$program_prefix&;$program_transform_name"
# Use a double $ so make ignores it.
test "$program_suffix" != NONE &&
  program_transform_name="s&\$&$program_suffix&;$program_transform_name"
# Double any \ or $.  echo might interpret backslashes.
# By default was `s,x,x', remove it if useless.
cat <<\_ACEOF >conftest.sed
s/[\\$]/&&/g;s/;s,x,x,$//
_ACEOF
program_transform_name=`echo $program_transform_name | sed -f conftest.sed`
rm -f conftest.sed

# expand $ac_aux_dir to an absolute path
am_aux_dir=`cd $ac_aux_dir && pwd`

test x"${MISSING+set}" = xset || MISSING="\${SHELL} $am_aux_dir/missing"
# Use eval to expand $SHELL
if eval "$MISSING --run true"; then
  am_missing_run="$MISSING --run "
else
  am_missing_run=
  { echo "$as_me:$LINENO: WARNING: \`missing' script is too old or missing" >&5
echo "$as_me: WARNING: \`missing' script is too old or missing" >&2;}
fi

{ echo "$as_me:$LINENO: checking for a thread-safe mkdir -p" >&5
echo $ECHO_N "checking for a thread-safe mkdir -p... $ECHO_C" >&6; }
if test -z "$MKDIR_P"; then
  if test "${ac_cv_path_mkdir+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH$PATH_SEPARATOR/opt/sfw/bin
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_prog in mkdir gmkdir; do
	 for ac_exec_ext in '' $ac_executable_extensions; do
	   { test -f "$as_dir/$ac_prog$ac_exec_ext" && $as_test_x "$as_dir/$ac_prog$ac_exec_ext"; } || continue
	   case `"$as_dir/$ac_prog$ac_exec_ext" --version 2>&1` in #(
	     'mkdir (GNU coreutils) '* | \
	     'mkdir (coreutils) '* | \
	     'mkdir (fileutils) '4.1*)
	       ac_cv_path_mkdir=$as_dir/$ac_prog$ac_exec_ext
	       break 3;;
	   esac
	 done
       done
done
IFS=$as_save_IFS

fi

  if test "${ac_cv_path_mkdir+set}" = set; then
    MKDIR_P="$ac_cv_path_mkdir -p"
  else
    # As a last resort, use the slow shell script.  Don't cache a
    # value for MKDIR_P within a source directory, because that will
    # break other packages using the cache if that directory is
    # removed, or if the value is a relative name.
    test -d ./--version && rmdir ./--version
    MKDIR_P="$ac_install_sh -d"
  fi
fi
{ echo "$as_me:$LINENO: result: $MKDIR_P" >&5
echo "${ECHO_T}$MKDIR_P" >&6; }

mkdir_p="$MKDIR_P"
case $mkdir_p in
  [\\/$]* | ?:[\\/]*) ;;
  */*) mkdir_p="\$(top_builddir)/$mkdir_p" ;;
esac

for ac_prog in gawk mawk nawk awk
do
  # Extract the first word of "$ac_prog", so it can be a program name with args.
set dummy $ac_prog; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_AWK+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$AWK"; then
  ac_cv_prog_AWK="$AWK" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_test_x "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_AWK="$ac_prog"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
AWK=$ac_cv_prog_AWK
if test -n "$AWK"; then
  { echo "$as_me:$LINENO: result: $AWK" >&5
echo "${ECHO_T}$AWK" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi


  test -n "$AWK" && break
done

{ echo "$as_me:$LINENO: checking whether ${MAKE-make} sets \$(MAKE)" >&5
echo $ECHO_N "checking whether ${MAKE-make} sets \$(MAKE)... $ECHO_C" >&6; }
set x ${MAKE-make}; ac_make=`echo "$2" | sed 's/+/p/g; s/[^a-zA-Z0-9_]/_/g'`
if { as_var=ac_cv_prog_make_${ac_make}_set; eval "test \"\${$as_var+set}\" = set"; }; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  cat >conftest.make <<\_ACEOF
SHELL = /bin/sh
all:
	@echo '@@@%%%=$(MAKE)=@@@%%%'
_ACEOF
# GNU make sometimes prints "make[1]: Entering...", which would confuse us.
case `${MAKE-make} -f conftest.make 2>/dev/null` in
  *@@@%%%=?*=@@@%%%*)
    eval ac_cv_prog_make_${ac_make}_set=yes;;
  *)
    eval ac_cv_prog_make_${ac_make}_set=no;;
esac
rm -f conftest.make
fi
if eval test \$ac_cv_prog_make_${ac_make}_set = yes; then
  { echo "$as_me:$LINENO: result: yes" >&5
echo "${ECHO_T}yes" >&6; }
  SET_MAKE=
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
  SET_MAKE="MAKE=${MAKE-make}"
fi

rm -rf .tst 2>/dev/null
mkdir .tst 2>/dev/null
if test -d .tst; then
  am__leading_dot=.
else
  am__leading_dot=_
fi
rmdir .tst 2>/dev/null

if test "`cd $srcdir && pwd`" != "`pwd`"; then
  # Use -I$(srcdir) only when $(srcdir) != ., so that make's output
  # is not polluted with repeated "-I."
  am__isrc=' -I$(srcdir)'
  # test to see if srcdir already configured
  if test -f $srcdir/config.status; then
    { { echo "$as_me:$LINENO: error: source directory already configured; run \"make distclean\" there first" >&5
echo "$as_me: error: source directory already configured; run \"make distclean\" there first" >&2;}
   { (exit 1); exit 1; }; }
  fi
fi

# test whether we have cygpath
if test -z "$CYGPATH_W"; then
  if (cygpath --version) >/dev/null 2>/dev/null; then
    CYGPATH_W='cygpath -w'
  else
    CYGPATH_W=echo
  fi
fi


# Define the identity of the package.
 PACKAGE='wwnd2008_winter'
 VERSION='1.0'


cat >>confdefs.h <<_ACEOF
#define PACKAGE "$PACKAGE"
_ACEOF


cat >>confdefs.h <<_ACEOF
#define VERSION "$VERSION"
_ACEOF

# Some tools Automake needs.

ACLOCAL=${ACLOCAL-"${am_missing_run}aclocal-${am__api_version}"}


AUTOCONF=${AUTOCONF-"${am_missing_run}autoconf"}


AUTOMAKE=${AUTOMAKE-"${am_missing_run}automake-${am__api_version}"}


AUTOHEADER=${AUTOHEADER-"${am_missing_run}autoheader"}


MAKEINFO=${MAKEINFO-"${am_missing_run}makeinfo"}

install_sh=${install_sh-"\$(SHELL) $am_aux_dir/install-sh"}

# Installed binaries are usually stripped using `strip' when the user
# run `make install-strip'.  However `strip' might not be the right
# tool to use in cross-compilation environments, therefore Automake
# will honor the `STRIP' environment variable to overrule this program.
if test "$cross_compiling" != no; then
  if test -n "$ac_tool_prefix"; then
  # Extract the first word of "${ac_tool_prefix}strip", so it can be a program name with args.
set dummy ${ac_tool_prefix}strip; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_STRIP+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$STRIP"; then
  ac_cv_prog_STRIP="$STRIP" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_test_x "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_STRIP="${ac_tool_prefix}strip"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
STRIP=$ac_cv_prog_STRIP
if test -n "$STRIP"; then
  { echo "$as_me:$LINENO: result: $STRIP" >&5
echo "${ECHO_T}$STRIP" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi


fi
if test -z "$ac_cv_prog_STRIP"; then
  ac_ct_STRIP=$STRIP
  # Extract the first word of "strip", so it can be a program name with args.
set dummy strip; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_ac_ct_STRIP+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$ac_ct_STRIP"; then
  ac_cv_prog_ac_ct_STRIP="$ac_ct_STRIP" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_test_x "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_ac_ct_STRIP="strip"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
ac_ct_STRIP=$ac_cv_prog_ac_ct_STRIP
if test -n "$ac_ct_STRIP"; then
  { echo "$as_me:$LINENO: result: $ac_ct_STRIP" >&5
echo "${ECHO_T}$ac_ct_STRIP" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi

  if test "x$ac_ct_STRIP" = x; then
    STRIP=":"
  else
    case $cross_compiling:$ac_tool_warned in
yes:)
{ echo "$as_me:$LINENO: WARNING: In the future, Autoconf will not detect cross-tools
whose name does not start with the host triplet.  If you think this
configuration is useful to you, please write to autoconf@gnu.org." >&5
echo "$as_me: WARNING: In the future, Autoconf will not detect cross-tools
whose name does not start with the host triplet.  If you think this
configuration is useful to you, please write to autoconf@gnu.org." >&2;}
ac_tool_warned=yes ;;
esac
    STRIP=$ac_ct_STRIP
  fi
else
  STRIP="$ac_cv_prog_STRIP"
fi

fi
INSTALL_STRIP_PROGRAM="\$(install_sh) -c -s"

# We need awk for the "check" target.  The system "awk" is bad on
# some platforms.
# Always define AMTAR for backward compatibility.

AMTAR=${AMTAR-"${am_missing_run}tar"}

am__tar='${AMTAR} chof - "$$tardir"'; am__untar='${AMTAR} xf -'






# Checks for programs.
#  AC_PROG_CXX needed to make sure OBJEXT is set (so target mostlyclean-compile
#  doesn't wreck havoc!).
ac_ext=c
ac_cpp='$CPP $CPPFLAGS'
ac_compile='$CC -c $CFLAGS $CPPFLAGS conftest.$ac_ext >&5'
ac_link='$CC -o conftest$ac_exeext $CFLAGS $CPPFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_c_compiler_gnu
if test -n "$ac_tool_prefix"; then
  # Extract the first word of "${ac_tool_prefix}gcc", so it can be a program name with args.
set dummy ${ac_tool_prefix}gcc; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_CC+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$CC"; then
  ac_cv_prog_CC="$CC" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_test_x "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_CC="${ac_tool_prefix}gcc"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
CC=$ac_cv_prog_CC
if test -n "$CC"; then
  { echo "$as_me:$LINENO: result: $CC" >&5
echo "${ECHO_T}$CC" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi


fi
if test -z "$ac_cv_prog_CC"; then
  ac_ct_CC=$CC
  # Extract the first word of "gcc", so it can be a program name with args.
set dummy gcc; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_ac_ct_CC+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$ac_ct_CC"; then
  ac_cv_prog_ac_ct_CC="$ac_ct_CC" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_test_x "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_ac_ct_CC="gcc"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
ac_ct_CC=$ac_cv_prog_ac_ct_CC
if test -n "$ac_ct_CC"; then
  { echo "$as_me:$LINENO: result: $ac_ct_CC" >&5
echo "${ECHO_T}$ac_ct_CC" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi

  if test "x$ac_ct_CC" = x; then
    CC=""
  else
    case $cross_compiling:$ac_tool_warned in
yes:)
{ echo "$as_me:$LINENO: WARNING: In the future, Autoconf will not detect cross-tools
whose name does not start with the host triplet.  If you think this
configuration is useful to you, please write to autoconf@gnu.org." >&5
echo "$as_me: WARNING: In the future, Autoconf will not detect cross-tools
whose name does not start with the host triplet.  If you think this
configuration is useful to you, please write to autoconf@gnu.org." >&2;}
ac_tool_warned=yes ;;
esac
    CC=$ac_ct_CC
  fi
else
  CC="$ac_cv_prog_CC"
fi

if test -z "$CC"; then
          if test -n "$ac_tool_prefix"; then
    # Extract the first word of "${ac_tool_prefix}cc", so it can be a program name with args.
set dummy ${ac_tool_prefix}cc; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_CC+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$CC"; then
  ac_cv_prog_CC="$CC" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_test_x "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_CC="${ac_tool_prefix}cc"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
CC=$ac_cv_prog_CC
if test -n "$CC"; then
  { echo "$as_me:$LINENO: result: $CC" >&5
echo "${ECHO_T}$CC" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi


  fi
fi
if test -z "$CC"; then
  # Extract the first word of "cc", so it can be a program name with args.
set dummy cc; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_CC+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$CC"; then
  ac_cv_prog_CC="$CC" # Let the user override the test.
else
  ac_prog_rejected=no
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_test_x "$as_dir/$ac_word$ac_exec_ext"; }; then
    if test "$as_dir/$ac_word$ac_exec_ext" = "/usr/ucb/cc"; then
       ac_prog_rejected=yes
       continue
     fi
    ac_cv_prog_CC="cc"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

if test $ac_prog_rejected = yes; then
  # We found a bogon in the path, so make sure we never use it.
  set dummy $ac_cv_prog_CC
  shift
  if test $# != 0; then
    # We chose a different compiler from the bogus one.
    # However, it has the same basename, so the bogon will be chosen
    # first if we set CC to just the basename; use the full file name.
    shift
    ac_cv_prog_CC="$as_dir/$ac_word${1+' '}$@"
  fi
fi
fi
fi
CC=$ac_cv_prog_CC
if test -n "$CC"; then
  { echo "$as_me:$LINENO: result: $CC" >&5
echo "${ECHO_T}$CC" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi


fi
if test -z "$CC"; then
  if test -n "$ac_tool_prefix"; then
  for ac_prog in cl.exe
  do
    # Extract the first word of "$ac_tool_prefix$ac_prog", so it can be a program name with args.
set dummy $ac_tool_prefix$ac_prog; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_CC+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$CC"; then
  ac_cv_prog_CC="$CC" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_test_x "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_CC="$ac_tool_prefix$ac_prog"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
CC=$ac_cv_prog_CC
if test -n "$CC"; then
  { echo "$as_me:$LINENO: result: $CC" >&5
echo "${ECHO_T}$CC" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi


    test -n "$CC" && break
  done
fi
if test -z "$CC"; then
  ac_ct_CC=$CC
  for ac_prog in cl.exe
do
  # Extract the first word of "$ac_prog", so it can be a program name with args.
set dummy $ac_prog; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_ac_ct_CC+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$ac_ct_CC"; then
  ac_cv_prog_ac_ct_CC="$ac_ct_CC" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_test_x "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_ac_ct_CC="$ac_prog"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
ac_ct_CC=$ac_cv_prog_ac_ct_CC
if test -n "$ac_ct_CC"; then
  { echo "$as_me:$LINENO: result: $ac_ct_CC" >&5
echo "${ECHO_T}$ac_ct_CC" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi


  test -n "$ac_ct_CC" && break
done

  if test "x$ac_ct_CC" = x; then
    CC=""
  else
    case $cross_compiling:$ac_tool_warned in
yes:)
{ echo "$as_me:$LINENO: WARNING: In the future, Autoconf will not detect cross-tools
whose name does not start with the host triplet.  If you think this
configuration is useful to you, please write to autoconf@gnu.org." >&5
echo "$as_me: WARNING: In the future, Autoconf will not detect cross-tools
whose name does not start with the host triplet.  If you think this
configuration is useful to you, please write to autoconf@gnu.org." >&2;}
ac_tool_warned=yes ;;
esac
    CC=$ac_ct_CC
  fi
fi

fi


test -z "$CC" && { { echo "$as_me:$LINENO: error: no acceptable C compiler found in \$PATH
See \`config.log' for more details." >&5
echo "$as_me: error: no acceptable C compiler found in \$PATH
See \`config.log' for more details." >&2;}
   { (exit 1); exit 1; }; }

# Provide some information about the compiler.
echo "$as_me:$LINENO: checking for C compiler version" >&5
ac_compiler=`set X $ac_compile; echo $2`
{ (ac_try="$ac_compiler --version >&5"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compiler --version >&5") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }
{ (ac_try="$ac_compiler -v >&5"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compiler -v >&5") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }
{ (ac_try="$ac_compiler -V >&5"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compiler -V >&5") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }

cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

int
main ()
{

  ;
  return 0;
}
_ACEOF
ac_clean_files_save=$ac_clean_files
ac_clean_files="$ac_clean_files a.out a.exe b.out"
# Try to create an executable without -o first, disregard a.out.
# It will help us diagnose broken compilers, and finding out an intuition
# of exeext.
{ echo "$as_me:$LINENO: checking for C compiler default output file name" >&5
echo $ECHO_N "checking for C compiler default output file name... $ECHO_C" >&6; }
ac_link_default=`echo "$ac_link" | sed 's/ -o *conftest[^ ]*//'`
#
# List of possible output files, starting from the most likely.
# The algorithm is not robust to junk in `.', hence go to wildcards (a.*)
# only as a last resort.  b.out is created by i960 compilers.
ac_files='a_out.exe a.exe conftest.exe a.out conftest a.* conftest.* b.out'
#
# The IRIX 6 linker writes into existing files which may not be
# executable, retaining their permissions.  Remove them first so a
# subsequent execution test works.
ac_rmfiles=
for ac_file in $ac_files
do
  case $ac_file in
    *.$ac_ext | *.xcoff | *.tds | *.d | *.pdb | *.xSYM | *.bb | *.bbg | *.map | *.inf | *.o | *.obj ) ;;
    * ) ac_rmfiles="$ac_rmfiles $ac_file";;
  esac
done
rm -f $ac_rmfiles

if { (ac_try="$ac_link_default"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link_default") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; then
  # Autoconf-2.13 could set the ac_cv_exeext variable to `no'.
# So ignore a value of `no', otherwise this would lead to `EXEEXT = no'
# in a Makefile.  We should not override ac_cv_exeext if it was cached,
# so that the user can short-circuit this test for compilers unknown to
# Autoconf.
for ac_file in $ac_files ''
do
  test -f "$ac_file" || continue
  case $ac_file in
    *.$ac_ext | *.xcoff | *.tds | *.d | *.pdb | *.xSYM | *.bb | *.bbg | *.map | *.inf | *.o | *.obj )
	;;
    [ab].out )
	# We found the default executable, but exeext='' is most
	# certainly right.
	break;;
    *.* )
        if test "${ac_cv_exeext+set}" = set && test "$ac_cv_exeext" != no;
	then :; else
	   ac_cv_exeext=`expr "$ac_file" : '[^.]*\(\..*\)'`
	fi
	# We set ac_cv_exeext here because the later test for it is not
	# safe: cross compilers may not add the suffix if given an `-o'
	# argument, so we may need to know it at that point already.
	# Even if this section looks crufty: it has the advantage of
	# actually working.
	break;;
    * )
	break;;
  esac
done
test "$ac_cv_exeext" = no && ac_cv_exeext=

else
  ac_file=''
fi

{ echo "$as_me:$LINENO: result: $ac_file" >&5
echo "${ECHO_T}$ac_file" >&6; }
if test -z "$ac_file"; then
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

{ { echo "$as_me:$LINENO: error: C compiler cannot create executables
See \`config.log' for more details." >&5
echo "$as_me: error: C compiler cannot create executables
See \`config.log' for more details." >&2;}
   { (exit 77); exit 77; }; }
fi

ac_exeext=$ac_cv_exeext

# Check that the compiler produces executables we can run.  If not, either
# the compiler is broken, or we cross compile.
{ echo "$as_me:$LINENO: checking whether the C compiler works" >&5
echo $ECHO_N "checking whether the C compiler works... $ECHO_C" >&6; }
# FIXME: These cross compiler hacks should be removed for Autoconf 3.0
# If not cross compiling, check that we can run a simple program.
if test "$cross_compiling" != yes; then
  if { ac_try='./$ac_file'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
    cross_compiling=no
  else
    if test "$cross_compiling" = maybe; then
	cross_compiling=yes
    else
	{ { echo "$as_me:$LINENO: error: cannot run C compiled programs.
If you meant to cross compile, use \`--host'.
See \`config.log' for more details." >&5
echo "$as_me: error: cannot run C compiled programs.
If you meant to cross compile, use \`--host'.
See \`config.log' for more details." >&2;}
   { (exit 1); exit 1; }; }
    fi
  fi
fi
{ echo "$as_me:$LINENO: result: yes" >&5
echo "${ECHO_T}yes" >&6; }

rm -f a.out a.exe conftest$ac_cv_exeext b.out
ac_clean_files=$ac_clean_files_save
# Check that the compiler produces executables we can run.  If not, either
# the compiler is broken, or we cross compile.
{ echo "$as_me:$LINENO: checking whether we are cross compiling" >&5
echo $ECHO_N "checking whether we are cross compiling... $ECHO_C" >&6; }
{ echo "$as_me:$LINENO: result: $cross_compiling" >&5
echo "${ECHO_T}$cross_compiling" >&6; }

{ echo "$as_me:$LINENO: checking for suffix of executables" >&5
echo $ECHO_N "checking for suffix of executables... $ECHO_C" >&6; }
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; then
  # If both `conftest.exe' and `conftest' are `present' (well, observable)
# catch `conftest.exe'.  For instance with Cygwin, `ls conftest' will
# work properly (i.e., refer to `conftest.exe'), while it won't with
# `rm'.
for ac_file in conftest.exe conftest conftest.*; do
  test -f "$ac_file" || continue
  case $ac_file in
    *.$ac_ext | *.xcoff | *.tds | *.d | *.pdb | *.xSYM | *.bb | *.bbg | *.map | *.inf | *.o | *.obj ) ;;
    *.* ) ac_cv_exeext=`expr "$ac_file" : '[^.]*\(\..*\)'`
	  break;;
    * ) break;;
  esac
done
else
  { { echo "$as_me:$LINENO: error: cannot compute suffix of executables: cannot compile and link
See \`config.log' for more details." >&5
echo "$as_me: error: cannot compute suffix of executables: cannot compile and link
See \`config.log' for more details." >&2;}
   { (exit 1); exit 1; }; }
fi

rm -f conftest$ac_cv_exeext
{ echo "$as_me:$LINENO: result: $ac_cv_exeext" >&5
echo "${ECHO_T}$ac_cv_exeext" >&6; }

rm -f conftest.$ac_ext
EXEEXT=$ac_cv_exeext
ac_exeext=$EXEEXT
{ echo "$as_me:$LINENO: checking for suffix of object files" >&5
echo $ECHO_N "checking for suffix of object files... $ECHO_C" >&6; }
if test "${ac_cv_objext+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

int
main ()
{

  ;
  return 0;
}
_ACEOF
rm -f conftest.o conftest.obj
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; then
  for ac_file in conftest.o conftest.obj conftest.*; do
  test -f "$ac_file" || continue;
  case $ac_file in
    *.$ac_ext | *.xcoff | *.tds | *.d | *.pdb | *.xSYM | *.bb | *.bbg | *.map | *.inf ) ;;
    *) ac_cv_objext=`expr "$ac_file" : '.*\.\(.*\)'`
       break;;
  esac
done
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

{ { echo "$as_me:$LINENO: error: cannot compute suffix of object files: cannot compile
See \`config.log' for more details." >&5
echo "$as_me: error: cannot compute suffix of object files: cannot compile
See \`config.log' for more details." >&2;}
   { (exit 1); exit 1; }; }
fi

rm -f conftest.$ac_cv_objext conftest.$ac_ext
fi
{ echo "$as_me:$LINENO: result: $ac_cv_objext" >&5
echo "${ECHO_T}$ac_cv_objext" >&6; }
OBJEXT=$ac_cv_objext
ac_objext=$OBJEXT
{ echo "$as_me:$LINENO: checking whether we are using the GNU C compiler" >&5
echo $ECHO_N "checking whether we are using the GNU C compiler... $ECHO_C" >&6; }
if test "${ac_cv_c_compiler_gnu+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

int
main ()
{
#ifndef __GNUC__
       choke me
#endif

  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_c_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest.$ac_objext; then
  ac_compiler_gnu=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_compiler_gnu=no
fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext
ac_cv_c_compiler_gnu=$ac_compiler_gnu

fi
{ echo "$as_me:$LINENO: result: $ac_cv_c_compiler_gnu" >&5
echo "${ECHO_T}$ac_cv_c_compiler_gnu" >&6; }
GCC=`test $ac_compiler_gnu = yes && echo yes`
ac_test_CFLAGS=${CFLAGS+set}
ac_save_CFLAGS=$CFLAGS
{ echo "$as_me:$LINENO: checking whether $CC accepts -g" >&5
echo $ECHO_N "checking whether $CC accepts -g... $ECHO_C" >&6; }
if test "${ac_cv_prog_cc_g+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  ac_save_c_werror_flag=$ac_c_werror_flag
   ac_c_werror_flag=yes
   ac_cv_prog_cc_g=no
   CFLAGS="-g"
   cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

int
main ()
{

  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_c_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest.$ac_objext; then
  ac_cv_prog_cc_g=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	CFLAGS=""
      cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

int
main ()
{

  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_c_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest.$ac_objext; then
  :
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_c_werror_flag=$ac_save_c_werror_flag
	 CFLAGS="-g"
	 cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

int
main ()
{

  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_c_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest.$ac_objext; then
  ac_cv_prog_cc_g=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5


fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext
fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext
fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext
   ac_c_werror_flag=$ac_save_c_werror_flag
fi
{ echo "$as_me:$LINENO: result: $ac_cv_prog_cc_g" >&5
echo "${ECHO_T}$ac_cv_prog_cc_g" >&6; }
if test "$ac_test_CFLAGS" = set; then
  CFLAGS=$ac_save_CFLAGS
elif test $ac_cv_prog_cc_g = yes; then
  if test "$GCC" = yes; then
    CFLAGS="-g -O2"
  else
    CFLAGS="-g"
  fi
else
  if test "$GCC" = yes; then
    CFLAGS="-O2"
  else
    CFLAGS=
  fi
fi
{ echo "$as_me:$LINENO: checking for $CC option to accept ISO C89" >&5
echo $ECHO_N "checking for $CC option to accept ISO C89... $ECHO_C" >&6; }
if test "${ac_cv_prog_cc_c89+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  ac_cv_prog_cc_c89=no
ac_save_CC=$CC
cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#include <stdarg.h>
#include <stdio.h>
#include <sys/types.h>
#include <sys/stat.h>
/* Most of the following tests are stolen from RCS 5.7's src/conf.sh.  */
struct buf { int x; };
FILE * (*rcsopen) (struct buf *, struct stat *, int);
static char *e (p, i)
     char **p;
     int i;
{
  return p[i];
}
static char *f (char * (*g) (char **, int), char **p, ...)
{
  char *s;
  va_list v;
  va_start (v,p);
  s = g (p, va_arg (v,int));
  va_end (v);
  return s;
}

/* OSF 4.0 Compaq cc is some sort of almost-ANSI by default.  It has
   function prototypes and stuff, but not '\xHH' hex character constants.
   These don't provoke an error unfortunately, instead are silently treated
   as 'x'.  The following induces an error, until -std is added to get
   proper ANSI mode.  Curiously '\x00'!='x' always comes out true, for an
   array size at least.  It's necessary to write '\x00'==0 to get something
   that's true only with -std.  */
int osf4_cc_array ['\x00' == 0 ? 1 : -1];

/* IBM C 6 for AIX is almost-ANSI by default, but it replaces macro parameters
   inside strings and character constants.  */
#define FOO(x) 'x'
int xlc6_cc_array[FOO(a) == 'x' ? 1 : -1];

int test (int i, double x);
struct s1 {int (*f) (int a);};
struct s2 {int (*f) (double a);};
int pairnames (int, char **, FILE *(*)(struct buf *, struct stat *, int), int, int);
int argc;
char **argv;
int
main ()
{
return f (e, argv, 0) != argv[0]  ||  f (e, argv, 1) != argv[1];
  ;
  return 0;
}
_ACEOF
for ac_arg in '' -qlanglvl=extc89 -qlanglvl=ansi -std \
	-Ae "-Aa -D_HPUX_SOURCE" "-Xc -D__EXTENSIONS__"
do
  CC="$ac_save_CC $ac_arg"
  rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_c_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest.$ac_objext; then
  ac_cv_prog_cc_c89=$ac_arg
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5


fi

rm -f core conftest.err conftest.$ac_objext
  test "x$ac_cv_prog_cc_c89" != "xno" && break
done
rm -f conftest.$ac_ext
CC=$ac_save_CC

fi
# AC_CACHE_VAL
case "x$ac_cv_prog_cc_c89" in
  x)
    { echo "$as_me:$LINENO: result: none needed" >&5
echo "${ECHO_T}none needed" >&6; } ;;
  xno)
    { echo "$as_me:$LINENO: result: unsupported" >&5
echo "${ECHO_T}unsupported" >&6; } ;;
  *)
    CC="$CC $ac_cv_prog_cc_c89"
    { echo "$as_me:$LINENO: result: $ac_cv_prog_cc_c89" >&5
echo "${ECHO_T}$ac_cv_prog_cc_c89" >&6; } ;;
esac


ac_ext=c
ac_cpp='$CPP $CPPFLAGS'
ac_compile='$CC -c $CFLAGS $CPPFLAGS conftest.$ac_ext >&5'
ac_link='$CC -o conftest$ac_exeext $CFLAGS $CPPFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_c_compiler_gnu
DEPDIR="${am__leading_dot}deps"

ac_config_commands="$ac_config_commands depfiles"


am_make=${MAKE-make}
cat > confinc << 'END'
am__doit:
	@echo done
.PHONY: am__doit
END
# If we don't find an include directive, just comment out the code.
{ echo "$as_me:$LINENO: checking for style of include used by $am_make" >&5
echo $ECHO_N "checking for style of include used by $am_make... $ECHO_C" >&6; }
am__include="#"
am__quote=
_am_result=none
# First try GNU make style include.
echo "include confinc" > confmf
# We grep out `Entering directory' and `Leaving directory'
# messages which can occur if `w' ends up in MAKEFLAGS.
# In particular we don't look at `^make:' because GNU make might
# be invoked under some other name (usually "gmake"), in which
# case it prints its new name instead of `make'.
if test "`$am_make -s -f confmf 2> /dev/null | grep -v 'ing directory'`" = "done"; then
   am__include=include
   am__quote=
   _am_result=GNU
fi
# Now try BSD make style include.
if test "$am__include" = "#"; then
   echo '.include "confinc"' > confmf
   if test "`$am_make -s -f confmf 2> /dev/null`" = "done"; then
      am__include=.include
      am__quote="\""
      _am_result=BSD
   fi
fi


{ echo "$as_me:$LINENO: result: $_am_result" >&5
echo "${ECHO_T}$_am_result" >&6; }
rm -f confinc confmf

# Check whether --enable-dependency-tracking was given.
if test "${enable_dependency_tracking+set}" = set; then
  enableval=$enable_dependency_tracking;
fi

if test "x$enable_dependency_tracking" != xno; then
  am_depcomp="$ac_aux_dir/depcomp"
  AMDEPBACKSLASH='\'
fi
 if test "x$enable_dependency_tracking" != xno; then
  AMDEP_TRUE=
  AMDEP_FALSE='#'
else
  AMDEP_TRUE='#'
  AMDEP_FALSE=
fi



depcc="$CC"   am_compiler_list=

{ echo "$as_me:$LINENO: checking dependency style of $depcc" >&5
echo $ECHO_N "checking dependency style of $depcc... $ECHO_C" >&6; }
if test "${am_cv_CC_dependencies_compiler_type+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -z "$AMDEP_TRUE" && test -f "$am_depcomp"; then
  # We make a subdir and do the tests there.  Otherwise we can end up
  # making bogus files that we don't know about and never remove.  For
  # instance it was reported that on HP-UX the gcc test will end up
  # making a dummy file named `D' -- because `-MD' means `put the output
  # in D'.
  mkdir conftest.dir
  # Copy depcomp to subdir because otherwise we won't find it if we're
  # using a relative directory.
  cp "$am_depcomp" conftest.dir
  cd conftest.dir
  # We will build objects and dependencies in a subdirectory because
  # it helps to detect inapplicable dependency modes.  For instance
  # both Tru64's cc and ICC support -MD to output dependencies as a
  # side effect of compilation, but ICC will put the dependencies in
  # the current directory while Tru64 will put them in the object
  # directory.
  mkdir sub

  am_cv_CC_dependencies_compiler_type=none
  if test "$am_compiler_list" = ""; then
     am_compiler_list=`sed -n 's/^#*\([a-zA-Z0-9]*\))$/\1/p' < ./depcomp`
  fi
  for depmode in $am_compiler_list; do
    # Setup a source with many dependencies, because some compilers
    # like to wrap large dependency lists on column 80 (with \), and
    # we should not choose a depcomp mode which is confused by this.
    #
    # We need to recreate these files for each test, as the compiler may
    # overwrite some of them when testing with obscure command lines.
    # This happens at least with the AIX C compiler.
    : > sub/conftest.c
    for i in 1 2 3 4 5 6; do
      echo '#include "conftst'$i'.h"' >> sub/conftest.c
      # Using `: > sub/conftst$i.h' creates only sub/conftst1.h with
      # Solaris 8's {/usr,}/bin/sh.
      touch sub/conftst$i.h
    done
    echo "${am__include} ${am__quote}sub/conftest.Po${am__quote}" > confmf

    case $depmode in
    nosideeffect)
      # after this tag, mechanisms are not by side-effect, so they'll
      # only be used when explicitly requested
      if test "x$enable_dependency_tracking" = xyes; then
	continue
      else
	break
      fi
      ;;
    none) break ;;
    esac
    # We check with `-c' and `-o' for the sake of the "dashmstdout"
    # mode.  It turns out that the SunPro C++ compiler does not properly
    # handle `-M -o', and we need to detect this.
    if depmode=$depmode \
       source=sub/conftest.c object=sub/conftest.${OBJEXT-o} \
       depfile=sub/conftest.Po tmpdepfile=sub/conftest.TPo \
       $SHELL ./depcomp $depcc -c -o sub/conftest.${OBJEXT-o} sub/conftest.c \
         >/dev/null 2>conftest.err &&
       grep sub/conftst1.h sub/conftest.Po > /dev/null 2>&1 &&
       grep sub/conftst6.h sub/conftest.Po > /dev/null 2>&1 &&
       grep sub/conftest.${OBJEXT-o} sub/conftest.Po > /dev/null 2>&1 &&
       ${MAKE-make} -s -f confmf > /dev/null 2>&1; then
      # icc doesn't choke on unknown options, it will just issue warnings
      # or remarks (even with -Werror).  So we grep stderr for any message
      # that says an option was ignored or not supported.
      # When given -MP, icc 7.0 and 7.1 complain thusly:
      #   icc: Command line warning: ignoring option '-M'; no argument required
      # The diagnosis changed in icc 8.0:
      #   icc: Command line remark: option '-MP' not supported
      if (grep 'ignoring option' conftest.err ||
          grep 'not supported' conftest.err) >/dev/null 2>&1; then :; else
        am_cv_CC_dependencies_compiler_type=$depmode
        break
      fi
    fi
  done

  cd ..
  rm -rf conftest.dir
else
  am_cv_CC_dependencies_compiler_type=none
fi

fi
{ echo "$as_me:$LINENO: result: $am_cv_CC_dependencies_compiler_type" >&5
echo "${ECHO_T}$am_cv_CC_dependencies_compiler_type" >&6; }
CCDEPMODE=depmode=$am_cv_CC_dependencies_compiler_type

 if
  test "x$enable_dependency_tracking" != xno \
  && test "$am_cv_CC_dependencies_compiler_type" = gcc3; then
  am__fastdepCC_TRUE=
  am__fastdepCC_FALSE='#'
else
  am__fastdepCC_TRUE='#'
  am__fastdepCC_FALSE=
fi


ac_ext=cpp
ac_cpp='$CXXCPP $CPPFLAGS'
ac_compile='$CXX -c $CXXFLAGS $CPPFLAGS conftest.$ac_ext >&5'
ac_link='$CXX -o conftest$ac_exeext $CXXFLAGS $CPPFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_cxx_compiler_gnu
if test -z "$CXX"; then
  if test -n "$CCC"; then
    CXX=$CCC
  else
    if test -n "$ac_tool_prefix"; then
  for ac_prog in g++ c++ gpp aCC CC cxx cc++ cl.exe FCC KCC RCC xlC_r xlC
  do
    # Extract the first word of "$ac_tool_prefix$ac_prog", so it can be a program name with args.
set dummy $ac_tool_prefix$ac_prog; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_CXX+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$CXX"; then
  ac_cv_prog_CXX="$CXX" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_test_x "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_CXX="$ac_tool_prefix$ac_prog"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
CXX=$ac_cv_prog_CXX
if test -n "$CXX"; then
  { echo "$as_me:$LINENO: result: $CXX" >&5
echo "${ECHO_T}$CXX" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi


    test -n "$CXX" && break
  done
fi
if test -z "$CXX"; then
  ac_ct_CXX=$CXX
  for ac_prog in g++ c++ gpp aCC CC cxx cc++ cl.exe FCC KCC RCC xlC_r xlC
do
  # Extract the first word of "$ac_prog", so it can be a program name with args.
set dummy $ac_prog; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_ac_ct_CXX+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$ac_ct_CXX"; then
  ac_cv_prog_ac_ct_CXX="$ac_ct_CXX" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_test_x "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_ac_ct_CXX="$ac_prog"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
ac_ct_CXX=$ac_cv_prog_ac_ct_CXX
if test -n "$ac_ct_CXX"; then
  { echo "$as_me:$LINENO: result: $ac_ct_CXX" >&5
echo "${ECHO_T}$ac_ct_CXX" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi


  test -n "$ac_ct_CXX" && break
done

  if test "x$ac_ct_CXX" = x; then
    CXX="g++"
  else
    case $cross_compiling:$ac_tool_warned in
yes:)
{ echo "$as_me:$LINENO: WARNING: In the future, Autoconf will not detect cross-tools
whose name does not start with the host triplet.  If you think this
configuration is useful to you, please write to autoconf@gnu.org." >&5
echo "$as_me: WARNING: In the future, Autoconf will not detect cross-tools
whose name does not start with the host triplet.  If you think this
configuration is useful to you, please write to autoconf@gnu.org." >&2;}
ac_tool_warned=yes ;;
esac
    CXX=$ac_ct_CXX
  fi
fi

  fi
fi
# Provide some information about the compiler.
echo "$as_me:$LINENO: checking for C++ compiler version" >&5
ac_compiler=`set X $ac_compile; echo $2`
{ (ac_try="$ac_compiler --version >&5"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compiler --version >&5") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }
{ (ac_try="$ac_compiler -v >&5"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compiler -v >&5") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }
{ (ac_try="$ac_compiler -V >&5"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compiler -V >&5") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }

{ echo "$as_me:$LINENO: checking whether we are using the GNU C++ compiler" >&5
echo $ECHO_N "checking whether we are using the GNU C++ compiler... $ECHO_C" >&6; }
if test "${ac_cv_cxx_compiler_gnu+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

int
main ()
{
#ifndef __GNUC__
       choke me
#endif

  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_cxx_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest.$ac_objext; then
  ac_compiler_gnu=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_compiler_gnu=no
fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext
ac_cv_cxx_compiler_gnu=$ac_compiler_gnu

fi
{ echo "$as_me:$LINENO: result: $ac_cv_cxx_compiler_gnu" >&5
echo "${ECHO_T}$ac_cv_cxx_compiler_gnu" >&6; }
GXX=`test $ac_compiler_gnu = yes && echo yes`
ac_test_CXXFLAGS=${CXXFLAGS+set}
ac_save_CXXFLAGS=$CXXFLAGS
{ echo "$as_me:$LINENO: checking whether $CXX accepts -g" >&5
echo $ECHO_N "checking whether $CXX accepts -g... $ECHO_C" >&6; }
if test "${ac_cv_prog_cxx_g+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  ac_save_cxx_werror_flag=$ac_cxx_werror_flag
   ac_cxx_werror_flag=yes
   ac_cv_prog_cxx_g=no
   CXXFLAGS="-g"
   cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

int
main ()
{

  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_cxx_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest.$ac_objext; then
  ac_cv_prog_cxx_g=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	CXXFLAGS=""
      cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

int
main ()
{

  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_cxx_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest.$ac_objext; then
  :
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_cxx_werror_flag=$ac_save_cxx_werror_flag
	 CXXFLAGS="-g"
	 cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

int
main ()
{

  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_cxx_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest.$ac_objext; then
  ac_cv_prog_cxx_g=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5


fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext
fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext
fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext
   ac_cxx_werror_flag=$ac_save_cxx_werror_flag
fi
{ echo "$as_me:$LINENO: result: $ac_cv_prog_cxx_g" >&5
echo "${ECHO_T}$ac_cv_prog_cxx_g" >&6; }
if test "$ac_test_CXXFLAGS" = set; then
  CXXFLAGS=$ac_save_CXXFLAGS
elif test $ac_cv_prog_cxx_g = yes; then
  if test "$GXX" = yes; then
    CXXFLAGS="-g -O2"
  else
    CXXFLAGS="-g"
  fi
else
  if test "$GXX" = yes; then
    CXXFLAGS="-O2"
  else
    CXXFLAGS=
  fi
fi
ac_ext=c
ac_cpp='$CPP $CPPFLAGS'
ac_compile='$CC -c $CFLAGS $CPPFLAGS conftest.$ac_ext >&5'
ac_link='$CC -o conftest$ac_exeext $CFLAGS $CPPFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_c_compiler_gnu

depcc="$CXX"  am_compiler_list=

{ echo "$as_me:$LINENO: checking dependency style of $depcc" >&5
echo $ECHO_N "checking dependency style of $depcc... $ECHO_C" >&6; }
if test "${am_cv_CXX_dependencies_compiler_type+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -z "$AMDEP_TRUE" && test -f "$am_depcomp"; then
  # We make a subdir and do the tests there.  Otherwise we can end up
  # making bogus files that we don't know about and never remove.  For
  # instance it was reported that on HP-UX the gcc test will end up
  # making a dummy file named `D' -- because `-MD' means `put the output
  # in D'.
  mkdir conftest.dir
  # Copy depcomp to subdir because otherwise we won't find it if we're
  # using a relative directory.
  cp "$am_depcomp" conftest.dir
  cd conftest.dir
  # We will build objects and dependencies in a subdirectory because
  # it helps to detect inapplicable dependency modes.  For instance
  # both Tru64's cc and ICC support -MD to output dependencies as a
  # side effect of compilation, but ICC will put the dependencies in
  # the current directory while Tru64 will put them in the object
  # directory.
  mkdir sub

  am_cv_CXX_dependencies_compiler_type=none
  if test "$am_compiler_list" = ""; then
     am_compiler_list=`sed -n 's/^#*\([a-zA-Z0-9]*\))$/\1/p' < ./depcomp`
  fi
  for depmode in $am_compiler_list; do
    # Setup a source with many dependencies, because some compilers
    # like to wrap large dependency lists on column 80 (with \), and
    # we should not choose a depcomp mode which is confused by this.
    #
    # We need to recreate these files for each test, as the compiler may
    # overwrite some of them when testing with obscure command lines.
    # This happens at least with the AIX C compiler.
    : > sub/conftest.c
    for i in 1 2 3 4 5 6; do
      echo '#include "conftst'$i'.h"' >> sub/conftest.c
      # Using `: > sub/conftst$i.h' creates only sub/conftst1.h with
      # Solaris 8's {/usr,}/bin/sh.
      touch sub/conftst$i.h
    done
    echo "${am__include} ${am__quote}sub/conftest.Po${am__quote}" > confmf

    case $depmode in
    nosideeffect)
      # after this tag, mechanisms are not by side-effect, so they'll
      # only be used when explicitly requested
      if test "x$enable_dependency_tracking" = xyes; then
	continue
      else
	break
      fi
      ;;
    none) break ;;
    esac
    # We check with `-c' and `-o' for the sake of the "dashmstdout"
    # mode.  It turns out that the SunPro C++ compiler does not properly
    # handle `-M -o', and we need to detect this.
    if depmode=$depmode \
       source=sub/conftest.c object=sub/conftest.${OBJEXT-o} \
       depfile=sub/conftest.Po tmpdepfile=sub/conftest.TPo \
       $SHELL ./depcomp $depcc -c -o sub/conftest.${OBJEXT-o} sub/conftest.c \
         >/dev/null 2>conftest.err &&
       grep sub/conftst1.h sub/conftest.Po > /dev/null 2>&1 &&
       grep sub/conftst6.h sub/conftest.Po > /dev/null 2>&1 &&
       grep sub/conftest.${OBJEXT-o} sub/conftest.Po > /dev/null 2>&1 &&
       ${MAKE-make} -s -f confmf > /dev/null 2>&1; then
      # icc doesn't choke on unknown options, it will just issue warnings
      # or remarks (even with -Werror).  So we grep stderr for any message
      # that says an option was ignored or not supported.
      # When given -MP, icc 7.0 and 7.1 complain thusly:
      #   icc: Command line warning: ignoring option '-M'; no argument required
      # The diagnosis changed in icc 8.0:
      #   icc: Command line remark: option '-MP' not supported
      if (grep 'ignoring option' conftest.err ||
          grep 'not supported' conftest.err) >/dev/null 2>&1; then :; else
        am_cv_CXX_dependencies_compiler_type=$depmode
        break
      fi
    fi
  done

  cd ..
  rm -rf conftest.dir
else
  am_cv_CXX_dependencies_compiler_type=none
fi

fi
{ echo "$as_me:$LINENO: result: $am_cv_CXX_dependencies_compiler_type" >&5
echo "${ECHO_T}$am_cv_CXX_dependencies_compiler_type" >&6; }
CXXDEPMODE=depmode=$am_cv_CXX_dependencies_compiler_type

 if
  test "x$enable_dependency_tracking" != xno \
  && test "$am_cv_CXX_dependencies_compiler_type" = gcc3; then
  am__fastdepCXX_TRUE=
  am__fastdepCXX_FALSE='#'
else
  am__fastdepCXX_TRUE='#'
  am__fastdepCXX_FALSE=
fi


# Check whether --enable-static was given.
if test "${enable_static+set}" = set; then
  enableval=$enable_static; p=${PACKAGE-default}
    case $enableval in
    yes) enable_static=yes ;;
    no) enable_static=no ;;
    *)
     enable_static=no
      # Look at the argument we got.  We use all the common list separators.
      lt_save_ifs="$IFS"; IFS="${IFS}$PATH_SEPARATOR,"
      for pkg in $enableval; do
	IFS="$lt_save_ifs"
	if test "X$pkg" = "X$p"; then
	  enable_static=yes
	fi
      done
      IFS="$lt_save_ifs"
      ;;
    esac
else
  enable_static=no
fi


# Check whether --enable-shared was given.
if test "${enable_shared+set}" = set; then
  enableval=$enable_shared; p=${PACKAGE-default}
    case $enableval in
    yes) enable_shared=yes ;;
    no) enable_shared=no ;;
    *)
      enable_shared=no
      # Look at the argument we got.  We use all the common list separators.
      lt_save_ifs="$IFS"; IFS="${IFS}$PATH_SEPARATOR,"
      for pkg in $enableval; do
	IFS="$lt_save_ifs"
	if test "X$pkg" = "X$p"; then
	  enable_shared=yes
	fi
      done
      IFS="$lt_save_ifs"
      ;;
    esac
else
  enable_shared=yes
fi


# Check whether --enable-fast-install was given.
if test "${enable_fast_install+set}" = set; then
  enableval=$enable_fast_install; p=${PACKAGE-default}
    case $enableval in
    yes) enable_fast_install=yes ;;
    no) enable_fast_install=no ;;
    *)
      enable_fast_install=no
      # Look at the argument we got.  We use all the common list separators.
      lt_save_ifs="$IFS"; IFS="${IFS}$PATH_SEPARATOR,"
      for pkg in $enableval; do
	IFS="$lt_save_ifs"
	if test "X$pkg" = "X$p"; then
	  enable_fast_install=yes
	fi
      done
      IFS="$lt_save_ifs"
      ;;
    esac
else
  enable_fast_install=yes
fi


# Make sure we can run config.sub.
$SHELL "$ac_aux_dir/config.sub" sun4 >/dev/null 2>&1 ||
  { { echo "$as_me:$LINENO: error: cannot run $SHELL $ac_aux_dir/config.sub" >&5
echo "$as_me: error: cannot run $SHELL $ac_aux_dir/config.sub" >&2;}
   { (exit 1); exit 1; }; }

{ echo "$as_me:$LINENO: checking build system type" >&5
echo $ECHO_N "checking build system type... $ECHO_C" >&6; }
if test "${ac_cv_build+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  ac_build_alias=$build_alias
test "x$ac_build_alias" = x &&
  ac_build_alias=`$SHELL "$ac_aux_dir/config.guess"`
test "x$ac_build_alias" = x &&
  { { echo "$as_me:$LINENO: error: cannot guess build type; you must specify one" >&5
echo "$as_me: error: cannot guess build type; you must specify one" >&2;}
   { (exit 1); exit 1; }; }
ac_cv_build=`$SHELL "$ac_aux_dir/config.sub" $ac_build_alias` ||
  { { echo "$as_me:$LINENO: error: $SHELL $ac_aux_dir/config.sub $ac_build_alias failed" >&5
echo "$as_me: error: $SHELL $ac_aux_dir/config.sub $ac_build_alias failed" >&2;}
   { (exit 1); exit 1; }; }

fi
{ echo "$as_me:$LINENO: result: $ac_cv_build" >&5
echo "${ECHO_T}$ac_cv_build" >&6; }
case $ac_cv_build in
*-*-*) ;;
*) { { echo "$as_me:$LINENO: error: invalid value of canonical build" >&5
echo "$as_me: error: invalid value of canonical build" >&2;}
   { (exit 1); exit 1; }; };;
esac
build=$ac_cv_build
ac_save_IFS=$IFS; IFS='-'
set x $ac_cv_build
shift
build_cpu=$1
build_vendor=$2
shift; shift
# Remember, the first character of IFS is used to create $*,
# except with old shells:
build_os=$*
IFS=$ac_save_IFS
case $build_os in *\ *) build_os=`echo "$build_os" | sed 's/ /-/g'`;; esac


{ echo "$as_me:$LINENO: checking host system type" >&5
echo $ECHO_N "checking host system type... $ECHO_C" >&6; }
if test "${ac_cv_host+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test "x$host_alias" = x; then
  ac_cv_host=$ac_cv_build
else
  ac_cv_host=`$SHELL "$ac_aux_dir/config.sub" $host_alias` ||
    { { echo "$as_me:$LINENO: error: $SHELL $ac_aux_dir/config.sub $host_alias failed" >&5
echo "$as_me: error: $SHELL $ac_aux_dir/config.sub $host_alias failed" >&2;}
   { (exit 1); exit 1; }; }
fi

fi
{ echo "$as_me:$LINENO: result: $ac_cv_host" >&5
echo "${ECHO_T}$ac_cv_host" >&6; }
case $ac_cv_host in
*-*-*) ;;
*) { { echo "$as_me:$LINENO: error: invalid value of canonical host" >&5
echo "$as_me: error: invalid value of canonical host" >&2;}
   { (exit 1); exit 1; }; };;
esac
host=$ac_cv_host
ac_save_IFS=$IFS; IFS='-'
set x $ac_cv_host
shift
host_cpu=$1
host_vendor=$2
shift; shift
# Remember, the first character of IFS is used to create $*,
# except with old shells:
host_os=$*
IFS=$ac_save_IFS
case $host_os in *\ *) host_os=`echo "$host_os" | sed 's/ /-/g'`;; esac


{ echo "$as_me:$LINENO: checking for a sed that does not truncate output" >&5
echo $ECHO_N "checking for a sed that does not truncate output... $ECHO_C" >&6; }
if test "${lt_cv_path_SED+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  # Loop through the user's path and test for sed and gsed.
# Then use that list of sed's as ones to test for truncation.
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for lt_ac_prog in sed gsed; do
    for ac_exec_ext in '' $ac_executable_extensions; do
      if { test -f "$as_dir/$lt_ac_prog$ac_exec_ext" && $as_test_x "$as_dir/$lt_ac_prog$ac_exec_ext"; }; then
        lt_ac_sed_list="$lt_ac_sed_list $as_dir/$lt_ac_prog$ac_exec_ext"
      fi
    done
  done
done
IFS=$as_save_IFS
lt_ac_max=0
lt_ac_count=0
# Add /usr/xpg4/bin/sed as it is typically found on Solaris
# along with /bin/sed that truncates output.
for lt_ac_sed in $lt_ac_sed_list /usr/xpg4/bin/sed; do
  test ! -f $lt_ac_sed && continue
  cat /dev/null > conftest.in
  lt_ac_count=0
  echo $ECHO_N "0123456789$ECHO_C" >conftest.in
  # Check for GNU sed and select it if it is found.
  if "$lt_ac_sed" --version 2>&1 < /dev/null | grep 'GNU' > /dev/null; then
    lt_cv_path_SED=$lt_ac_sed
    break
  fi
  while true; do
    cat conftest.in conftest.in >conftest.tmp
    mv conftest.tmp conftest.in
    cp conftest.in conftest.nl
    echo >>conftest.nl
    $lt_ac_sed -e 's/a$//' < conftest.nl >conftest.out || break
    cmp -s conftest.out conftest.nl || break
    # 10000 chars as input seems more than enough
    test $lt_ac_count -gt 10 && break
    lt_ac_count=`expr $lt_ac_count + 1`
    if test $lt_ac_count -gt $lt_ac_max; then
      lt_ac_max=$lt_ac_count
      lt_cv_path_SED=$lt_ac_sed
    fi
  done
done

fi

SED=$lt_cv_path_SED

{ echo "$as_me:$LINENO: result: $SED" >&5
echo "${ECHO_T}$SED" >&6; }

{ echo "$as_me:$LINENO: checking for grep that handles long lines and -e" >&5
echo $ECHO_N "checking for grep that handles long lines and -e... $ECHO_C" >&6; }
if test "${ac_cv_path_GREP+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  # Extract the first word of "grep ggrep" to use in msg output
if test -z "$GREP"; then
set dummy grep ggrep; ac_prog_name=$2
if test "${ac_cv_path_GREP+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  ac_path_GREP_found=false
# Loop through the user's path and test for each of PROGNAME-LIST
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH$PATH_SEPARATOR/usr/xpg4/bin
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_prog in grep ggrep; do
  for ac_exec_ext in '' $ac_executable_extensions; do
    ac_path_GREP="$as_dir/$ac_prog$ac_exec_ext"
    { test -f "$ac_path_GREP" && $as_test_x "$ac_path_GREP"; } || continue
    # Check for GNU ac_path_GREP and select it if it is found.
  # Check for GNU $ac_path_GREP
case `"$ac_path_GREP" --version 2>&1` in
*GNU*)
  ac_cv_path_GREP="$ac_path_GREP" ac_path_GREP_found=:;;
*)
  ac_count=0
  echo $ECHO_N "0123456789$ECHO_C" >"conftest.in"
  while :
  do
    cat "conftest.in" "conftest.in" >"conftest.tmp"
    mv "conftest.tmp" "conftest.in"
    cp "conftest.in" "conftest.nl"
    echo 'GREP' >> "conftest.nl"
    "$ac_path_GREP" -e 'GREP$' -e '-(cannot match)-' < "conftest.nl" >"conftest.out" 2>/dev/null || break
    diff "conftest.out" "conftest.nl" >/dev/null 2>&1 || break
    ac_count=`expr $ac_count + 1`
    if test $ac_count -gt ${ac_path_GREP_max-0}; then
      # Best one so far, save it but keep looking for a better one
      ac_cv_path_GREP="$ac_path_GREP"
      ac_path_GREP_max=$ac_count
    fi
    # 10*(2^10) chars as input seems more than enough
    test $ac_count -gt 10 && break
  done
  rm -f conftest.in conftest.tmp conftest.nl conftest.out;;
esac


    $ac_path_GREP_found && break 3
  done
done

done
IFS=$as_save_IFS


fi

GREP="$ac_cv_path_GREP"
if test -z "$GREP"; then
  { { echo "$as_me:$LINENO: error: no acceptable $ac_prog_name could be found in $PATH$PATH_SEPARATOR/usr/xpg4/bin" >&5
echo "$as_me: error: no acceptable $ac_prog_name could be found in $PATH$PATH_SEPARATOR/usr/xpg4/bin" >&2;}
   { (exit 1); exit 1; }; }
fi

else
  ac_cv_path_GREP=$GREP
fi


fi
{ echo "$as_me:$LINENO: result: $ac_cv_path_GREP" >&5
echo "${ECHO_T}$ac_cv_path_GREP" >&6; }
 GREP="$ac_cv_path_GREP"


{ echo "$as_me:$LINENO: checking for egrep" >&5
echo $ECHO_N "checking for egrep... $ECHO_C" >&6; }
if test "${ac_cv_path_EGREP+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if echo a | $GREP -E '(a|b)' >/dev/null 2>&1
   then ac_cv_path_EGREP="$GREP -E"
   else
     # Extract the first word of "egrep" to use in msg output
if test -z "$EGREP"; then
set dummy egrep; ac_prog_name=$2
if test "${ac_cv_path_EGREP+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  ac_path_EGREP_found=false
# Loop through the user's path and test for each of PROGNAME-LIST
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH$PATH_SEPARATOR/usr/xpg4/bin
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_prog in egrep; do
  for ac_exec_ext in '' $ac_executable_extensions; do
    ac_path_EGREP="$as_dir/$ac_prog$ac_exec_ext"
    { test -f "$ac_path_EGREP" && $as_test_x "$ac_path_EGREP"; } || continue
    # Check for GNU ac_path_EGREP and select it if it is found.
  # Check for GNU $ac_path_EGREP
case `"$ac_path_EGREP" --version 2>&1` in
*GNU*)
  ac_cv_path_EGREP="$ac_path_EGREP" ac_path_EGREP_found=:;;
*)
  ac_count=0
  echo $ECHO_N "0123456789$ECHO_C" >"conftest.in"
  while :
  do
    cat "conftest.in" "conftest.in" >"conftest.tmp"
    mv "conftest.tmp" "conftest.in"
    cp "conftest.in" "conftest.nl"
    echo 'EGREP' >> "conftest.nl"
    "$ac_path_EGREP" 'EGREP$' < "conftest.nl" >"conftest.out" 2>/dev/null || break
    diff "conftest.out" "conftest.nl" >/dev/null 2>&1 || break
    ac_count=`expr $ac_count + 1`
    if test $ac_count -gt ${ac_path_EGREP_max-0}; then
      # Best one so far, save it but keep looking for a better one
      ac_cv_path_EGREP="$ac_path_EGREP"
      ac_path_EGREP_max=$ac_count
    fi
    # 10*(2^10) chars as input seems more than enough
    test $ac_count -gt 10 && break
  done
  rm -f conftest.in conftest.tmp conftest.nl conftest.out;;
esac


    $ac_path_EGREP_found && break 3
  done
done

done
IFS=$as_save_IFS


fi

EGREP="$ac_cv_path_EGREP"
if test -z "$EGREP"; then
  { { echo "$as_me:$LINENO: error: no acceptable $ac_prog_name could be found in $PATH$PATH_SEPARATOR/usr/xpg4/bin" >&5
echo "$as_me: error: no acceptable $ac_prog_name could be found in $PATH$PATH_SEPARATOR/usr/xpg4/bin" >&2;}
   { (exit 1); exit 1; }; }
fi

else
  ac_cv_path_EGREP=$EGREP
fi


   fi
fi
{ echo "$as_me:$LINENO: result: $ac_cv_path_EGREP" >&5
echo "${ECHO_T}$ac_cv_path_EGREP" >&6; }
 EGREP="$ac_cv_path_EGREP"



# Check whether --with-gnu-ld was given.
if test "${with_gnu_ld+set}" = set; then
  withval=$with_gnu_ld; test "$withval" = no || with_gnu_ld=yes
else
  with_gnu_ld=no
fi

ac_prog=ld
if test "$GCC" = yes; then
  # Check if gcc -print-prog-name=ld gives a path.
  { echo "$as_me:$LINENO: checking for ld used by $CC" >&5
echo $ECHO_N "checking for ld used by $CC... $ECHO_C" >&6; }
  case $host in
  *-*-mingw*)
    # gcc leaves a trailing carriage return which upsets mingw
    ac_prog=`($CC -print-prog-name=ld) 2>&5 | tr -d '\015'` ;;
  *)
    ac_prog=`($CC -print-prog-name=ld) 2>&5` ;;
  esac
  case $ac_prog in
    # Accept absolute paths.
    [\\/]* | ?:[\\/]*)
      re_direlt='/[^/][^/]*/\.\./'
      # Canonicalize the pathname of ld
      ac_prog=`echo $ac_prog| $SED 's%\\\\%/%g'`
      while echo $ac_prog | grep "$re_direlt" > /dev/null 2>&1; do
	ac_prog=`echo $ac_prog| $SED "s%$re_direlt%/%"`
      done
      test -z "$LD" && LD="$ac_prog"
      ;;
  "")
    # If it fails, then pretend we aren't using GCC.
    ac_prog=ld
    ;;
  *)
    # If it is relative, then search for the first ld in PATH.
    with_gnu_ld=unknown
    ;;
  esac
elif test "$with_gnu_ld" = yes; then
  { echo "$as_me:$LINENO: checking for GNU ld" >&5
echo $ECHO_N "checking for GNU ld... $ECHO_C" >&6; }
else
  { echo "$as_me:$LINENO: checking for non-GNU ld" >&5
echo $ECHO_N "checking for non-GNU ld... $ECHO_C" >&6; }
fi
if test "${lt_cv_path_LD+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -z "$LD"; then
  lt_save_ifs="$IFS"; IFS=$PATH_SEPARATOR
  for ac_dir in $PATH; do
    IFS="$lt_save_ifs"
    test -z "$ac_dir" && ac_dir=.
    if test -f "$ac_dir/$ac_prog" || test -f "$ac_dir/$ac_prog$ac_exeext"; then
      lt_cv_path_LD="$ac_dir/$ac_prog"
      # Check to see if the program is GNU ld.  I'd rather use --version,
      # but apparently some variants of GNU ld only accept -v.
      # Break only if it was the GNU/non-GNU ld that we prefer.
      case `"$lt_cv_path_LD" -v 2>&1 </dev/null` in
      *GNU* | *'with BFD'*)
	test "$with_gnu_ld" != no && break
	;;
      *)
	test "$with_gnu_ld" != yes && break
	;;
      esac
    fi
  done
  IFS="$lt_save_ifs"
else
  lt_cv_path_LD="$LD" # Let the user override the test with a path.
fi
fi

LD="$lt_cv_path_LD"
if test -n "$LD"; then
  { echo "$as_me:$LINENO: result: $LD" >&5
echo "${ECHO_T}$LD" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi
test -z "$LD" && { { echo "$as_me:$LINENO: error: no acceptable ld found in \$PATH" >&5
echo "$as_me: error: no acceptable ld found in \$PATH" >&2;}
   { (exit 1); exit 1; }; }
{ echo "$as_me:$LINENO: checking if the linker ($LD) is GNU ld" >&5
echo $ECHO_N "checking if the linker ($LD) is GNU ld... $ECHO_C" >&6; }
if test "${lt_cv_prog_gnu_ld+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  # I'd rather use --version here, but apparently some GNU lds only accept -v.
case `$LD -v 2>&1 </dev/null` in
*GNU* | *'with BFD'*)
  lt_cv_prog_gnu_ld=yes
  ;;
*)
  lt_cv_prog_gnu_ld=no
  ;;
esac
fi
{ echo "$as_me:$LINENO: result: $lt_cv_prog_gnu_ld" >&5
echo "${ECHO_T}$lt_cv_prog_gnu_ld" >&6; }
with_gnu_ld=$lt_cv_prog_gnu_ld


{ echo "$as_me:$LINENO: checking for $LD option to reload object files" >&5
echo $ECHO_N "checking for $LD option to reload object files... $ECHO_C" >&6; }
if test "${lt_cv_ld_reload_flag+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  lt_cv_ld_reload_flag='-r'
fi
{ echo "$as_me:$LINENO: result: $lt_cv_ld_reload_flag" >&5
echo "${ECHO_T}$lt_cv_ld_reload_flag" >&6; }
reload_flag=$lt_cv_ld_reload_flag
case $reload_flag in
"" | " "*) ;;
*) reload_flag=" $reload_flag" ;;
esac
reload_cmds='$LD$reload_flag -o $output$reload_objs'
case $host_os in
  darwin*)
    if test "$GCC" = yes; then
      reload_cmds='$LTCC $LTCFLAGS -nostdlib ${wl}-r -o $output$reload_objs'
    else
      reload_cmds='$LD$reload_flag -o $output$reload_objs'
    fi
    ;;
esac

{ echo "$as_me:$LINENO: checking for BSD-compatible nm" >&5
echo $ECHO_N "checking for BSD-compatible nm... $ECHO_C" >&6; }
if test "${lt_cv_path_NM+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$NM"; then
  # Let the user override the test.
  lt_cv_path_NM="$NM"
else
  lt_nm_to_check="${ac_tool_prefix}nm"
  if test -n "$ac_tool_prefix" && test "$build" = "$host"; then
    lt_nm_to_check="$lt_nm_to_check nm"
  fi
  for lt_tmp_nm in $lt_nm_to_check; do
    lt_save_ifs="$IFS"; IFS=$PATH_SEPARATOR
    for ac_dir in $PATH /usr/ccs/bin/elf /usr/ccs/bin /usr/ucb /bin; do
      IFS="$lt_save_ifs"
      test -z "$ac_dir" && ac_dir=.
      tmp_nm="$ac_dir/$lt_tmp_nm"
      if test -f "$tmp_nm" || test -f "$tmp_nm$ac_exeext" ; then
	# Check to see if the nm accepts a BSD-compat flag.
	# Adding the `sed 1q' prevents false positives on HP-UX, which says:
	#   nm: unknown option "B" ignored
	# Tru64's nm complains that /dev/null is an invalid object file
	case `"$tmp_nm" -B /dev/null 2>&1 | sed '1q'` in
	*/dev/null* | *'Invalid file or object type'*)
	  lt_cv_path_NM="$tmp_nm -B"
	  break
	  ;;
	*)
	  case `"$tmp_nm" -p /dev/null 2>&1 | sed '1q'` in
	  */dev/null*)
	    lt_cv_path_NM="$tmp_nm -p"
	    break
	    ;;
	  *)
	    lt_cv_path_NM=${lt_cv_path_NM="$tmp_nm"} # keep the first match, but
	    continue # so that we can try to find one that supports BSD flags
	    ;;
	  esac
	  ;;
	esac
      fi
    done
    IFS="$lt_save_ifs"
  done
  test -z "$lt_cv_path_NM" && lt_cv_path_NM=nm
fi
fi
{ echo "$as_me:$LINENO: result: $lt_cv_path_NM" >&5
echo "${ECHO_T}$lt_cv_path_NM" >&6; }
NM="$lt_cv_path_NM"

{ echo "$as_me:$LINENO: checking whether ln -s works" >&5
echo $ECHO_N "checking whether ln -s works... $ECHO_C" >&6; }
LN_S=$as_ln_s
if test "$LN_S" = "ln -s"; then
  { echo "$as_me:$LINENO: result: yes" >&5
echo "${ECHO_T}yes" >&6; }
else
  { echo "$as_me:$LINENO: result: no, using $LN_S" >&5
echo "${ECHO_T}no, using $LN_S" >&6; }
fi

{ echo "$as_me:$LINENO: checking how to recognize dependent libraries" >&5
echo $ECHO_N "checking how to recognize dependent libraries... $ECHO_C" >&6; }
if test "${lt_cv_deplibs_check_method+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  lt_cv_file_magic_cmd='$MAGIC_CMD'
lt_cv_file_magic_test_file=
lt_cv_deplibs_check_method='unknown'
# Need to set the preceding variable on all platforms that support
# interlibrary dependencies.
# 'none' -- dependencies not supported.
# `unknown' -- same as none, but documents that we really don't know.
# 'pass_all' -- all dependencies passed with no checks.
# 'test_compile' -- check by making test program.
# 'file_magic [[regex]]' -- check by looking for files in library path
# which responds to the $file_magic_cmd with a given extended regex.
# If you have `file' or equivalent on your system and you're not sure
# whether `pass_all' will *always* work, you probably want this one.

case $host_os in
aix4* | aix5*)
  lt_cv_deplibs_check_method=pass_all
  ;;

beos*)
  lt_cv_deplibs_check_method=pass_all
  ;;

bsdi[45]*)
  lt_cv_deplibs_check_method='file_magic ELF [0-9][0-9]*-bit [ML]SB (shared object|dynamic lib)'
  lt_cv_file_magic_cmd='/usr/bin/file -L'
  lt_cv_file_magic_test_file=/shlib/libc.so
  ;;

cygwin*)
  # func_win32_libid is a shell function defined in ltmain.sh
  lt_cv_deplibs_check_method='file_magic ^x86 archive import|^x86 DLL'
  lt_cv_file_magic_cmd='func_win32_libid'
  ;;

mingw* | pw32*)
  # Base MSYS/MinGW do not provide the 'file' command needed by
  # func_win32_libid shell function, so use a weaker test based on 'objdump',
  # unless we find 'file', for example because we are cross-compiling.
  if ( file / ) >/dev/null 2>&1; then
    lt_cv_deplibs_check_method='file_magic ^x86 archive import|^x86 DLL'
    lt_cv_file_magic_cmd='func_win32_libid'
  else
    lt_cv_deplibs_check_method='file_magic file format pei*-i386(.*architecture: i386)?'
    lt_cv_file_magic_cmd='$OBJDUMP -f'
  fi
  ;;

darwin* | rhapsody*)
  lt_cv_deplibs_check_method=pass_all
  ;;

freebsd* | dragonfly*)
  if echo __ELF__ | $CC -E - | grep __ELF__ > /dev/null; then
    case $host_cpu in
    i*86 )
      # Not sure whether the presence of OpenBSD here was a mistake.
      # Let's accept both of them until this is cleared up.
      lt_cv_deplibs_check_method='file_magic (FreeBSD|OpenBSD|DragonFly)/i[3-9]86 (compact )?demand paged shared library'
      lt_cv_file_magic_cmd=/usr/bin/file
      lt_cv_file_magic_test_file=`echo /usr/lib/libc.so.*`
      ;;
    esac
  else
    lt_cv_deplibs_check_method=pass_all
  fi
  ;;

gnu*)
  lt_cv_deplibs_check_method=pass_all
  ;;

hpux10.20* | hpux11*)
  lt_cv_file_magic_cmd=/usr/bin/file
  case $host_cpu in
  ia64*)
    lt_cv_deplibs_check_method='file_magic (s[0-9][0-9][0-9]|ELF-[0-9][0-9]) shared object file - IA64'
    lt_cv_file_magic_test_file=/usr/lib/hpux32/libc.so
    ;;
  hppa*64*)
    lt_cv_deplibs_check_method='file_magic (s[0-9][0-9][0-9]|ELF-[0-9][0-9]) shared object file - PA-RISC [0-9].[0-9]'
    lt_cv_file_magic_test_file=/usr/lib/pa20_64/libc.sl
    ;;
  *)
    lt_cv_deplibs_check_method='file_magic (s[0-9][0-9][0-9]|PA-RISC[0-9].[0-9]) shared library'
    lt_cv_file_magic_test_file=/usr/lib/libc.sl
    ;;
  esac
  ;;

interix[3-9]*)
  # PIC code is broken on Interix 3.x, that's why |\.a not |_pic\.a here
  lt_cv_deplibs_check_method='match_pattern /lib[^/]+(\.so|\.a)$'
  ;;

irix5* | irix6* | nonstopux*)
  case $LD in
  *-32|*"-32 ") libmagic=32-bit;;
  *-n32|*"-n32 ") libmagic=N32;;
  *-64|*"-64 ") libmagic=64-bit;;
  *) libmagic=never-match;;
  esac
  lt_cv_deplibs_check_method=pass_all
  ;;

# This must be Linux ELF.
linux* | k*bsd*-gnu)
  lt_cv_deplibs_check_method=pass_all
  ;;

netbsd*)
  if echo __ELF__ | $CC -E - | grep __ELF__ > /dev/null; then
    lt_cv_deplibs_check_method='match_pattern /lib[^/]+(\.so\.[0-9]+\.[0-9]+|_pic\.a)$'
  else
    lt_cv_deplibs_check_method='match_pattern /lib[^/]+(\.so|_pic\.a)$'
  fi
  ;;

newos6*)
  lt_cv_deplibs_check_method='file_magic ELF [0-9][0-9]*-bit [ML]SB (executable|dynamic lib)'
  lt_cv_file_magic_cmd=/usr/bin/file
  lt_cv_file_magic_test_file=/usr/lib/libnls.so
  ;;

nto-qnx*)
  lt_cv_deplibs_check_method=unknown
  ;;

openbsd*)
  if test -z "`echo __ELF__ | $CC -E - | grep __ELF__`" || test "$host_os-$host_cpu" = "openbsd2.8-powerpc"; then
    lt_cv_deplibs_check_method='match_pattern /lib[^/]+(\.so\.[0-9]+\.[0-9]+|\.so|_pic\.a)$'
  else
    lt_cv_deplibs_check_method='match_pattern /lib[^/]+(\.so\.[0-9]+\.[0-9]+|_pic\.a)$'
  fi
  ;;

osf3* | osf4* | osf5*)
  lt_cv_deplibs_check_method=pass_all
  ;;

rdos*)
  lt_cv_deplibs_check_method=pass_all
  ;;

solaris*)
  lt_cv_deplibs_check_method=pass_all
  ;;

sysv4 | sysv4.3*)
  case $host_vendor in
  motorola)
    lt_cv_deplibs_check_method='file_magic ELF [0-9][0-9]*-bit [ML]SB (shared object|dynamic lib) M[0-9][0-9]* Version [0-9]'
    lt_cv_file_magic_test_file=`echo /usr/lib/libc.so*`
    ;;
  ncr)
    lt_cv_deplibs_check_method=pass_all
    ;;
  sequent)
    lt_cv_file_magic_cmd='/bin/file'
    lt_cv_deplibs_check_method='file_magic ELF [0-9][0-9]*-bit [LM]SB (shared object|dynamic lib )'
    ;;
  sni)
    lt_cv_file_magic_cmd='/bin/file'
    lt_cv_deplibs_check_method="file_magic ELF [0-9][0-9]*-bit [LM]SB dynamic lib"
    lt_cv_file_magic_test_file=/lib/libc.so
    ;;
  siemens)
    lt_cv_deplibs_check_method=pass_all
    ;;
  pc)
    lt_cv_deplibs_check_method=pass_all
    ;;
  esac
  ;;

sysv5* | sco3.2v5* | sco5v6* | unixware* | OpenUNIX* | sysv4*uw2*)
  lt_cv_deplibs_check_method=pass_all
  ;;
esac

fi
{ echo "$as_me:$LINENO: result: $lt_cv_deplibs_check_method" >&5
echo "${ECHO_T}$lt_cv_deplibs_check_method" >&6; }
file_magic_cmd=$lt_cv_file_magic_cmd
deplibs_check_method=$lt_cv_deplibs_check_method
test -z "$deplibs_check_method" && deplibs_check_method=unknown




# If no C compiler was specified, use CC.
LTCC=${LTCC-"$CC"}

# If no C compiler flags were specified, use CFLAGS.
LTCFLAGS=${LTCFLAGS-"$CFLAGS"}

# Allow CC to be a program name with arguments.
compiler=$CC


# Check whether --enable-libtool-lock was given.
if test "${enable_libtool_lock+set}" = set; then
  enableval=$enable_libtool_lock;
fi

test "x$enable_libtool_lock" != xno && enable_libtool_lock=yes

# Some flags need to be propagated to the compiler or linker for good
# libtool support.
case $host in
ia64-*-hpux*)
  # Find out which ABI we are using.
  echo 'int i;' > conftest.$ac_ext
  if { (eval echo "$as_me:$LINENO: \"$ac_compile\"") >&5
  (eval $ac_compile) 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; then
    case `/usr/bin/file conftest.$ac_objext` in
    *ELF-32*)
      HPUX_IA64_MODE="32"
      ;;
    *ELF-64*)
      HPUX_IA64_MODE="64"
      ;;
    esac
  fi
  rm -rf conftest*
  ;;
*-*-irix6*)
  # Find out which ABI we are using.
  echo '#line 4793 "configure"' > conftest.$ac_ext
  if { (eval echo "$as_me:$LINENO: \"$ac_compile\"") >&5
  (eval $ac_compile) 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; then
   if test "$lt_cv_prog_gnu_ld" = yes; then
    case `/usr/bin/file conftest.$ac_objext` in
    *32-bit*)
      LD="${LD-ld} -melf32bsmip"
      ;;
    *N32*)
      LD="${LD-ld} -melf32bmipn32"
      ;;
    *64-bit*)
      LD="${LD-ld} -melf64bmip"
      ;;
    esac
   else
    case `/usr/bin/file conftest.$ac_objext` in
    *32-bit*)
      LD="${LD-ld} -32"
      ;;
    *N32*)
      LD="${LD-ld} -n32"
      ;;
    *64-bit*)
      LD="${LD-ld} -64"
      ;;
    esac
   fi
  fi
  rm -rf conftest*
  ;;

x86_64-*kfreebsd*-gnu|x86_64-*linux*|ppc*-*linux*|powerpc*-*linux*| \
s390*-*linux*|sparc*-*linux*)
  # Find out which ABI we are using.
  echo 'int i;' > conftest.$ac_ext
  if { (eval echo "$as_me:$LINENO: \"$ac_compile\"") >&5
  (eval $ac_compile) 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; then
    case `/usr/bin/file conftest.o` in
    *32-bit*)
      case $host in
        x86_64-*kfreebsd*-gnu)
          LD="${LD-ld} -m elf_i386_fbsd"
          ;;
        x86_64-*linux*)
          LD="${LD-ld} -m elf_i386"
          ;;
        ppc64-*linux*|powerpc64-*linux*)
          LD="${LD-ld} -m elf32ppclinux"
          ;;
        s390x-*linux*)
          LD="${LD-ld} -m elf_s390"
          ;;
        sparc64-*linux*)
          LD="${LD-ld} -m elf32_sparc"
          ;;
      esac
      ;;
    *64-bit*)
      case $host in
        x86_64-*kfreebsd*-gnu)
          LD="${LD-ld} -m elf_x86_64_fbsd"
          ;;
        x86_64-*linux*)
          LD="${LD-ld} -m elf_x86_64"
          ;;
        ppc*-*linux*|powerpc*-*linux*)
          LD="${LD-ld} -m elf64ppc"
          ;;
        s390*-*linux*)
          LD="${LD-ld} -m elf64_s390"
          ;;
        sparc*-*linux*)
          LD="${LD-ld} -m elf64_sparc"
          ;;
      esac
      ;;
    esac
  fi
  rm -rf conftest*
  ;;

*-*-sco3.2v5*)
  # On SCO OpenServer 5, we need -belf to get full-featured binaries.
  SAVE_CFLAGS="$CFLAGS"
  CFLAGS="$CFLAGS -belf"
  { echo "$as_me:$LINENO: checking whether the C compiler needs -belf" >&5
echo $ECHO_N "checking whether the C compiler needs -belf... $ECHO_C" >&6; }
if test "${lt_cv_cc_needs_belf+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  ac_ext=c
ac_cpp='$CPP $CPPFLAGS'
ac_compile='$CC -c $CFLAGS $CPPFLAGS conftest.$ac_ext >&5'
ac_link='$CC -o conftest$ac_exeext $CFLAGS $CPPFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_c_compiler_gnu

     cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

int
main ()
{

  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_c_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest$ac_exeext &&
       $as_test_x conftest$ac_exeext; then
  lt_cv_cc_needs_belf=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	lt_cv_cc_needs_belf=no
fi

rm -f core conftest.err conftest.$ac_objext conftest_ipa8_conftest.oo \
      conftest$ac_exeext conftest.$ac_ext
     ac_ext=c
ac_cpp='$CPP $CPPFLAGS'
ac_compile='$CC -c $CFLAGS $CPPFLAGS conftest.$ac_ext >&5'
ac_link='$CC -o conftest$ac_exeext $CFLAGS $CPPFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_c_compiler_gnu

fi
{ echo "$as_me:$LINENO: result: $lt_cv_cc_needs_belf" >&5
echo "${ECHO_T}$lt_cv_cc_needs_belf" >&6; }
  if test x"$lt_cv_cc_needs_belf" != x"yes"; then
    # this is probably gcc 2.8.0, egcs 1.0 or newer; no need for -belf
    CFLAGS="$SAVE_CFLAGS"
  fi
  ;;
sparc*-*solaris*)
  # Find out which ABI we are using.
  echo 'int i;' > conftest.$ac_ext
  if { (eval echo "$as_me:$LINENO: \"$ac_compile\"") >&5
  (eval $ac_compile) 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; then
    case `/usr/bin/file conftest.o` in
    *64-bit*)
      case $lt_cv_prog_gnu_ld in
      yes*) LD="${LD-ld} -m elf64_sparc" ;;
      *)    LD="${LD-ld} -64" ;;
      esac
      ;;
    esac
  fi
  rm -rf conftest*
  ;;


esac

need_locks="$enable_libtool_lock"


ac_ext=c
ac_cpp='$CPP $CPPFLAGS'
ac_compile='$CC -c $CFLAGS $CPPFLAGS conftest.$ac_ext >&5'
ac_link='$CC -o conftest$ac_exeext $CFLAGS $CPPFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_c_compiler_gnu
{ echo "$as_me:$LINENO: checking how to run the C preprocessor" >&5
echo $ECHO_N "checking how to run the C preprocessor... $ECHO_C" >&6; }
# On Suns, sometimes $CPP names a directory.
if test -n "$CPP" && test -d "$CPP"; then
  CPP=
fi
if test -z "$CPP"; then
  if test "${ac_cv_prog_CPP+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
      # Double quotes because CPP needs to be expanded
    for CPP in "$CC -E" "$CC -E -traditional-cpp" "/lib/cpp"
    do
      ac_preproc_ok=false
for ac_c_preproc_warn_flag in '' yes
do
  # Use a header file that comes with gcc, so configuring glibc
  # with a fresh cross-compiler works.
  # Prefer <limits.h> to <assert.h> if __STDC__ is defined, since
  # <limits.h> exists even on freestanding compilers.
  # On the NeXT, cc -E runs the code through the compiler's parser,
  # not just through cpp. "Syntax error" is here to catch this case.
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#ifdef __STDC__
# include <limits.h>
#else
# include <assert.h>
#endif
		     Syntax error
_ACEOF
if { (ac_try="$ac_cpp conftest.$ac_ext"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_cpp conftest.$ac_ext") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } >/dev/null && {
	 test -z "$ac_c_preproc_warn_flag$ac_c_werror_flag" ||
	 test ! -s conftest.err
       }; then
  :
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

  # Broken: fails on valid input.
continue
fi

rm -f conftest.err conftest.$ac_ext

  # OK, works on sane cases.  Now check whether nonexistent headers
  # can be detected and how.
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#include <ac_nonexistent.h>
_ACEOF
if { (ac_try="$ac_cpp conftest.$ac_ext"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_cpp conftest.$ac_ext") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } >/dev/null && {
	 test -z "$ac_c_preproc_warn_flag$ac_c_werror_flag" ||
	 test ! -s conftest.err
       }; then
  # Broken: success on invalid input.
continue
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

  # Passes both tests.
ac_preproc_ok=:
break
fi

rm -f conftest.err conftest.$ac_ext

done
# Because of `break', _AC_PREPROC_IFELSE's cleaning code was skipped.
rm -f conftest.err conftest.$ac_ext
if $ac_preproc_ok; then
  break
fi

    done
    ac_cv_prog_CPP=$CPP

fi
  CPP=$ac_cv_prog_CPP
else
  ac_cv_prog_CPP=$CPP
fi
{ echo "$as_me:$LINENO: result: $CPP" >&5
echo "${ECHO_T}$CPP" >&6; }
ac_preproc_ok=false
for ac_c_preproc_warn_flag in '' yes
do
  # Use a header file that comes with gcc, so configuring glibc
  # with a fresh cross-compiler works.
  # Prefer <limits.h> to <assert.h> if __STDC__ is defined, since
  # <limits.h> exists even on freestanding compilers.
  # On the NeXT, cc -E runs the code through the compiler's parser,
  # not just through cpp. "Syntax error" is here to catch this case.
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#ifdef __STDC__
# include <limits.h>
#else
# include <assert.h>
#endif
		     Syntax error
_ACEOF
if { (ac_try="$ac_cpp conftest.$ac_ext"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_cpp conftest.$ac_ext") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } >/dev/null && {
	 test -z "$ac_c_preproc_warn_flag$ac_c_werror_flag" ||
	 test ! -s conftest.err
       }; then
  :
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

  # Broken: fails on valid input.
continue
fi

rm -f conftest.err conftest.$ac_ext

  # OK, works on sane cases.  Now check whether nonexistent headers
  # can be detected and how.
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#include <ac_nonexistent.h>
_ACEOF
if { (ac_try="$ac_cpp conftest.$ac_ext"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_cpp conftest.$ac_ext") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } >/dev/null && {
	 test -z "$ac_c_preproc_warn_flag$ac_c_werror_flag" ||
	 test ! -s conftest.err
       }; then
  # Broken: success on invalid input.
continue
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

  # Passes both tests.
ac_preproc_ok=:
break
fi

rm -f conftest.err conftest.$ac_ext

done
# Because of `break', _AC_PREPROC_IFELSE's cleaning code was skipped.
rm -f conftest.err conftest.$ac_ext
if $ac_preproc_ok; then
  :
else
  { { echo "$as_me:$LINENO: error: C preprocessor \"$CPP\" fails sanity check
See \`config.log' for more details." >&5
echo "$as_me: error: C preprocessor \"$CPP\" fails sanity check
See \`config.log' for more details." >&2;}
   { (exit 1); exit 1; }; }
fi

ac_ext=c
ac_cpp='$CPP $CPPFLAGS'
ac_compile='$CC -c $CFLAGS $CPPFLAGS conftest.$ac_ext >&5'
ac_link='$CC -o conftest$ac_exeext $CFLAGS $CPPFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_c_compiler_gnu


{ echo "$as_me:$LINENO: checking for ANSI C header files" >&5
echo $ECHO_N "checking for ANSI C header files... $ECHO_C" >&6; }
if test "${ac_cv_header_stdc+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#include <stdlib.h>
#include <stdarg.h>
#include <string.h>
#include <float.h>

int
main ()
{

  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_c_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest.$ac_objext; then
  ac_cv_header_stdc=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_cv_header_stdc=no
fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext

if test $ac_cv_header_stdc = yes; then
  # SunOS 4.x string.h does not declare mem*, contrary to ANSI.
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#include <string.h>

_ACEOF
if (eval "$ac_cpp conftest.$ac_ext") 2>&5 |
  $EGREP "memchr" >/dev/null 2>&1; then
  :
else
  ac_cv_header_stdc=no
fi
rm -f conftest*

fi

if test $ac_cv_header_stdc = yes; then
  # ISC 2.0.2 stdlib.h does not declare free, contrary to ANSI.
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#include <stdlib.h>

_ACEOF
if (eval "$ac_cpp conftest.$ac_ext") 2>&5 |
  $EGREP "free" >/dev/null 2>&1; then
  :
else
  ac_cv_header_stdc=no
fi
rm -f conftest*

fi

if test $ac_cv_header_stdc = yes; then
  # /bin/cc in Irix-4.0.5 gets non-ANSI ctype macros unless using -ansi.
  if test "$cross_compiling" = yes; then
  :
else
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#include <ctype.h>
#include <stdlib.h>
#if ((' ' & 0x0FF) == 0x020)
# define ISLOWER(c) ('a' <= (c) && (c) <= 'z')
# define TOUPPER(c) (ISLOWER(c) ? 'A' + ((c) - 'a') : (c))
#else
# define ISLOWER(c) \
		   (('a' <= (c) && (c) <= 'i') \
		     || ('j' <= (c) && (c) <= 'r') \
		     || ('s' <= (c) && (c) <= 'z'))
# define TOUPPER(c) (ISLOWER(c) ? ((c) | 0x40) : (c))
#endif

#define XOR(e, f) (((e) && !(f)) || (!(e) && (f)))
int
main ()
{
  int i;
  for (i = 0; i < 256; i++)
    if (XOR (islower (i), ISLOWER (i))
	|| toupper (i) != TOUPPER (i))
      return 2;
  return 0;
}
_ACEOF
rm -f conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && { ac_try='./conftest$ac_exeext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  :
else
  echo "$as_me: program exited with status $ac_status" >&5
echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

( exit $ac_status )
ac_cv_header_stdc=no
fi
rm -f core *.core core.conftest.* gmon.out bb.out conftest$ac_exeext conftest.$ac_objext conftest.$ac_ext
fi


fi
fi
{ echo "$as_me:$LINENO: result: $ac_cv_header_stdc" >&5
echo "${ECHO_T}$ac_cv_header_stdc" >&6; }
if test $ac_cv_header_stdc = yes; then

cat >>confdefs.h <<\_ACEOF
#define STDC_HEADERS 1
_ACEOF

fi

# On IRIX 5.3, sys/types and inttypes.h are conflicting.









for ac_header in sys/types.h sys/stat.h stdlib.h string.h memory.h strings.h \
		  inttypes.h stdint.h unistd.h
do
as_ac_Header=`echo "ac_cv_header_$ac_header" | $as_tr_sh`
{ echo "$as_me:$LINENO: checking for $ac_header" >&5
echo $ECHO_N "checking for $ac_header... $ECHO_C" >&6; }
if { as_var=$as_ac_Header; eval "test \"\${$as_var+set}\" = set"; }; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
$ac_includes_default

#include <$ac_header>
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_c_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest.$ac_objext; then
  eval "$as_ac_Header=yes"
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	eval "$as_ac_Header=no"
fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext
fi
ac_res=`eval echo '${'$as_ac_Header'}'`
	       { echo "$as_me:$LINENO: result: $ac_res" >&5
echo "${ECHO_T}$ac_res" >&6; }
if test `eval echo '${'$as_ac_Header'}'` = yes; then
  cat >>confdefs.h <<_ACEOF
#define `echo "HAVE_$ac_header" | $as_tr_cpp` 1
_ACEOF

fi

done



for ac_header in dlfcn.h
do
as_ac_Header=`echo "ac_cv_header_$ac_header" | $as_tr_sh`
if { as_var=$as_ac_Header; eval "test \"\${$as_var+set}\" = set"; }; then
  { echo "$as_me:$LINENO: checking for $ac_header" >&5
echo $ECHO_N "checking for $ac_header... $ECHO_C" >&6; }
if { as_var=$as_ac_Header; eval "test \"\${$as_var+set}\" = set"; }; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
fi
ac_res=`eval echo '${'$as_ac_Header'}'`
	       { echo "$as_me:$LINENO: result: $ac_res" >&5
echo "${ECHO_T}$ac_res" >&6; }
else
  # Is the header compilable?
{ echo "$as_me:$LINENO: checking $ac_header usability" >&5
echo $ECHO_N "checking $ac_header usability... $ECHO_C" >&6; }
cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
$ac_includes_default
#include <$ac_header>
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_c_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest.$ac_objext; then
  ac_header_compiler=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_header_compiler=no
fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext
{ echo "$as_me:$LINENO: result: $ac_header_compiler" >&5
echo "${ECHO_T}$ac_header_compiler" >&6; }

# Is the header present?
{ echo "$as_me:$LINENO: checking $ac_header presence" >&5
echo $ECHO_N "checking $ac_header presence... $ECHO_C" >&6; }
cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#include <$ac_header>
_ACEOF
if { (ac_try="$ac_cpp conftest.$ac_ext"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_cpp conftest.$ac_ext") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } >/dev/null && {
	 test -z "$ac_c_preproc_warn_flag$ac_c_werror_flag" ||
	 test ! -s conftest.err
       }; then
  ac_header_preproc=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

  ac_header_preproc=no
fi

rm -f conftest.err conftest.$ac_ext
{ echo "$as_me:$LINENO: result: $ac_header_preproc" >&5
echo "${ECHO_T}$ac_header_preproc" >&6; }

# So?  What about this header?
case $ac_header_compiler:$ac_header_preproc:$ac_c_preproc_warn_flag in
  yes:no: )
    { echo "$as_me:$LINENO: WARNING: $ac_header: accepted by the compiler, rejected by the preprocessor!" >&5
echo "$as_me: WARNING: $ac_header: accepted by the compiler, rejected by the preprocessor!" >&2;}
    { echo "$as_me:$LINENO: WARNING: $ac_header: proceeding with the compiler's result" >&5
echo "$as_me: WARNING: $ac_header: proceeding with the compiler's result" >&2;}
    ac_header_preproc=yes
    ;;
  no:yes:* )
    { echo "$as_me:$LINENO: WARNING: $ac_header: present but cannot be compiled" >&5
echo "$as_me: WARNING: $ac_header: present but cannot be compiled" >&2;}
    { echo "$as_me:$LINENO: WARNING: $ac_header:     check for missing prerequisite headers?" >&5
echo "$as_me: WARNING: $ac_header:     check for missing prerequisite headers?" >&2;}
    { echo "$as_me:$LINENO: WARNING: $ac_header: see the Autoconf documentation" >&5
echo "$as_me: WARNING: $ac_header: see the Autoconf documentation" >&2;}
    { echo "$as_me:$LINENO: WARNING: $ac_header:     section \"Present But Cannot Be Compiled\"" >&5
echo "$as_me: WARNING: $ac_header:     section \"Present But Cannot Be Compiled\"" >&2;}
    { echo "$as_me:$LINENO: WARNING: $ac_header: proceeding with the preprocessor's result" >&5
echo "$as_me: WARNING: $ac_header: proceeding with the preprocessor's result" >&2;}
    { echo "$as_me:$LINENO: WARNING: $ac_header: in the future, the compiler will take precedence" >&5
echo "$as_me: WARNING: $ac_header: in the future, the compiler will take precedence" >&2;}
    ( cat <<\_ASBOX
## ---------------------------------- ##
## Report this to winter@alum.mit.edu ##
## ---------------------------------- ##
_ASBOX
     ) | sed "s/^/$as_me: WARNING:     /" >&2
    ;;
esac
{ echo "$as_me:$LINENO: checking for $ac_header" >&5
echo $ECHO_N "checking for $ac_header... $ECHO_C" >&6; }
if { as_var=$as_ac_Header; eval "test \"\${$as_var+set}\" = set"; }; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  eval "$as_ac_Header=\$ac_header_preproc"
fi
ac_res=`eval echo '${'$as_ac_Header'}'`
	       { echo "$as_me:$LINENO: result: $ac_res" >&5
echo "${ECHO_T}$ac_res" >&6; }

fi
if test `eval echo '${'$as_ac_Header'}'` = yes; then
  cat >>confdefs.h <<_ACEOF
#define `echo "HAVE_$ac_header" | $as_tr_cpp` 1
_ACEOF

fi

done



if test -n "$CXX" && ( test "X$CXX" != "Xno" &&
    ( (test "X$CXX" = "Xg++" && `g++ -v >/dev/null 2>&1` ) ||
    (test "X$CXX" != "Xg++"))) ; then
  ac_ext=cpp
ac_cpp='$CXXCPP $CPPFLAGS'
ac_compile='$CXX -c $CXXFLAGS $CPPFLAGS conftest.$ac_ext >&5'
ac_link='$CXX -o conftest$ac_exeext $CXXFLAGS $CPPFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_cxx_compiler_gnu
{ echo "$as_me:$LINENO: checking how to run the C++ preprocessor" >&5
echo $ECHO_N "checking how to run the C++ preprocessor... $ECHO_C" >&6; }
if test -z "$CXXCPP"; then
  if test "${ac_cv_prog_CXXCPP+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
      # Double quotes because CXXCPP needs to be expanded
    for CXXCPP in "$CXX -E" "/lib/cpp"
    do
      ac_preproc_ok=false
for ac_cxx_preproc_warn_flag in '' yes
do
  # Use a header file that comes with gcc, so configuring glibc
  # with a fresh cross-compiler works.
  # Prefer <limits.h> to <assert.h> if __STDC__ is defined, since
  # <limits.h> exists even on freestanding compilers.
  # On the NeXT, cc -E runs the code through the compiler's parser,
  # not just through cpp. "Syntax error" is here to catch this case.
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#ifdef __STDC__
# include <limits.h>
#else
# include <assert.h>
#endif
		     Syntax error
_ACEOF
if { (ac_try="$ac_cpp conftest.$ac_ext"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_cpp conftest.$ac_ext") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } >/dev/null && {
	 test -z "$ac_cxx_preproc_warn_flag$ac_cxx_werror_flag" ||
	 test ! -s conftest.err
       }; then
  :
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

  # Broken: fails on valid input.
continue
fi

rm -f conftest.err conftest.$ac_ext

  # OK, works on sane cases.  Now check whether nonexistent headers
  # can be detected and how.
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#include <ac_nonexistent.h>
_ACEOF
if { (ac_try="$ac_cpp conftest.$ac_ext"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_cpp conftest.$ac_ext") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } >/dev/null && {
	 test -z "$ac_cxx_preproc_warn_flag$ac_cxx_werror_flag" ||
	 test ! -s conftest.err
       }; then
  # Broken: success on invalid input.
continue
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

  # Passes both tests.
ac_preproc_ok=:
break
fi

rm -f conftest.err conftest.$ac_ext

done
# Because of `break', _AC_PREPROC_IFELSE's cleaning code was skipped.
rm -f conftest.err conftest.$ac_ext
if $ac_preproc_ok; then
  break
fi

    done
    ac_cv_prog_CXXCPP=$CXXCPP

fi
  CXXCPP=$ac_cv_prog_CXXCPP
else
  ac_cv_prog_CXXCPP=$CXXCPP
fi
{ echo "$as_me:$LINENO: result: $CXXCPP" >&5
echo "${ECHO_T}$CXXCPP" >&6; }
ac_preproc_ok=false
for ac_cxx_preproc_warn_flag in '' yes
do
  # Use a header file that comes with gcc, so configuring glibc
  # with a fresh cross-compiler works.
  # Prefer <limits.h> to <assert.h> if __STDC__ is defined, since
  # <limits.h> exists even on freestanding compilers.
  # On the NeXT, cc -E runs the code through the compiler's parser,
  # not just through cpp. "Syntax error" is here to catch this case.
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#ifdef __STDC__
# include <limits.h>
#else
# include <assert.h>
#endif
		     Syntax error
_ACEOF
if { (ac_try="$ac_cpp conftest.$ac_ext"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_cpp conftest.$ac_ext") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } >/dev/null && {
	 test -z "$ac_cxx_preproc_warn_flag$ac_cxx_werror_flag" ||
	 test ! -s conftest.err
       }; then
  :
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

  # Broken: fails on valid input.
continue
fi

rm -f conftest.err conftest.$ac_ext

  # OK, works on sane cases.  Now check whether nonexistent headers
  # can be detected and how.
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#include <ac_nonexistent.h>
_ACEOF
if { (ac_try="$ac_cpp conftest.$ac_ext"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_cpp conftest.$ac_ext") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } >/dev/null && {
	 test -z "$ac_cxx_preproc_warn_flag$ac_cxx_werror_flag" ||
	 test ! -s conftest.err
       }; then
  # Broken: success on invalid input.
continue
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

  # Passes both tests.
ac_preproc_ok=:
break
fi

rm -f conftest.err conftest.$ac_ext

done
# Because of `break', _AC_PREPROC_IFELSE's cleaning code was skipped.
rm -f conftest.err conftest.$ac_ext
if $ac_preproc_ok; then
  :
else
  { { echo "$as_me:$LINENO: error: C++ preprocessor \"$CXXCPP\" fails sanity check
See \`config.log' for more details." >&5
echo "$as_me: error: C++ preprocessor \"$CXXCPP\" fails sanity check
See \`config.log' for more details." >&2;}
   { (exit 1); exit 1; }; }
fi

ac_ext=cpp
ac_cpp='$CXXCPP $CPPFLAGS'
ac_compile='$CXX -c $CXXFLAGS $CPPFLAGS conftest.$ac_ext >&5'
ac_link='$CXX -o conftest$ac_exeext $CXXFLAGS $CPPFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_cxx_compiler_gnu

fi


ac_ext=f
ac_compile='$F77 -c $FFLAGS conftest.$ac_ext >&5'
ac_link='$F77 -o conftest$ac_exeext $FFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_f77_compiler_gnu
if test -n "$ac_tool_prefix"; then
  for ac_prog in g77 xlf f77 frt pgf77 cf77 fort77 fl32 af77 xlf90 f90 pgf90 pghpf epcf90 gfortran g95 xlf95 f95 fort ifort ifc efc pgf95 lf95 ftn
  do
    # Extract the first word of "$ac_tool_prefix$ac_prog", so it can be a program name with args.
set dummy $ac_tool_prefix$ac_prog; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_F77+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$F77"; then
  ac_cv_prog_F77="$F77" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_test_x "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_F77="$ac_tool_prefix$ac_prog"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
F77=$ac_cv_prog_F77
if test -n "$F77"; then
  { echo "$as_me:$LINENO: result: $F77" >&5
echo "${ECHO_T}$F77" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi


    test -n "$F77" && break
  done
fi
if test -z "$F77"; then
  ac_ct_F77=$F77
  for ac_prog in g77 xlf f77 frt pgf77 cf77 fort77 fl32 af77 xlf90 f90 pgf90 pghpf epcf90 gfortran g95 xlf95 f95 fort ifort ifc efc pgf95 lf95 ftn
do
  # Extract the first word of "$ac_prog", so it can be a program name with args.
set dummy $ac_prog; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_ac_ct_F77+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$ac_ct_F77"; then
  ac_cv_prog_ac_ct_F77="$ac_ct_F77" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_test_x "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_ac_ct_F77="$ac_prog"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
ac_ct_F77=$ac_cv_prog_ac_ct_F77
if test -n "$ac_ct_F77"; then
  { echo "$as_me:$LINENO: result: $ac_ct_F77" >&5
echo "${ECHO_T}$ac_ct_F77" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi


  test -n "$ac_ct_F77" && break
done

  if test "x$ac_ct_F77" = x; then
    F77=""
  else
    case $cross_compiling:$ac_tool_warned in
yes:)
{ echo "$as_me:$LINENO: WARNING: In the future, Autoconf will not detect cross-tools
whose name does not start with the host triplet.  If you think this
configuration is useful to you, please write to autoconf@gnu.org." >&5
echo "$as_me: WARNING: In the future, Autoconf will not detect cross-tools
whose name does not start with the host triplet.  If you think this
configuration is useful to you, please write to autoconf@gnu.org." >&2;}
ac_tool_warned=yes ;;
esac
    F77=$ac_ct_F77
  fi
fi


# Provide some information about the compiler.
echo "$as_me:$LINENO: checking for Fortran 77 compiler version" >&5
ac_compiler=`set X $ac_compile; echo $2`
{ (ac_try="$ac_compiler --version >&5"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compiler --version >&5") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }
{ (ac_try="$ac_compiler -v >&5"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compiler -v >&5") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }
{ (ac_try="$ac_compiler -V >&5"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compiler -V >&5") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }
rm -f a.out

# If we don't use `.F' as extension, the preprocessor is not run on the
# input file.  (Note that this only needs to work for GNU compilers.)
ac_save_ext=$ac_ext
ac_ext=F
{ echo "$as_me:$LINENO: checking whether we are using the GNU Fortran 77 compiler" >&5
echo $ECHO_N "checking whether we are using the GNU Fortran 77 compiler... $ECHO_C" >&6; }
if test "${ac_cv_f77_compiler_gnu+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  cat >conftest.$ac_ext <<_ACEOF
      program main
#ifndef __GNUC__
       choke me
#endif

      end
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_f77_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest.$ac_objext; then
  ac_compiler_gnu=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_compiler_gnu=no
fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext
ac_cv_f77_compiler_gnu=$ac_compiler_gnu

fi
{ echo "$as_me:$LINENO: result: $ac_cv_f77_compiler_gnu" >&5
echo "${ECHO_T}$ac_cv_f77_compiler_gnu" >&6; }
ac_ext=$ac_save_ext
ac_test_FFLAGS=${FFLAGS+set}
ac_save_FFLAGS=$FFLAGS
FFLAGS=
{ echo "$as_me:$LINENO: checking whether $F77 accepts -g" >&5
echo $ECHO_N "checking whether $F77 accepts -g... $ECHO_C" >&6; }
if test "${ac_cv_prog_f77_g+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  FFLAGS=-g
cat >conftest.$ac_ext <<_ACEOF
      program main

      end
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_f77_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest.$ac_objext; then
  ac_cv_prog_f77_g=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_cv_prog_f77_g=no
fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext

fi
{ echo "$as_me:$LINENO: result: $ac_cv_prog_f77_g" >&5
echo "${ECHO_T}$ac_cv_prog_f77_g" >&6; }
if test "$ac_test_FFLAGS" = set; then
  FFLAGS=$ac_save_FFLAGS
elif test $ac_cv_prog_f77_g = yes; then
  if test "x$ac_cv_f77_compiler_gnu" = xyes; then
    FFLAGS="-g -O2"
  else
    FFLAGS="-g"
  fi
else
  if test "x$ac_cv_f77_compiler_gnu" = xyes; then
    FFLAGS="-O2"
  else
    FFLAGS=
  fi
fi

G77=`test $ac_compiler_gnu = yes && echo yes`
ac_ext=c
ac_cpp='$CPP $CPPFLAGS'
ac_compile='$CC -c $CFLAGS $CPPFLAGS conftest.$ac_ext >&5'
ac_link='$CC -o conftest$ac_exeext $CFLAGS $CPPFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_c_compiler_gnu



# Autoconf 2.13's AC_OBJEXT and AC_EXEEXT macros only works for C compilers!

# find the maximum length of command line arguments
{ echo "$as_me:$LINENO: checking the maximum length of command line arguments" >&5
echo $ECHO_N "checking the maximum length of command line arguments... $ECHO_C" >&6; }
if test "${lt_cv_sys_max_cmd_len+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
    i=0
  teststring="ABCD"

  case $build_os in
  msdosdjgpp*)
    # On DJGPP, this test can blow up pretty badly due to problems in libc
    # (any single argument exceeding 2000 bytes causes a buffer overrun
    # during glob expansion).  Even if it were fixed, the result of this
    # check would be larger than it should be.
    lt_cv_sys_max_cmd_len=12288;    # 12K is about right
    ;;

  gnu*)
    # Under GNU Hurd, this test is not required because there is
    # no limit to the length of command line arguments.
    # Libtool will interpret -1 as no limit whatsoever
    lt_cv_sys_max_cmd_len=-1;
    ;;

  cygwin* | mingw*)
    # On Win9x/ME, this test blows up -- it succeeds, but takes
    # about 5 minutes as the teststring grows exponentially.
    # Worse, since 9x/ME are not pre-emptively multitasking,
    # you end up with a "frozen" computer, even though with patience
    # the test eventually succeeds (with a max line length of 256k).
    # Instead, let's just punt: use the minimum linelength reported by
    # all of the supported platforms: 8192 (on NT/2K/XP).
    lt_cv_sys_max_cmd_len=8192;
    ;;

  amigaos*)
    # On AmigaOS with pdksh, this test takes hours, literally.
    # So we just punt and use a minimum line length of 8192.
    lt_cv_sys_max_cmd_len=8192;
    ;;

  netbsd* | freebsd* | openbsd* | darwin* | dragonfly*)
    # This has been around since 386BSD, at least.  Likely further.
    if test -x /sbin/sysctl; then
      lt_cv_sys_max_cmd_len=`/sbin/sysctl -n kern.argmax`
    elif test -x /usr/sbin/sysctl; then
      lt_cv_sys_max_cmd_len=`/usr/sbin/sysctl -n kern.argmax`
    else
      lt_cv_sys_max_cmd_len=65536	# usable default for all BSDs
    fi
    # And add a safety zone
    lt_cv_sys_max_cmd_len=`expr $lt_cv_sys_max_cmd_len \/ 4`
    lt_cv_sys_max_cmd_len=`expr $lt_cv_sys_max_cmd_len \* 3`
    ;;

  interix*)
    # We know the value 262144 and hardcode it with a safety zone (like BSD)
    lt_cv_sys_max_cmd_len=196608
    ;;

  osf*)
    # Dr. Hans Ekkehard Plesser reports seeing a kernel panic running configure
    # due to this test when exec_disable_arg_limit is 1 on Tru64. It is not
    # nice to cause kernel panics so lets avoid the loop below.
    # First set a reasonable default.
    lt_cv_sys_max_cmd_len=16384
    #
    if test -x /sbin/sysconfig; then
      case `/sbin/sysconfig -q proc exec_disable_arg_limit` in
        *1*) lt_cv_sys_max_cmd_len=-1 ;;
      esac
    fi
    ;;
  sco3.2v5*)
    lt_cv_sys_max_cmd_len=102400
    ;;
  sysv5* | sco5v6* | sysv4.2uw2*)
    kargmax=`grep ARG_MAX /etc/conf/cf.d/stune 2>/dev/null`
    if test -n "$kargmax"; then
      lt_cv_sys_max_cmd_len=`echo $kargmax | sed 's/.*[ 	]//'`
    else
      lt_cv_sys_max_cmd_len=32768
    fi
    ;;
  *)
    lt_cv_sys_max_cmd_len=`(getconf ARG_MAX) 2> /dev/null`
    if test -n "$lt_cv_sys_max_cmd_len"; then
      lt_cv_sys_max_cmd_len=`expr $lt_cv_sys_max_cmd_len \/ 4`
      lt_cv_sys_max_cmd_len=`expr $lt_cv_sys_max_cmd_len \* 3`
    else
      SHELL=${SHELL-${CONFIG_SHELL-/bin/sh}}
      while (test "X"`$SHELL $0 --fallback-echo "X$teststring" 2>/dev/null` \
	       = "XX$teststring") >/dev/null 2>&1 &&
	      new_result=`expr "X$teststring" : ".*" 2>&1` &&
	      lt_cv_sys_max_cmd_len=$new_result &&
	      test $i != 17 # 1/2 MB should be enough
      do
        i=`expr $i + 1`
        teststring=$teststring$teststring
      done
      teststring=
      # Add a significant safety factor because C++ compilers can tack on massive
      # amounts of additional arguments before passing them to the linker.
      # It appears as though 1/2 is a usable value.
      lt_cv_sys_max_cmd_len=`expr $lt_cv_sys_max_cmd_len \/ 2`
    fi
    ;;
  esac

fi

if test -n $lt_cv_sys_max_cmd_len ; then
  { echo "$as_me:$LINENO: result: $lt_cv_sys_max_cmd_len" >&5
echo "${ECHO_T}$lt_cv_sys_max_cmd_len" >&6; }
else
  { echo "$as_me:$LINENO: result: none" >&5
echo "${ECHO_T}none" >&6; }
fi





# Check for command to grab the raw symbol name followed by C symbol from nm.
{ echo "$as_me:$LINENO: checking command to parse $NM output from $compiler object" >&5
echo $ECHO_N "checking command to parse $NM output from $compiler object... $ECHO_C" >&6; }
if test "${lt_cv_sys_global_symbol_pipe+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else

# These are sane defaults that work on at least a few old systems.
# [They come from Ultrix.  What could be older than Ultrix?!! ;)]

# Character class describing NM global symbol codes.
symcode='[BCDEGRST]'

# Regexp to match symbols that can be accessed directly from C.
sympat='\([_A-Za-z][_A-Za-z0-9]*\)'

# Transform an extracted symbol line into a proper C declaration
lt_cv_sys_global_symbol_to_cdecl="sed -n -e 's/^. .* \(.*\)$/extern int \1;/p'"

# Transform an extracted symbol line into symbol name and symbol address
lt_cv_sys_global_symbol_to_c_name_address="sed -n -e 's/^: \([^ ]*\) $/  {\\\"\1\\\", (lt_ptr) 0},/p' -e 's/^$symcode \([^ ]*\) \([^ ]*\)$/  {\"\2\", (lt_ptr) \&\2},/p'"

# Define system-specific variables.
case $host_os in
aix*)
  symcode='[BCDT]'
  ;;
cygwin* | mingw* | pw32*)
  symcode='[ABCDGISTW]'
  ;;
hpux*) # Its linker distinguishes data from code symbols
  if test "$host_cpu" = ia64; then
    symcode='[ABCDEGRST]'
  fi
  lt_cv_sys_global_symbol_to_cdecl="sed -n -e 's/^T .* \(.*\)$/extern int \1();/p' -e 's/^$symcode* .* \(.*\)$/extern char \1;/p'"
  lt_cv_sys_global_symbol_to_c_name_address="sed -n -e 's/^: \([^ ]*\) $/  {\\\"\1\\\", (lt_ptr) 0},/p' -e 's/^$symcode* \([^ ]*\) \([^ ]*\)$/  {\"\2\", (lt_ptr) \&\2},/p'"
  ;;
linux* | k*bsd*-gnu)
  if test "$host_cpu" = ia64; then
    symcode='[ABCDGIRSTW]'
    lt_cv_sys_global_symbol_to_cdecl="sed -n -e 's/^T .* \(.*\)$/extern int \1();/p' -e 's/^$symcode* .* \(.*\)$/extern char \1;/p'"
    lt_cv_sys_global_symbol_to_c_name_address="sed -n -e 's/^: \([^ ]*\) $/  {\\\"\1\\\", (lt_ptr) 0},/p' -e 's/^$symcode* \([^ ]*\) \([^ ]*\)$/  {\"\2\", (lt_ptr) \&\2},/p'"
  fi
  ;;
irix* | nonstopux*)
  symcode='[BCDEGRST]'
  ;;
osf*)
  symcode='[BCDEGQRST]'
  ;;
solaris*)
  symcode='[BDRT]'
  ;;
sco3.2v5*)
  symcode='[DT]'
  ;;
sysv4.2uw2*)
  symcode='[DT]'
  ;;
sysv5* | sco5v6* | unixware* | OpenUNIX*)
  symcode='[ABDT]'
  ;;
sysv4)
  symcode='[DFNSTU]'
  ;;
esac

# Handle CRLF in mingw tool chain
opt_cr=
case $build_os in
mingw*)
  opt_cr=`echo 'x\{0,1\}' | tr x '\015'` # option cr in regexp
  ;;
esac

# If we're using GNU nm, then use its standard symbol codes.
case `$NM -V 2>&1` in
*GNU* | *'with BFD'*)
  symcode='[ABCDGIRSTW]' ;;
esac

# Try without a prefix undercore, then with it.
for ac_symprfx in "" "_"; do

  # Transform symcode, sympat, and symprfx into a raw symbol and a C symbol.
  symxfrm="\\1 $ac_symprfx\\2 \\2"

  # Write the raw and C identifiers.
  lt_cv_sys_global_symbol_pipe="sed -n -e 's/^.*[ 	]\($symcode$symcode*\)[ 	][ 	]*$ac_symprfx$sympat$opt_cr$/$symxfrm/p'"

  # Check to see that the pipe works correctly.
  pipe_works=no

  rm -f conftest*
  cat > conftest.$ac_ext <<EOF
#ifdef __cplusplus
extern "C" {
#endif
char nm_test_var;
void nm_test_func(){}
#ifdef __cplusplus
}
#endif
int main(){nm_test_var='a';nm_test_func();return(0);}
EOF

  if { (eval echo "$as_me:$LINENO: \"$ac_compile\"") >&5
  (eval $ac_compile) 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; then
    # Now try to grab the symbols.
    nlist=conftest.nm
    if { (eval echo "$as_me:$LINENO: \"$NM conftest.$ac_objext \| $lt_cv_sys_global_symbol_pipe \> $nlist\"") >&5
  (eval $NM conftest.$ac_objext \| $lt_cv_sys_global_symbol_pipe \> $nlist) 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && test -s "$nlist"; then
      # Try sorting and uniquifying the output.
      if sort "$nlist" | uniq > "$nlist"T; then
	mv -f "$nlist"T "$nlist"
      else
	rm -f "$nlist"T
      fi

      # Make sure that we snagged all the symbols we need.
      if grep ' nm_test_var$' "$nlist" >/dev/null; then
	if grep ' nm_test_func$' "$nlist" >/dev/null; then
	  cat <<EOF > conftest.$ac_ext
#ifdef __cplusplus
extern "C" {
#endif

EOF
	  # Now generate the symbol file.
	  eval "$lt_cv_sys_global_symbol_to_cdecl"' < "$nlist" | grep -v main >> conftest.$ac_ext'

	  cat <<EOF >> conftest.$ac_ext
#if defined (__STDC__) && __STDC__
# define lt_ptr_t void *
#else
# define lt_ptr_t char *
# define const
#endif

/* The mapping between symbol names and symbols. */
const struct {
  const char *name;
  lt_ptr_t address;
}
lt_preloaded_symbols[] =
{
EOF
	  $SED "s/^$symcode$symcode* \(.*\) \(.*\)$/  {\"\2\", (lt_ptr_t) \&\2},/" < "$nlist" | grep -v main >> conftest.$ac_ext
	  cat <<\EOF >> conftest.$ac_ext
  {0, (lt_ptr_t) 0}
};

#ifdef __cplusplus
}
#endif
EOF
	  # Now try linking the two files.
	  mv conftest.$ac_objext conftstm.$ac_objext
	  lt_save_LIBS="$LIBS"
	  lt_save_CFLAGS="$CFLAGS"
	  LIBS="conftstm.$ac_objext"
	  CFLAGS="$CFLAGS$lt_prog_compiler_no_builtin_flag"
	  if { (eval echo "$as_me:$LINENO: \"$ac_link\"") >&5
  (eval $ac_link) 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && test -s conftest${ac_exeext}; then
	    pipe_works=yes
	  fi
	  LIBS="$lt_save_LIBS"
	  CFLAGS="$lt_save_CFLAGS"
	else
	  echo "cannot find nm_test_func in $nlist" >&5
	fi
      else
	echo "cannot find nm_test_var in $nlist" >&5
      fi
    else
      echo "cannot run $lt_cv_sys_global_symbol_pipe" >&5
    fi
  else
    echo "$progname: failed program was:" >&5
    cat conftest.$ac_ext >&5
  fi
  rm -f conftest* conftst*

  # Do not use the global_symbol_pipe unless it works.
  if test "$pipe_works" = yes; then
    break
  else
    lt_cv_sys_global_symbol_pipe=
  fi
done

fi

if test -z "$lt_cv_sys_global_symbol_pipe"; then
  lt_cv_sys_global_symbol_to_cdecl=
fi
if test -z "$lt_cv_sys_global_symbol_pipe$lt_cv_sys_global_symbol_to_cdecl"; then
  { echo "$as_me:$LINENO: result: failed" >&5
echo "${ECHO_T}failed" >&6; }
else
  { echo "$as_me:$LINENO: result: ok" >&5
echo "${ECHO_T}ok" >&6; }
fi

{ echo "$as_me:$LINENO: checking for objdir" >&5
echo $ECHO_N "checking for objdir... $ECHO_C" >&6; }
if test "${lt_cv_objdir+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  rm -f .libs 2>/dev/null
mkdir .libs 2>/dev/null
if test -d .libs; then
  lt_cv_objdir=.libs
else
  # MS-DOS does not allow filenames that begin with a dot.
  lt_cv_objdir=_libs
fi
rmdir .libs 2>/dev/null
fi
{ echo "$as_me:$LINENO: result: $lt_cv_objdir" >&5
echo "${ECHO_T}$lt_cv_objdir" >&6; }
objdir=$lt_cv_objdir





case $host_os in
aix3*)
  # AIX sometimes has problems with the GCC collect2 program.  For some
  # reason, if we set the COLLECT_NAMES environment variable, the problems
  # vanish in a puff of smoke.
  if test "X${COLLECT_NAMES+set}" != Xset; then
    COLLECT_NAMES=
    export COLLECT_NAMES
  fi
  ;;
esac

# Sed substitution that helps us do robust quoting.  It backslashifies
# metacharacters that are still active within double-quoted strings.
Xsed='sed -e 1s/^X//'
sed_quote_subst='s/\([\\"\\`$\\\\]\)/\\\1/g'

# Same as above, but do not quote variable references.
double_quote_subst='s/\([\\"\\`\\\\]\)/\\\1/g'

# Sed substitution to delay expansion of an escaped shell variable in a
# double_quote_subst'ed string.
delay_variable_subst='s/\\\\\\\\\\\$/\\\\\\$/g'

# Sed substitution to avoid accidental globbing in evaled expressions
no_glob_subst='s/\*/\\\*/g'

# Constants:
rm="rm -f"

# Global variables:
default_ofile=libtool
can_build_shared=yes

# All known linkers require a `.a' archive for static linking (except MSVC,
# which needs '.lib').
libext=a
ltmain="$ac_aux_dir/ltmain.sh"
ofile="$default_ofile"
with_gnu_ld="$lt_cv_prog_gnu_ld"

if test -n "$ac_tool_prefix"; then
  # Extract the first word of "${ac_tool_prefix}ar", so it can be a program name with args.
set dummy ${ac_tool_prefix}ar; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_AR+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$AR"; then
  ac_cv_prog_AR="$AR" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_test_x "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_AR="${ac_tool_prefix}ar"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
AR=$ac_cv_prog_AR
if test -n "$AR"; then
  { echo "$as_me:$LINENO: result: $AR" >&5
echo "${ECHO_T}$AR" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi


fi
if test -z "$ac_cv_prog_AR"; then
  ac_ct_AR=$AR
  # Extract the first word of "ar", so it can be a program name with args.
set dummy ar; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_ac_ct_AR+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$ac_ct_AR"; then
  ac_cv_prog_ac_ct_AR="$ac_ct_AR" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_test_x "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_ac_ct_AR="ar"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
ac_ct_AR=$ac_cv_prog_ac_ct_AR
if test -n "$ac_ct_AR"; then
  { echo "$as_me:$LINENO: result: $ac_ct_AR" >&5
echo "${ECHO_T}$ac_ct_AR" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi

  if test "x$ac_ct_AR" = x; then
    AR="false"
  else
    case $cross_compiling:$ac_tool_warned in
yes:)
{ echo "$as_me:$LINENO: WARNING: In the future, Autoconf will not detect cross-tools
whose name does not start with the host triplet.  If you think this
configuration is useful to you, please write to autoconf@gnu.org." >&5
echo "$as_me: WARNING: In the future, Autoconf will not detect cross-tools
whose name does not start with the host triplet.  If you think this
configuration is useful to you, please write to autoconf@gnu.org." >&2;}
ac_tool_warned=yes ;;
esac
    AR=$ac_ct_AR
  fi
else
  AR="$ac_cv_prog_AR"
fi

if test -n "$ac_tool_prefix"; then
  # Extract the first word of "${ac_tool_prefix}ranlib", so it can be a program name with args.
set dummy ${ac_tool_prefix}ranlib; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_RANLIB+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$RANLIB"; then
  ac_cv_prog_RANLIB="$RANLIB" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_test_x "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_RANLIB="${ac_tool_prefix}ranlib"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
RANLIB=$ac_cv_prog_RANLIB
if test -n "$RANLIB"; then
  { echo "$as_me:$LINENO: result: $RANLIB" >&5
echo "${ECHO_T}$RANLIB" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi


fi
if test -z "$ac_cv_prog_RANLIB"; then
  ac_ct_RANLIB=$RANLIB
  # Extract the first word of "ranlib", so it can be a program name with args.
set dummy ranlib; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_ac_ct_RANLIB+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$ac_ct_RANLIB"; then
  ac_cv_prog_ac_ct_RANLIB="$ac_ct_RANLIB" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_test_x "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_ac_ct_RANLIB="ranlib"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
ac_ct_RANLIB=$ac_cv_prog_ac_ct_RANLIB
if test -n "$ac_ct_RANLIB"; then
  { echo "$as_me:$LINENO: result: $ac_ct_RANLIB" >&5
echo "${ECHO_T}$ac_ct_RANLIB" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi

  if test "x$ac_ct_RANLIB" = x; then
    RANLIB=":"
  else
    case $cross_compiling:$ac_tool_warned in
yes:)
{ echo "$as_me:$LINENO: WARNING: In the future, Autoconf will not detect cross-tools
whose name does not start with the host triplet.  If you think this
configuration is useful to you, please write to autoconf@gnu.org." >&5
echo "$as_me: WARNING: In the future, Autoconf will not detect cross-tools
whose name does not start with the host triplet.  If you think this
configuration is useful to you, please write to autoconf@gnu.org." >&2;}
ac_tool_warned=yes ;;
esac
    RANLIB=$ac_ct_RANLIB
  fi
else
  RANLIB="$ac_cv_prog_RANLIB"
fi

if test -n "$ac_tool_prefix"; then
  # Extract the first word of "${ac_tool_prefix}strip", so it can be a program name with args.
set dummy ${ac_tool_prefix}strip; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_STRIP+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$STRIP"; then
  ac_cv_prog_STRIP="$STRIP" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_test_x "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_STRIP="${ac_tool_prefix}strip"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
STRIP=$ac_cv_prog_STRIP
if test -n "$STRIP"; then
  { echo "$as_me:$LINENO: result: $STRIP" >&5
echo "${ECHO_T}$STRIP" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi


fi
if test -z "$ac_cv_prog_STRIP"; then
  ac_ct_STRIP=$STRIP
  # Extract the first word of "strip", so it can be a program name with args.
set dummy strip; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_ac_ct_STRIP+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$ac_ct_STRIP"; then
  ac_cv_prog_ac_ct_STRIP="$ac_ct_STRIP" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_test_x "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_ac_ct_STRIP="strip"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
ac_ct_STRIP=$ac_cv_prog_ac_ct_STRIP
if test -n "$ac_ct_STRIP"; then
  { echo "$as_me:$LINENO: result: $ac_ct_STRIP" >&5
echo "${ECHO_T}$ac_ct_STRIP" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi

  if test "x$ac_ct_STRIP" = x; then
    STRIP=":"
  else
    case $cross_compiling:$ac_tool_warned in
yes:)
{ echo "$as_me:$LINENO: WARNING: In the future, Autoconf will not detect cross-tools
whose name does not start with the host triplet.  If you think this
configuration is useful to you, please write to autoconf@gnu.org." >&5
echo "$as_me: WARNING: In the future, Autoconf will not detect cross-tools
whose name does not start with the host triplet.  If you think this
configuration is useful to you, please write to autoconf@gnu.org." >&2;}
ac_tool_warned=yes ;;
esac
    STRIP=$ac_ct_STRIP
  fi
else
  STRIP="$ac_cv_prog_STRIP"
fi


old_CC="$CC"
old_CFLAGS="$CFLAGS"

# Set sane defaults for various variables
test -z "$AR" && AR=ar
test -z "$AR_FLAGS" && AR_FLAGS=cru
test -z "$AS" && AS=as
test -z "$CC" && CC=cc
test -z "$LTCC" && LTCC=$CC
test -z "$LTCFLAGS" && LTCFLAGS=$CFLAGS
test -z "$DLLTOOL" && DLLTOOL=dlltool
test -z "$LD" && LD=ld
test -z "$LN_S" && LN_S="ln -s"
test -z "$MAGIC_CMD" && MAGIC_CMD=file
test -z "$NM" && NM=nm
test -z "$SED" && SED=sed
test -z "$OBJDUMP" && OBJDUMP=objdump
test -z "$RANLIB" && RANLIB=:
test -z "$STRIP" && STRIP=:
test -z "$ac_objext" && ac_objext=o

# Determine commands to create old-style static archives.
old_archive_cmds='$AR $AR_FLAGS $oldlib$oldobjs'
old_postinstall_cmds='chmod 644 $oldlib'
old_postuninstall_cmds=

if test -n "$RANLIB"; then
  case $host_os in
  openbsd*)
    old_postinstall_cmds="$old_postinstall_cmds~\$RANLIB -t \$oldlib"
    ;;
  *)
    old_postinstall_cmds="$old_postinstall_cmds~\$RANLIB \$oldlib"
    ;;
  esac
  old_archive_cmds="$old_archive_cmds~\$RANLIB \$oldlib"
fi

for cc_temp in $compiler""; do
  case $cc_temp in
    compile | *[\\/]compile | ccache | *[\\/]ccache ) ;;
    distcc | *[\\/]distcc | purify | *[\\/]purify ) ;;
    \-*) ;;
    *) break;;
  esac
done
cc_basename=`$echo "X$cc_temp" | $Xsed -e 's%.*/%%' -e "s%^$host_alias-%%"`


# Only perform the check for file, if the check method requires it
case $deplibs_check_method in
file_magic*)
  if test "$file_magic_cmd" = '$MAGIC_CMD'; then
    { echo "$as_me:$LINENO: checking for ${ac_tool_prefix}file" >&5
echo $ECHO_N "checking for ${ac_tool_prefix}file... $ECHO_C" >&6; }
if test "${lt_cv_path_MAGIC_CMD+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  case $MAGIC_CMD in
[\\/*] |  ?:[\\/]*)
  lt_cv_path_MAGIC_CMD="$MAGIC_CMD" # Let the user override the test with a path.
  ;;
*)
  lt_save_MAGIC_CMD="$MAGIC_CMD"
  lt_save_ifs="$IFS"; IFS=$PATH_SEPARATOR
  ac_dummy="/usr/bin$PATH_SEPARATOR$PATH"
  for ac_dir in $ac_dummy; do
    IFS="$lt_save_ifs"
    test -z "$ac_dir" && ac_dir=.
    if test -f $ac_dir/${ac_tool_prefix}file; then
      lt_cv_path_MAGIC_CMD="$ac_dir/${ac_tool_prefix}file"
      if test -n "$file_magic_test_file"; then
	case $deplibs_check_method in
	"file_magic "*)
	  file_magic_regex=`expr "$deplibs_check_method" : "file_magic \(.*\)"`
	  MAGIC_CMD="$lt_cv_path_MAGIC_CMD"
	  if eval $file_magic_cmd \$file_magic_test_file 2> /dev/null |
	    $EGREP "$file_magic_regex" > /dev/null; then
	    :
	  else
	    cat <<EOF 1>&2

*** Warning: the command libtool uses to detect shared libraries,
*** $file_magic_cmd, produces output that libtool cannot recognize.
*** The result is that libtool may fail to recognize shared libraries
*** as such.  This will affect the creation of libtool libraries that
*** depend on shared libraries, but programs linked with such libtool
*** libraries will work regardless of this problem.  Nevertheless, you
*** may want to report the problem to your system manager and/or to
*** bug-libtool@gnu.org

EOF
	  fi ;;
	esac
      fi
      break
    fi
  done
  IFS="$lt_save_ifs"
  MAGIC_CMD="$lt_save_MAGIC_CMD"
  ;;
esac
fi

MAGIC_CMD="$lt_cv_path_MAGIC_CMD"
if test -n "$MAGIC_CMD"; then
  { echo "$as_me:$LINENO: result: $MAGIC_CMD" >&5
echo "${ECHO_T}$MAGIC_CMD" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi

if test -z "$lt_cv_path_MAGIC_CMD"; then
  if test -n "$ac_tool_prefix"; then
    { echo "$as_me:$LINENO: checking for file" >&5
echo $ECHO_N "checking for file... $ECHO_C" >&6; }
if test "${lt_cv_path_MAGIC_CMD+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  case $MAGIC_CMD in
[\\/*] |  ?:[\\/]*)
  lt_cv_path_MAGIC_CMD="$MAGIC_CMD" # Let the user override the test with a path.
  ;;
*)
  lt_save_MAGIC_CMD="$MAGIC_CMD"
  lt_save_ifs="$IFS"; IFS=$PATH_SEPARATOR
  ac_dummy="/usr/bin$PATH_SEPARATOR$PATH"
  for ac_dir in $ac_dummy; do
    IFS="$lt_save_ifs"
    test -z "$ac_dir" && ac_dir=.
    if test -f $ac_dir/file; then
      lt_cv_path_MAGIC_CMD="$ac_dir/file"
      if test -n "$file_magic_test_file"; then
	case $deplibs_check_method in
	"file_magic "*)
	  file_magic_regex=`expr "$deplibs_check_method" : "file_magic \(.*\)"`
	  MAGIC_CMD="$lt_cv_path_MAGIC_CMD"
	  if eval $file_magic_cmd \$file_magic_test_file 2> /dev/null |
	    $EGREP "$file_magic_regex" > /dev/null; then
	    :
	  else
	    cat <<EOF 1>&2

*** Warning: the command libtool uses to detect shared libraries,
*** $file_magic_cmd, produces output that libtool cannot recognize.
*** The result is that libtool may fail to recognize shared libraries
*** as such.  This will affect the creation of libtool libraries that
*** depend on shared libraries, but programs linked with such libtool
*** libraries will work regardless of this problem.  Nevertheless, you
*** may want to report the problem to your system manager and/or to
*** bug-libtool@gnu.org

EOF
	  fi ;;
	esac
      fi
      break
    fi
  done
  IFS="$lt_save_ifs"
  MAGIC_CMD="$lt_save_MAGIC_CMD"
  ;;
esac
fi

MAGIC_CMD="$lt_cv_path_MAGIC_CMD"
if test -n "$MAGIC_CMD"; then
  { echo "$as_me:$LINENO: result: $MAGIC_CMD" >&5
echo "${ECHO_T}$MAGIC_CMD" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi

  else
    MAGIC_CMD=:
  fi
fi

  fi
  ;;
esac

enable_dlopen=no
enable_win32_dll=no

# Check whether --enable-libtool-lock was given.
if test "${enable_libtool_lock+set}" = set; then
  enableval=$enable_libtool_lock;
fi

test "x$enable_libtool_lock" != xno && enable_libtool_lock=yes


# Check whether --with-pic was given.
if test "${with_pic+set}" = set; then
  withval=$with_pic; pic_mode="$withval"
else
  pic_mode=default
fi

test -z "$pic_mode" && pic_mode=default

# Use C for the default configuration in the libtool script
tagname=
lt_save_CC="$CC"
ac_ext=c
ac_cpp='$CPP $CPPFLAGS'
ac_compile='$CC -c $CFLAGS $CPPFLAGS conftest.$ac_ext >&5'
ac_link='$CC -o conftest$ac_exeext $CFLAGS $CPPFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_c_compiler_gnu


# Source file extension for C test sources.
ac_ext=c

# Object file extension for compiled C test sources.
objext=o
objext=$objext

# Code to be used in simple compile tests
lt_simple_compile_test_code="int some_variable = 0;"

# Code to be used in simple link tests
lt_simple_link_test_code='int main(){return(0);}'


# If no C compiler was specified, use CC.
LTCC=${LTCC-"$CC"}

# If no C compiler flags were specified, use CFLAGS.
LTCFLAGS=${LTCFLAGS-"$CFLAGS"}

# Allow CC to be a program name with arguments.
compiler=$CC


# save warnings/boilerplate of simple test code
ac_outfile=conftest.$ac_objext
echo "$lt_simple_compile_test_code" >conftest.$ac_ext
eval "$ac_compile" 2>&1 >/dev/null | $SED '/^$/d; /^ *+/d' >conftest.err
_lt_compiler_boilerplate=`cat conftest.err`
$rm conftest*

ac_outfile=conftest.$ac_objext
echo "$lt_simple_link_test_code" >conftest.$ac_ext
eval "$ac_link" 2>&1 >/dev/null | $SED '/^$/d; /^ *+/d' >conftest.err
_lt_linker_boilerplate=`cat conftest.err`
$rm conftest*



lt_prog_compiler_no_builtin_flag=

if test "$GCC" = yes; then
  lt_prog_compiler_no_builtin_flag=' -fno-builtin'


{ echo "$as_me:$LINENO: checking if $compiler supports -fno-rtti -fno-exceptions" >&5
echo $ECHO_N "checking if $compiler supports -fno-rtti -fno-exceptions... $ECHO_C" >&6; }
if test "${lt_cv_prog_compiler_rtti_exceptions+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  lt_cv_prog_compiler_rtti_exceptions=no
  ac_outfile=conftest.$ac_objext
   echo "$lt_simple_compile_test_code" > conftest.$ac_ext
   lt_compiler_flag="-fno-rtti -fno-exceptions"
   # Insert the option either (1) after the last *FLAGS variable, or
   # (2) before a word containing "conftest.", or (3) at the end.
   # Note that $ac_compile itself does not contain backslashes and begins
   # with a dollar sign (not a hyphen), so the echo should work correctly.
   # The option is referenced via a variable to avoid confusing sed.
   lt_compile=`echo "$ac_compile" | $SED \
   -e 's:.*FLAGS}\{0,1\} :&$lt_compiler_flag :; t' \
   -e 's: [^ ]*conftest\.: $lt_compiler_flag&:; t' \
   -e 's:$: $lt_compiler_flag:'`
   (eval echo "\"\$as_me:7063: $lt_compile\"" >&5)
   (eval "$lt_compile" 2>conftest.err)
   ac_status=$?
   cat conftest.err >&5
   echo "$as_me:7067: \$? = $ac_status" >&5
   if (exit $ac_status) && test -s "$ac_outfile"; then
     # The compiler can only warn and ignore the option if not recognized
     # So say no if there are warnings other than the usual output.
     $echo "X$_lt_compiler_boilerplate" | $Xsed -e '/^$/d' >conftest.exp
     $SED '/^$/d; /^ *+/d' conftest.err >conftest.er2
     if test ! -s conftest.er2 || diff conftest.exp conftest.er2 >/dev/null; then
       lt_cv_prog_compiler_rtti_exceptions=yes
     fi
   fi
   $rm conftest*

fi
{ echo "$as_me:$LINENO: result: $lt_cv_prog_compiler_rtti_exceptions" >&5
echo "${ECHO_T}$lt_cv_prog_compiler_rtti_exceptions" >&6; }

if test x"$lt_cv_prog_compiler_rtti_exceptions" = xyes; then
    lt_prog_compiler_no_builtin_flag="$lt_prog_compiler_no_builtin_flag -fno-rtti -fno-exceptions"
else
    :
fi

fi

lt_prog_compiler_wl=
lt_prog_compiler_pic=
lt_prog_compiler_static=

{ echo "$as_me:$LINENO: checking for $compiler option to produce PIC" >&5
echo $ECHO_N "checking for $compiler option to produce PIC... $ECHO_C" >&6; }

  if test "$GCC" = yes; then
    lt_prog_compiler_wl='-Wl,'
    lt_prog_compiler_static='-static'

    case $host_os in
      aix*)
      # All AIX code is PIC.
      if test "$host_cpu" = ia64; then
	# AIX 5 now supports IA64 processor
	lt_prog_compiler_static='-Bstatic'
      fi
      ;;

    amigaos*)
      # FIXME: we need at least 68020 code to build shared libraries, but
      # adding the `-m68020' flag to GCC prevents building anything better,
      # like `-m68040'.
      lt_prog_compiler_pic='-m68020 -resident32 -malways-restore-a4'
      ;;

    beos* | irix5* | irix6* | nonstopux* | osf3* | osf4* | osf5*)
      # PIC is the default for these OSes.
      ;;

    mingw* | cygwin* | pw32* | os2*)
      # This hack is so that the source file can tell whether it is being
      # built for inclusion in a dll (and should export symbols for example).
      # Although the cygwin gcc ignores -fPIC, still need this for old-style
      # (--disable-auto-import) libraries
      lt_prog_compiler_pic='-DDLL_EXPORT'
      ;;

    darwin* | rhapsody*)
      # PIC is the default on this platform
      # Common symbols not allowed in MH_DYLIB files
      lt_prog_compiler_pic='-fno-common'
      ;;

    interix[3-9]*)
      # Interix 3.x gcc -fpic/-fPIC options generate broken code.
      # Instead, we relocate shared libraries at runtime.
      ;;

    msdosdjgpp*)
      # Just because we use GCC doesn't mean we suddenly get shared libraries
      # on systems that don't support them.
      lt_prog_compiler_can_build_shared=no
      enable_shared=no
      ;;

    sysv4*MP*)
      if test -d /usr/nec; then
	lt_prog_compiler_pic=-Kconform_pic
      fi
      ;;

    hpux*)
      # PIC is the default for IA64 HP-UX and 64-bit HP-UX, but
      # not for PA HP-UX.
      case $host_cpu in
      hppa*64*|ia64*)
	# +Z the default
	;;
      *)
	lt_prog_compiler_pic='-fPIC'
	;;
      esac
      ;;

    *)
      lt_prog_compiler_pic='-fPIC'
      ;;
    esac
  else
    # PORTME Check for flag to pass linker flags through the system compiler.
    case $host_os in
    aix*)
      lt_prog_compiler_wl='-Wl,'
      if test "$host_cpu" = ia64; then
	# AIX 5 now supports IA64 processor
	lt_prog_compiler_static='-Bstatic'
      else
	lt_prog_compiler_static='-bnso -bI:/lib/syscalls.exp'
      fi
      ;;
      darwin*)
        # PIC is the default on this platform
        # Common symbols not allowed in MH_DYLIB files
       case $cc_basename in
         xlc*)
         lt_prog_compiler_pic='-qnocommon'
         lt_prog_compiler_wl='-Wl,'
         ;;
       esac
       ;;

    mingw* | cygwin* | pw32* | os2*)
      # This hack is so that the source file can tell whether it is being
      # built for inclusion in a dll (and should export symbols for example).
      lt_prog_compiler_pic='-DDLL_EXPORT'
      ;;

    hpux9* | hpux10* | hpux11*)
      lt_prog_compiler_wl='-Wl,'
      # PIC is the default for IA64 HP-UX and 64-bit HP-UX, but
      # not for PA HP-UX.
      case $host_cpu in
      hppa*64*|ia64*)
	# +Z the default
	;;
      *)
	lt_prog_compiler_pic='+Z'
	;;
      esac
      # Is there a better lt_prog_compiler_static that works with the bundled CC?
      lt_prog_compiler_static='${wl}-a ${wl}archive'
      ;;

    irix5* | irix6* | nonstopux*)
      lt_prog_compiler_wl='-Wl,'
      # PIC (with -KPIC) is the default.
      lt_prog_compiler_static='-non_shared'
      ;;

    newsos6)
      lt_prog_compiler_pic='-KPIC'
      lt_prog_compiler_static='-Bstatic'
      ;;

    linux* | k*bsd*-gnu)
      case $cc_basename in
      icc* | ecc*)
	lt_prog_compiler_wl='-Wl,'
	lt_prog_compiler_pic='-KPIC'
	lt_prog_compiler_static='-static'
        ;;
      pgcc* | pgf77* | pgf90* | pgf95*)
        # Portland Group compilers (*not* the Pentium gcc compiler,
	# which looks to be a dead project)
	lt_prog_compiler_wl='-Wl,'
	lt_prog_compiler_pic='-fpic'
	lt_prog_compiler_static='-Bstatic'
        ;;
      ccc*)
        lt_prog_compiler_wl='-Wl,'
        # All Alpha code is PIC.
        lt_prog_compiler_static='-non_shared'
        ;;
      *)
        case `$CC -V 2>&1 | sed 5q` in
	*Sun\ C*)
	  # Sun C 5.9
	  lt_prog_compiler_pic='-KPIC'
	  lt_prog_compiler_static='-Bstatic'
	  lt_prog_compiler_wl='-Wl,'
	  ;;
	*Sun\ F*)
	  # Sun Fortran 8.3 passes all unrecognized flags to the linker
	  lt_prog_compiler_pic='-KPIC'
	  lt_prog_compiler_static='-Bstatic'
	  lt_prog_compiler_wl=''
	  ;;
	esac
	;;
      esac
      ;;

    osf3* | osf4* | osf5*)
      lt_prog_compiler_wl='-Wl,'
      # All OSF/1 code is PIC.
      lt_prog_compiler_static='-non_shared'
      ;;

    rdos*)
      lt_prog_compiler_static='-non_shared'
      ;;

    solaris*)
      lt_prog_compiler_pic='-KPIC'
      lt_prog_compiler_static='-Bstatic'
      case $cc_basename in
      f77* | f90* | f95*)
	lt_prog_compiler_wl='-Qoption ld ';;
      *)
	lt_prog_compiler_wl='-Wl,';;
      esac
      ;;

    sunos4*)
      lt_prog_compiler_wl='-Qoption ld '
      lt_prog_compiler_pic='-PIC'
      lt_prog_compiler_static='-Bstatic'
      ;;

    sysv4 | sysv4.2uw2* | sysv4.3*)
      lt_prog_compiler_wl='-Wl,'
      lt_prog_compiler_pic='-KPIC'
      lt_prog_compiler_static='-Bstatic'
      ;;

    sysv4*MP*)
      if test -d /usr/nec ;then
	lt_prog_compiler_pic='-Kconform_pic'
	lt_prog_compiler_static='-Bstatic'
      fi
      ;;

    sysv5* | unixware* | sco3.2v5* | sco5v6* | OpenUNIX*)
      lt_prog_compiler_wl='-Wl,'
      lt_prog_compiler_pic='-KPIC'
      lt_prog_compiler_static='-Bstatic'
      ;;

    unicos*)
      lt_prog_compiler_wl='-Wl,'
      lt_prog_compiler_can_build_shared=no
      ;;

    uts4*)
      lt_prog_compiler_pic='-pic'
      lt_prog_compiler_static='-Bstatic'
      ;;

    *)
      lt_prog_compiler_can_build_shared=no
      ;;
    esac
  fi

{ echo "$as_me:$LINENO: result: $lt_prog_compiler_pic" >&5
echo "${ECHO_T}$lt_prog_compiler_pic" >&6; }

#
# Check to make sure the PIC flag actually works.
#
if test -n "$lt_prog_compiler_pic"; then

{ echo "$as_me:$LINENO: checking if $compiler PIC flag $lt_prog_compiler_pic works" >&5
echo $ECHO_N "checking if $compiler PIC flag $lt_prog_compiler_pic works... $ECHO_C" >&6; }
if test "${lt_prog_compiler_pic_works+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  lt_prog_compiler_pic_works=no
  ac_outfile=conftest.$ac_objext
   echo "$lt_simple_compile_test_code" > conftest.$ac_ext
   lt_compiler_flag="$lt_prog_compiler_pic -DPIC"
   # Insert the option either (1) after the last *FLAGS variable, or
   # (2) before a word containing "conftest.", or (3) at the end.
   # Note that $ac_compile itself does not contain backslashes and begins
   # with a dollar sign (not a hyphen), so the echo should work correctly.
   # The option is referenced via a variable to avoid confusing sed.
   lt_compile=`echo "$ac_compile" | $SED \
   -e 's:.*FLAGS}\{0,1\} :&$lt_compiler_flag :; t' \
   -e 's: [^ ]*conftest\.: $lt_compiler_flag&:; t' \
   -e 's:$: $lt_compiler_flag:'`
   (eval echo "\"\$as_me:7353: $lt_compile\"" >&5)
   (eval "$lt_compile" 2>conftest.err)
   ac_status=$?
   cat conftest.err >&5
   echo "$as_me:7357: \$? = $ac_status" >&5
   if (exit $ac_status) && test -s "$ac_outfile"; then
     # The compiler can only warn and ignore the option if not recognized
     # So say no if there are warnings other than the usual output.
     $echo "X$_lt_compiler_boilerplate" | $Xsed -e '/^$/d' >conftest.exp
     $SED '/^$/d; /^ *+/d' conftest.err >conftest.er2
     if test ! -s conftest.er2 || diff conftest.exp conftest.er2 >/dev/null; then
       lt_prog_compiler_pic_works=yes
     fi
   fi
   $rm conftest*

fi
{ echo "$as_me:$LINENO: result: $lt_prog_compiler_pic_works" >&5
echo "${ECHO_T}$lt_prog_compiler_pic_works" >&6; }

if test x"$lt_prog_compiler_pic_works" = xyes; then
    case $lt_prog_compiler_pic in
     "" | " "*) ;;
     *) lt_prog_compiler_pic=" $lt_prog_compiler_pic" ;;
     esac
else
    lt_prog_compiler_pic=
     lt_prog_compiler_can_build_shared=no
fi

fi
case $host_os in
  # For platforms which do not support PIC, -DPIC is meaningless:
  *djgpp*)
    lt_prog_compiler_pic=
    ;;
  *)
    lt_prog_compiler_pic="$lt_prog_compiler_pic -DPIC"
    ;;
esac

#
# Check to make sure the static flag actually works.
#
wl=$lt_prog_compiler_wl eval lt_tmp_static_flag=\"$lt_prog_compiler_static\"
{ echo "$as_me:$LINENO: checking if $compiler static flag $lt_tmp_static_flag works" >&5
echo $ECHO_N "checking if $compiler static flag $lt_tmp_static_flag works... $ECHO_C" >&6; }
if test "${lt_prog_compiler_static_works+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  lt_prog_compiler_static_works=no
   save_LDFLAGS="$LDFLAGS"
   LDFLAGS="$LDFLAGS $lt_tmp_static_flag"
   echo "$lt_simple_link_test_code" > conftest.$ac_ext
   if (eval $ac_link 2>conftest.err) && test -s conftest$ac_exeext; then
     # The linker can only warn and ignore the option if not recognized
     # So say no if there are warnings
     if test -s conftest.err; then
       # Append any errors to the config.log.
       cat conftest.err 1>&5
       $echo "X$_lt_linker_boilerplate" | $Xsed -e '/^$/d' > conftest.exp
       $SED '/^$/d; /^ *+/d' conftest.err >conftest.er2
       if diff conftest.exp conftest.er2 >/dev/null; then
         lt_prog_compiler_static_works=yes
       fi
     else
       lt_prog_compiler_static_works=yes
     fi
   fi
   $rm conftest*
   LDFLAGS="$save_LDFLAGS"

fi
{ echo "$as_me:$LINENO: result: $lt_prog_compiler_static_works" >&5
echo "${ECHO_T}$lt_prog_compiler_static_works" >&6; }

if test x"$lt_prog_compiler_static_works" = xyes; then
    :
else
    lt_prog_compiler_static=
fi


{ echo "$as_me:$LINENO: checking if $compiler supports -c -o file.$ac_objext" >&5
echo $ECHO_N "checking if $compiler supports -c -o file.$ac_objext... $ECHO_C" >&6; }
if test "${lt_cv_prog_compiler_c_o+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  lt_cv_prog_compiler_c_o=no
   $rm -r conftest 2>/dev/null
   mkdir conftest
   cd conftest
   mkdir out
   echo "$lt_simple_compile_test_code" > conftest.$ac_ext

   lt_compiler_flag="-o out/conftest2.$ac_objext"
   # Insert the option either (1) after the last *FLAGS variable, or
   # (2) before a word containing "conftest.", or (3) at the end.
   # Note that $ac_compile itself does not contain backslashes and begins
   # with a dollar sign (not a hyphen), so the echo should work correctly.
   lt_compile=`echo "$ac_compile" | $SED \
   -e 's:.*FLAGS}\{0,1\} :&$lt_compiler_flag :; t' \
   -e 's: [^ ]*conftest\.: $lt_compiler_flag&:; t' \
   -e 's:$: $lt_compiler_flag:'`
   (eval echo "\"\$as_me:7457: $lt_compile\"" >&5)
   (eval "$lt_compile" 2>out/conftest.err)
   ac_status=$?
   cat out/conftest.err >&5
   echo "$as_me:7461: \$? = $ac_status" >&5
   if (exit $ac_status) && test -s out/conftest2.$ac_objext
   then
     # The compiler can only warn and ignore the option if not recognized
     # So say no if there are warnings
     $echo "X$_lt_compiler_boilerplate" | $Xsed -e '/^$/d' > out/conftest.exp
     $SED '/^$/d; /^ *+/d' out/conftest.err >out/conftest.er2
     if test ! -s out/conftest.er2 || diff out/conftest.exp out/conftest.er2 >/dev/null; then
       lt_cv_prog_compiler_c_o=yes
     fi
   fi
   chmod u+w . 2>&5
   $rm conftest*
   # SGI C++ compiler will create directory out/ii_files/ for
   # template instantiation
   test -d out/ii_files && $rm out/ii_files/* && rmdir out/ii_files
   $rm out/* && rmdir out
   cd ..
   rmdir conftest
   $rm conftest*

fi
{ echo "$as_me:$LINENO: result: $lt_cv_prog_compiler_c_o" >&5
echo "${ECHO_T}$lt_cv_prog_compiler_c_o" >&6; }


hard_links="nottested"
if test "$lt_cv_prog_compiler_c_o" = no && test "$need_locks" != no; then
  # do not overwrite the value of need_locks provided by the user
  { echo "$as_me:$LINENO: checking if we can lock with hard links" >&5
echo $ECHO_N "checking if we can lock with hard links... $ECHO_C" >&6; }
  hard_links=yes
  $rm conftest*
  ln conftest.a conftest.b 2>/dev/null && hard_links=no
  touch conftest.a
  ln conftest.a conftest.b 2>&5 || hard_links=no
  ln conftest.a conftest.b 2>/dev/null && hard_links=no
  { echo "$as_me:$LINENO: result: $hard_links" >&5
echo "${ECHO_T}$hard_links" >&6; }
  if test "$hard_links" = no; then
    { echo "$as_me:$LINENO: WARNING: \`$CC' does not support \`-c -o', so \`make -j' may be unsafe" >&5
echo "$as_me: WARNING: \`$CC' does not support \`-c -o', so \`make -j' may be unsafe" >&2;}
    need_locks=warn
  fi
else
  need_locks=no
fi

{ echo "$as_me:$LINENO: checking whether the $compiler linker ($LD) supports shared libraries" >&5
echo $ECHO_N "checking whether the $compiler linker ($LD) supports shared libraries... $ECHO_C" >&6; }

  runpath_var=
  allow_undefined_flag=
  enable_shared_with_static_runtimes=no
  archive_cmds=
  archive_expsym_cmds=
  old_archive_From_new_cmds=
  old_archive_from_expsyms_cmds=
  export_dynamic_flag_spec=
  whole_archive_flag_spec=
  thread_safe_flag_spec=
  hardcode_libdir_flag_spec=
  hardcode_libdir_flag_spec_ld=
  hardcode_libdir_separator=
  hardcode_direct=no
  hardcode_minus_L=no
  hardcode_shlibpath_var=unsupported
  link_all_deplibs=unknown
  hardcode_automatic=no
  module_cmds=
  module_expsym_cmds=
  always_export_symbols=no
  export_symbols_cmds='$NM $libobjs $convenience | $global_symbol_pipe | $SED '\''s/.* //'\'' | sort | uniq > $export_symbols'
  # include_expsyms should be a list of space-separated symbols to be *always*
  # included in the symbol list
  include_expsyms=
  # exclude_expsyms can be an extended regexp of symbols to exclude
  # it will be wrapped by ` (' and `)$', so one must not match beginning or
  # end of line.  Example: `a|bc|.*d.*' will exclude the symbols `a' and `bc',
  # as well as any symbol that contains `d'.
  exclude_expsyms="_GLOBAL_OFFSET_TABLE_"
  # Although _GLOBAL_OFFSET_TABLE_ is a valid symbol C name, most a.out
  # platforms (ab)use it in PIC code, but their linkers get confused if
  # the symbol is explicitly referenced.  Since portable code cannot
  # rely on this symbol name, it's probably fine to never include it in
  # preloaded symbol tables.
  extract_expsyms_cmds=
  # Just being paranoid about ensuring that cc_basename is set.
  for cc_temp in $compiler""; do
  case $cc_temp in
    compile | *[\\/]compile | ccache | *[\\/]ccache ) ;;
    distcc | *[\\/]distcc | purify | *[\\/]purify ) ;;
    \-*) ;;
    *) break;;
  esac
done
cc_basename=`$echo "X$cc_temp" | $Xsed -e 's%.*/%%' -e "s%^$host_alias-%%"`

  case $host_os in
  cygwin* | mingw* | pw32*)
    # FIXME: the MSVC++ port hasn't been tested in a loooong time
    # When not using gcc, we currently assume that we are using
    # Microsoft Visual C++.
    if test "$GCC" != yes; then
      with_gnu_ld=no
    fi
    ;;
  interix*)
    # we just hope/assume this is gcc and not c89 (= MSVC++)
    with_gnu_ld=yes
    ;;
  openbsd*)
    with_gnu_ld=no
    ;;
  esac

  ld_shlibs=yes
  if test "$with_gnu_ld" = yes; then
    # If archive_cmds runs LD, not CC, wlarc should be empty
    wlarc='${wl}'

    # Set some defaults for GNU ld with shared library support. These
    # are reset later if shared libraries are not supported. Putting them
    # here allows them to be overridden if necessary.
    runpath_var=LD_RUN_PATH
    hardcode_libdir_flag_spec='${wl}--rpath ${wl}$libdir'
    export_dynamic_flag_spec='${wl}--export-dynamic'
    # ancient GNU ld didn't support --whole-archive et. al.
    if $LD --help 2>&1 | grep 'no-whole-archive' > /dev/null; then
	whole_archive_flag_spec="$wlarc"'--whole-archive$convenience '"$wlarc"'--no-whole-archive'
      else
  	whole_archive_flag_spec=
    fi
    supports_anon_versioning=no
    case `$LD -v 2>/dev/null` in
      *\ [01].* | *\ 2.[0-9].* | *\ 2.10.*) ;; # catch versions < 2.11
      *\ 2.11.93.0.2\ *) supports_anon_versioning=yes ;; # RH7.3 ...
      *\ 2.11.92.0.12\ *) supports_anon_versioning=yes ;; # Mandrake 8.2 ...
      *\ 2.11.*) ;; # other 2.11 versions
      *) supports_anon_versioning=yes ;;
    esac

    # See if GNU ld supports shared libraries.
    case $host_os in
    aix3* | aix4* | aix5*)
      # On AIX/PPC, the GNU linker is very broken
      if test "$host_cpu" != ia64; then
	ld_shlibs=no
	cat <<EOF 1>&2

*** Warning: the GNU linker, at least up to release 2.9.1, is reported
*** to be unable to reliably create shared libraries on AIX.
*** Therefore, libtool is disabling shared libraries support.  If you
*** really care for shared libraries, you may want to modify your PATH
*** so that a non-GNU linker is found, and then restart.

EOF
      fi
      ;;

    amigaos*)
      archive_cmds='$rm $output_objdir/a2ixlibrary.data~$echo "#define NAME $libname" > $output_objdir/a2ixlibrary.data~$echo "#define LIBRARY_ID 1" >> $output_objdir/a2ixlibrary.data~$echo "#define VERSION $major" >> $output_objdir/a2ixlibrary.data~$echo "#define REVISION $revision" >> $output_objdir/a2ixlibrary.data~$AR $AR_FLAGS $lib $libobjs~$RANLIB $lib~(cd $output_objdir && a2ixlibrary -32)'
      hardcode_libdir_flag_spec='-L$libdir'
      hardcode_minus_L=yes

      # Samuel A. Falvo II <kc5tja@dolphin.openprojects.net> reports
      # that the semantics of dynamic libraries on AmigaOS, at least up
      # to version 4, is to share data among multiple programs linked
      # with the same dynamic library.  Since this doesn't match the
      # behavior of shared libraries on other platforms, we can't use
      # them.
      ld_shlibs=no
      ;;

    beos*)
      if $LD --help 2>&1 | grep ': supported targets:.* elf' > /dev/null; then
	allow_undefined_flag=unsupported
	# Joseph Beckenbach <jrb3@best.com> says some releases of gcc
	# support --undefined.  This deserves some investigation.  FIXME
	archive_cmds='$CC -nostart $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname -o $lib'
      else
	ld_shlibs=no
      fi
      ;;

    cygwin* | mingw* | pw32*)
      # _LT_AC_TAGVAR(hardcode_libdir_flag_spec, ) is actually meaningless,
      # as there is no search path for DLLs.
      hardcode_libdir_flag_spec='-L$libdir'
      allow_undefined_flag=unsupported
      always_export_symbols=no
      enable_shared_with_static_runtimes=yes
      export_symbols_cmds='$NM $libobjs $convenience | $global_symbol_pipe | $SED -e '\''/^[BCDGRS][ ]/s/.*[ ]\([^ ]*\)/\1 DATA/'\'' -e '\''/^[AITW][ ]/s/.*[ ]//'\'' | sort | uniq > $export_symbols'

      if $LD --help 2>&1 | grep 'auto-import' > /dev/null; then
        archive_cmds='$CC -shared $libobjs $deplibs $compiler_flags -o $output_objdir/$soname ${wl}--enable-auto-image-base -Xlinker --out-implib -Xlinker $lib'
	# If the export-symbols file already is a .def file (1st line
	# is EXPORTS), use it as is; otherwise, prepend...
	archive_expsym_cmds='if test "x`$SED 1q $export_symbols`" = xEXPORTS; then
	  cp $export_symbols $output_objdir/$soname.def;
	else
	  echo EXPORTS > $output_objdir/$soname.def;
	  cat $export_symbols >> $output_objdir/$soname.def;
	fi~
	$CC -shared $output_objdir/$soname.def $libobjs $deplibs $compiler_flags -o $output_objdir/$soname ${wl}--enable-auto-image-base -Xlinker --out-implib -Xlinker $lib'
      else
	ld_shlibs=no
      fi
      ;;

    interix[3-9]*)
      hardcode_direct=no
      hardcode_shlibpath_var=no
      hardcode_libdir_flag_spec='${wl}-rpath,$libdir'
      export_dynamic_flag_spec='${wl}-E'
      # Hack: On Interix 3.x, we cannot compile PIC because of a broken gcc.
      # Instead, shared libraries are loaded at an image base (0x10000000 by
      # default) and relocated if they conflict, which is a slow very memory
      # consuming and fragmenting process.  To avoid this, we pick a random,
      # 256 KiB-aligned image base between 0x50000000 and 0x6FFC0000 at link
      # time.  Moving up from 0x10000000 also allows more sbrk(2) space.
      archive_cmds='$CC -shared $pic_flag $libobjs $deplibs $compiler_flags ${wl}-h,$soname ${wl}--image-base,`expr ${RANDOM-$$} % 4096 / 2 \* 262144 + 1342177280` -o $lib'
      archive_expsym_cmds='sed "s,^,_," $export_symbols >$output_objdir/$soname.expsym~$CC -shared $pic_flag $libobjs $deplibs $compiler_flags ${wl}-h,$soname ${wl}--retain-symbols-file,$output_objdir/$soname.expsym ${wl}--image-base,`expr ${RANDOM-$$} % 4096 / 2 \* 262144 + 1342177280` -o $lib'
      ;;

    gnu* | linux* | k*bsd*-gnu)
      if $LD --help 2>&1 | grep ': supported targets:.* elf' > /dev/null; then
	tmp_addflag=
	case $cc_basename,$host_cpu in
	pgcc*)				# Portland Group C compiler
	  whole_archive_flag_spec='${wl}--whole-archive`for conv in $convenience\"\"; do test  -n \"$conv\" && new_convenience=\"$new_convenience,$conv\"; done; $echo \"$new_convenience\"` ${wl}--no-whole-archive'
	  tmp_addflag=' $pic_flag'
	  ;;
	pgf77* | pgf90* | pgf95*)	# Portland Group f77 and f90 compilers
	  whole_archive_flag_spec='${wl}--whole-archive`for conv in $convenience\"\"; do test  -n \"$conv\" && new_convenience=\"$new_convenience,$conv\"; done; $echo \"$new_convenience\"` ${wl}--no-whole-archive'
	  tmp_addflag=' $pic_flag -Mnomain' ;;
	ecc*,ia64* | icc*,ia64*)		# Intel C compiler on ia64
	  tmp_addflag=' -i_dynamic' ;;
	efc*,ia64* | ifort*,ia64*)	# Intel Fortran compiler on ia64
	  tmp_addflag=' -i_dynamic -nofor_main' ;;
	ifc* | ifort*)			# Intel Fortran compiler
	  tmp_addflag=' -nofor_main' ;;
	esac
	case `$CC -V 2>&1 | sed 5q` in
	*Sun\ C*)			# Sun C 5.9
	  whole_archive_flag_spec='${wl}--whole-archive`new_convenience=; for conv in $convenience\"\"; do test -z \"$conv\" || new_convenience=\"$new_convenience,$conv\"; done; $echo \"$new_convenience\"` ${wl}--no-whole-archive'
	  tmp_sharedflag='-G' ;;
	*Sun\ F*)			# Sun Fortran 8.3
	  tmp_sharedflag='-G' ;;
	*)
	  tmp_sharedflag='-shared' ;;
	esac
	archive_cmds='$CC '"$tmp_sharedflag""$tmp_addflag"' $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname -o $lib'

	if test $supports_anon_versioning = yes; then
	  archive_expsym_cmds='$echo "{ global:" > $output_objdir/$libname.ver~
  cat $export_symbols | sed -e "s/\(.*\)/\1;/" >> $output_objdir/$libname.ver~
  $echo "local: *; };" >> $output_objdir/$libname.ver~
	  $CC '"$tmp_sharedflag""$tmp_addflag"' $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname ${wl}-version-script ${wl}$output_objdir/$libname.ver -o $lib'
	fi
      else
	ld_shlibs=no
      fi
      ;;

    netbsd*)
      if echo __ELF__ | $CC -E - | grep __ELF__ >/dev/null; then
	archive_cmds='$LD -Bshareable $libobjs $deplibs $linker_flags -o $lib'
	wlarc=
      else
	archive_cmds='$CC -shared $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname -o $lib'
	archive_expsym_cmds='$CC -shared $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname ${wl}-retain-symbols-file $wl$export_symbols -o $lib'
      fi
      ;;

    solaris*)
      if $LD -v 2>&1 | grep 'BFD 2\.8' > /dev/null; then
	ld_shlibs=no
	cat <<EOF 1>&2

*** Warning: The releases 2.8.* of the GNU linker cannot reliably
*** create shared libraries on Solaris systems.  Therefore, libtool
*** is disabling shared libraries support.  We urge you to upgrade GNU
*** binutils to release 2.9.1 or newer.  Another option is to modify
*** your PATH or compiler configuration so that the native linker is
*** used, and then restart.

EOF
      elif $LD --help 2>&1 | grep ': supported targets:.* elf' > /dev/null; then
	archive_cmds='$CC -shared $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname -o $lib'
	archive_expsym_cmds='$CC -shared $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname ${wl}-retain-symbols-file $wl$export_symbols -o $lib'
      else
	ld_shlibs=no
      fi
      ;;

    sysv5* | sco3.2v5* | sco5v6* | unixware* | OpenUNIX*)
      case `$LD -v 2>&1` in
        *\ [01].* | *\ 2.[0-9].* | *\ 2.1[0-5].*)
	ld_shlibs=no
	cat <<_LT_EOF 1>&2

*** Warning: Releases of the GNU linker prior to 2.16.91.0.3 can not
*** reliably create shared libraries on SCO systems.  Therefore, libtool
*** is disabling shared libraries support.  We urge you to upgrade GNU
*** binutils to release 2.16.91.0.3 or newer.  Another option is to modify
*** your PATH or compiler configuration so that the native linker is
*** used, and then restart.

_LT_EOF
	;;
	*)
	  if $LD --help 2>&1 | grep ': supported targets:.* elf' > /dev/null; then
	    hardcode_libdir_flag_spec='`test -z "$SCOABSPATH" && echo ${wl}-rpath,$libdir`'
	    archive_cmds='$CC -shared $libobjs $deplibs $compiler_flags ${wl}-soname,\${SCOABSPATH:+${install_libdir}/}$soname -o $lib'
	    archive_expsym_cmds='$CC -shared $libobjs $deplibs $compiler_flags ${wl}-soname,\${SCOABSPATH:+${install_libdir}/}$soname,-retain-symbols-file,$export_symbols -o $lib'
	  else
	    ld_shlibs=no
	  fi
	;;
      esac
      ;;

    sunos4*)
      archive_cmds='$LD -assert pure-text -Bshareable -o $lib $libobjs $deplibs $linker_flags'
      wlarc=
      hardcode_direct=yes
      hardcode_shlibpath_var=no
      ;;

    *)
      if $LD --help 2>&1 | grep ': supported targets:.* elf' > /dev/null; then
	archive_cmds='$CC -shared $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname -o $lib'
	archive_expsym_cmds='$CC -shared $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname ${wl}-retain-symbols-file $wl$export_symbols -o $lib'
      else
	ld_shlibs=no
      fi
      ;;
    esac

    if test "$ld_shlibs" = no; then
      runpath_var=
      hardcode_libdir_flag_spec=
      export_dynamic_flag_spec=
      whole_archive_flag_spec=
    fi
  else
    # PORTME fill in a description of your system's linker (not GNU ld)
    case $host_os in
    aix3*)
      allow_undefined_flag=unsupported
      always_export_symbols=yes
      archive_expsym_cmds='$LD -o $output_objdir/$soname $libobjs $deplibs $linker_flags -bE:$export_symbols -T512 -H512 -bM:SRE~$AR $AR_FLAGS $lib $output_objdir/$soname'
      # Note: this linker hardcodes the directories in LIBPATH if there
      # are no directories specified by -L.
      hardcode_minus_L=yes
      if test "$GCC" = yes && test -z "$lt_prog_compiler_static"; then
	# Neither direct hardcoding nor static linking is supported with a
	# broken collect2.
	hardcode_direct=unsupported
      fi
      ;;

    aix4* | aix5*)
      if test "$host_cpu" = ia64; then
	# On IA64, the linker does run time linking by default, so we don't
	# have to do anything special.
	aix_use_runtimelinking=no
	exp_sym_flag='-Bexport'
	no_entry_flag=""
      else
	# If we're using GNU nm, then we don't want the "-C" option.
	# -C means demangle to AIX nm, but means don't demangle with GNU nm
	if $NM -V 2>&1 | grep 'GNU' > /dev/null; then
	  export_symbols_cmds='$NM -Bpg $libobjs $convenience | awk '\''{ if (((\$2 == "T") || (\$2 == "D") || (\$2 == "B")) && (substr(\$3,1,1) != ".")) { print \$3 } }'\'' | sort -u > $export_symbols'
	else
	  export_symbols_cmds='$NM -BCpg $libobjs $convenience | awk '\''{ if (((\$2 == "T") || (\$2 == "D") || (\$2 == "B")) && (substr(\$3,1,1) != ".")) { print \$3 } }'\'' | sort -u > $export_symbols'
	fi
	aix_use_runtimelinking=no

	# Test if we are trying to use run time linking or normal
	# AIX style linking. If -brtl is somewhere in LDFLAGS, we
	# need to do runtime linking.
	case $host_os in aix4.[23]|aix4.[23].*|aix5*)
	  for ld_flag in $LDFLAGS; do
  	  if (test $ld_flag = "-brtl" || test $ld_flag = "-Wl,-brtl"); then
  	    aix_use_runtimelinking=yes
  	    break
  	  fi
	  done
	  ;;
	esac

	exp_sym_flag='-bexport'
	no_entry_flag='-bnoentry'
      fi

      # When large executables or shared objects are built, AIX ld can
      # have problems creating the table of contents.  If linking a library
      # or program results in "error TOC overflow" add -mminimal-toc to
      # CXXFLAGS/CFLAGS for g++/gcc.  In the cases where that is not
      # enough to fix the problem, add -Wl,-bbigtoc to LDFLAGS.

      archive_cmds=''
      hardcode_direct=yes
      hardcode_libdir_separator=':'
      link_all_deplibs=yes

      if test "$GCC" = yes; then
	case $host_os in aix4.[012]|aix4.[012].*)
	# We only want to do this on AIX 4.2 and lower, the check
	# below for broken collect2 doesn't work under 4.3+
	  collect2name=`${CC} -print-prog-name=collect2`
	  if test -f "$collect2name" && \
  	   strings "$collect2name" | grep resolve_lib_name >/dev/null
	  then
  	  # We have reworked collect2
  	  :
	  else
  	  # We have old collect2
  	  hardcode_direct=unsupported
  	  # It fails to find uninstalled libraries when the uninstalled
  	  # path is not listed in the libpath.  Setting hardcode_minus_L
  	  # to unsupported forces relinking
  	  hardcode_minus_L=yes
  	  hardcode_libdir_flag_spec='-L$libdir'
  	  hardcode_libdir_separator=
	  fi
	  ;;
	esac
	shared_flag='-shared'
	if test "$aix_use_runtimelinking" = yes; then
	  shared_flag="$shared_flag "'${wl}-G'
	fi
      else
	# not using gcc
	if test "$host_cpu" = ia64; then
  	# VisualAge C++, Version 5.5 for AIX 5L for IA-64, Beta 3 Release
  	# chokes on -Wl,-G. The following line is correct:
	  shared_flag='-G'
	else
	  if test "$aix_use_runtimelinking" = yes; then
	    shared_flag='${wl}-G'
	  else
	    shared_flag='${wl}-bM:SRE'
	  fi
	fi
      fi

      # It seems that -bexpall does not export symbols beginning with
      # underscore (_), so it is better to generate a list of symbols to export.
      always_export_symbols=yes
      if test "$aix_use_runtimelinking" = yes; then
	# Warning - without using the other runtime loading flags (-brtl),
	# -berok will link without error, but may produce a broken library.
	allow_undefined_flag='-berok'
       # Determine the default libpath from the value encoded in an empty executable.
       cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

int
main ()
{

  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_c_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest$ac_exeext &&
       $as_test_x conftest$ac_exeext; then

lt_aix_libpath_sed='
    /Import File Strings/,/^$/ {
	/^0/ {
	    s/^0  *\(.*\)$/\1/
	    p
	}
    }'
aix_libpath=`dump -H conftest$ac_exeext 2>/dev/null | $SED -n -e "$lt_aix_libpath_sed"`
# Check for a 64-bit object if we didn't find anything.
if test -z "$aix_libpath"; then
  aix_libpath=`dump -HX64 conftest$ac_exeext 2>/dev/null | $SED -n -e "$lt_aix_libpath_sed"`
fi
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5


fi

rm -f core conftest.err conftest.$ac_objext conftest_ipa8_conftest.oo \
      conftest$ac_exeext conftest.$ac_ext
if test -z "$aix_libpath"; then aix_libpath="/usr/lib:/lib"; fi

       hardcode_libdir_flag_spec='${wl}-blibpath:$libdir:'"$aix_libpath"
	archive_expsym_cmds="\$CC"' -o $output_objdir/$soname $libobjs $deplibs '"\${wl}$no_entry_flag"' $compiler_flags `if test "x${allow_undefined_flag}" != "x"; then echo "${wl}${allow_undefined_flag}"; else :; fi` '"\${wl}$exp_sym_flag:\$export_symbols $shared_flag"
       else
	if test "$host_cpu" = ia64; then
	  hardcode_libdir_flag_spec='${wl}-R $libdir:/usr/lib:/lib'
	  allow_undefined_flag="-z nodefs"
	  archive_expsym_cmds="\$CC $shared_flag"' -o $output_objdir/$soname $libobjs $deplibs '"\${wl}$no_entry_flag"' $compiler_flags ${wl}${allow_undefined_flag} '"\${wl}$exp_sym_flag:\$export_symbols"
	else
	 # Determine the default libpath from the value encoded in an empty executable.
	 cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

int
main ()
{

  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_c_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest$ac_exeext &&
       $as_test_x conftest$ac_exeext; then

lt_aix_libpath_sed='
    /Import File Strings/,/^$/ {
	/^0/ {
	    s/^0  *\(.*\)$/\1/
	    p
	}
    }'
aix_libpath=`dump -H conftest$ac_exeext 2>/dev/null | $SED -n -e "$lt_aix_libpath_sed"`
# Check for a 64-bit object if we didn't find anything.
if test -z "$aix_libpath"; then
  aix_libpath=`dump -HX64 conftest$ac_exeext 2>/dev/null | $SED -n -e "$lt_aix_libpath_sed"`
fi
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5


fi

rm -f core conftest.err conftest.$ac_objext conftest_ipa8_conftest.oo \
      conftest$ac_exeext conftest.$ac_ext
if test -z "$aix_libpath"; then aix_libpath="/usr/lib:/lib"; fi

	 hardcode_libdir_flag_spec='${wl}-blibpath:$libdir:'"$aix_libpath"
	  # Warning - without using the other run time loading flags,
	  # -berok will link without error, but may produce a broken library.
	  no_undefined_flag=' ${wl}-bernotok'
	  allow_undefined_flag=' ${wl}-berok'
	  # Exported symbols can be pulled into shared objects from archives
	  whole_archive_flag_spec='$convenience'
	  archive_cmds_need_lc=yes
	  # This is similar to how AIX traditionally builds its shared libraries.
	  archive_expsym_cmds="\$CC $shared_flag"' -o $output_objdir/$soname $libobjs $deplibs ${wl}-bnoentry $compiler_flags ${wl}-bE:$export_symbols${allow_undefined_flag}~$AR $AR_FLAGS $output_objdir/$libname$release.a $output_objdir/$soname'
	fi
      fi
      ;;

    amigaos*)
      archive_cmds='$rm $output_objdir/a2ixlibrary.data~$echo "#define NAME $libname" > $output_objdir/a2ixlibrary.data~$echo "#define LIBRARY_ID 1" >> $output_objdir/a2ixlibrary.data~$echo "#define VERSION $major" >> $output_objdir/a2ixlibrary.data~$echo "#define REVISION $revision" >> $output_objdir/a2ixlibrary.data~$AR $AR_FLAGS $lib $libobjs~$RANLIB $lib~(cd $output_objdir && a2ixlibrary -32)'
      hardcode_libdir_flag_spec='-L$libdir'
      hardcode_minus_L=yes
      # see comment about different semantics on the GNU ld section
      ld_shlibs=no
      ;;

    bsdi[45]*)
      export_dynamic_flag_spec=-rdynamic
      ;;

    cygwin* | mingw* | pw32*)
      # When not using gcc, we currently assume that we are using
      # Microsoft Visual C++.
      # hardcode_libdir_flag_spec is actually meaningless, as there is
      # no search path for DLLs.
      hardcode_libdir_flag_spec=' '
      allow_undefined_flag=unsupported
      # Tell ltmain to make .lib files, not .a files.
      libext=lib
      # Tell ltmain to make .dll files, not .so files.
      shrext_cmds=".dll"
      # FIXME: Setting linknames here is a bad hack.
      archive_cmds='$CC -o $lib $libobjs $compiler_flags `echo "$deplibs" | $SED -e '\''s/ -lc$//'\''` -link -dll~linknames='
      # The linker will automatically build a .lib file if we build a DLL.
      old_archive_From_new_cmds='true'
      # FIXME: Should let the user specify the lib program.
      old_archive_cmds='lib -OUT:$oldlib$oldobjs$old_deplibs'
      fix_srcfile_path='`cygpath -w "$srcfile"`'
      enable_shared_with_static_runtimes=yes
      ;;

    darwin* | rhapsody*)
      case $host_os in
        rhapsody* | darwin1.[012])
         allow_undefined_flag='${wl}-undefined ${wl}suppress'
         ;;
       *) # Darwin 1.3 on
         if test -z ${MACOSX_DEPLOYMENT_TARGET} ; then
           allow_undefined_flag='${wl}-flat_namespace ${wl}-undefined ${wl}suppress'
         else
           case ${MACOSX_DEPLOYMENT_TARGET} in
             10.[012])
               allow_undefined_flag='${wl}-flat_namespace ${wl}-undefined ${wl}suppress'
               ;;
             10.*)
               allow_undefined_flag='${wl}-undefined ${wl}dynamic_lookup'
               ;;
           esac
         fi
         ;;
      esac
      archive_cmds_need_lc=no
      hardcode_direct=no
      hardcode_automatic=yes
      hardcode_shlibpath_var=unsupported
      whole_archive_flag_spec=''
      link_all_deplibs=yes
    if test "$GCC" = yes ; then
    	output_verbose_link_cmd='echo'
        archive_cmds='$CC -dynamiclib $allow_undefined_flag -o $lib $libobjs $deplibs $compiler_flags -install_name $rpath/$soname $verstring'
      module_cmds='$CC $allow_undefined_flag -o $lib -bundle $libobjs $deplibs$compiler_flags'
      # Don't fix this by using the ld -exported_symbols_list flag, it doesn't exist in older darwin lds
      archive_expsym_cmds='sed -e "s,#.*,," -e "s,^[    ]*,," -e "s,^\(..*\),_&," < $export_symbols > $output_objdir/${libname}-symbols.expsym~$CC -dynamiclib $allow_undefined_flag -o $lib $libobjs $deplibs $compiler_flags -install_name $rpath/$soname $verstring~nmedit -s $output_objdir/${libname}-symbols.expsym ${lib}'
      module_expsym_cmds='sed -e "s,#.*,," -e "s,^[    ]*,," -e "s,^\(..*\),_&," < $export_symbols > $output_objdir/${libname}-symbols.expsym~$CC $allow_undefined_flag  -o $lib -bundle $libobjs $deplibs$compiler_flags~nmedit -s $output_objdir/${libname}-symbols.expsym ${lib}'
    else
      case $cc_basename in
        xlc*)
         output_verbose_link_cmd='echo'
         archive_cmds='$CC -qmkshrobj $allow_undefined_flag -o $lib $libobjs $deplibs $compiler_flags ${wl}-install_name ${wl}`echo $rpath/$soname` $xlcverstring'
         module_cmds='$CC $allow_undefined_flag -o $lib -bundle $libobjs $deplibs$compiler_flags'
          # Don't fix this by using the ld -exported_symbols_list flag, it doesn't exist in older darwin lds
         archive_expsym_cmds='sed -e "s,#.*,," -e "s,^[    ]*,," -e "s,^\(..*\),_&," < $export_symbols > $output_objdir/${libname}-symbols.expsym~$CC -qmkshrobj $allow_undefined_flag -o $lib $libobjs $deplibs $compiler_flags ${wl}-install_name ${wl}$rpath/$soname $xlcverstring~nmedit -s $output_objdir/${libname}-symbols.expsym ${lib}'
          module_expsym_cmds='sed -e "s,#.*,," -e "s,^[    ]*,," -e "s,^\(..*\),_&," < $export_symbols > $output_objdir/${libname}-symbols.expsym~$CC $allow_undefined_flag  -o $lib -bundle $libobjs $deplibs$compiler_flags~nmedit -s $output_objdir/${libname}-symbols.expsym ${lib}'
          ;;
       *)
         ld_shlibs=no
          ;;
      esac
    fi
      ;;

    dgux*)
      archive_cmds='$LD -G -h $soname -o $lib $libobjs $deplibs $linker_flags'
      hardcode_libdir_flag_spec='-L$libdir'
      hardcode_shlibpath_var=no
      ;;

    freebsd1*)
      ld_shlibs=no
      ;;

    # FreeBSD 2.2.[012] allows us to include c++rt0.o to get C++ constructor
    # support.  Future versions do this automatically, but an explicit c++rt0.o
    # does not break anything, and helps significantly (at the cost of a little
    # extra space).
    freebsd2.2*)
      archive_cmds='$LD -Bshareable -o $lib $libobjs $deplibs $linker_flags /usr/lib/c++rt0.o'
      hardcode_libdir_flag_spec='-R$libdir'
      hardcode_direct=yes
      hardcode_shlibpath_var=no
      ;;

    # Unfortunately, older versions of FreeBSD 2 do not have this feature.
    freebsd2*)
      archive_cmds='$LD -Bshareable -o $lib $libobjs $deplibs $linker_flags'
      hardcode_direct=yes
      hardcode_minus_L=yes
      hardcode_shlibpath_var=no
      ;;

    # FreeBSD 3 and greater uses gcc -shared to do shared libraries.
    freebsd* | dragonfly*)
      archive_cmds='$CC -shared -o $lib $libobjs $deplibs $compiler_flags'
      hardcode_libdir_flag_spec='-R$libdir'
      hardcode_direct=yes
      hardcode_shlibpath_var=no
      ;;

    hpux9*)
      if test "$GCC" = yes; then
	archive_cmds='$rm $output_objdir/$soname~$CC -shared -fPIC ${wl}+b ${wl}$install_libdir -o $output_objdir/$soname $libobjs $deplibs $compiler_flags~test $output_objdir/$soname = $lib || mv $output_objdir/$soname $lib'
      else
	archive_cmds='$rm $output_objdir/$soname~$LD -b +b $install_libdir -o $output_objdir/$soname $libobjs $deplibs $linker_flags~test $output_objdir/$soname = $lib || mv $output_objdir/$soname $lib'
      fi
      hardcode_libdir_flag_spec='${wl}+b ${wl}$libdir'
      hardcode_libdir_separator=:
      hardcode_direct=yes

      # hardcode_minus_L: Not really in the search PATH,
      # but as the default location of the library.
      hardcode_minus_L=yes
      export_dynamic_flag_spec='${wl}-E'
      ;;

    hpux10*)
      if test "$GCC" = yes -a "$with_gnu_ld" = no; then
	archive_cmds='$CC -shared -fPIC ${wl}+h ${wl}$soname ${wl}+b ${wl}$install_libdir -o $lib $libobjs $deplibs $compiler_flags'
      else
	archive_cmds='$LD -b +h $soname +b $install_libdir -o $lib $libobjs $deplibs $linker_flags'
      fi
      if test "$with_gnu_ld" = no; then
	hardcode_libdir_flag_spec='${wl}+b ${wl}$libdir'
	hardcode_libdir_separator=:

	hardcode_direct=yes
	export_dynamic_flag_spec='${wl}-E'

	# hardcode_minus_L: Not really in the search PATH,
	# but as the default location of the library.
	hardcode_minus_L=yes
      fi
      ;;

    hpux11*)
      if test "$GCC" = yes -a "$with_gnu_ld" = no; then
	case $host_cpu in
	hppa*64*)
	  archive_cmds='$CC -shared ${wl}+h ${wl}$soname -o $lib $libobjs $deplibs $compiler_flags'
	  ;;
	ia64*)
	  archive_cmds='$CC -shared ${wl}+h ${wl}$soname ${wl}+nodefaultrpath -o $lib $libobjs $deplibs $compiler_flags'
	  ;;
	*)
	  archive_cmds='$CC -shared -fPIC ${wl}+h ${wl}$soname ${wl}+b ${wl}$install_libdir -o $lib $libobjs $deplibs $compiler_flags'
	  ;;
	esac
      else
	case $host_cpu in
	hppa*64*)
	  archive_cmds='$CC -b ${wl}+h ${wl}$soname -o $lib $libobjs $deplibs $compiler_flags'
	  ;;
	ia64*)
	  archive_cmds='$CC -b ${wl}+h ${wl}$soname ${wl}+nodefaultrpath -o $lib $libobjs $deplibs $compiler_flags'
	  ;;
	*)
	  archive_cmds='$CC -b ${wl}+h ${wl}$soname ${wl}+b ${wl}$install_libdir -o $lib $libobjs $deplibs $compiler_flags'
	  ;;
	esac
      fi
      if test "$with_gnu_ld" = no; then
	hardcode_libdir_flag_spec='${wl}+b ${wl}$libdir'
	hardcode_libdir_separator=:

	case $host_cpu in
	hppa*64*|ia64*)
	  hardcode_libdir_flag_spec_ld='+b $libdir'
	  hardcode_direct=no
	  hardcode_shlibpath_var=no
	  ;;
	*)
	  hardcode_direct=yes
	  export_dynamic_flag_spec='${wl}-E'

	  # hardcode_minus_L: Not really in the search PATH,
	  # but as the default location of the library.
	  hardcode_minus_L=yes
	  ;;
	esac
      fi
      ;;

    irix5* | irix6* | nonstopux*)
      if test "$GCC" = yes; then
	archive_cmds='$CC -shared $libobjs $deplibs $compiler_flags ${wl}-soname ${wl}$soname `test -n "$verstring" && echo ${wl}-set_version ${wl}$verstring` ${wl}-update_registry ${wl}${output_objdir}/so_locations -o $lib'
      else
	archive_cmds='$LD -shared $libobjs $deplibs $linker_flags -soname $soname `test -n "$verstring" && echo -set_version $verstring` -update_registry ${output_objdir}/so_locations -o $lib'
	hardcode_libdir_flag_spec_ld='-rpath $libdir'
      fi
      hardcode_libdir_flag_spec='${wl}-rpath ${wl}$libdir'
      hardcode_libdir_separator=:
      link_all_deplibs=yes
      ;;

    netbsd*)
      if echo __ELF__ | $CC -E - | grep __ELF__ >/dev/null; then
	archive_cmds='$LD -Bshareable -o $lib $libobjs $deplibs $linker_flags'  # a.out
      else
	archive_cmds='$LD -shared -o $lib $libobjs $deplibs $linker_flags'      # ELF
      fi
      hardcode_libdir_flag_spec='-R$libdir'
      hardcode_direct=yes
      hardcode_shlibpath_var=no
      ;;

    newsos6)
      archive_cmds='$LD -G -h $soname -o $lib $libobjs $deplibs $linker_flags'
      hardcode_direct=yes
      hardcode_libdir_flag_spec='${wl}-rpath ${wl}$libdir'
      hardcode_libdir_separator=:
      hardcode_shlibpath_var=no
      ;;

    openbsd*)
      if test -f /usr/libexec/ld.so; then
	hardcode_direct=yes
	hardcode_shlibpath_var=no
	if test -z "`echo __ELF__ | $CC -E - | grep __ELF__`" || test "$host_os-$host_cpu" = "openbsd2.8-powerpc"; then
	  archive_cmds='$CC -shared $pic_flag -o $lib $libobjs $deplibs $compiler_flags'
	  archive_expsym_cmds='$CC -shared $pic_flag -o $lib $libobjs $deplibs $compiler_flags ${wl}-retain-symbols-file,$export_symbols'
	  hardcode_libdir_flag_spec='${wl}-rpath,$libdir'
	  export_dynamic_flag_spec='${wl}-E'
	else
	  case $host_os in
	   openbsd[01].* | openbsd2.[0-7] | openbsd2.[0-7].*)
	     archive_cmds='$LD -Bshareable -o $lib $libobjs $deplibs $linker_flags'
	     hardcode_libdir_flag_spec='-R$libdir'
	     ;;
	   *)
	     archive_cmds='$CC -shared $pic_flag -o $lib $libobjs $deplibs $compiler_flags'
	     hardcode_libdir_flag_spec='${wl}-rpath,$libdir'
	     ;;
	  esac
        fi
      else
	ld_shlibs=no
      fi
      ;;

    os2*)
      hardcode_libdir_flag_spec='-L$libdir'
      hardcode_minus_L=yes
      allow_undefined_flag=unsupported
      archive_cmds='$echo "LIBRARY $libname INITINSTANCE" > $output_objdir/$libname.def~$echo "DESCRIPTION \"$libname\"" >> $output_objdir/$libname.def~$echo DATA >> $output_objdir/$libname.def~$echo " SINGLE NONSHARED" >> $output_objdir/$libname.def~$echo EXPORTS >> $output_objdir/$libname.def~emxexp $libobjs >> $output_objdir/$libname.def~$CC -Zdll -Zcrtdll -o $lib $libobjs $deplibs $compiler_flags $output_objdir/$libname.def'
      old_archive_From_new_cmds='emximp -o $output_objdir/$libname.a $output_objdir/$libname.def'
      ;;

    osf3*)
      if test "$GCC" = yes; then
	allow_undefined_flag=' ${wl}-expect_unresolved ${wl}\*'
	archive_cmds='$CC -shared${allow_undefined_flag} $libobjs $deplibs $compiler_flags ${wl}-soname ${wl}$soname `test -n "$verstring" && echo ${wl}-set_version ${wl}$verstring` ${wl}-update_registry ${wl}${output_objdir}/so_locations -o $lib'
      else
	allow_undefined_flag=' -expect_unresolved \*'
	archive_cmds='$LD -shared${allow_undefined_flag} $libobjs $deplibs $linker_flags -soname $soname `test -n "$verstring" && echo -set_version $verstring` -update_registry ${output_objdir}/so_locations -o $lib'
      fi
      hardcode_libdir_flag_spec='${wl}-rpath ${wl}$libdir'
      hardcode_libdir_separator=:
      ;;

    osf4* | osf5*)	# as osf3* with the addition of -msym flag
      if test "$GCC" = yes; then
	allow_undefined_flag=' ${wl}-expect_unresolved ${wl}\*'
	archive_cmds='$CC -shared${allow_undefined_flag} $libobjs $deplibs $compiler_flags ${wl}-msym ${wl}-soname ${wl}$soname `test -n "$verstring" && echo ${wl}-set_version ${wl}$verstring` ${wl}-update_registry ${wl}${output_objdir}/so_locations -o $lib'
	hardcode_libdir_flag_spec='${wl}-rpath ${wl}$libdir'
      else
	allow_undefined_flag=' -expect_unresolved \*'
	archive_cmds='$LD -shared${allow_undefined_flag} $libobjs $deplibs $linker_flags -msym -soname $soname `test -n "$verstring" && echo -set_version $verstring` -update_registry ${output_objdir}/so_locations -o $lib'
	archive_expsym_cmds='for i in `cat $export_symbols`; do printf "%s %s\\n" -exported_symbol "\$i" >> $lib.exp; done; echo "-hidden">> $lib.exp~
	$LD -shared${allow_undefined_flag} -input $lib.exp $linker_flags $libobjs $deplibs -soname $soname `test -n "$verstring" && echo -set_version $verstring` -update_registry ${output_objdir}/so_locations -o $lib~$rm $lib.exp'

	# Both c and cxx compiler support -rpath directly
	hardcode_libdir_flag_spec='-rpath $libdir'
      fi
      hardcode_libdir_separator=:
      ;;

    solaris*)
      no_undefined_flag=' -z text'
      if test "$GCC" = yes; then
	wlarc='${wl}'
	archive_cmds='$CC -shared ${wl}-h ${wl}$soname -o $lib $libobjs $deplibs $compiler_flags'
	archive_expsym_cmds='$echo "{ global:" > $lib.exp~cat $export_symbols | $SED -e "s/\(.*\)/\1;/" >> $lib.exp~$echo "local: *; };" >> $lib.exp~
	  $CC -shared ${wl}-M ${wl}$lib.exp ${wl}-h ${wl}$soname -o $lib $libobjs $deplibs $compiler_flags~$rm $lib.exp'
      else
	wlarc=''
	archive_cmds='$LD -G${allow_undefined_flag} -h $soname -o $lib $libobjs $deplibs $linker_flags'
	archive_expsym_cmds='$echo "{ global:" > $lib.exp~cat $export_symbols | $SED -e "s/\(.*\)/\1;/" >> $lib.exp~$echo "local: *; };" >> $lib.exp~
  	$LD -G${allow_undefined_flag} -M $lib.exp -h $soname -o $lib $libobjs $deplibs $linker_flags~$rm $lib.exp'
      fi
      hardcode_libdir_flag_spec='-R$libdir'
      hardcode_shlibpath_var=no
      case $host_os in
      solaris2.[0-5] | solaris2.[0-5].*) ;;
      *)
	# The compiler driver will combine and reorder linker options,
	# but understands `-z linker_flag'.  GCC discards it without `$wl',
	# but is careful enough not to reorder.
 	# Supported since Solaris 2.6 (maybe 2.5.1?)
	if test "$GCC" = yes; then
	  whole_archive_flag_spec='${wl}-z ${wl}allextract$convenience ${wl}-z ${wl}defaultextract'
	else
	  whole_archive_flag_spec='-z allextract$convenience -z defaultextract'
	fi
	;;
      esac
      link_all_deplibs=yes
      ;;

    sunos4*)
      if test "x$host_vendor" = xsequent; then
	# Use $CC to link under sequent, because it throws in some extra .o
	# files that make .init and .fini sections work.
	archive_cmds='$CC -G ${wl}-h $soname -o $lib $libobjs $deplibs $compiler_flags'
      else
	archive_cmds='$LD -assert pure-text -Bstatic -o $lib $libobjs $deplibs $linker_flags'
      fi
      hardcode_libdir_flag_spec='-L$libdir'
      hardcode_direct=yes
      hardcode_minus_L=yes
      hardcode_shlibpath_var=no
      ;;

    sysv4)
      case $host_vendor in
	sni)
	  archive_cmds='$LD -G -h $soname -o $lib $libobjs $deplibs $linker_flags'
	  hardcode_direct=yes # is this really true???
	;;
	siemens)
	  ## LD is ld it makes a PLAMLIB
	  ## CC just makes a GrossModule.
	  archive_cmds='$LD -G -o $lib $libobjs $deplibs $linker_flags'
	  reload_cmds='$CC -r -o $output$reload_objs'
	  hardcode_direct=no
        ;;
	motorola)
	  archive_cmds='$LD -G -h $soname -o $lib $libobjs $deplibs $linker_flags'
	  hardcode_direct=no #Motorola manual says yes, but my tests say they lie
	;;
      esac
      runpath_var='LD_RUN_PATH'
      hardcode_shlibpath_var=no
      ;;

    sysv4.3*)
      archive_cmds='$LD -G -h $soname -o $lib $libobjs $deplibs $linker_flags'
      hardcode_shlibpath_var=no
      export_dynamic_flag_spec='-Bexport'
      ;;

    sysv4*MP*)
      if test -d /usr/nec; then
	archive_cmds='$LD -G -h $soname -o $lib $libobjs $deplibs $linker_flags'
	hardcode_shlibpath_var=no
	runpath_var=LD_RUN_PATH
	hardcode_runpath_var=yes
	ld_shlibs=yes
      fi
      ;;

    sysv4*uw2* | sysv5OpenUNIX* | sysv5UnixWare7.[01].[10]* | unixware7* | sco3.2v5.0.[024]*)
      no_undefined_flag='${wl}-z,text'
      archive_cmds_need_lc=no
      hardcode_shlibpath_var=no
      runpath_var='LD_RUN_PATH'

      if test "$GCC" = yes; then
	archive_cmds='$CC -shared ${wl}-h,$soname -o $lib $libobjs $deplibs $compiler_flags'
	archive_expsym_cmds='$CC -shared ${wl}-Bexport:$export_symbols ${wl}-h,$soname -o $lib $libobjs $deplibs $compiler_flags'
      else
	archive_cmds='$CC -G ${wl}-h,$soname -o $lib $libobjs $deplibs $compiler_flags'
	archive_expsym_cmds='$CC -G ${wl}-Bexport:$export_symbols ${wl}-h,$soname -o $lib $libobjs $deplibs $compiler_flags'
      fi
      ;;

    sysv5* | sco3.2v5* | sco5v6*)
      # Note: We can NOT use -z defs as we might desire, because we do not
      # link with -lc, and that would cause any symbols used from libc to
      # always be unresolved, which means just about no library would
      # ever link correctly.  If we're not using GNU ld we use -z text
      # though, which does catch some bad symbols but isn't as heavy-handed
      # as -z defs.
      no_undefined_flag='${wl}-z,text'
      allow_undefined_flag='${wl}-z,nodefs'
      archive_cmds_need_lc=no
      hardcode_shlibpath_var=no
      hardcode_libdir_flag_spec='`test -z "$SCOABSPATH" && echo ${wl}-R,$libdir`'
      hardcode_libdir_separator=':'
      link_all_deplibs=yes
      export_dynamic_flag_spec='${wl}-Bexport'
      runpath_var='LD_RUN_PATH'

      if test "$GCC" = yes; then
	archive_cmds='$CC -shared ${wl}-h,\${SCOABSPATH:+${install_libdir}/}$soname -o $lib $libobjs $deplibs $compiler_flags'
	archive_expsym_cmds='$CC -shared ${wl}-Bexport:$export_symbols ${wl}-h,\${SCOABSPATH:+${install_libdir}/}$soname -o $lib $libobjs $deplibs $compiler_flags'
      else
	archive_cmds='$CC -G ${wl}-h,\${SCOABSPATH:+${install_libdir}/}$soname -o $lib $libobjs $deplibs $compiler_flags'
	archive_expsym_cmds='$CC -G ${wl}-Bexport:$export_symbols ${wl}-h,\${SCOABSPATH:+${install_libdir}/}$soname -o $lib $libobjs $deplibs $compiler_flags'
      fi
      ;;

    uts4*)
      archive_cmds='$LD -G -h $soname -o $lib $libobjs $deplibs $linker_flags'
      hardcode_libdir_flag_spec='-L$libdir'
      hardcode_shlibpath_var=no
      ;;

    *)
      ld_shlibs=no
      ;;
    esac
  fi

{ echo "$as_me:$LINENO: result: $ld_shlibs" >&5
echo "${ECHO_T}$ld_shlibs" >&6; }
test "$ld_shlibs" = no && can_build_shared=no

#
# Do we need to explicitly link libc?
#
case "x$archive_cmds_need_lc" in
x|xyes)
  # Assume -lc should be added
  archive_cmds_need_lc=yes

  if test "$enable_shared" = yes && test "$GCC" = yes; then
    case $archive_cmds in
    *'~'*)
      # FIXME: we may have to deal with multi-command sequences.
      ;;
    '$CC '*)
      # Test whether the compiler implicitly links with -lc since on some
      # systems, -lgcc has to come before -lc. If gcc already passes -lc
      # to ld, don't add -lc before -lgcc.
      { echo "$as_me:$LINENO: checking whether -lc should be explicitly linked in" >&5
echo $ECHO_N "checking whether -lc should be explicitly linked in... $ECHO_C" >&6; }
      $rm conftest*
      echo "$lt_simple_compile_test_code" > conftest.$ac_ext

      if { (eval echo "$as_me:$LINENO: \"$ac_compile\"") >&5
  (eval $ac_compile) 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } 2>conftest.err; then
        soname=conftest
        lib=conftest
        libobjs=conftest.$ac_objext
        deplibs=
        wl=$lt_prog_compiler_wl
	pic_flag=$lt_prog_compiler_pic
        compiler_flags=-v
        linker_flags=-v
        verstring=
        output_objdir=.
        libname=conftest
        lt_save_allow_undefined_flag=$allow_undefined_flag
        allow_undefined_flag=
        if { (eval echo "$as_me:$LINENO: \"$archive_cmds 2\>\&1 \| grep \" -lc \" \>/dev/null 2\>\&1\"") >&5
  (eval $archive_cmds 2\>\&1 \| grep \" -lc \" \>/dev/null 2\>\&1) 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }
        then
	  archive_cmds_need_lc=no
        else
	  archive_cmds_need_lc=yes
        fi
        allow_undefined_flag=$lt_save_allow_undefined_flag
      else
        cat conftest.err 1>&5
      fi
      $rm conftest*
      { echo "$as_me:$LINENO: result: $archive_cmds_need_lc" >&5
echo "${ECHO_T}$archive_cmds_need_lc" >&6; }
      ;;
    esac
  fi
  ;;
esac

{ echo "$as_me:$LINENO: checking dynamic linker characteristics" >&5
echo $ECHO_N "checking dynamic linker characteristics... $ECHO_C" >&6; }
library_names_spec=
libname_spec='lib$name'
soname_spec=
shrext_cmds=".so"
postinstall_cmds=
postuninstall_cmds=
finish_cmds=
finish_eval=
shlibpath_var=
shlibpath_overrides_runpath=unknown
version_type=none
dynamic_linker="$host_os ld.so"
sys_lib_dlsearch_path_spec="/lib /usr/lib"

if test "$GCC" = yes; then
  case $host_os in
    darwin*) lt_awk_arg="/^libraries:/,/LR/" ;;
    *) lt_awk_arg="/^libraries:/" ;;
  esac
  lt_search_path_spec=`$CC -print-search-dirs | awk $lt_awk_arg | $SED -e "s/^libraries://" -e "s,=/,/,g"`
  if echo "$lt_search_path_spec" | grep ';' >/dev/null ; then
    # if the path contains ";" then we assume it to be the separator
    # otherwise default to the standard path separator (i.e. ":") - it is
    # assumed that no part of a normal pathname contains ";" but that should
    # okay in the real world where ";" in dirpaths is itself problematic.
    lt_search_path_spec=`echo "$lt_search_path_spec" | $SED -e 's/;/ /g'`
  else
    lt_search_path_spec=`echo "$lt_search_path_spec" | $SED  -e "s/$PATH_SEPARATOR/ /g"`
  fi
  # Ok, now we have the path, separated by spaces, we can step through it
  # and add multilib dir if necessary.
  lt_tmp_lt_search_path_spec=
  lt_multi_os_dir=`$CC $CPPFLAGS $CFLAGS $LDFLAGS -print-multi-os-directory 2>/dev/null`
  for lt_sys_path in $lt_search_path_spec; do
    if test -d "$lt_sys_path/$lt_multi_os_dir"; then
      lt_tmp_lt_search_path_spec="$lt_tmp_lt_search_path_spec $lt_sys_path/$lt_multi_os_dir"
    else
      test -d "$lt_sys_path" && \
	lt_tmp_lt_search_path_spec="$lt_tmp_lt_search_path_spec $lt_sys_path"
    fi
  done
  lt_search_path_spec=`echo $lt_tmp_lt_search_path_spec | awk '
BEGIN {RS=" "; FS="/|\n";} {
  lt_foo="";
  lt_count=0;
  for (lt_i = NF; lt_i > 0; lt_i--) {
    if ($lt_i != "" && $lt_i != ".") {
      if ($lt_i == "..") {
        lt_count++;
      } else {
        if (lt_count == 0) {
          lt_foo="/" $lt_i lt_foo;
        } else {
          lt_count--;
        }
      }
    }
  }
  if (lt_foo != "") { lt_freq[lt_foo]++; }
  if (lt_freq[lt_foo] == 1) { print lt_foo; }
}'`
  sys_lib_search_path_spec=`echo $lt_search_path_spec`
else
  sys_lib_search_path_spec="/lib /usr/lib /usr/local/lib"
fi
need_lib_prefix=unknown
hardcode_into_libs=no

# when you set need_version to no, make sure it does not cause -set_version
# flags to be left without arguments
need_version=unknown

case $host_os in
aix3*)
  version_type=linux
  library_names_spec='${libname}${release}${shared_ext}$versuffix $libname.a'
  shlibpath_var=LIBPATH

  # AIX 3 has no versioning support, so we append a major version to the name.
  soname_spec='${libname}${release}${shared_ext}$major'
  ;;

aix4* | aix5*)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  hardcode_into_libs=yes
  if test "$host_cpu" = ia64; then
    # AIX 5 supports IA64
    library_names_spec='${libname}${release}${shared_ext}$major ${libname}${release}${shared_ext}$versuffix $libname${shared_ext}'
    shlibpath_var=LD_LIBRARY_PATH
  else
    # With GCC up to 2.95.x, collect2 would create an import file
    # for dependence libraries.  The import file would start with
    # the line `#! .'.  This would cause the generated library to
    # depend on `.', always an invalid library.  This was fixed in
    # development snapshots of GCC prior to 3.0.
    case $host_os in
      aix4 | aix4.[01] | aix4.[01].*)
      if { echo '#if __GNUC__ > 2 || (__GNUC__ == 2 && __GNUC_MINOR__ >= 97)'
	   echo ' yes '
	   echo '#endif'; } | ${CC} -E - | grep yes > /dev/null; then
	:
      else
	can_build_shared=no
      fi
      ;;
    esac
    # AIX (on Power*) has no versioning support, so currently we can not hardcode correct
    # soname into executable. Probably we can add versioning support to
    # collect2, so additional links can be useful in future.
    if test "$aix_use_runtimelinking" = yes; then
      # If using run time linking (on AIX 4.2 or later) use lib<name>.so
      # instead of lib<name>.a to let people know that these are not
      # typical AIX shared libraries.
      library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
    else
      # We preserve .a as extension for shared libraries through AIX4.2
      # and later when we are not doing run time linking.
      library_names_spec='${libname}${release}.a $libname.a'
      soname_spec='${libname}${release}${shared_ext}$major'
    fi
    shlibpath_var=LIBPATH
  fi
  ;;

amigaos*)
  library_names_spec='$libname.ixlibrary $libname.a'
  # Create ${libname}_ixlibrary.a entries in /sys/libs.
  finish_eval='for lib in `ls $libdir/*.ixlibrary 2>/dev/null`; do libname=`$echo "X$lib" | $Xsed -e '\''s%^.*/\([^/]*\)\.ixlibrary$%\1%'\''`; test $rm /sys/libs/${libname}_ixlibrary.a; $show "cd /sys/libs && $LN_S $lib ${libname}_ixlibrary.a"; cd /sys/libs && $LN_S $lib ${libname}_ixlibrary.a || exit 1; done'
  ;;

beos*)
  library_names_spec='${libname}${shared_ext}'
  dynamic_linker="$host_os ld.so"
  shlibpath_var=LIBRARY_PATH
  ;;

bsdi[45]*)
  version_type=linux
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  finish_cmds='PATH="\$PATH:/sbin" ldconfig $libdir'
  shlibpath_var=LD_LIBRARY_PATH
  sys_lib_search_path_spec="/shlib /usr/lib /usr/X11/lib /usr/contrib/lib /lib /usr/local/lib"
  sys_lib_dlsearch_path_spec="/shlib /usr/lib /usr/local/lib"
  # the default ld.so.conf also contains /usr/contrib/lib and
  # /usr/X11R6/lib (/usr/X11 is a link to /usr/X11R6), but let us allow
  # libtool to hard-code these into programs
  ;;

cygwin* | mingw* | pw32*)
  version_type=windows
  shrext_cmds=".dll"
  need_version=no
  need_lib_prefix=no

  case $GCC,$host_os in
  yes,cygwin* | yes,mingw* | yes,pw32*)
    library_names_spec='$libname.dll.a'
    # DLL is installed to $(libdir)/../bin by postinstall_cmds
    postinstall_cmds='base_file=`basename \${file}`~
      dlpath=`$SHELL 2>&1 -c '\''. $dir/'\''\${base_file}'\''i;echo \$dlname'\''`~
      dldir=$destdir/`dirname \$dlpath`~
      test -d \$dldir || mkdir -p \$dldir~
      $install_prog $dir/$dlname \$dldir/$dlname~
      chmod a+x \$dldir/$dlname'
    postuninstall_cmds='dldll=`$SHELL 2>&1 -c '\''. $file; echo \$dlname'\''`~
      dlpath=$dir/\$dldll~
       $rm \$dlpath'
    shlibpath_overrides_runpath=yes

    case $host_os in
    cygwin*)
      # Cygwin DLLs use 'cyg' prefix rather than 'lib'
      soname_spec='`echo ${libname} | sed -e 's/^lib/cyg/'``echo ${release} | $SED -e 's/[.]/-/g'`${versuffix}${shared_ext}'
      sys_lib_search_path_spec="/usr/lib /lib/w32api /lib /usr/local/lib"
      ;;
    mingw*)
      # MinGW DLLs use traditional 'lib' prefix
      soname_spec='${libname}`echo ${release} | $SED -e 's/[.]/-/g'`${versuffix}${shared_ext}'
      sys_lib_search_path_spec=`$CC -print-search-dirs | grep "^libraries:" | $SED -e "s/^libraries://" -e "s,=/,/,g"`
      if echo "$sys_lib_search_path_spec" | grep ';[c-zC-Z]:/' >/dev/null; then
        # It is most probably a Windows format PATH printed by
        # mingw gcc, but we are running on Cygwin. Gcc prints its search
        # path with ; separators, and with drive letters. We can handle the
        # drive letters (cygwin fileutils understands them), so leave them,
        # especially as we might pass files found there to a mingw objdump,
        # which wouldn't understand a cygwinified path. Ahh.
        sys_lib_search_path_spec=`echo "$sys_lib_search_path_spec" | $SED -e 's/;/ /g'`
      else
        sys_lib_search_path_spec=`echo "$sys_lib_search_path_spec" | $SED  -e "s/$PATH_SEPARATOR/ /g"`
      fi
      ;;
    pw32*)
      # pw32 DLLs use 'pw' prefix rather than 'lib'
      library_names_spec='`echo ${libname} | sed -e 's/^lib/pw/'``echo ${release} | $SED -e 's/[.]/-/g'`${versuffix}${shared_ext}'
      ;;
    esac
    ;;

  *)
    library_names_spec='${libname}`echo ${release} | $SED -e 's/[.]/-/g'`${versuffix}${shared_ext} $libname.lib'
    ;;
  esac
  dynamic_linker='Win32 ld.exe'
  # FIXME: first we should search . and the directory the executable is in
  shlibpath_var=PATH
  ;;

darwin* | rhapsody*)
  dynamic_linker="$host_os dyld"
  version_type=darwin
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${versuffix}$shared_ext ${libname}${release}${major}$shared_ext ${libname}$shared_ext'
  soname_spec='${libname}${release}${major}$shared_ext'
  shlibpath_overrides_runpath=yes
  shlibpath_var=DYLD_LIBRARY_PATH
  shrext_cmds='`test .$module = .yes && echo .so || echo .dylib`'

  sys_lib_search_path_spec="$sys_lib_search_path_spec /usr/local/lib"
  sys_lib_dlsearch_path_spec='/usr/local/lib /lib /usr/lib'
  ;;

dgux*)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname$shared_ext'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  ;;

freebsd1*)
  dynamic_linker=no
  ;;

freebsd* | dragonfly*)
  # DragonFly does not have aout.  When/if they implement a new
  # versioning mechanism, adjust this.
  if test -x /usr/bin/objformat; then
    objformat=`/usr/bin/objformat`
  else
    case $host_os in
    freebsd[123]*) objformat=aout ;;
    *) objformat=elf ;;
    esac
  fi
  version_type=freebsd-$objformat
  case $version_type in
    freebsd-elf*)
      library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext} $libname${shared_ext}'
      need_version=no
      need_lib_prefix=no
      ;;
    freebsd-*)
      library_names_spec='${libname}${release}${shared_ext}$versuffix $libname${shared_ext}$versuffix'
      need_version=yes
      ;;
  esac
  shlibpath_var=LD_LIBRARY_PATH
  case $host_os in
  freebsd2*)
    shlibpath_overrides_runpath=yes
    ;;
  freebsd3.[01]* | freebsdelf3.[01]*)
    shlibpath_overrides_runpath=yes
    hardcode_into_libs=yes
    ;;
  freebsd3.[2-9]* | freebsdelf3.[2-9]* | \
  freebsd4.[0-5] | freebsdelf4.[0-5] | freebsd4.1.1 | freebsdelf4.1.1)
    shlibpath_overrides_runpath=no
    hardcode_into_libs=yes
    ;;
  *) # from 4.6 on, and DragonFly
    shlibpath_overrides_runpath=yes
    hardcode_into_libs=yes
    ;;
  esac
  ;;

gnu*)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}${major} ${libname}${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  hardcode_into_libs=yes
  ;;

hpux9* | hpux10* | hpux11*)
  # Give a soname corresponding to the major version so that dld.sl refuses to
  # link against other versions.
  version_type=sunos
  need_lib_prefix=no
  need_version=no
  case $host_cpu in
  ia64*)
    shrext_cmds='.so'
    hardcode_into_libs=yes
    dynamic_linker="$host_os dld.so"
    shlibpath_var=LD_LIBRARY_PATH
    shlibpath_overrides_runpath=yes # Unless +noenvvar is specified.
    library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
    soname_spec='${libname}${release}${shared_ext}$major'
    if test "X$HPUX_IA64_MODE" = X32; then
      sys_lib_search_path_spec="/usr/lib/hpux32 /usr/local/lib/hpux32 /usr/local/lib"
    else
      sys_lib_search_path_spec="/usr/lib/hpux64 /usr/local/lib/hpux64"
    fi
    sys_lib_dlsearch_path_spec=$sys_lib_search_path_spec
    ;;
   hppa*64*)
     shrext_cmds='.sl'
     hardcode_into_libs=yes
     dynamic_linker="$host_os dld.sl"
     shlibpath_var=LD_LIBRARY_PATH # How should we handle SHLIB_PATH
     shlibpath_overrides_runpath=yes # Unless +noenvvar is specified.
     library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
     soname_spec='${libname}${release}${shared_ext}$major'
     sys_lib_search_path_spec="/usr/lib/pa20_64 /usr/ccs/lib/pa20_64"
     sys_lib_dlsearch_path_spec=$sys_lib_search_path_spec
     ;;
   *)
    shrext_cmds='.sl'
    dynamic_linker="$host_os dld.sl"
    shlibpath_var=SHLIB_PATH
    shlibpath_overrides_runpath=no # +s is required to enable SHLIB_PATH
    library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
    soname_spec='${libname}${release}${shared_ext}$major'
    ;;
  esac
  # HP-UX runs *really* slowly unless shared libraries are mode 555.
  postinstall_cmds='chmod 555 $lib'
  ;;

interix[3-9]*)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major ${libname}${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  dynamic_linker='Interix 3.x ld.so.1 (PE, like ELF)'
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=no
  hardcode_into_libs=yes
  ;;

irix5* | irix6* | nonstopux*)
  case $host_os in
    nonstopux*) version_type=nonstopux ;;
    *)
	if test "$lt_cv_prog_gnu_ld" = yes; then
		version_type=linux
	else
		version_type=irix
	fi ;;
  esac
  need_lib_prefix=no
  need_version=no
  soname_spec='${libname}${release}${shared_ext}$major'
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major ${libname}${release}${shared_ext} $libname${shared_ext}'
  case $host_os in
  irix5* | nonstopux*)
    libsuff= shlibsuff=
    ;;
  *)
    case $LD in # libtool.m4 will add one of these switches to LD
    *-32|*"-32 "|*-melf32bsmip|*"-melf32bsmip ")
      libsuff= shlibsuff= libmagic=32-bit;;
    *-n32|*"-n32 "|*-melf32bmipn32|*"-melf32bmipn32 ")
      libsuff=32 shlibsuff=N32 libmagic=N32;;
    *-64|*"-64 "|*-melf64bmip|*"-melf64bmip ")
      libsuff=64 shlibsuff=64 libmagic=64-bit;;
    *) libsuff= shlibsuff= libmagic=never-match;;
    esac
    ;;
  esac
  shlibpath_var=LD_LIBRARY${shlibsuff}_PATH
  shlibpath_overrides_runpath=no
  sys_lib_search_path_spec="/usr/lib${libsuff} /lib${libsuff} /usr/local/lib${libsuff}"
  sys_lib_dlsearch_path_spec="/usr/lib${libsuff} /lib${libsuff}"
  hardcode_into_libs=yes
  ;;

# No shared lib support for Linux oldld, aout, or coff.
linux*oldld* | linux*aout* | linux*coff*)
  dynamic_linker=no
  ;;

# This must be Linux ELF.
linux* | k*bsd*-gnu)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  finish_cmds='PATH="\$PATH:/sbin" ldconfig -n $libdir'
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=no
  # This implies no fast_install, which is unacceptable.
  # Some rework will be needed to allow for fast_install
  # before this can be enabled.
  hardcode_into_libs=yes

  # Append ld.so.conf contents to the search path
  if test -f /etc/ld.so.conf; then
    lt_ld_extra=`awk '/^include / { system(sprintf("cd /etc; cat %s 2>/dev/null", \$2)); skip = 1; } { if (!skip) print \$0; skip = 0; }' < /etc/ld.so.conf | $SED -e 's/#.*//;/^[ 	]*hwcap[ 	]/d;s/[:,	]/ /g;s/=[^=]*$//;s/=[^= ]* / /g;/^$/d' | tr '\n' ' '`
    sys_lib_dlsearch_path_spec="/lib /usr/lib $lt_ld_extra"
  fi

  # We used to test for /lib/ld.so.1 and disable shared libraries on
  # powerpc, because MkLinux only supported shared libraries with the
  # GNU dynamic linker.  Since this was broken with cross compilers,
  # most powerpc-linux boxes support dynamic linking these days and
  # people can always --disable-shared, the test was removed, and we
  # assume the GNU/Linux dynamic linker is in use.
  dynamic_linker='GNU/Linux ld.so'
  ;;

netbsd*)
  version_type=sunos
  need_lib_prefix=no
  need_version=no
  if echo __ELF__ | $CC -E - | grep __ELF__ >/dev/null; then
    library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${shared_ext}$versuffix'
    finish_cmds='PATH="\$PATH:/sbin" ldconfig -m $libdir'
    dynamic_linker='NetBSD (a.out) ld.so'
  else
    library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major ${libname}${shared_ext}'
    soname_spec='${libname}${release}${shared_ext}$major'
    dynamic_linker='NetBSD ld.elf_so'
  fi
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=yes
  hardcode_into_libs=yes
  ;;

newsos6)
  version_type=linux
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=yes
  ;;

nto-qnx*)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=yes
  ;;

openbsd*)
  version_type=sunos
  sys_lib_dlsearch_path_spec="/usr/lib"
  need_lib_prefix=no
  # Some older versions of OpenBSD (3.3 at least) *do* need versioned libs.
  case $host_os in
    openbsd3.3 | openbsd3.3.*) need_version=yes ;;
    *)                         need_version=no  ;;
  esac
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${shared_ext}$versuffix'
  finish_cmds='PATH="\$PATH:/sbin" ldconfig -m $libdir'
  shlibpath_var=LD_LIBRARY_PATH
  if test -z "`echo __ELF__ | $CC -E - | grep __ELF__`" || test "$host_os-$host_cpu" = "openbsd2.8-powerpc"; then
    case $host_os in
      openbsd2.[89] | openbsd2.[89].*)
	shlibpath_overrides_runpath=no
	;;
      *)
	shlibpath_overrides_runpath=yes
	;;
      esac
  else
    shlibpath_overrides_runpath=yes
  fi
  ;;

os2*)
  libname_spec='$name'
  shrext_cmds=".dll"
  need_lib_prefix=no
  library_names_spec='$libname${shared_ext} $libname.a'
  dynamic_linker='OS/2 ld.exe'
  shlibpath_var=LIBPATH
  ;;

osf3* | osf4* | osf5*)
  version_type=osf
  need_lib_prefix=no
  need_version=no
  soname_spec='${libname}${release}${shared_ext}$major'
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  shlibpath_var=LD_LIBRARY_PATH
  sys_lib_search_path_spec="/usr/shlib /usr/ccs/lib /usr/lib/cmplrs/cc /usr/lib /usr/local/lib /var/shlib"
  sys_lib_dlsearch_path_spec="$sys_lib_search_path_spec"
  ;;

rdos*)
  dynamic_linker=no
  ;;

solaris*)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=yes
  hardcode_into_libs=yes
  # ldd complains unless libraries are executable
  postinstall_cmds='chmod +x $lib'
  ;;

sunos4*)
  version_type=sunos
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${shared_ext}$versuffix'
  finish_cmds='PATH="\$PATH:/usr/etc" ldconfig $libdir'
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=yes
  if test "$with_gnu_ld" = yes; then
    need_lib_prefix=no
  fi
  need_version=yes
  ;;

sysv4 | sysv4.3*)
  version_type=linux
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  case $host_vendor in
    sni)
      shlibpath_overrides_runpath=no
      need_lib_prefix=no
      export_dynamic_flag_spec='${wl}-Blargedynsym'
      runpath_var=LD_RUN_PATH
      ;;
    siemens)
      need_lib_prefix=no
      ;;
    motorola)
      need_lib_prefix=no
      need_version=no
      shlibpath_overrides_runpath=no
      sys_lib_search_path_spec='/lib /usr/lib /usr/ccs/lib'
      ;;
  esac
  ;;

sysv4*MP*)
  if test -d /usr/nec ;then
    version_type=linux
    library_names_spec='$libname${shared_ext}.$versuffix $libname${shared_ext}.$major $libname${shared_ext}'
    soname_spec='$libname${shared_ext}.$major'
    shlibpath_var=LD_LIBRARY_PATH
  fi
  ;;

sysv5* | sco3.2v5* | sco5v6* | unixware* | OpenUNIX* | sysv4*uw2*)
  version_type=freebsd-elf
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext} $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  hardcode_into_libs=yes
  if test "$with_gnu_ld" = yes; then
    sys_lib_search_path_spec='/usr/local/lib /usr/gnu/lib /usr/ccs/lib /usr/lib /lib'
    shlibpath_overrides_runpath=no
  else
    sys_lib_search_path_spec='/usr/ccs/lib /usr/lib'
    shlibpath_overrides_runpath=yes
    case $host_os in
      sco3.2v5*)
        sys_lib_search_path_spec="$sys_lib_search_path_spec /lib"
	;;
    esac
  fi
  sys_lib_dlsearch_path_spec='/usr/lib'
  ;;

uts4*)
  version_type=linux
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  ;;

*)
  dynamic_linker=no
  ;;
esac
{ echo "$as_me:$LINENO: result: $dynamic_linker" >&5
echo "${ECHO_T}$dynamic_linker" >&6; }
test "$dynamic_linker" = no && can_build_shared=no

variables_saved_for_relink="PATH $shlibpath_var $runpath_var"
if test "$GCC" = yes; then
  variables_saved_for_relink="$variables_saved_for_relink GCC_EXEC_PREFIX COMPILER_PATH LIBRARY_PATH"
fi

{ echo "$as_me:$LINENO: checking how to hardcode library paths into programs" >&5
echo $ECHO_N "checking how to hardcode library paths into programs... $ECHO_C" >&6; }
hardcode_action=
if test -n "$hardcode_libdir_flag_spec" || \
   test -n "$runpath_var" || \
   test "X$hardcode_automatic" = "Xyes" ; then

  # We can hardcode non-existant directories.
  if test "$hardcode_direct" != no &&
     # If the only mechanism to avoid hardcoding is shlibpath_var, we
     # have to relink, otherwise we might link with an installed library
     # when we should be linking with a yet-to-be-installed one
     ## test "$_LT_AC_TAGVAR(hardcode_shlibpath_var, )" != no &&
     test "$hardcode_minus_L" != no; then
    # Linking always hardcodes the temporary library directory.
    hardcode_action=relink
  else
    # We can link without hardcoding, and we can hardcode nonexisting dirs.
    hardcode_action=immediate
  fi
else
  # We cannot hardcode anything, or else we can only hardcode existing
  # directories.
  hardcode_action=unsupported
fi
{ echo "$as_me:$LINENO: result: $hardcode_action" >&5
echo "${ECHO_T}$hardcode_action" >&6; }

if test "$hardcode_action" = relink; then
  # Fast installation is not supported
  enable_fast_install=no
elif test "$shlibpath_overrides_runpath" = yes ||
     test "$enable_shared" = no; then
  # Fast installation is not necessary
  enable_fast_install=needless
fi

striplib=
old_striplib=
{ echo "$as_me:$LINENO: checking whether stripping libraries is possible" >&5
echo $ECHO_N "checking whether stripping libraries is possible... $ECHO_C" >&6; }
if test -n "$STRIP" && $STRIP -V 2>&1 | grep "GNU strip" >/dev/null; then
  test -z "$old_striplib" && old_striplib="$STRIP --strip-debug"
  test -z "$striplib" && striplib="$STRIP --strip-unneeded"
  { echo "$as_me:$LINENO: result: yes" >&5
echo "${ECHO_T}yes" >&6; }
else
# FIXME - insert some real tests, host_os isn't really good enough
  case $host_os in
   darwin*)
       if test -n "$STRIP" ; then
         striplib="$STRIP -x"
         old_striplib="$STRIP -S"
         { echo "$as_me:$LINENO: result: yes" >&5
echo "${ECHO_T}yes" >&6; }
       else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi
       ;;
   *)
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
    ;;
  esac
fi

if test "x$enable_dlopen" != xyes; then
  enable_dlopen=unknown
  enable_dlopen_self=unknown
  enable_dlopen_self_static=unknown
else
  lt_cv_dlopen=no
  lt_cv_dlopen_libs=

  case $host_os in
  beos*)
    lt_cv_dlopen="load_add_on"
    lt_cv_dlopen_libs=
    lt_cv_dlopen_self=yes
    ;;

  mingw* | pw32*)
    lt_cv_dlopen="LoadLibrary"
    lt_cv_dlopen_libs=
   ;;

  cygwin*)
    lt_cv_dlopen="dlopen"
    lt_cv_dlopen_libs=
   ;;

  darwin*)
  # if libdl is installed we need to link against it
    { echo "$as_me:$LINENO: checking for dlopen in -ldl" >&5
echo $ECHO_N "checking for dlopen in -ldl... $ECHO_C" >&6; }
if test "${ac_cv_lib_dl_dlopen+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  ac_check_lib_save_LIBS=$LIBS
LIBS="-ldl  $LIBS"
cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

/* Override any GCC internal prototype to avoid an error.
   Use char because int might match the return type of a GCC
   builtin and then its argument prototype would still apply.  */
#ifdef __cplusplus
extern "C"
#endif
char dlopen ();
int
main ()
{
return dlopen ();
  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_c_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest$ac_exeext &&
       $as_test_x conftest$ac_exeext; then
  ac_cv_lib_dl_dlopen=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_cv_lib_dl_dlopen=no
fi

rm -f core conftest.err conftest.$ac_objext conftest_ipa8_conftest.oo \
      conftest$ac_exeext conftest.$ac_ext
LIBS=$ac_check_lib_save_LIBS
fi
{ echo "$as_me:$LINENO: result: $ac_cv_lib_dl_dlopen" >&5
echo "${ECHO_T}$ac_cv_lib_dl_dlopen" >&6; }
if test $ac_cv_lib_dl_dlopen = yes; then
  lt_cv_dlopen="dlopen" lt_cv_dlopen_libs="-ldl"
else

    lt_cv_dlopen="dyld"
    lt_cv_dlopen_libs=
    lt_cv_dlopen_self=yes

fi

   ;;

  *)
    { echo "$as_me:$LINENO: checking for shl_load" >&5
echo $ECHO_N "checking for shl_load... $ECHO_C" >&6; }
if test "${ac_cv_func_shl_load+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
/* Define shl_load to an innocuous variant, in case <limits.h> declares shl_load.
   For example, HP-UX 11i <limits.h> declares gettimeofday.  */
#define shl_load innocuous_shl_load

/* System header to define __stub macros and hopefully few prototypes,
    which can conflict with char shl_load (); below.
    Prefer <limits.h> to <assert.h> if __STDC__ is defined, since
    <limits.h> exists even on freestanding compilers.  */

#ifdef __STDC__
# include <limits.h>
#else
# include <assert.h>
#endif

#undef shl_load

/* Override any GCC internal prototype to avoid an error.
   Use char because int might match the return type of a GCC
   builtin and then its argument prototype would still apply.  */
#ifdef __cplusplus
extern "C"
#endif
char shl_load ();
/* The GNU C library defines this for functions which it implements
    to always fail with ENOSYS.  Some functions are actually named
    something starting with __ and the normal name is an alias.  */
#if defined __stub_shl_load || defined __stub___shl_load
choke me
#endif

int
main ()
{
return shl_load ();
  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_c_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest$ac_exeext &&
       $as_test_x conftest$ac_exeext; then
  ac_cv_func_shl_load=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_cv_func_shl_load=no
fi

rm -f core conftest.err conftest.$ac_objext conftest_ipa8_conftest.oo \
      conftest$ac_exeext conftest.$ac_ext
fi
{ echo "$as_me:$LINENO: result: $ac_cv_func_shl_load" >&5
echo "${ECHO_T}$ac_cv_func_shl_load" >&6; }
if test $ac_cv_func_shl_load = yes; then
  lt_cv_dlopen="shl_load"
else
  { echo "$as_me:$LINENO: checking for shl_load in -ldld" >&5
echo $ECHO_N "checking for shl_load in -ldld... $ECHO_C" >&6; }
if test "${ac_cv_lib_dld_shl_load+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  ac_check_lib_save_LIBS=$LIBS
LIBS="-ldld  $LIBS"
cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

/* Override any GCC internal prototype to avoid an error.
   Use char because int might match the return type of a GCC
   builtin and then its argument prototype would still apply.  */
#ifdef __cplusplus
extern "C"
#endif
char shl_load ();
int
main ()
{
return shl_load ();
  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_c_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest$ac_exeext &&
       $as_test_x conftest$ac_exeext; then
  ac_cv_lib_dld_shl_load=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_cv_lib_dld_shl_load=no
fi

rm -f core conftest.err conftest.$ac_objext conftest_ipa8_conftest.oo \
      conftest$ac_exeext conftest.$ac_ext
LIBS=$ac_check_lib_save_LIBS
fi
{ echo "$as_me:$LINENO: result: $ac_cv_lib_dld_shl_load" >&5
echo "${ECHO_T}$ac_cv_lib_dld_shl_load" >&6; }
if test $ac_cv_lib_dld_shl_load = yes; then
  lt_cv_dlopen="shl_load" lt_cv_dlopen_libs="-ldld"
else
  { echo "$as_me:$LINENO: checking for dlopen" >&5
echo $ECHO_N "checking for dlopen... $ECHO_C" >&6; }
if test "${ac_cv_func_dlopen+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
/* Define dlopen to an innocuous variant, in case <limits.h> declares dlopen.
   For example, HP-UX 11i <limits.h> declares gettimeofday.  */
#define dlopen innocuous_dlopen

/* System header to define __stub macros and hopefully few prototypes,
    which can conflict with char dlopen (); below.
    Prefer <limits.h> to <assert.h> if __STDC__ is defined, since
    <limits.h> exists even on freestanding compilers.  */

#ifdef __STDC__
# include <limits.h>
#else
# include <assert.h>
#endif

#undef dlopen

/* Override any GCC internal prototype to avoid an error.
   Use char because int might match the return type of a GCC
   builtin and then its argument prototype would still apply.  */
#ifdef __cplusplus
extern "C"
#endif
char dlopen ();
/* The GNU C library defines this for functions which it implements
    to always fail with ENOSYS.  Some functions are actually named
    something starting with __ and the normal name is an alias.  */
#if defined __stub_dlopen || defined __stub___dlopen
choke me
#endif

int
main ()
{
return dlopen ();
  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_c_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest$ac_exeext &&
       $as_test_x conftest$ac_exeext; then
  ac_cv_func_dlopen=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_cv_func_dlopen=no
fi

rm -f core conftest.err conftest.$ac_objext conftest_ipa8_conftest.oo \
      conftest$ac_exeext conftest.$ac_ext
fi
{ echo "$as_me:$LINENO: result: $ac_cv_func_dlopen" >&5
echo "${ECHO_T}$ac_cv_func_dlopen" >&6; }
if test $ac_cv_func_dlopen = yes; then
  lt_cv_dlopen="dlopen"
else
  { echo "$as_me:$LINENO: checking for dlopen in -ldl" >&5
echo $ECHO_N "checking for dlopen in -ldl... $ECHO_C" >&6; }
if test "${ac_cv_lib_dl_dlopen+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  ac_check_lib_save_LIBS=$LIBS
LIBS="-ldl  $LIBS"
cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

/* Override any GCC internal prototype to avoid an error.
   Use char because int might match the return type of a GCC
   builtin and then its argument prototype would still apply.  */
#ifdef __cplusplus
extern "C"
#endif
char dlopen ();
int
main ()
{
return dlopen ();
  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_c_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest$ac_exeext &&
       $as_test_x conftest$ac_exeext; then
  ac_cv_lib_dl_dlopen=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_cv_lib_dl_dlopen=no
fi

rm -f core conftest.err conftest.$ac_objext conftest_ipa8_conftest.oo \
      conftest$ac_exeext conftest.$ac_ext
LIBS=$ac_check_lib_save_LIBS
fi
{ echo "$as_me:$LINENO: result: $ac_cv_lib_dl_dlopen" >&5
echo "${ECHO_T}$ac_cv_lib_dl_dlopen" >&6; }
if test $ac_cv_lib_dl_dlopen = yes; then
  lt_cv_dlopen="dlopen" lt_cv_dlopen_libs="-ldl"
else
  { echo "$as_me:$LINENO: checking for dlopen in -lsvld" >&5
echo $ECHO_N "checking for dlopen in -lsvld... $ECHO_C" >&6; }
if test "${ac_cv_lib_svld_dlopen+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  ac_check_lib_save_LIBS=$LIBS
LIBS="-lsvld  $LIBS"
cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

/* Override any GCC internal prototype to avoid an error.
   Use char because int might match the return type of a GCC
   builtin and then its argument prototype would still apply.  */
#ifdef __cplusplus
extern "C"
#endif
char dlopen ();
int
main ()
{
return dlopen ();
  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_c_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest$ac_exeext &&
       $as_test_x conftest$ac_exeext; then
  ac_cv_lib_svld_dlopen=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_cv_lib_svld_dlopen=no
fi

rm -f core conftest.err conftest.$ac_objext conftest_ipa8_conftest.oo \
      conftest$ac_exeext conftest.$ac_ext
LIBS=$ac_check_lib_save_LIBS
fi
{ echo "$as_me:$LINENO: result: $ac_cv_lib_svld_dlopen" >&5
echo "${ECHO_T}$ac_cv_lib_svld_dlopen" >&6; }
if test $ac_cv_lib_svld_dlopen = yes; then
  lt_cv_dlopen="dlopen" lt_cv_dlopen_libs="-lsvld"
else
  { echo "$as_me:$LINENO: checking for dld_link in -ldld" >&5
echo $ECHO_N "checking for dld_link in -ldld... $ECHO_C" >&6; }
if test "${ac_cv_lib_dld_dld_link+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  ac_check_lib_save_LIBS=$LIBS
LIBS="-ldld  $LIBS"
cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

/* Override any GCC internal prototype to avoid an error.
   Use char because int might match the return type of a GCC
   builtin and then its argument prototype would still apply.  */
#ifdef __cplusplus
extern "C"
#endif
char dld_link ();
int
main ()
{
return dld_link ();
  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_c_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest$ac_exeext &&
       $as_test_x conftest$ac_exeext; then
  ac_cv_lib_dld_dld_link=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_cv_lib_dld_dld_link=no
fi

rm -f core conftest.err conftest.$ac_objext conftest_ipa8_conftest.oo \
      conftest$ac_exeext conftest.$ac_ext
LIBS=$ac_check_lib_save_LIBS
fi
{ echo "$as_me:$LINENO: result: $ac_cv_lib_dld_dld_link" >&5
echo "${ECHO_T}$ac_cv_lib_dld_dld_link" >&6; }
if test $ac_cv_lib_dld_dld_link = yes; then
  lt_cv_dlopen="dld_link" lt_cv_dlopen_libs="-ldld"
fi


fi


fi


fi


fi


fi

    ;;
  esac

  if test "x$lt_cv_dlopen" != xno; then
    enable_dlopen=yes
  else
    enable_dlopen=no
  fi

  case $lt_cv_dlopen in
  dlopen)
    save_CPPFLAGS="$CPPFLAGS"
    test "x$ac_cv_header_dlfcn_h" = xyes && CPPFLAGS="$CPPFLAGS -DHAVE_DLFCN_H"

    save_LDFLAGS="$LDFLAGS"
    wl=$lt_prog_compiler_wl eval LDFLAGS=\"\$LDFLAGS $export_dynamic_flag_spec\"

    save_LIBS="$LIBS"
    LIBS="$lt_cv_dlopen_libs $LIBS"

    { echo "$as_me:$LINENO: checking whether a program can dlopen itself" >&5
echo $ECHO_N "checking whether a program can dlopen itself... $ECHO_C" >&6; }
if test "${lt_cv_dlopen_self+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  	  if test "$cross_compiling" = yes; then :
  lt_cv_dlopen_self=cross
else
  lt_dlunknown=0; lt_dlno_uscore=1; lt_dlneed_uscore=2
  lt_status=$lt_dlunknown
  cat > conftest.$ac_ext <<EOF
#line 9806 "configure"
#include "confdefs.h"

#if HAVE_DLFCN_H
#include <dlfcn.h>
#endif

#include <stdio.h>

#ifdef RTLD_GLOBAL
#  define LT_DLGLOBAL		RTLD_GLOBAL
#else
#  ifdef DL_GLOBAL
#    define LT_DLGLOBAL		DL_GLOBAL
#  else
#    define LT_DLGLOBAL		0
#  endif
#endif

/* We may have to define LT_DLLAZY_OR_NOW in the command line if we
   find out it does not work in some platform. */
#ifndef LT_DLLAZY_OR_NOW
#  ifdef RTLD_LAZY
#    define LT_DLLAZY_OR_NOW		RTLD_LAZY
#  else
#    ifdef DL_LAZY
#      define LT_DLLAZY_OR_NOW		DL_LAZY
#    else
#      ifdef RTLD_NOW
#        define LT_DLLAZY_OR_NOW	RTLD_NOW
#      else
#        ifdef DL_NOW
#          define LT_DLLAZY_OR_NOW	DL_NOW
#        else
#          define LT_DLLAZY_OR_NOW	0
#        endif
#      endif
#    endif
#  endif
#endif

#ifdef __cplusplus
extern "C" void exit (int);
#endif

void fnord() { int i=42;}
int main ()
{
  void *self = dlopen (0, LT_DLGLOBAL|LT_DLLAZY_OR_NOW);
  int status = $lt_dlunknown;

  if (self)
    {
      if (dlsym (self,"fnord"))       status = $lt_dlno_uscore;
      else if (dlsym( self,"_fnord")) status = $lt_dlneed_uscore;
      /* dlclose (self); */
    }
  else
    puts (dlerror ());

    exit (status);
}
EOF
  if { (eval echo "$as_me:$LINENO: \"$ac_link\"") >&5
  (eval $ac_link) 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && test -s conftest${ac_exeext} 2>/dev/null; then
    (./conftest; exit; ) >&5 2>/dev/null
    lt_status=$?
    case x$lt_status in
      x$lt_dlno_uscore) lt_cv_dlopen_self=yes ;;
      x$lt_dlneed_uscore) lt_cv_dlopen_self=yes ;;
      x$lt_dlunknown|x*) lt_cv_dlopen_self=no ;;
    esac
  else :
    # compilation failed
    lt_cv_dlopen_self=no
  fi
fi
rm -fr conftest*


fi
{ echo "$as_me:$LINENO: result: $lt_cv_dlopen_self" >&5
echo "${ECHO_T}$lt_cv_dlopen_self" >&6; }

    if test "x$lt_cv_dlopen_self" = xyes; then
      wl=$lt_prog_compiler_wl eval LDFLAGS=\"\$LDFLAGS $lt_prog_compiler_static\"
      { echo "$as_me:$LINENO: checking whether a statically linked program can dlopen itself" >&5
echo $ECHO_N "checking whether a statically linked program can dlopen itself... $ECHO_C" >&6; }
if test "${lt_cv_dlopen_self_static+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  	  if test "$cross_compiling" = yes; then :
  lt_cv_dlopen_self_static=cross
else
  lt_dlunknown=0; lt_dlno_uscore=1; lt_dlneed_uscore=2
  lt_status=$lt_dlunknown
  cat > conftest.$ac_ext <<EOF
#line 9906 "configure"
#include "confdefs.h"

#if HAVE_DLFCN_H
#include <dlfcn.h>
#endif

#include <stdio.h>

#ifdef RTLD_GLOBAL
#  define LT_DLGLOBAL		RTLD_GLOBAL
#else
#  ifdef DL_GLOBAL
#    define LT_DLGLOBAL		DL_GLOBAL
#  else
#    define LT_DLGLOBAL		0
#  endif
#endif

/* We may have to define LT_DLLAZY_OR_NOW in the command line if we
   find out it does not work in some platform. */
#ifndef LT_DLLAZY_OR_NOW
#  ifdef RTLD_LAZY
#    define LT_DLLAZY_OR_NOW		RTLD_LAZY
#  else
#    ifdef DL_LAZY
#      define LT_DLLAZY_OR_NOW		DL_LAZY
#    else
#      ifdef RTLD_NOW
#        define LT_DLLAZY_OR_NOW	RTLD_NOW
#      else
#        ifdef DL_NOW
#          define LT_DLLAZY_OR_NOW	DL_NOW
#        else
#          define LT_DLLAZY_OR_NOW	0
#        endif
#      endif
#    endif
#  endif
#endif

#ifdef __cplusplus
extern "C" void exit (int);
#endif

void fnord() { int i=42;}
int main ()
{
  void *self = dlopen (0, LT_DLGLOBAL|LT_DLLAZY_OR_NOW);
  int status = $lt_dlunknown;

  if (self)
    {
      if (dlsym (self,"fnord"))       status = $lt_dlno_uscore;
      else if (dlsym( self,"_fnord")) status = $lt_dlneed_uscore;
      /* dlclose (self); */
    }
  else
    puts (dlerror ());

    exit (status);
}
EOF
  if { (eval echo "$as_me:$LINENO: \"$ac_link\"") >&5
  (eval $ac_link) 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && test -s conftest${ac_exeext} 2>/dev/null; then
    (./conftest; exit; ) >&5 2>/dev/null
    lt_status=$?
    case x$lt_status in
      x$lt_dlno_uscore) lt_cv_dlopen_self_static=yes ;;
      x$lt_dlneed_uscore) lt_cv_dlopen_self_static=yes ;;
      x$lt_dlunknown|x*) lt_cv_dlopen_self_static=no ;;
    esac
  else :
    # compilation failed
    lt_cv_dlopen_self_static=no
  fi
fi
rm -fr conftest*


fi
{ echo "$as_me:$LINENO: result: $lt_cv_dlopen_self_static" >&5
echo "${ECHO_T}$lt_cv_dlopen_self_static" >&6; }
    fi

    CPPFLAGS="$save_CPPFLAGS"
    LDFLAGS="$save_LDFLAGS"
    LIBS="$save_LIBS"
    ;;
  esac

  case $lt_cv_dlopen_self in
  yes|no) enable_dlopen_self=$lt_cv_dlopen_self ;;
  *) enable_dlopen_self=unknown ;;
  esac

  case $lt_cv_dlopen_self_static in
  yes|no) enable_dlopen_self_static=$lt_cv_dlopen_self_static ;;
  *) enable_dlopen_self_static=unknown ;;
  esac
fi


# Report which library types will actually be built
{ echo "$as_me:$LINENO: checking if libtool supports shared libraries" >&5
echo $ECHO_N "checking if libtool supports shared libraries... $ECHO_C" >&6; }
{ echo "$as_me:$LINENO: result: $can_build_shared" >&5
echo "${ECHO_T}$can_build_shared" >&6; }

{ echo "$as_me:$LINENO: checking whether to build shared libraries" >&5
echo $ECHO_N "checking whether to build shared libraries... $ECHO_C" >&6; }
test "$can_build_shared" = "no" && enable_shared=no

# On AIX, shared libraries and static libraries use the same namespace, and
# are all built from PIC.
case $host_os in
aix3*)
  test "$enable_shared" = yes && enable_static=no
  if test -n "$RANLIB"; then
    archive_cmds="$archive_cmds~\$RANLIB \$lib"
    postinstall_cmds='$RANLIB $lib'
  fi
  ;;

aix4* | aix5*)
  if test "$host_cpu" != ia64 && test "$aix_use_runtimelinking" = no ; then
    test "$enable_shared" = yes && enable_static=no
  fi
    ;;
esac
{ echo "$as_me:$LINENO: result: $enable_shared" >&5
echo "${ECHO_T}$enable_shared" >&6; }

{ echo "$as_me:$LINENO: checking whether to build static libraries" >&5
echo $ECHO_N "checking whether to build static libraries... $ECHO_C" >&6; }
# Make sure either enable_shared or enable_static is yes.
test "$enable_shared" = yes || enable_static=yes
{ echo "$as_me:$LINENO: result: $enable_static" >&5
echo "${ECHO_T}$enable_static" >&6; }

# The else clause should only fire when bootstrapping the
# libtool distribution, otherwise you forgot to ship ltmain.sh
# with your package, and you will get complaints that there are
# no rules to generate ltmain.sh.
if test -f "$ltmain"; then
  # See if we are running on zsh, and set the options which allow our commands through
  # without removal of \ escapes.
  if test -n "${ZSH_VERSION+set}" ; then
    setopt NO_GLOB_SUBST
  fi
  # Now quote all the things that may contain metacharacters while being
  # careful not to overquote the AC_SUBSTed values.  We take copies of the
  # variables and quote the copies for generation of the libtool script.
  for var in echo old_CC old_CFLAGS AR AR_FLAGS EGREP RANLIB LN_S LTCC LTCFLAGS NM \
    SED SHELL STRIP \
    libname_spec library_names_spec soname_spec extract_expsyms_cmds \
    old_striplib striplib file_magic_cmd finish_cmds finish_eval \
    deplibs_check_method reload_flag reload_cmds need_locks \
    lt_cv_sys_global_symbol_pipe lt_cv_sys_global_symbol_to_cdecl \
    lt_cv_sys_global_symbol_to_c_name_address \
    sys_lib_search_path_spec sys_lib_dlsearch_path_spec \
    old_postinstall_cmds old_postuninstall_cmds \
    compiler \
    CC \
    LD \
    lt_prog_compiler_wl \
    lt_prog_compiler_pic \
    lt_prog_compiler_static \
    lt_prog_compiler_no_builtin_flag \
    export_dynamic_flag_spec \
    thread_safe_flag_spec \
    whole_archive_flag_spec \
    enable_shared_with_static_runtimes \
    old_archive_cmds \
    old_archive_from_new_cmds \
    predep_objects \
    postdep_objects \
    predeps \
    postdeps \
    compiler_lib_search_path \
    archive_cmds \
    archive_expsym_cmds \
    postinstall_cmds \
    postuninstall_cmds \
    old_archive_from_expsyms_cmds \
    allow_undefined_flag \
    no_undefined_flag \
    export_symbols_cmds \
    hardcode_libdir_flag_spec \
    hardcode_libdir_flag_spec_ld \
    hardcode_libdir_separator \
    hardcode_automatic \
    module_cmds \
    module_expsym_cmds \
    lt_cv_prog_compiler_c_o \
    fix_srcfile_path \
    exclude_expsyms \
    include_expsyms; do

    case $var in
    old_archive_cmds | \
    old_archive_from_new_cmds | \
    archive_cmds | \
    archive_expsym_cmds | \
    module_cmds | \
    module_expsym_cmds | \
    old_archive_from_expsyms_cmds | \
    export_symbols_cmds | \
    extract_expsyms_cmds | reload_cmds | finish_cmds | \
    postinstall_cmds | postuninstall_cmds | \
    old_postinstall_cmds | old_postuninstall_cmds | \
    sys_lib_search_path_spec | sys_lib_dlsearch_path_spec)
      # Double-quote double-evaled strings.
      eval "lt_$var=\\\"\`\$echo \"X\$$var\" | \$Xsed -e \"\$double_quote_subst\" -e \"\$sed_quote_subst\" -e \"\$delay_variable_subst\"\`\\\""
      ;;
    *)
      eval "lt_$var=\\\"\`\$echo \"X\$$var\" | \$Xsed -e \"\$sed_quote_subst\"\`\\\""
      ;;
    esac
  done

  case $lt_echo in
  *'\$0 --fallback-echo"')
    lt_echo=`$echo "X$lt_echo" | $Xsed -e 's/\\\\\\\$0 --fallback-echo"$/$0 --fallback-echo"/'`
    ;;
  esac

cfgfile="${ofile}T"
  trap "$rm \"$cfgfile\"; exit 1" 1 2 15
  $rm -f "$cfgfile"
  { echo "$as_me:$LINENO: creating $ofile" >&5
echo "$as_me: creating $ofile" >&6;}

  cat <<__EOF__ >> "$cfgfile"
#! $SHELL

# `$echo "$cfgfile" | sed 's%^.*/%%'` - Provide generalized library-building support services.
# Generated automatically by $PROGRAM (GNU $PACKAGE $VERSION$TIMESTAMP)
# NOTE: Changes made to this file will be lost: look at ltmain.sh.
#
# Copyright (C) 1996, 1997, 1998, 1999, 2000, 2001, 2002, 2003, 2004, 2005, 2006, 2007
# Free Software Foundation, Inc.
#
# This file is part of GNU Libtool:
# Originally by Gordon Matzigkeit <gord@gnu.ai.mit.edu>, 1996
#
# This program is free software; you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation; either version 2 of the License, or
# (at your option) any later version.
#
# This program is distributed in the hope that it will be useful, but
# WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the GNU
# General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program; if not, write to the Free Software
# Foundation, Inc., 51 Franklin Street, Fifth Floor, Boston, MA 02110-1301, USA.
#
# As a special exception to the GNU General Public License, if you
# distribute this file as part of a program that contains a
# configuration script generated by Autoconf, you may include it under
# the same distribution terms that you use for the rest of that program.

# A sed program that does not truncate output.
SED=$lt_SED

# Sed that helps us avoid accidentally triggering echo(1) options like -n.
Xsed="$SED -e 1s/^X//"

# The HP-UX ksh and POSIX shell print the target directory to stdout
# if CDPATH is set.
(unset CDPATH) >/dev/null 2>&1 && unset CDPATH

# The names of the tagged configurations supported by this script.
available_tags=

# ### BEGIN LIBTOOL CONFIG

# Libtool was configured on host `(hostname || uname -n) 2>/dev/null | sed 1q`:

# Shell to use when invoking shell scripts.
SHELL=$lt_SHELL

# Whether or not to build shared libraries.
build_libtool_libs=$enable_shared

# Whether or not to build static libraries.
build_old_libs=$enable_static

# Whether or not to add -lc for building shared libraries.
build_libtool_need_lc=$archive_cmds_need_lc

# Whether or not to disallow shared libs when runtime libs are static
allow_libtool_libs_with_static_runtimes=$enable_shared_with_static_runtimes

# Whether or not to optimize for fast installation.
fast_install=$enable_fast_install

# The host system.
host_alias=$host_alias
host=$host
host_os=$host_os

# The build system.
build_alias=$build_alias
build=$build
build_os=$build_os

# An echo program that does not interpret backslashes.
echo=$lt_echo

# The archiver.
AR=$lt_AR
AR_FLAGS=$lt_AR_FLAGS

# A C compiler.
LTCC=$lt_LTCC

# LTCC compiler flags.
LTCFLAGS=$lt_LTCFLAGS

# A language-specific compiler.
CC=$lt_compiler

# Is the compiler the GNU C compiler?
with_gcc=$GCC

# An ERE matcher.
EGREP=$lt_EGREP

# The linker used to build libraries.
LD=$lt_LD

# Whether we need hard or soft links.
LN_S=$lt_LN_S

# A BSD-compatible nm program.
NM=$lt_NM

# A symbol stripping program
STRIP=$lt_STRIP

# Used to examine libraries when file_magic_cmd begins "file"
MAGIC_CMD=$MAGIC_CMD

# Used on cygwin: DLL creation program.
DLLTOOL="$DLLTOOL"

# Used on cygwin: object dumper.
OBJDUMP="$OBJDUMP"

# Used on cygwin: assembler.
AS="$AS"

# The name of the directory that contains temporary libtool files.
objdir=$objdir

# How to create reloadable object files.
reload_flag=$lt_reload_flag
reload_cmds=$lt_reload_cmds

# How to pass a linker flag through the compiler.
wl=$lt_lt_prog_compiler_wl

# Object file suffix (normally "o").
objext="$ac_objext"

# Old archive suffix (normally "a").
libext="$libext"

# Shared library suffix (normally ".so").
shrext_cmds='$shrext_cmds'

# Executable file suffix (normally "").
exeext="$exeext"

# Additional compiler flags for building library objects.
pic_flag=$lt_lt_prog_compiler_pic
pic_mode=$pic_mode

# What is the maximum length of a command?
max_cmd_len=$lt_cv_sys_max_cmd_len

# Does compiler simultaneously support -c and -o options?
compiler_c_o=$lt_lt_cv_prog_compiler_c_o

# Must we lock files when doing compilation?
need_locks=$lt_need_locks

# Do we need the lib prefix for modules?
need_lib_prefix=$need_lib_prefix

# Do we need a version for libraries?
need_version=$need_version

# Whether dlopen is supported.
dlopen_support=$enable_dlopen

# Whether dlopen of programs is supported.
dlopen_self=$enable_dlopen_self

# Whether dlopen of statically linked programs is supported.
dlopen_self_static=$enable_dlopen_self_static

# Compiler flag to prevent dynamic linking.
link_static_flag=$lt_lt_prog_compiler_static

# Compiler flag to turn off builtin functions.
no_builtin_flag=$lt_lt_prog_compiler_no_builtin_flag

# Compiler flag to allow reflexive dlopens.
export_dynamic_flag_spec=$lt_export_dynamic_flag_spec

# Compiler flag to generate shared objects directly from archives.
whole_archive_flag_spec=$lt_whole_archive_flag_spec

# Compiler flag to generate thread-safe objects.
thread_safe_flag_spec=$lt_thread_safe_flag_spec

# Library versioning type.
version_type=$version_type

# Format of library name prefix.
libname_spec=$lt_libname_spec

# List of archive names.  First name is the real one, the rest are links.
# The last name is the one that the linker finds with -lNAME.
library_names_spec=$lt_library_names_spec

# The coded name of the library, if different from the real name.
soname_spec=$lt_soname_spec

# Commands used to build and install an old-style archive.
RANLIB=$lt_RANLIB
old_archive_cmds=$lt_old_archive_cmds
old_postinstall_cmds=$lt_old_postinstall_cmds
old_postuninstall_cmds=$lt_old_postuninstall_cmds

# Create an old-style archive from a shared archive.
old_archive_from_new_cmds=$lt_old_archive_from_new_cmds

# Create a temporary old-style archive to link instead of a shared archive.
old_archive_from_expsyms_cmds=$lt_old_archive_from_expsyms_cmds

# Commands used to build and install a shared archive.
archive_cmds=$lt_archive_cmds
archive_expsym_cmds=$lt_archive_expsym_cmds
postinstall_cmds=$lt_postinstall_cmds
postuninstall_cmds=$lt_postuninstall_cmds

# Commands used to build a loadable module (assumed same as above if empty)
module_cmds=$lt_module_cmds
module_expsym_cmds=$lt_module_expsym_cmds

# Commands to strip libraries.
old_striplib=$lt_old_striplib
striplib=$lt_striplib

# Dependencies to place before the objects being linked to create a
# shared library.
predep_objects=$lt_predep_objects

# Dependencies to place after the objects being linked to create a
# shared library.
postdep_objects=$lt_postdep_objects

# Dependencies to place before the objects being linked to create a
# shared library.
predeps=$lt_predeps

# Dependencies to place after the objects being linked to create a
# shared library.
postdeps=$lt_postdeps

# The library search path used internally by the compiler when linking
# a shared library.
compiler_lib_search_path=$lt_compiler_lib_search_path

# Method to check whether dependent libraries are shared objects.
deplibs_check_method=$lt_deplibs_check_method

# Command to use when deplibs_check_method == file_magic.
file_magic_cmd=$lt_file_magic_cmd

# Flag that allows shared libraries with undefined symbols to be built.
allow_undefined_flag=$lt_allow_undefined_flag

# Flag that forces no undefined symbols.
no_undefined_flag=$lt_no_undefined_flag

# Commands used to finish a libtool library installation in a directory.
finish_cmds=$lt_finish_cmds

# Same as above, but a single script fragment to be evaled but not shown.
finish_eval=$lt_finish_eval

# Take the output of nm and produce a listing of raw symbols and C names.
global_symbol_pipe=$lt_lt_cv_sys_global_symbol_pipe

# Transform the output of nm in a proper C declaration
global_symbol_to_cdecl=$lt_lt_cv_sys_global_symbol_to_cdecl

# Transform the output of nm in a C name address pair
global_symbol_to_c_name_address=$lt_lt_cv_sys_global_symbol_to_c_name_address

# This is the shared library runtime path variable.
runpath_var=$runpath_var

# This is the shared library path variable.
shlibpath_var=$shlibpath_var

# Is shlibpath searched before the hard-coded library search path?
shlibpath_overrides_runpath=$shlibpath_overrides_runpath

# How to hardcode a shared library path into an executable.
hardcode_action=$hardcode_action

# Whether we should hardcode library paths into libraries.
hardcode_into_libs=$hardcode_into_libs

# Flag to hardcode \$libdir into a binary during linking.
# This must work even if \$libdir does not exist.
hardcode_libdir_flag_spec=$lt_hardcode_libdir_flag_spec

# If ld is used when linking, flag to hardcode \$libdir into
# a binary during linking. This must work even if \$libdir does
# not exist.
hardcode_libdir_flag_spec_ld=$lt_hardcode_libdir_flag_spec_ld

# Whether we need a single -rpath flag with a separated argument.
hardcode_libdir_separator=$lt_hardcode_libdir_separator

# Set to yes if using DIR/libNAME${shared_ext} during linking hardcodes DIR into the
# resulting binary.
hardcode_direct=$hardcode_direct

# Set to yes if using the -LDIR flag during linking hardcodes DIR into the
# resulting binary.
hardcode_minus_L=$hardcode_minus_L

# Set to yes if using SHLIBPATH_VAR=DIR during linking hardcodes DIR into
# the resulting binary.
hardcode_shlibpath_var=$hardcode_shlibpath_var

# Set to yes if building a shared library automatically hardcodes DIR into the library
# and all subsequent libraries and executables linked against it.
hardcode_automatic=$hardcode_automatic

# Variables whose values should be saved in libtool wrapper scripts and
# restored at relink time.
variables_saved_for_relink="$variables_saved_for_relink"

# Whether libtool must link a program against all its dependency libraries.
link_all_deplibs=$link_all_deplibs

# Compile-time system search path for libraries
sys_lib_search_path_spec=$lt_sys_lib_search_path_spec

# Run-time system search path for libraries
sys_lib_dlsearch_path_spec=$lt_sys_lib_dlsearch_path_spec

# Fix the shell variable \$srcfile for the compiler.
fix_srcfile_path=$lt_fix_srcfile_path

# Set to yes if exported symbols are required.
always_export_symbols=$always_export_symbols

# The commands to list exported symbols.
export_symbols_cmds=$lt_export_symbols_cmds

# The commands to extract the exported symbol list from a shared archive.
extract_expsyms_cmds=$lt_extract_expsyms_cmds

# Symbols that should not be listed in the preloaded symbols.
exclude_expsyms=$lt_exclude_expsyms

# Symbols that must always be exported.
include_expsyms=$lt_include_expsyms

# ### END LIBTOOL CONFIG

__EOF__


  case $host_os in
  aix3*)
    cat <<\EOF >> "$cfgfile"

# AIX sometimes has problems with the GCC collect2 program.  For some
# reason, if we set the COLLECT_NAMES environment variable, the problems
# vanish in a puff of smoke.
if test "X${COLLECT_NAMES+set}" != Xset; then
  COLLECT_NAMES=
  export COLLECT_NAMES
fi
EOF
    ;;
  esac

  # We use sed instead of cat because bash on DJGPP gets confused if
  # if finds mixed CR/LF and LF-only lines.  Since sed operates in
  # text mode, it properly converts lines to CR/LF.  This bash problem
  # is reportedly fixed, but why not run on old versions too?
  sed '$q' "$ltmain" >> "$cfgfile" || (rm -f "$cfgfile"; exit 1)

  mv -f "$cfgfile" "$ofile" || \
    (rm -f "$ofile" && cp "$cfgfile" "$ofile" && rm -f "$cfgfile")
  chmod +x "$ofile"

else
  # If there is no Makefile yet, we rely on a make rule to execute
  # `config.status --recheck' to rerun these tests and create the
  # libtool script then.
  ltmain_in=`echo $ltmain | sed -e 's/\.sh$/.in/'`
  if test -f "$ltmain_in"; then
    test -f Makefile && make "$ltmain"
  fi
fi


ac_ext=c
ac_cpp='$CPP $CPPFLAGS'
ac_compile='$CC -c $CFLAGS $CPPFLAGS conftest.$ac_ext >&5'
ac_link='$CC -o conftest$ac_exeext $CFLAGS $CPPFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_c_compiler_gnu

CC="$lt_save_CC"


# Check whether --with-tags was given.
if test "${with_tags+set}" = set; then
  withval=$with_tags; tagnames="$withval"
fi


if test -f "$ltmain" && test -n "$tagnames"; then
  if test ! -f "${ofile}"; then
    { echo "$as_me:$LINENO: WARNING: output file \`$ofile' does not exist" >&5
echo "$as_me: WARNING: output file \`$ofile' does not exist" >&2;}
  fi

  if test -z "$LTCC"; then
    eval "`$SHELL ${ofile} --config | grep '^LTCC='`"
    if test -z "$LTCC"; then
      { echo "$as_me:$LINENO: WARNING: output file \`$ofile' does not look like a libtool script" >&5
echo "$as_me: WARNING: output file \`$ofile' does not look like a libtool script" >&2;}
    else
      { echo "$as_me:$LINENO: WARNING: using \`LTCC=$LTCC', extracted from \`$ofile'" >&5
echo "$as_me: WARNING: using \`LTCC=$LTCC', extracted from \`$ofile'" >&2;}
    fi
  fi
  if test -z "$LTCFLAGS"; then
    eval "`$SHELL ${ofile} --config | grep '^LTCFLAGS='`"
  fi

  # Extract list of available tagged configurations in $ofile.
  # Note that this assumes the entire list is on one line.
  available_tags=`grep "^available_tags=" "${ofile}" | $SED -e 's/available_tags=\(.*$\)/\1/' -e 's/\"//g'`

  lt_save_ifs="$IFS"; IFS="${IFS}$PATH_SEPARATOR,"
  for tagname in $tagnames; do
    IFS="$lt_save_ifs"
    # Check whether tagname contains only valid characters
    case `$echo "X$tagname" | $Xsed -e 's:[-_ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrstuvwxyz1234567890,/]::g'` in
    "") ;;
    *)  { { echo "$as_me:$LINENO: error: invalid tag name: $tagname" >&5
echo "$as_me: error: invalid tag name: $tagname" >&2;}
   { (exit 1); exit 1; }; }
	;;
    esac

    if grep "^# ### BEGIN LIBTOOL TAG CONFIG: $tagname$" < "${ofile}" > /dev/null
    then
      { { echo "$as_me:$LINENO: error: tag name \"$tagname\" already exists" >&5
echo "$as_me: error: tag name \"$tagname\" already exists" >&2;}
   { (exit 1); exit 1; }; }
    fi

    # Update the list of available tags.
    if test -n "$tagname"; then
      echo appending configuration tag \"$tagname\" to $ofile

      case $tagname in
      CXX)
	if test -n "$CXX" && ( test "X$CXX" != "Xno" &&
	    ( (test "X$CXX" = "Xg++" && `g++ -v >/dev/null 2>&1` ) ||
	    (test "X$CXX" != "Xg++"))) ; then
	  ac_ext=cpp
ac_cpp='$CXXCPP $CPPFLAGS'
ac_compile='$CXX -c $CXXFLAGS $CPPFLAGS conftest.$ac_ext >&5'
ac_link='$CXX -o conftest$ac_exeext $CXXFLAGS $CPPFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_cxx_compiler_gnu




archive_cmds_need_lc_CXX=no
allow_undefined_flag_CXX=
always_export_symbols_CXX=no
archive_expsym_cmds_CXX=
export_dynamic_flag_spec_CXX=
hardcode_direct_CXX=no
hardcode_libdir_flag_spec_CXX=
hardcode_libdir_flag_spec_ld_CXX=
hardcode_libdir_separator_CXX=
hardcode_minus_L_CXX=no
hardcode_shlibpath_var_CXX=unsupported
hardcode_automatic_CXX=no
module_cmds_CXX=
module_expsym_cmds_CXX=
link_all_deplibs_CXX=unknown
old_archive_cmds_CXX=$old_archive_cmds
no_undefined_flag_CXX=
whole_archive_flag_spec_CXX=
enable_shared_with_static_runtimes_CXX=no

# Dependencies to place before and after the object being linked:
predep_objects_CXX=
postdep_objects_CXX=
predeps_CXX=
postdeps_CXX=
compiler_lib_search_path_CXX=

# Source file extension for C++ test sources.
ac_ext=cpp

# Object file extension for compiled C++ test sources.
objext=o
objext_CXX=$objext

# Code to be used in simple compile tests
lt_simple_compile_test_code="int some_variable = 0;"

# Code to be used in simple link tests
lt_simple_link_test_code='int main(int, char *[]) { return(0); }'

# ltmain only uses $CC for tagged configurations so make sure $CC is set.

# If no C compiler was specified, use CC.
LTCC=${LTCC-"$CC"}

# If no C compiler flags were specified, use CFLAGS.
LTCFLAGS=${LTCFLAGS-"$CFLAGS"}

# Allow CC to be a program name with arguments.
compiler=$CC


# save warnings/boilerplate of simple test code
ac_outfile=conftest.$ac_objext
echo "$lt_simple_compile_test_code" >conftest.$ac_ext
eval "$ac_compile" 2>&1 >/dev/null | $SED '/^$/d; /^ *+/d' >conftest.err
_lt_compiler_boilerplate=`cat conftest.err`
$rm conftest*

ac_outfile=conftest.$ac_objext
echo "$lt_simple_link_test_code" >conftest.$ac_ext
eval "$ac_link" 2>&1 >/dev/null | $SED '/^$/d; /^ *+/d' >conftest.err
_lt_linker_boilerplate=`cat conftest.err`
$rm conftest*


# Allow CC to be a program name with arguments.
lt_save_CC=$CC
lt_save_LD=$LD
lt_save_GCC=$GCC
GCC=$GXX
lt_save_with_gnu_ld=$with_gnu_ld
lt_save_path_LD=$lt_cv_path_LD
if test -n "${lt_cv_prog_gnu_ldcxx+set}"; then
  lt_cv_prog_gnu_ld=$lt_cv_prog_gnu_ldcxx
else
  $as_unset lt_cv_prog_gnu_ld
fi
if test -n "${lt_cv_path_LDCXX+set}"; then
  lt_cv_path_LD=$lt_cv_path_LDCXX
else
  $as_unset lt_cv_path_LD
fi
test -z "${LDCXX+set}" || LD=$LDCXX
CC=${CXX-"c++"}
compiler=$CC
compiler_CXX=$CC
for cc_temp in $compiler""; do
  case $cc_temp in
    compile | *[\\/]compile | ccache | *[\\/]ccache ) ;;
    distcc | *[\\/]distcc | purify | *[\\/]purify ) ;;
    \-*) ;;
    *) break;;
  esac
done
cc_basename=`$echo "X$cc_temp" | $Xsed -e 's%.*/%%' -e "s%^$host_alias-%%"`


# We don't want -fno-exception wen compiling C++ code, so set the
# no_builtin_flag separately
if test "$GXX" = yes; then
  lt_prog_compiler_no_builtin_flag_CXX=' -fno-builtin'
else
  lt_prog_compiler_no_builtin_flag_CXX=
fi

if test "$GXX" = yes; then
  # Set up default GNU C++ configuration


# Check whether --with-gnu-ld was given.
if test "${with_gnu_ld+set}" = set; then
  withval=$with_gnu_ld; test "$withval" = no || with_gnu_ld=yes
else
  with_gnu_ld=no
fi

ac_prog=ld
if test "$GCC" = yes; then
  # Check if gcc -print-prog-name=ld gives a path.
  { echo "$as_me:$LINENO: checking for ld used by $CC" >&5
echo $ECHO_N "checking for ld used by $CC... $ECHO_C" >&6; }
  case $host in
  *-*-mingw*)
    # gcc leaves a trailing carriage return which upsets mingw
    ac_prog=`($CC -print-prog-name=ld) 2>&5 | tr -d '\015'` ;;
  *)
    ac_prog=`($CC -print-prog-name=ld) 2>&5` ;;
  esac
  case $ac_prog in
    # Accept absolute paths.
    [\\/]* | ?:[\\/]*)
      re_direlt='/[^/][^/]*/\.\./'
      # Canonicalize the pathname of ld
      ac_prog=`echo $ac_prog| $SED 's%\\\\%/%g'`
      while echo $ac_prog | grep "$re_direlt" > /dev/null 2>&1; do
	ac_prog=`echo $ac_prog| $SED "s%$re_direlt%/%"`
      done
      test -z "$LD" && LD="$ac_prog"
      ;;
  "")
    # If it fails, then pretend we aren't using GCC.
    ac_prog=ld
    ;;
  *)
    # If it is relative, then search for the first ld in PATH.
    with_gnu_ld=unknown
    ;;
  esac
elif test "$with_gnu_ld" = yes; then
  { echo "$as_me:$LINENO: checking for GNU ld" >&5
echo $ECHO_N "checking for GNU ld... $ECHO_C" >&6; }
else
  { echo "$as_me:$LINENO: checking for non-GNU ld" >&5
echo $ECHO_N "checking for non-GNU ld... $ECHO_C" >&6; }
fi
if test "${lt_cv_path_LD+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -z "$LD"; then
  lt_save_ifs="$IFS"; IFS=$PATH_SEPARATOR
  for ac_dir in $PATH; do
    IFS="$lt_save_ifs"
    test -z "$ac_dir" && ac_dir=.
    if test -f "$ac_dir/$ac_prog" || test -f "$ac_dir/$ac_prog$ac_exeext"; then
      lt_cv_path_LD="$ac_dir/$ac_prog"
      # Check to see if the program is GNU ld.  I'd rather use --version,
      # but apparently some variants of GNU ld only accept -v.
      # Break only if it was the GNU/non-GNU ld that we prefer.
      case `"$lt_cv_path_LD" -v 2>&1 </dev/null` in
      *GNU* | *'with BFD'*)
	test "$with_gnu_ld" != no && break
	;;
      *)
	test "$with_gnu_ld" != yes && break
	;;
      esac
    fi
  done
  IFS="$lt_save_ifs"
else
  lt_cv_path_LD="$LD" # Let the user override the test with a path.
fi
fi

LD="$lt_cv_path_LD"
if test -n "$LD"; then
  { echo "$as_me:$LINENO: result: $LD" >&5
echo "${ECHO_T}$LD" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi
test -z "$LD" && { { echo "$as_me:$LINENO: error: no acceptable ld found in \$PATH" >&5
echo "$as_me: error: no acceptable ld found in \$PATH" >&2;}
   { (exit 1); exit 1; }; }
{ echo "$as_me:$LINENO: checking if the linker ($LD) is GNU ld" >&5
echo $ECHO_N "checking if the linker ($LD) is GNU ld... $ECHO_C" >&6; }
if test "${lt_cv_prog_gnu_ld+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  # I'd rather use --version here, but apparently some GNU lds only accept -v.
case `$LD -v 2>&1 </dev/null` in
*GNU* | *'with BFD'*)
  lt_cv_prog_gnu_ld=yes
  ;;
*)
  lt_cv_prog_gnu_ld=no
  ;;
esac
fi
{ echo "$as_me:$LINENO: result: $lt_cv_prog_gnu_ld" >&5
echo "${ECHO_T}$lt_cv_prog_gnu_ld" >&6; }
with_gnu_ld=$lt_cv_prog_gnu_ld



  # Check if GNU C++ uses GNU ld as the underlying linker, since the
  # archiving commands below assume that GNU ld is being used.
  if test "$with_gnu_ld" = yes; then
    archive_cmds_CXX='$CC -shared -nostdlib $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags ${wl}-soname $wl$soname -o $lib'
    archive_expsym_cmds_CXX='$CC -shared -nostdlib $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags ${wl}-soname $wl$soname ${wl}-retain-symbols-file $wl$export_symbols -o $lib'

    hardcode_libdir_flag_spec_CXX='${wl}--rpath ${wl}$libdir'
    export_dynamic_flag_spec_CXX='${wl}--export-dynamic'

    # If archive_cmds runs LD, not CC, wlarc should be empty
    # XXX I think wlarc can be eliminated in ltcf-cxx, but I need to
    #     investigate it a little bit more. (MM)
    wlarc='${wl}'

    # ancient GNU ld didn't support --whole-archive et. al.
    if eval "`$CC -print-prog-name=ld` --help 2>&1" | \
	grep 'no-whole-archive' > /dev/null; then
      whole_archive_flag_spec_CXX="$wlarc"'--whole-archive$convenience '"$wlarc"'--no-whole-archive'
    else
      whole_archive_flag_spec_CXX=
    fi
  else
    with_gnu_ld=no
    wlarc=

    # A generic and very simple default shared library creation
    # command for GNU C++ for the case where it uses the native
    # linker, instead of GNU ld.  If possible, this setting should
    # overridden to take advantage of the native linker features on
    # the platform it is being used on.
    archive_cmds_CXX='$CC -shared -nostdlib $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags -o $lib'
  fi

  # Commands to make compiler produce verbose output that lists
  # what "hidden" libraries, object files and flags are used when
  # linking a shared library.
  output_verbose_link_cmd='$CC -shared $CFLAGS -v conftest.$objext 2>&1 | grep "\-L"'

else
  GXX=no
  with_gnu_ld=no
  wlarc=
fi

# PORTME: fill in a description of your system's C++ link characteristics
{ echo "$as_me:$LINENO: checking whether the $compiler linker ($LD) supports shared libraries" >&5
echo $ECHO_N "checking whether the $compiler linker ($LD) supports shared libraries... $ECHO_C" >&6; }
ld_shlibs_CXX=yes
case $host_os in
  aix3*)
    # FIXME: insert proper C++ library support
    ld_shlibs_CXX=no
    ;;
  aix4* | aix5*)
    if test "$host_cpu" = ia64; then
      # On IA64, the linker does run time linking by default, so we don't
      # have to do anything special.
      aix_use_runtimelinking=no
      exp_sym_flag='-Bexport'
      no_entry_flag=""
    else
      aix_use_runtimelinking=no

      # Test if we are trying to use run time linking or normal
      # AIX style linking. If -brtl is somewhere in LDFLAGS, we
      # need to do runtime linking.
      case $host_os in aix4.[23]|aix4.[23].*|aix5*)
	for ld_flag in $LDFLAGS; do
	  case $ld_flag in
	  *-brtl*)
	    aix_use_runtimelinking=yes
	    break
	    ;;
	  esac
	done
	;;
      esac

      exp_sym_flag='-bexport'
      no_entry_flag='-bnoentry'
    fi

    # When large executables or shared objects are built, AIX ld can
    # have problems creating the table of contents.  If linking a library
    # or program results in "error TOC overflow" add -mminimal-toc to
    # CXXFLAGS/CFLAGS for g++/gcc.  In the cases where that is not
    # enough to fix the problem, add -Wl,-bbigtoc to LDFLAGS.

    archive_cmds_CXX=''
    hardcode_direct_CXX=yes
    hardcode_libdir_separator_CXX=':'
    link_all_deplibs_CXX=yes

    if test "$GXX" = yes; then
      case $host_os in aix4.[012]|aix4.[012].*)
      # We only want to do this on AIX 4.2 and lower, the check
      # below for broken collect2 doesn't work under 4.3+
	collect2name=`${CC} -print-prog-name=collect2`
	if test -f "$collect2name" && \
	   strings "$collect2name" | grep resolve_lib_name >/dev/null
	then
	  # We have reworked collect2
	  :
	else
	  # We have old collect2
	  hardcode_direct_CXX=unsupported
	  # It fails to find uninstalled libraries when the uninstalled
	  # path is not listed in the libpath.  Setting hardcode_minus_L
	  # to unsupported forces relinking
	  hardcode_minus_L_CXX=yes
	  hardcode_libdir_flag_spec_CXX='-L$libdir'
	  hardcode_libdir_separator_CXX=
	fi
	;;
      esac
      shared_flag='-shared'
      if test "$aix_use_runtimelinking" = yes; then
	shared_flag="$shared_flag "'${wl}-G'
      fi
    else
      # not using gcc
      if test "$host_cpu" = ia64; then
	# VisualAge C++, Version 5.5 for AIX 5L for IA-64, Beta 3 Release
	# chokes on -Wl,-G. The following line is correct:
	shared_flag='-G'
      else
	if test "$aix_use_runtimelinking" = yes; then
	  shared_flag='${wl}-G'
	else
	  shared_flag='${wl}-bM:SRE'
	fi
      fi
    fi

    # It seems that -bexpall does not export symbols beginning with
    # underscore (_), so it is better to generate a list of symbols to export.
    always_export_symbols_CXX=yes
    if test "$aix_use_runtimelinking" = yes; then
      # Warning - without using the other runtime loading flags (-brtl),
      # -berok will link without error, but may produce a broken library.
      allow_undefined_flag_CXX='-berok'
      # Determine the default libpath from the value encoded in an empty executable.
      cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

int
main ()
{

  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_cxx_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest$ac_exeext &&
       $as_test_x conftest$ac_exeext; then

lt_aix_libpath_sed='
    /Import File Strings/,/^$/ {
	/^0/ {
	    s/^0  *\(.*\)$/\1/
	    p
	}
    }'
aix_libpath=`dump -H conftest$ac_exeext 2>/dev/null | $SED -n -e "$lt_aix_libpath_sed"`
# Check for a 64-bit object if we didn't find anything.
if test -z "$aix_libpath"; then
  aix_libpath=`dump -HX64 conftest$ac_exeext 2>/dev/null | $SED -n -e "$lt_aix_libpath_sed"`
fi
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5


fi

rm -f core conftest.err conftest.$ac_objext conftest_ipa8_conftest.oo \
      conftest$ac_exeext conftest.$ac_ext
if test -z "$aix_libpath"; then aix_libpath="/usr/lib:/lib"; fi

      hardcode_libdir_flag_spec_CXX='${wl}-blibpath:$libdir:'"$aix_libpath"

      archive_expsym_cmds_CXX="\$CC"' -o $output_objdir/$soname $libobjs $deplibs '"\${wl}$no_entry_flag"' $compiler_flags `if test "x${allow_undefined_flag}" != "x"; then echo "${wl}${allow_undefined_flag}"; else :; fi` '"\${wl}$exp_sym_flag:\$export_symbols $shared_flag"
     else
      if test "$host_cpu" = ia64; then
	hardcode_libdir_flag_spec_CXX='${wl}-R $libdir:/usr/lib:/lib'
	allow_undefined_flag_CXX="-z nodefs"
	archive_expsym_cmds_CXX="\$CC $shared_flag"' -o $output_objdir/$soname $libobjs $deplibs '"\${wl}$no_entry_flag"' $compiler_flags ${wl}${allow_undefined_flag} '"\${wl}$exp_sym_flag:\$export_symbols"
      else
	# Determine the default libpath from the value encoded in an empty executable.
	cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

int
main ()
{

  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_cxx_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest$ac_exeext &&
       $as_test_x conftest$ac_exeext; then

lt_aix_libpath_sed='
    /Import File Strings/,/^$/ {
	/^0/ {
	    s/^0  *\(.*\)$/\1/
	    p
	}
    }'
aix_libpath=`dump -H conftest$ac_exeext 2>/dev/null | $SED -n -e "$lt_aix_libpath_sed"`
# Check for a 64-bit object if we didn't find anything.
if test -z "$aix_libpath"; then
  aix_libpath=`dump -HX64 conftest$ac_exeext 2>/dev/null | $SED -n -e "$lt_aix_libpath_sed"`
fi
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5


fi

rm -f core conftest.err conftest.$ac_objext conftest_ipa8_conftest.oo \
      conftest$ac_exeext conftest.$ac_ext
if test -z "$aix_libpath"; then aix_libpath="/usr/lib:/lib"; fi

	hardcode_libdir_flag_spec_CXX='${wl}-blibpath:$libdir:'"$aix_libpath"
	# Warning - without using the other run time loading flags,
	# -berok will link without error, but may produce a broken library.
	no_undefined_flag_CXX=' ${wl}-bernotok'
	allow_undefined_flag_CXX=' ${wl}-berok'
	# Exported symbols can be pulled into shared objects from archives
	whole_archive_flag_spec_CXX='$convenience'
	archive_cmds_need_lc_CXX=yes
	# This is similar to how AIX traditionally builds its shared libraries.
	archive_expsym_cmds_CXX="\$CC $shared_flag"' -o $output_objdir/$soname $libobjs $deplibs ${wl}-bnoentry $compiler_flags ${wl}-bE:$export_symbols${allow_undefined_flag}~$AR $AR_FLAGS $output_objdir/$libname$release.a $output_objdir/$soname'
      fi
    fi
    ;;

  beos*)
    if $LD --help 2>&1 | grep ': supported targets:.* elf' > /dev/null; then
      allow_undefined_flag_CXX=unsupported
      # Joseph Beckenbach <jrb3@best.com> says some releases of gcc
      # support --undefined.  This deserves some investigation.  FIXME
      archive_cmds_CXX='$CC -nostart $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname -o $lib'
    else
      ld_shlibs_CXX=no
    fi
    ;;

  chorus*)
    case $cc_basename in
      *)
	# FIXME: insert proper C++ library support
	ld_shlibs_CXX=no
	;;
    esac
    ;;

  cygwin* | mingw* | pw32*)
    # _LT_AC_TAGVAR(hardcode_libdir_flag_spec, CXX) is actually meaningless,
    # as there is no search path for DLLs.
    hardcode_libdir_flag_spec_CXX='-L$libdir'
    allow_undefined_flag_CXX=unsupported
    always_export_symbols_CXX=no
    enable_shared_with_static_runtimes_CXX=yes

    if $LD --help 2>&1 | grep 'auto-import' > /dev/null; then
      archive_cmds_CXX='$CC -shared -nostdlib $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags -o $output_objdir/$soname ${wl}--enable-auto-image-base -Xlinker --out-implib -Xlinker $lib'
      # If the export-symbols file already is a .def file (1st line
      # is EXPORTS), use it as is; otherwise, prepend...
      archive_expsym_cmds_CXX='if test "x`$SED 1q $export_symbols`" = xEXPORTS; then
	cp $export_symbols $output_objdir/$soname.def;
      else
	echo EXPORTS > $output_objdir/$soname.def;
	cat $export_symbols >> $output_objdir/$soname.def;
      fi~
      $CC -shared -nostdlib $output_objdir/$soname.def $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags -o $output_objdir/$soname ${wl}--enable-auto-image-base -Xlinker --out-implib -Xlinker $lib'
    else
      ld_shlibs_CXX=no
    fi
  ;;
      darwin* | rhapsody*)
        case $host_os in
        rhapsody* | darwin1.[012])
         allow_undefined_flag_CXX='${wl}-undefined ${wl}suppress'
         ;;
       *) # Darwin 1.3 on
         if test -z ${MACOSX_DEPLOYMENT_TARGET} ; then
           allow_undefined_flag_CXX='${wl}-flat_namespace ${wl}-undefined ${wl}suppress'
         else
           case ${MACOSX_DEPLOYMENT_TARGET} in
             10.[012])
               allow_undefined_flag_CXX='${wl}-flat_namespace ${wl}-undefined ${wl}suppress'
               ;;
             10.*)
               allow_undefined_flag_CXX='${wl}-undefined ${wl}dynamic_lookup'
               ;;
           esac
         fi
         ;;
        esac
      archive_cmds_need_lc_CXX=no
      hardcode_direct_CXX=no
      hardcode_automatic_CXX=yes
      hardcode_shlibpath_var_CXX=unsupported
      whole_archive_flag_spec_CXX=''
      link_all_deplibs_CXX=yes

    if test "$GXX" = yes ; then
      lt_int_apple_cc_single_mod=no
      output_verbose_link_cmd='echo'
      if $CC -dumpspecs 2>&1 | $EGREP 'single_module' >/dev/null ; then
       lt_int_apple_cc_single_mod=yes
      fi
      if test "X$lt_int_apple_cc_single_mod" = Xyes ; then
       archive_cmds_CXX='$CC -dynamiclib -single_module $allow_undefined_flag -o $lib $libobjs $deplibs $compiler_flags -install_name $rpath/$soname $verstring'
      else
          archive_cmds_CXX='$CC -r -keep_private_externs -nostdlib -o ${lib}-master.o $libobjs~$CC -dynamiclib $allow_undefined_flag -o $lib ${lib}-master.o $deplibs $compiler_flags -install_name $rpath/$soname $verstring'
        fi
        module_cmds_CXX='$CC $allow_undefined_flag -o $lib -bundle $libobjs $deplibs$compiler_flags'
        # Don't fix this by using the ld -exported_symbols_list flag, it doesn't exist in older darwin lds
          if test "X$lt_int_apple_cc_single_mod" = Xyes ; then
            archive_expsym_cmds_CXX='sed -e "s,#.*,," -e "s,^[    ]*,," -e "s,^\(..*\),_&," < $export_symbols > $output_objdir/${libname}-symbols.expsym~$CC -dynamiclib -single_module $allow_undefined_flag -o $lib $libobjs $deplibs $compiler_flags -install_name $rpath/$soname $verstring~nmedit -s $output_objdir/${libname}-symbols.expsym ${lib}'
          else
            archive_expsym_cmds_CXX='sed -e "s,#.*,," -e "s,^[    ]*,," -e "s,^\(..*\),_&," < $export_symbols > $output_objdir/${libname}-symbols.expsym~$CC -r -keep_private_externs -nostdlib -o ${lib}-master.o $libobjs~$CC -dynamiclib $allow_undefined_flag -o $lib ${lib}-master.o $deplibs $compiler_flags -install_name $rpath/$soname $verstring~nmedit -s $output_objdir/${libname}-symbols.expsym ${lib}'
          fi
            module_expsym_cmds_CXX='sed -e "s,#.*,," -e "s,^[    ]*,," -e "s,^\(..*\),_&," < $export_symbols > $output_objdir/${libname}-symbols.expsym~$CC $allow_undefined_flag  -o $lib -bundle $libobjs $deplibs$compiler_flags~nmedit -s $output_objdir/${libname}-symbols.expsym ${lib}'
      else
      case $cc_basename in
        xlc*)
         output_verbose_link_cmd='echo'
          archive_cmds_CXX='$CC -qmkshrobj ${wl}-single_module $allow_undefined_flag -o $lib $libobjs $deplibs $compiler_flags ${wl}-install_name ${wl}`echo $rpath/$soname` $xlcverstring'
          module_cmds_CXX='$CC $allow_undefined_flag -o $lib -bundle $libobjs $deplibs$compiler_flags'
          # Don't fix this by using the ld -exported_symbols_list flag, it doesn't exist in older darwin lds
          archive_expsym_cmds_CXX='sed -e "s,#.*,," -e "s,^[    ]*,," -e "s,^\(..*\),_&," < $export_symbols > $output_objdir/${libname}-symbols.expsym~$CC -qmkshrobj ${wl}-single_module $allow_undefined_flag -o $lib $libobjs $deplibs $compiler_flags ${wl}-install_name ${wl}$rpath/$soname $xlcverstring~nmedit -s $output_objdir/${libname}-symbols.expsym ${lib}'
          module_expsym_cmds_CXX='sed -e "s,#.*,," -e "s,^[    ]*,," -e "s,^\(..*\),_&," < $export_symbols > $output_objdir/${libname}-symbols.expsym~$CC $allow_undefined_flag  -o $lib -bundle $libobjs $deplibs$compiler_flags~nmedit -s $output_objdir/${libname}-symbols.expsym ${lib}'
          ;;
       *)
         ld_shlibs_CXX=no
          ;;
      esac
      fi
        ;;

  dgux*)
    case $cc_basename in
      ec++*)
	# FIXME: insert proper C++ library support
	ld_shlibs_CXX=no
	;;
      ghcx*)
	# Green Hills C++ Compiler
	# FIXME: insert proper C++ library support
	ld_shlibs_CXX=no
	;;
      *)
	# FIXME: insert proper C++ library support
	ld_shlibs_CXX=no
	;;
    esac
    ;;
  freebsd[12]*)
    # C++ shared libraries reported to be fairly broken before switch to ELF
    ld_shlibs_CXX=no
    ;;
  freebsd-elf*)
    archive_cmds_need_lc_CXX=no
    ;;
  freebsd* | dragonfly*)
    # FreeBSD 3 and later use GNU C++ and GNU ld with standard ELF
    # conventions
    ld_shlibs_CXX=yes
    ;;
  gnu*)
    ;;
  hpux9*)
    hardcode_libdir_flag_spec_CXX='${wl}+b ${wl}$libdir'
    hardcode_libdir_separator_CXX=:
    export_dynamic_flag_spec_CXX='${wl}-E'
    hardcode_direct_CXX=yes
    hardcode_minus_L_CXX=yes # Not in the search PATH,
				# but as the default
				# location of the library.

    case $cc_basename in
    CC*)
      # FIXME: insert proper C++ library support
      ld_shlibs_CXX=no
      ;;
    aCC*)
      archive_cmds_CXX='$rm $output_objdir/$soname~$CC -b ${wl}+b ${wl}$install_libdir -o $output_objdir/$soname $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags~test $output_objdir/$soname = $lib || mv $output_objdir/$soname $lib'
      # Commands to make compiler produce verbose output that lists
      # what "hidden" libraries, object files and flags are used when
      # linking a shared library.
      #
      # There doesn't appear to be a way to prevent this compiler from
      # explicitly linking system object files so we need to strip them
      # from the output so that they don't get included in the library
      # dependencies.
      output_verbose_link_cmd='templist=`($CC -b $CFLAGS -v conftest.$objext 2>&1) | grep "[-]L"`; list=""; for z in $templist; do case $z in conftest.$objext) list="$list $z";; *.$objext);; *) list="$list $z";;esac; done; echo $list'
      ;;
    *)
      if test "$GXX" = yes; then
        archive_cmds_CXX='$rm $output_objdir/$soname~$CC -shared -nostdlib -fPIC ${wl}+b ${wl}$install_libdir -o $output_objdir/$soname $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags~test $output_objdir/$soname = $lib || mv $output_objdir/$soname $lib'
      else
        # FIXME: insert proper C++ library support
        ld_shlibs_CXX=no
      fi
      ;;
    esac
    ;;
  hpux10*|hpux11*)
    if test $with_gnu_ld = no; then
      hardcode_libdir_flag_spec_CXX='${wl}+b ${wl}$libdir'
      hardcode_libdir_separator_CXX=:

      case $host_cpu in
      hppa*64*|ia64*) ;;
      *)
	export_dynamic_flag_spec_CXX='${wl}-E'
        ;;
      esac
    fi
    case $host_cpu in
    hppa*64*|ia64*)
      hardcode_direct_CXX=no
      hardcode_shlibpath_var_CXX=no
      ;;
    *)
      hardcode_direct_CXX=yes
      hardcode_minus_L_CXX=yes # Not in the search PATH,
					      # but as the default
					      # location of the library.
      ;;
    esac

    case $cc_basename in
      CC*)
	# FIXME: insert proper C++ library support
	ld_shlibs_CXX=no
	;;
      aCC*)
	case $host_cpu in
	hppa*64*)
	  archive_cmds_CXX='$CC -b ${wl}+h ${wl}$soname -o $lib $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags'
	  ;;
	ia64*)
	  archive_cmds_CXX='$CC -b ${wl}+h ${wl}$soname ${wl}+nodefaultrpath -o $lib $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags'
	  ;;
	*)
	  archive_cmds_CXX='$CC -b ${wl}+h ${wl}$soname ${wl}+b ${wl}$install_libdir -o $lib $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags'
	  ;;
	esac
	# Commands to make compiler produce verbose output that lists
	# what "hidden" libraries, object files and flags are used when
	# linking a shared library.
	#
	# There doesn't appear to be a way to prevent this compiler from
	# explicitly linking system object files so we need to strip them
	# from the output so that they don't get included in the library
	# dependencies.
	output_verbose_link_cmd='templist=`($CC -b $CFLAGS -v conftest.$objext 2>&1) | grep "\-L"`; list=""; for z in $templist; do case $z in conftest.$objext) list="$list $z";; *.$objext);; *) list="$list $z";;esac; done; echo $list'
	;;
      *)
	if test "$GXX" = yes; then
	  if test $with_gnu_ld = no; then
	    case $host_cpu in
	    hppa*64*)
	      archive_cmds_CXX='$CC -shared -nostdlib -fPIC ${wl}+h ${wl}$soname -o $lib $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags'
	      ;;
	    ia64*)
	      archive_cmds_CXX='$CC -shared -nostdlib -fPIC ${wl}+h ${wl}$soname ${wl}+nodefaultrpath -o $lib $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags'
	      ;;
	    *)
	      archive_cmds_CXX='$CC -shared -nostdlib -fPIC ${wl}+h ${wl}$soname ${wl}+b ${wl}$install_libdir -o $lib $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags'
	      ;;
	    esac
	  fi
	else
	  # FIXME: insert proper C++ library support
	  ld_shlibs_CXX=no
	fi
	;;
    esac
    ;;
  interix[3-9]*)
    hardcode_direct_CXX=no
    hardcode_shlibpath_var_CXX=no
    hardcode_libdir_flag_spec_CXX='${wl}-rpath,$libdir'
    export_dynamic_flag_spec_CXX='${wl}-E'
    # Hack: On Interix 3.x, we cannot compile PIC because of a broken gcc.
    # Instead, shared libraries are loaded at an image base (0x10000000 by
    # default) and relocated if they conflict, which is a slow very memory
    # consuming and fragmenting process.  To avoid this, we pick a random,
    # 256 KiB-aligned image base between 0x50000000 and 0x6FFC0000 at link
    # time.  Moving up from 0x10000000 also allows more sbrk(2) space.
    archive_cmds_CXX='$CC -shared $pic_flag $libobjs $deplibs $compiler_flags ${wl}-h,$soname ${wl}--image-base,`expr ${RANDOM-$$} % 4096 / 2 \* 262144 + 1342177280` -o $lib'
    archive_expsym_cmds_CXX='sed "s,^,_," $export_symbols >$output_objdir/$soname.expsym~$CC -shared $pic_flag $libobjs $deplibs $compiler_flags ${wl}-h,$soname ${wl}--retain-symbols-file,$output_objdir/$soname.expsym ${wl}--image-base,`expr ${RANDOM-$$} % 4096 / 2 \* 262144 + 1342177280` -o $lib'
    ;;
  irix5* | irix6*)
    case $cc_basename in
      CC*)
	# SGI C++
	archive_cmds_CXX='$CC -shared -all -multigot $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags -soname $soname `test -n "$verstring" && echo -set_version $verstring` -update_registry ${output_objdir}/so_locations -o $lib'

	# Archives containing C++ object files must be created using
	# "CC -ar", where "CC" is the IRIX C++ compiler.  This is
	# necessary to make sure instantiated templates are included
	# in the archive.
	old_archive_cmds_CXX='$CC -ar -WR,-u -o $oldlib $oldobjs'
	;;
      *)
	if test "$GXX" = yes; then
	  if test "$with_gnu_ld" = no; then
	    archive_cmds_CXX='$CC -shared -nostdlib $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags ${wl}-soname ${wl}$soname `test -n "$verstring" && echo ${wl}-set_version ${wl}$verstring` ${wl}-update_registry ${wl}${output_objdir}/so_locations -o $lib'
	  else
	    archive_cmds_CXX='$CC -shared -nostdlib $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags ${wl}-soname ${wl}$soname `test -n "$verstring" && echo ${wl}-set_version ${wl}$verstring` -o $lib'
	  fi
	fi
	link_all_deplibs_CXX=yes
	;;
    esac
    hardcode_libdir_flag_spec_CXX='${wl}-rpath ${wl}$libdir'
    hardcode_libdir_separator_CXX=:
    ;;
  linux* | k*bsd*-gnu)
    case $cc_basename in
      KCC*)
	# Kuck and Associates, Inc. (KAI) C++ Compiler

	# KCC will only create a shared library if the output file
	# ends with ".so" (or ".sl" for HP-UX), so rename the library
	# to its proper name (with version) after linking.
	archive_cmds_CXX='tempext=`echo $shared_ext | $SED -e '\''s/\([^()0-9A-Za-z{}]\)/\\\\\1/g'\''`; templib=`echo $lib | $SED -e "s/\${tempext}\..*/.so/"`; $CC $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags --soname $soname -o \$templib; mv \$templib $lib'
	archive_expsym_cmds_CXX='tempext=`echo $shared_ext | $SED -e '\''s/\([^()0-9A-Za-z{}]\)/\\\\\1/g'\''`; templib=`echo $lib | $SED -e "s/\${tempext}\..*/.so/"`; $CC $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags --soname $soname -o \$templib ${wl}-retain-symbols-file,$export_symbols; mv \$templib $lib'
	# Commands to make compiler produce verbose output that lists
	# what "hidden" libraries, object files and flags are used when
	# linking a shared library.
	#
	# There doesn't appear to be a way to prevent this compiler from
	# explicitly linking system object files so we need to strip them
	# from the output so that they don't get included in the library
	# dependencies.
	output_verbose_link_cmd='templist=`$CC $CFLAGS -v conftest.$objext -o libconftest$shared_ext 2>&1 | grep "ld"`; rm -f libconftest$shared_ext; list=""; for z in $templist; do case $z in conftest.$objext) list="$list $z";; *.$objext);; *) list="$list $z";;esac; done; echo $list'

	hardcode_libdir_flag_spec_CXX='${wl}--rpath,$libdir'
	export_dynamic_flag_spec_CXX='${wl}--export-dynamic'

	# Archives containing C++ object files must be created using
	# "CC -Bstatic", where "CC" is the KAI C++ compiler.
	old_archive_cmds_CXX='$CC -Bstatic -o $oldlib $oldobjs'
	;;
      icpc*)
	# Intel C++
	with_gnu_ld=yes
	# version 8.0 and above of icpc choke on multiply defined symbols
	# if we add $predep_objects and $postdep_objects, however 7.1 and
	# earlier do not add the objects themselves.
	case `$CC -V 2>&1` in
	*"Version 7."*)
  	  archive_cmds_CXX='$CC -shared $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags ${wl}-soname $wl$soname -o $lib'
  	  archive_expsym_cmds_CXX='$CC -shared $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags ${wl}-soname $wl$soname ${wl}-retain-symbols-file $wl$export_symbols -o $lib'
	  ;;
	*)  # Version 8.0 or newer
	  tmp_idyn=
	  case $host_cpu in
	    ia64*) tmp_idyn=' -i_dynamic';;
	  esac
  	  archive_cmds_CXX='$CC -shared'"$tmp_idyn"' $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname -o $lib'
	  archive_expsym_cmds_CXX='$CC -shared'"$tmp_idyn"' $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname ${wl}-retain-symbols-file $wl$export_symbols -o $lib'
	  ;;
	esac
	archive_cmds_need_lc_CXX=no
	hardcode_libdir_flag_spec_CXX='${wl}-rpath,$libdir'
	export_dynamic_flag_spec_CXX='${wl}--export-dynamic'
	whole_archive_flag_spec_CXX='${wl}--whole-archive$convenience ${wl}--no-whole-archive'
	;;
      pgCC*)
        # Portland Group C++ compiler
	archive_cmds_CXX='$CC -shared $pic_flag $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags ${wl}-soname ${wl}$soname -o $lib'
  	archive_expsym_cmds_CXX='$CC -shared $pic_flag $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags ${wl}-soname ${wl}$soname ${wl}-retain-symbols-file ${wl}$export_symbols -o $lib'

	hardcode_libdir_flag_spec_CXX='${wl}--rpath ${wl}$libdir'
	export_dynamic_flag_spec_CXX='${wl}--export-dynamic'
	whole_archive_flag_spec_CXX='${wl}--whole-archive`for conv in $convenience\"\"; do test  -n \"$conv\" && new_convenience=\"$new_convenience,$conv\"; done; $echo \"$new_convenience\"` ${wl}--no-whole-archive'
        ;;
      cxx*)
	# Compaq C++
	archive_cmds_CXX='$CC -shared $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags ${wl}-soname $wl$soname -o $lib'
	archive_expsym_cmds_CXX='$CC -shared $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags ${wl}-soname $wl$soname  -o $lib ${wl}-retain-symbols-file $wl$export_symbols'

	runpath_var=LD_RUN_PATH
	hardcode_libdir_flag_spec_CXX='-rpath $libdir'
	hardcode_libdir_separator_CXX=:

	# Commands to make compiler produce verbose output that lists
	# what "hidden" libraries, object files and flags are used when
	# linking a shared library.
	#
	# There doesn't appear to be a way to prevent this compiler from
	# explicitly linking system object files so we need to strip them
	# from the output so that they don't get included in the library
	# dependencies.
	output_verbose_link_cmd='templist=`$CC -shared $CFLAGS -v conftest.$objext 2>&1 | grep "ld"`; templist=`echo $templist | $SED "s/\(^.*ld.*\)\( .*ld .*$\)/\1/"`; list=""; for z in $templist; do case $z in conftest.$objext) list="$list $z";; *.$objext);; *) list="$list $z";;esac; done; echo $list'
	;;
      *)
	case `$CC -V 2>&1 | sed 5q` in
	*Sun\ C*)
	  # Sun C++ 5.9
	  no_undefined_flag_CXX=' -zdefs'
	  archive_cmds_CXX='$CC -G${allow_undefined_flag} -h$soname -o $lib $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags'
	  archive_expsym_cmds_CXX='$CC -G${allow_undefined_flag} -h$soname -o $lib $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags ${wl}-retain-symbols-file ${wl}$export_symbols'
	  hardcode_libdir_flag_spec_CXX='-R$libdir'
	  whole_archive_flag_spec_CXX='${wl}--whole-archive`new_convenience=; for conv in $convenience\"\"; do test -z \"$conv\" || new_convenience=\"$new_convenience,$conv\"; done; $echo \"$new_convenience\"` ${wl}--no-whole-archive'

	  # Not sure whether something based on
	  # $CC $CFLAGS -v conftest.$objext -o libconftest$shared_ext 2>&1
	  # would be better.
	  output_verbose_link_cmd='echo'

	  # Archives containing C++ object files must be created using
	  # "CC -xar", where "CC" is the Sun C++ compiler.  This is
	  # necessary to make sure instantiated templates are included
	  # in the archive.
	  old_archive_cmds_CXX='$CC -xar -o $oldlib $oldobjs'
	  ;;
	esac
	;;
    esac
    ;;
  lynxos*)
    # FIXME: insert proper C++ library support
    ld_shlibs_CXX=no
    ;;
  m88k*)
    # FIXME: insert proper C++ library support
    ld_shlibs_CXX=no
    ;;
  mvs*)
    case $cc_basename in
      cxx*)
	# FIXME: insert proper C++ library support
	ld_shlibs_CXX=no
	;;
      *)
	# FIXME: insert proper C++ library support
	ld_shlibs_CXX=no
	;;
    esac
    ;;
  netbsd*)
    if echo __ELF__ | $CC -E - | grep __ELF__ >/dev/null; then
      archive_cmds_CXX='$LD -Bshareable  -o $lib $predep_objects $libobjs $deplibs $postdep_objects $linker_flags'
      wlarc=
      hardcode_libdir_flag_spec_CXX='-R$libdir'
      hardcode_direct_CXX=yes
      hardcode_shlibpath_var_CXX=no
    fi
    # Workaround some broken pre-1.5 toolchains
    output_verbose_link_cmd='$CC -shared $CFLAGS -v conftest.$objext 2>&1 | grep conftest.$objext | $SED -e "s:-lgcc -lc -lgcc::"'
    ;;
  openbsd2*)
    # C++ shared libraries are fairly broken
    ld_shlibs_CXX=no
    ;;
  openbsd*)
    if test -f /usr/libexec/ld.so; then
      hardcode_direct_CXX=yes
      hardcode_shlibpath_var_CXX=no
      archive_cmds_CXX='$CC -shared $pic_flag $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags -o $lib'
      hardcode_libdir_flag_spec_CXX='${wl}-rpath,$libdir'
      if test -z "`echo __ELF__ | $CC -E - | grep __ELF__`" || test "$host_os-$host_cpu" = "openbsd2.8-powerpc"; then
	archive_expsym_cmds_CXX='$CC -shared $pic_flag $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags ${wl}-retain-symbols-file,$export_symbols -o $lib'
	export_dynamic_flag_spec_CXX='${wl}-E'
	whole_archive_flag_spec_CXX="$wlarc"'--whole-archive$convenience '"$wlarc"'--no-whole-archive'
      fi
      output_verbose_link_cmd='echo'
    else
      ld_shlibs_CXX=no
    fi
    ;;
  osf3*)
    case $cc_basename in
      KCC*)
	# Kuck and Associates, Inc. (KAI) C++ Compiler

	# KCC will only create a shared library if the output file
	# ends with ".so" (or ".sl" for HP-UX), so rename the library
	# to its proper name (with version) after linking.
	archive_cmds_CXX='tempext=`echo $shared_ext | $SED -e '\''s/\([^()0-9A-Za-z{}]\)/\\\\\1/g'\''`; templib=`echo $lib | $SED -e "s/\${tempext}\..*/.so/"`; $CC $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags --soname $soname -o \$templib; mv \$templib $lib'

	hardcode_libdir_flag_spec_CXX='${wl}-rpath,$libdir'
	hardcode_libdir_separator_CXX=:

	# Archives containing C++ object files must be created using
	# "CC -Bstatic", where "CC" is the KAI C++ compiler.
	old_archive_cmds_CXX='$CC -Bstatic -o $oldlib $oldobjs'

	;;
      RCC*)
	# Rational C++ 2.4.1
	# FIXME: insert proper C++ library support
	ld_shlibs_CXX=no
	;;
      cxx*)
	allow_undefined_flag_CXX=' ${wl}-expect_unresolved ${wl}\*'
	archive_cmds_CXX='$CC -shared${allow_undefined_flag} $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags ${wl}-soname $soname `test -n "$verstring" && echo ${wl}-set_version $verstring` -update_registry ${output_objdir}/so_locations -o $lib'

	hardcode_libdir_flag_spec_CXX='${wl}-rpath ${wl}$libdir'
	hardcode_libdir_separator_CXX=:

	# Commands to make compiler produce verbose output that lists
	# what "hidden" libraries, object files and flags are used when
	# linking a shared library.
	#
	# There doesn't appear to be a way to prevent this compiler from
	# explicitly linking system object files so we need to strip them
	# from the output so that they don't get included in the library
	# dependencies.
	output_verbose_link_cmd='templist=`$CC -shared $CFLAGS -v conftest.$objext 2>&1 | grep "ld" | grep -v "ld:"`; templist=`echo $templist | $SED "s/\(^.*ld.*\)\( .*ld.*$\)/\1/"`; list=""; for z in $templist; do case $z in conftest.$objext) list="$list $z";; *.$objext);; *) list="$list $z";;esac; done; echo $list'
	;;
      *)
	if test "$GXX" = yes && test "$with_gnu_ld" = no; then
	  allow_undefined_flag_CXX=' ${wl}-expect_unresolved ${wl}\*'
	  archive_cmds_CXX='$CC -shared -nostdlib ${allow_undefined_flag} $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags ${wl}-soname ${wl}$soname `test -n "$verstring" && echo ${wl}-set_version ${wl}$verstring` ${wl}-update_registry ${wl}${output_objdir}/so_locations -o $lib'

	  hardcode_libdir_flag_spec_CXX='${wl}-rpath ${wl}$libdir'
	  hardcode_libdir_separator_CXX=:

	  # Commands to make compiler produce verbose output that lists
	  # what "hidden" libraries, object files and flags are used when
	  # linking a shared library.
	  output_verbose_link_cmd='$CC -shared $CFLAGS -v conftest.$objext 2>&1 | grep "\-L"'

	else
	  # FIXME: insert proper C++ library support
	  ld_shlibs_CXX=no
	fi
	;;
    esac
    ;;
  osf4* | osf5*)
    case $cc_basename in
      KCC*)
	# Kuck and Associates, Inc. (KAI) C++ Compiler

	# KCC will only create a shared library if the output file
	# ends with ".so" (or ".sl" for HP-UX), so rename the library
	# to its proper name (with version) after linking.
	archive_cmds_CXX='tempext=`echo $shared_ext | $SED -e '\''s/\([^()0-9A-Za-z{}]\)/\\\\\1/g'\''`; templib=`echo $lib | $SED -e "s/\${tempext}\..*/.so/"`; $CC $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags --soname $soname -o \$templib; mv \$templib $lib'

	hardcode_libdir_flag_spec_CXX='${wl}-rpath,$libdir'
	hardcode_libdir_separator_CXX=:

	# Archives containing C++ object files must be created using
	# the KAI C++ compiler.
	old_archive_cmds_CXX='$CC -o $oldlib $oldobjs'
	;;
      RCC*)
	# Rational C++ 2.4.1
	# FIXME: insert proper C++ library support
	ld_shlibs_CXX=no
	;;
      cxx*)
	allow_undefined_flag_CXX=' -expect_unresolved \*'
	archive_cmds_CXX='$CC -shared${allow_undefined_flag} $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags -msym -soname $soname `test -n "$verstring" && echo -set_version $verstring` -update_registry ${output_objdir}/so_locations -o $lib'
	archive_expsym_cmds_CXX='for i in `cat $export_symbols`; do printf "%s %s\\n" -exported_symbol "\$i" >> $lib.exp; done~
	  echo "-hidden">> $lib.exp~
	  $CC -shared$allow_undefined_flag $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags -msym -soname $soname -Wl,-input -Wl,$lib.exp  `test -n "$verstring" && echo -set_version	$verstring` -update_registry ${output_objdir}/so_locations -o $lib~
	  $rm $lib.exp'

	hardcode_libdir_flag_spec_CXX='-rpath $libdir'
	hardcode_libdir_separator_CXX=:

	# Commands to make compiler produce verbose output that lists
	# what "hidden" libraries, object files and flags are used when
	# linking a shared library.
	#
	# There doesn't appear to be a way to prevent this compiler from
	# explicitly linking system object files so we need to strip them
	# from the output so that they don't get included in the library
	# dependencies.
	output_verbose_link_cmd='templist=`$CC -shared $CFLAGS -v conftest.$objext 2>&1 | grep "ld" | grep -v "ld:"`; templist=`echo $templist | $SED "s/\(^.*ld.*\)\( .*ld.*$\)/\1/"`; list=""; for z in $templist; do case $z in conftest.$objext) list="$list $z";; *.$objext);; *) list="$list $z";;esac; done; echo $list'
	;;
      *)
	if test "$GXX" = yes && test "$with_gnu_ld" = no; then
	  allow_undefined_flag_CXX=' ${wl}-expect_unresolved ${wl}\*'
	 archive_cmds_CXX='$CC -shared -nostdlib ${allow_undefined_flag} $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags ${wl}-msym ${wl}-soname ${wl}$soname `test -n "$verstring" && echo ${wl}-set_version ${wl}$verstring` ${wl}-update_registry ${wl}${output_objdir}/so_locations -o $lib'

	  hardcode_libdir_flag_spec_CXX='${wl}-rpath ${wl}$libdir'
	  hardcode_libdir_separator_CXX=:

	  # Commands to make compiler produce verbose output that lists
	  # what "hidden" libraries, object files and flags are used when
	  # linking a shared library.
	  output_verbose_link_cmd='$CC -shared $CFLAGS -v conftest.$objext 2>&1 | grep "\-L"'

	else
	  # FIXME: insert proper C++ library support
	  ld_shlibs_CXX=no
	fi
	;;
    esac
    ;;
  psos*)
    # FIXME: insert proper C++ library support
    ld_shlibs_CXX=no
    ;;
  sunos4*)
    case $cc_basename in
      CC*)
	# Sun C++ 4.x
	# FIXME: insert proper C++ library support
	ld_shlibs_CXX=no
	;;
      lcc*)
	# Lucid
	# FIXME: insert proper C++ library support
	ld_shlibs_CXX=no
	;;
      *)
	# FIXME: insert proper C++ library support
	ld_shlibs_CXX=no
	;;
    esac
    ;;
  solaris*)
    case $cc_basename in
      CC*)
	# Sun C++ 4.2, 5.x and Centerline C++
        archive_cmds_need_lc_CXX=yes
	no_undefined_flag_CXX=' -zdefs'
	archive_cmds_CXX='$CC -G${allow_undefined_flag}  -h$soname -o $lib $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags'
	archive_expsym_cmds_CXX='$echo "{ global:" > $lib.exp~cat $export_symbols | $SED -e "s/\(.*\)/\1;/" >> $lib.exp~$echo "local: *; };" >> $lib.exp~
	$CC -G${allow_undefined_flag}  ${wl}-M ${wl}$lib.exp -h$soname -o $lib $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags~$rm $lib.exp'

	hardcode_libdir_flag_spec_CXX='-R$libdir'
	hardcode_shlibpath_var_CXX=no
	case $host_os in
	  solaris2.[0-5] | solaris2.[0-5].*) ;;
	  *)
	    # The compiler driver will combine and reorder linker options,
	    # but understands `-z linker_flag'.
	    # Supported since Solaris 2.6 (maybe 2.5.1?)
	    whole_archive_flag_spec_CXX='-z allextract$convenience -z defaultextract'
	    ;;
	esac
	link_all_deplibs_CXX=yes

	output_verbose_link_cmd='echo'

	# Archives containing C++ object files must be created using
	# "CC -xar", where "CC" is the Sun C++ compiler.  This is
	# necessary to make sure instantiated templates are included
	# in the archive.
	old_archive_cmds_CXX='$CC -xar -o $oldlib $oldobjs'
	;;
      gcx*)
	# Green Hills C++ Compiler
	archive_cmds_CXX='$CC -shared $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags ${wl}-h $wl$soname -o $lib'

	# The C++ compiler must be used to create the archive.
	old_archive_cmds_CXX='$CC $LDFLAGS -archive -o $oldlib $oldobjs'
	;;
      *)
	# GNU C++ compiler with Solaris linker
	if test "$GXX" = yes && test "$with_gnu_ld" = no; then
	  no_undefined_flag_CXX=' ${wl}-z ${wl}defs'
	  if $CC --version | grep -v '^2\.7' > /dev/null; then
	    archive_cmds_CXX='$CC -shared -nostdlib $LDFLAGS $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags ${wl}-h $wl$soname -o $lib'
	    archive_expsym_cmds_CXX='$echo "{ global:" > $lib.exp~cat $export_symbols | $SED -e "s/\(.*\)/\1;/" >> $lib.exp~$echo "local: *; };" >> $lib.exp~
		$CC -shared -nostdlib ${wl}-M $wl$lib.exp -o $lib $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags~$rm $lib.exp'

	    # Commands to make compiler produce verbose output that lists
	    # what "hidden" libraries, object files and flags are used when
	    # linking a shared library.
	    output_verbose_link_cmd="$CC -shared $CFLAGS -v conftest.$objext 2>&1 | grep \"\-L\""
	  else
	    # g++ 2.7 appears to require `-G' NOT `-shared' on this
	    # platform.
	    archive_cmds_CXX='$CC -G -nostdlib $LDFLAGS $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags ${wl}-h $wl$soname -o $lib'
	    archive_expsym_cmds_CXX='$echo "{ global:" > $lib.exp~cat $export_symbols | $SED -e "s/\(.*\)/\1;/" >> $lib.exp~$echo "local: *; };" >> $lib.exp~
		$CC -G -nostdlib ${wl}-M $wl$lib.exp -o $lib $predep_objects $libobjs $deplibs $postdep_objects $compiler_flags~$rm $lib.exp'

	    # Commands to make compiler produce verbose output that lists
	    # what "hidden" libraries, object files and flags are used when
	    # linking a shared library.
	    output_verbose_link_cmd="$CC -G $CFLAGS -v conftest.$objext 2>&1 | grep \"\-L\""
	  fi

	  hardcode_libdir_flag_spec_CXX='${wl}-R $wl$libdir'
	  case $host_os in
	  solaris2.[0-5] | solaris2.[0-5].*) ;;
	  *)
	    whole_archive_flag_spec_CXX='${wl}-z ${wl}allextract$convenience ${wl}-z ${wl}defaultextract'
	    ;;
	  esac
	fi
	;;
    esac
    ;;
  sysv4*uw2* | sysv5OpenUNIX* | sysv5UnixWare7.[01].[10]* | unixware7* | sco3.2v5.0.[024]*)
    no_undefined_flag_CXX='${wl}-z,text'
    archive_cmds_need_lc_CXX=no
    hardcode_shlibpath_var_CXX=no
    runpath_var='LD_RUN_PATH'

    case $cc_basename in
      CC*)
	archive_cmds_CXX='$CC -G ${wl}-h,$soname -o $lib $libobjs $deplibs $compiler_flags'
	archive_expsym_cmds_CXX='$CC -G ${wl}-Bexport:$export_symbols ${wl}-h,$soname -o $lib $libobjs $deplibs $compiler_flags'
	;;
      *)
	archive_cmds_CXX='$CC -shared ${wl}-h,$soname -o $lib $libobjs $deplibs $compiler_flags'
	archive_expsym_cmds_CXX='$CC -shared ${wl}-Bexport:$export_symbols ${wl}-h,$soname -o $lib $libobjs $deplibs $compiler_flags'
	;;
    esac
    ;;
  sysv5* | sco3.2v5* | sco5v6*)
    # Note: We can NOT use -z defs as we might desire, because we do not
    # link with -lc, and that would cause any symbols used from libc to
    # always be unresolved, which means just about no library would
    # ever link correctly.  If we're not using GNU ld we use -z text
    # though, which does catch some bad symbols but isn't as heavy-handed
    # as -z defs.
    # For security reasons, it is highly recommended that you always
    # use absolute paths for naming shared libraries, and exclude the
    # DT_RUNPATH tag from executables and libraries.  But doing so
    # requires that you compile everything twice, which is a pain.
    # So that behaviour is only enabled if SCOABSPATH is set to a
    # non-empty value in the environment.  Most likely only useful for
    # creating official distributions of packages.
    # This is a hack until libtool officially supports absolute path
    # names for shared libraries.
    no_undefined_flag_CXX='${wl}-z,text'
    allow_undefined_flag_CXX='${wl}-z,nodefs'
    archive_cmds_need_lc_CXX=no
    hardcode_shlibpath_var_CXX=no
    hardcode_libdir_flag_spec_CXX='`test -z "$SCOABSPATH" && echo ${wl}-R,$libdir`'
    hardcode_libdir_separator_CXX=':'
    link_all_deplibs_CXX=yes
    export_dynamic_flag_spec_CXX='${wl}-Bexport'
    runpath_var='LD_RUN_PATH'

    case $cc_basename in
      CC*)
	archive_cmds_CXX='$CC -G ${wl}-h,\${SCOABSPATH:+${install_libdir}/}$soname -o $lib $libobjs $deplibs $compiler_flags'
	archive_expsym_cmds_CXX='$CC -G ${wl}-Bexport:$export_symbols ${wl}-h,\${SCOABSPATH:+${install_libdir}/}$soname -o $lib $libobjs $deplibs $compiler_flags'
	;;
      *)
	archive_cmds_CXX='$CC -shared ${wl}-h,\${SCOABSPATH:+${install_libdir}/}$soname -o $lib $libobjs $deplibs $compiler_flags'
	archive_expsym_cmds_CXX='$CC -shared ${wl}-Bexport:$export_symbols ${wl}-h,\${SCOABSPATH:+${install_libdir}/}$soname -o $lib $libobjs $deplibs $compiler_flags'
	;;
    esac
    ;;
  tandem*)
    case $cc_basename in
      NCC*)
	# NonStop-UX NCC 3.20
	# FIXME: insert proper C++ library support
	ld_shlibs_CXX=no
	;;
      *)
	# FIXME: insert proper C++ library support
	ld_shlibs_CXX=no
	;;
    esac
    ;;
  vxworks*)
    # FIXME: insert proper C++ library support
    ld_shlibs_CXX=no
    ;;
  *)
    # FIXME: insert proper C++ library support
    ld_shlibs_CXX=no
    ;;
esac
{ echo "$as_me:$LINENO: result: $ld_shlibs_CXX" >&5
echo "${ECHO_T}$ld_shlibs_CXX" >&6; }
test "$ld_shlibs_CXX" = no && can_build_shared=no

GCC_CXX="$GXX"
LD_CXX="$LD"


cat > conftest.$ac_ext <<EOF
class Foo
{
public:
  Foo (void) { a = 0; }
private:
  int a;
};
EOF

if { (eval echo "$as_me:$LINENO: \"$ac_compile\"") >&5
  (eval $ac_compile) 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; then
  # Parse the compiler output and extract the necessary
  # objects, libraries and library flags.

  # Sentinel used to keep track of whether or not we are before
  # the conftest object file.
  pre_test_object_deps_done=no

  # The `*' in the case matches for architectures that use `case' in
  # $output_verbose_cmd can trigger glob expansion during the loop
  # eval without this substitution.
  output_verbose_link_cmd=`$echo "X$output_verbose_link_cmd" | $Xsed -e "$no_glob_subst"`

  for p in `eval $output_verbose_link_cmd`; do
    case $p in

    -L* | -R* | -l*)
       # Some compilers place space between "-{L,R}" and the path.
       # Remove the space.
       if test $p = "-L" \
	  || test $p = "-R"; then
	 prev=$p
	 continue
       else
	 prev=
       fi

       if test "$pre_test_object_deps_done" = no; then
	 case $p in
	 -L* | -R*)
	   # Internal compiler library paths should come after those
	   # provided the user.  The postdeps already come after the
	   # user supplied libs so there is no need to process them.
	   if test -z "$compiler_lib_search_path_CXX"; then
	     compiler_lib_search_path_CXX="${prev}${p}"
	   else
	     compiler_lib_search_path_CXX="${compiler_lib_search_path_CXX} ${prev}${p}"
	   fi
	   ;;
	 # The "-l" case would never come before the object being
	 # linked, so don't bother handling this case.
	 esac
       else
	 if test -z "$postdeps_CXX"; then
	   postdeps_CXX="${prev}${p}"
	 else
	   postdeps_CXX="${postdeps_CXX} ${prev}${p}"
	 fi
       fi
       ;;

    *.$objext)
       # This assumes that the test object file only shows up
       # once in the compiler output.
       if test "$p" = "conftest.$objext"; then
	 pre_test_object_deps_done=yes
	 continue
       fi

       if test "$pre_test_object_deps_done" = no; then
	 if test -z "$predep_objects_CXX"; then
	   predep_objects_CXX="$p"
	 else
	   predep_objects_CXX="$predep_objects_CXX $p"
	 fi
       else
	 if test -z "$postdep_objects_CXX"; then
	   postdep_objects_CXX="$p"
	 else
	   postdep_objects_CXX="$postdep_objects_CXX $p"
	 fi
       fi
       ;;

    *) ;; # Ignore the rest.

    esac
  done

  # Clean up.
  rm -f a.out a.exe
else
  echo "libtool.m4: error: problem compiling CXX test program"
fi

$rm -f confest.$objext

# PORTME: override above test on systems where it is broken
case $host_os in
interix[3-9]*)
  # Interix 3.5 installs completely hosed .la files for C++, so rather than
  # hack all around it, let's just trust "g++" to DTRT.
  predep_objects_CXX=
  postdep_objects_CXX=
  postdeps_CXX=
  ;;

linux*)
  case `$CC -V 2>&1 | sed 5q` in
  *Sun\ C*)
    # Sun C++ 5.9
    #
    # The more standards-conforming stlport4 library is
    # incompatible with the Cstd library. Avoid specifying
    # it if it's in CXXFLAGS. Ignore libCrun as
    # -library=stlport4 depends on it.
    case " $CXX $CXXFLAGS " in
    *" -library=stlport4 "*)
      solaris_use_stlport4=yes
      ;;
    esac
    if test "$solaris_use_stlport4" != yes; then
      postdeps_CXX='-library=Cstd -library=Crun'
    fi
    ;;
  esac
  ;;

solaris*)
  case $cc_basename in
  CC*)
    # The more standards-conforming stlport4 library is
    # incompatible with the Cstd library. Avoid specifying
    # it if it's in CXXFLAGS. Ignore libCrun as
    # -library=stlport4 depends on it.
    case " $CXX $CXXFLAGS " in
    *" -library=stlport4 "*)
      solaris_use_stlport4=yes
      ;;
    esac

    # Adding this requires a known-good setup of shared libraries for
    # Sun compiler versions before 5.6, else PIC objects from an old
    # archive will be linked into the output, leading to subtle bugs.
    if test "$solaris_use_stlport4" != yes; then
      postdeps_CXX='-library=Cstd -library=Crun'
    fi
    ;;
  esac
  ;;
esac


case " $postdeps_CXX " in
*" -lc "*) archive_cmds_need_lc_CXX=no ;;
esac

lt_prog_compiler_wl_CXX=
lt_prog_compiler_pic_CXX=
lt_prog_compiler_static_CXX=

{ echo "$as_me:$LINENO: checking for $compiler option to produce PIC" >&5
echo $ECHO_N "checking for $compiler option to produce PIC... $ECHO_C" >&6; }

  # C++ specific cases for pic, static, wl, etc.
  if test "$GXX" = yes; then
    lt_prog_compiler_wl_CXX='-Wl,'
    lt_prog_compiler_static_CXX='-static'

    case $host_os in
    aix*)
      # All AIX code is PIC.
      if test "$host_cpu" = ia64; then
	# AIX 5 now supports IA64 processor
	lt_prog_compiler_static_CXX='-Bstatic'
      fi
      ;;
    amigaos*)
      # FIXME: we need at least 68020 code to build shared libraries, but
      # adding the `-m68020' flag to GCC prevents building anything better,
      # like `-m68040'.
      lt_prog_compiler_pic_CXX='-m68020 -resident32 -malways-restore-a4'
      ;;
    beos* | irix5* | irix6* | nonstopux* | osf3* | osf4* | osf5*)
      # PIC is the default for these OSes.
      ;;
    mingw* | cygwin* | os2* | pw32*)
      # This hack is so that the source file can tell whether it is being
      # built for inclusion in a dll (and should export symbols for example).
      # Although the cygwin gcc ignores -fPIC, still need this for old-style
      # (--disable-auto-import) libraries
      lt_prog_compiler_pic_CXX='-DDLL_EXPORT'
      ;;
    darwin* | rhapsody*)
      # PIC is the default on this platform
      # Common symbols not allowed in MH_DYLIB files
      lt_prog_compiler_pic_CXX='-fno-common'
      ;;
    *djgpp*)
      # DJGPP does not support shared libraries at all
      lt_prog_compiler_pic_CXX=
      ;;
    interix[3-9]*)
      # Interix 3.x gcc -fpic/-fPIC options generate broken code.
      # Instead, we relocate shared libraries at runtime.
      ;;
    sysv4*MP*)
      if test -d /usr/nec; then
	lt_prog_compiler_pic_CXX=-Kconform_pic
      fi
      ;;
    hpux*)
      # PIC is the default for IA64 HP-UX and 64-bit HP-UX, but
      # not for PA HP-UX.
      case $host_cpu in
      hppa*64*|ia64*)
	;;
      *)
	lt_prog_compiler_pic_CXX='-fPIC'
	;;
      esac
      ;;
    *)
      lt_prog_compiler_pic_CXX='-fPIC'
      ;;
    esac
  else
    case $host_os in
      aix4* | aix5*)
	# All AIX code is PIC.
	if test "$host_cpu" = ia64; then
	  # AIX 5 now supports IA64 processor
	  lt_prog_compiler_static_CXX='-Bstatic'
	else
	  lt_prog_compiler_static_CXX='-bnso -bI:/lib/syscalls.exp'
	fi
	;;
      chorus*)
	case $cc_basename in
	cxch68*)
	  # Green Hills C++ Compiler
	  # _LT_AC_TAGVAR(lt_prog_compiler_static, CXX)="--no_auto_instantiation -u __main -u __premain -u _abort -r $COOL_DIR/lib/libOrb.a $MVME_DIR/lib/CC/libC.a $MVME_DIR/lib/classix/libcx.s.a"
	  ;;
	esac
	;;
       darwin*)
         # PIC is the default on this platform
         # Common symbols not allowed in MH_DYLIB files
         case $cc_basename in
           xlc*)
           lt_prog_compiler_pic_CXX='-qnocommon'
           lt_prog_compiler_wl_CXX='-Wl,'
           ;;
         esac
       ;;
      dgux*)
	case $cc_basename in
	  ec++*)
	    lt_prog_compiler_pic_CXX='-KPIC'
	    ;;
	  ghcx*)
	    # Green Hills C++ Compiler
	    lt_prog_compiler_pic_CXX='-pic'
	    ;;
	  *)
	    ;;
	esac
	;;
      freebsd* | dragonfly*)
	# FreeBSD uses GNU C++
	;;
      hpux9* | hpux10* | hpux11*)
	case $cc_basename in
	  CC*)
	    lt_prog_compiler_wl_CXX='-Wl,'
	    lt_prog_compiler_static_CXX='${wl}-a ${wl}archive'
	    if test "$host_cpu" != ia64; then
	      lt_prog_compiler_pic_CXX='+Z'
	    fi
	    ;;
	  aCC*)
	    lt_prog_compiler_wl_CXX='-Wl,'
	    lt_prog_compiler_static_CXX='${wl}-a ${wl}archive'
	    case $host_cpu in
	    hppa*64*|ia64*)
	      # +Z the default
	      ;;
	    *)
	      lt_prog_compiler_pic_CXX='+Z'
	      ;;
	    esac
	    ;;
	  *)
	    ;;
	esac
	;;
      interix*)
	# This is c89, which is MS Visual C++ (no shared libs)
	# Anyone wants to do a port?
	;;
      irix5* | irix6* | nonstopux*)
	case $cc_basename in
	  CC*)
	    lt_prog_compiler_wl_CXX='-Wl,'
	    lt_prog_compiler_static_CXX='-non_shared'
	    # CC pic flag -KPIC is the default.
	    ;;
	  *)
	    ;;
	esac
	;;
      linux* | k*bsd*-gnu)
	case $cc_basename in
	  KCC*)
	    # KAI C++ Compiler
	    lt_prog_compiler_wl_CXX='--backend -Wl,'
	    lt_prog_compiler_pic_CXX='-fPIC'
	    ;;
	  icpc* | ecpc*)
	    # Intel C++
	    lt_prog_compiler_wl_CXX='-Wl,'
	    lt_prog_compiler_pic_CXX='-KPIC'
	    lt_prog_compiler_static_CXX='-static'
	    ;;
	  pgCC*)
	    # Portland Group C++ compiler.
	    lt_prog_compiler_wl_CXX='-Wl,'
	    lt_prog_compiler_pic_CXX='-fpic'
	    lt_prog_compiler_static_CXX='-Bstatic'
	    ;;
	  cxx*)
	    # Compaq C++
	    # Make sure the PIC flag is empty.  It appears that all Alpha
	    # Linux and Compaq Tru64 Unix objects are PIC.
	    lt_prog_compiler_pic_CXX=
	    lt_prog_compiler_static_CXX='-non_shared'
	    ;;
	  *)
	    case `$CC -V 2>&1 | sed 5q` in
	    *Sun\ C*)
	      # Sun C++ 5.9
	      lt_prog_compiler_pic_CXX='-KPIC'
	      lt_prog_compiler_static_CXX='-Bstatic'
	      lt_prog_compiler_wl_CXX='-Qoption ld '
	      ;;
	    esac
	    ;;
	esac
	;;
      lynxos*)
	;;
      m88k*)
	;;
      mvs*)
	case $cc_basename in
	  cxx*)
	    lt_prog_compiler_pic_CXX='-W c,exportall'
	    ;;
	  *)
	    ;;
	esac
	;;
      netbsd*)
	;;
      osf3* | osf4* | osf5*)
	case $cc_basename in
	  KCC*)
	    lt_prog_compiler_wl_CXX='--backend -Wl,'
	    ;;
	  RCC*)
	    # Rational C++ 2.4.1
	    lt_prog_compiler_pic_CXX='-pic'
	    ;;
	  cxx*)
	    # Digital/Compaq C++
	    lt_prog_compiler_wl_CXX='-Wl,'
	    # Make sure the PIC flag is empty.  It appears that all Alpha
	    # Linux and Compaq Tru64 Unix objects are PIC.
	    lt_prog_compiler_pic_CXX=
	    lt_prog_compiler_static_CXX='-non_shared'
	    ;;
	  *)
	    ;;
	esac
	;;
      psos*)
	;;
      solaris*)
	case $cc_basename in
	  CC*)
	    # Sun C++ 4.2, 5.x and Centerline C++
	    lt_prog_compiler_pic_CXX='-KPIC'
	    lt_prog_compiler_static_CXX='-Bstatic'
	    lt_prog_compiler_wl_CXX='-Qoption ld '
	    ;;
	  gcx*)
	    # Green Hills C++ Compiler
	    lt_prog_compiler_pic_CXX='-PIC'
	    ;;
	  *)
	    ;;
	esac
	;;
      sunos4*)
	case $cc_basename in
	  CC*)
	    # Sun C++ 4.x
	    lt_prog_compiler_pic_CXX='-pic'
	    lt_prog_compiler_static_CXX='-Bstatic'
	    ;;
	  lcc*)
	    # Lucid
	    lt_prog_compiler_pic_CXX='-pic'
	    ;;
	  *)
	    ;;
	esac
	;;
      tandem*)
	case $cc_basename in
	  NCC*)
	    # NonStop-UX NCC 3.20
	    lt_prog_compiler_pic_CXX='-KPIC'
	    ;;
	  *)
	    ;;
	esac
	;;
      sysv5* | unixware* | sco3.2v5* | sco5v6* | OpenUNIX*)
	case $cc_basename in
	  CC*)
	    lt_prog_compiler_wl_CXX='-Wl,'
	    lt_prog_compiler_pic_CXX='-KPIC'
	    lt_prog_compiler_static_CXX='-Bstatic'
	    ;;
	esac
	;;
      vxworks*)
	;;
      *)
	lt_prog_compiler_can_build_shared_CXX=no
	;;
    esac
  fi

{ echo "$as_me:$LINENO: result: $lt_prog_compiler_pic_CXX" >&5
echo "${ECHO_T}$lt_prog_compiler_pic_CXX" >&6; }

#
# Check to make sure the PIC flag actually works.
#
if test -n "$lt_prog_compiler_pic_CXX"; then

{ echo "$as_me:$LINENO: checking if $compiler PIC flag $lt_prog_compiler_pic_CXX works" >&5
echo $ECHO_N "checking if $compiler PIC flag $lt_prog_compiler_pic_CXX works... $ECHO_C" >&6; }
if test "${lt_prog_compiler_pic_works_CXX+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  lt_prog_compiler_pic_works_CXX=no
  ac_outfile=conftest.$ac_objext
   echo "$lt_simple_compile_test_code" > conftest.$ac_ext
   lt_compiler_flag="$lt_prog_compiler_pic_CXX -DPIC"
   # Insert the option either (1) after the last *FLAGS variable, or
   # (2) before a word containing "conftest.", or (3) at the end.
   # Note that $ac_compile itself does not contain backslashes and begins
   # with a dollar sign (not a hyphen), so the echo should work correctly.
   # The option is referenced via a variable to avoid confusing sed.
   lt_compile=`echo "$ac_compile" | $SED \
   -e 's:.*FLAGS}\{0,1\} :&$lt_compiler_flag :; t' \
   -e 's: [^ ]*conftest\.: $lt_compiler_flag&:; t' \
   -e 's:$: $lt_compiler_flag:'`
   (eval echo "\"\$as_me:12326: $lt_compile\"" >&5)
   (eval "$lt_compile" 2>conftest.err)
   ac_status=$?
   cat conftest.err >&5
   echo "$as_me:12330: \$? = $ac_status" >&5
   if (exit $ac_status) && test -s "$ac_outfile"; then
     # The compiler can only warn and ignore the option if not recognized
     # So say no if there are warnings other than the usual output.
     $echo "X$_lt_compiler_boilerplate" | $Xsed -e '/^$/d' >conftest.exp
     $SED '/^$/d; /^ *+/d' conftest.err >conftest.er2
     if test ! -s conftest.er2 || diff conftest.exp conftest.er2 >/dev/null; then
       lt_prog_compiler_pic_works_CXX=yes
     fi
   fi
   $rm conftest*

fi
{ echo "$as_me:$LINENO: result: $lt_prog_compiler_pic_works_CXX" >&5
echo "${ECHO_T}$lt_prog_compiler_pic_works_CXX" >&6; }

if test x"$lt_prog_compiler_pic_works_CXX" = xyes; then
    case $lt_prog_compiler_pic_CXX in
     "" | " "*) ;;
     *) lt_prog_compiler_pic_CXX=" $lt_prog_compiler_pic_CXX" ;;
     esac
else
    lt_prog_compiler_pic_CXX=
     lt_prog_compiler_can_build_shared_CXX=no
fi

fi
case $host_os in
  # For platforms which do not support PIC, -DPIC is meaningless:
  *djgpp*)
    lt_prog_compiler_pic_CXX=
    ;;
  *)
    lt_prog_compiler_pic_CXX="$lt_prog_compiler_pic_CXX -DPIC"
    ;;
esac

#
# Check to make sure the static flag actually works.
#
wl=$lt_prog_compiler_wl_CXX eval lt_tmp_static_flag=\"$lt_prog_compiler_static_CXX\"
{ echo "$as_me:$LINENO: checking if $compiler static flag $lt_tmp_static_flag works" >&5
echo $ECHO_N "checking if $compiler static flag $lt_tmp_static_flag works... $ECHO_C" >&6; }
if test "${lt_prog_compiler_static_works_CXX+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  lt_prog_compiler_static_works_CXX=no
   save_LDFLAGS="$LDFLAGS"
   LDFLAGS="$LDFLAGS $lt_tmp_static_flag"
   echo "$lt_simple_link_test_code" > conftest.$ac_ext
   if (eval $ac_link 2>conftest.err) && test -s conftest$ac_exeext; then
     # The linker can only warn and ignore the option if not recognized
     # So say no if there are warnings
     if test -s conftest.err; then
       # Append any errors to the config.log.
       cat conftest.err 1>&5
       $echo "X$_lt_linker_boilerplate" | $Xsed -e '/^$/d' > conftest.exp
       $SED '/^$/d; /^ *+/d' conftest.err >conftest.er2
       if diff conftest.exp conftest.er2 >/dev/null; then
         lt_prog_compiler_static_works_CXX=yes
       fi
     else
       lt_prog_compiler_static_works_CXX=yes
     fi
   fi
   $rm conftest*
   LDFLAGS="$save_LDFLAGS"

fi
{ echo "$as_me:$LINENO: result: $lt_prog_compiler_static_works_CXX" >&5
echo "${ECHO_T}$lt_prog_compiler_static_works_CXX" >&6; }

if test x"$lt_prog_compiler_static_works_CXX" = xyes; then
    :
else
    lt_prog_compiler_static_CXX=
fi


{ echo "$as_me:$LINENO: checking if $compiler supports -c -o file.$ac_objext" >&5
echo $ECHO_N "checking if $compiler supports -c -o file.$ac_objext... $ECHO_C" >&6; }
if test "${lt_cv_prog_compiler_c_o_CXX+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  lt_cv_prog_compiler_c_o_CXX=no
   $rm -r conftest 2>/dev/null
   mkdir conftest
   cd conftest
   mkdir out
   echo "$lt_simple_compile_test_code" > conftest.$ac_ext

   lt_compiler_flag="-o out/conftest2.$ac_objext"
   # Insert the option either (1) after the last *FLAGS variable, or
   # (2) before a word containing "conftest.", or (3) at the end.
   # Note that $ac_compile itself does not contain backslashes and begins
   # with a dollar sign (not a hyphen), so the echo should work correctly.
   lt_compile=`echo "$ac_compile" | $SED \
   -e 's:.*FLAGS}\{0,1\} :&$lt_compiler_flag :; t' \
   -e 's: [^ ]*conftest\.: $lt_compiler_flag&:; t' \
   -e 's:$: $lt_compiler_flag:'`
   (eval echo "\"\$as_me:12430: $lt_compile\"" >&5)
   (eval "$lt_compile" 2>out/conftest.err)
   ac_status=$?
   cat out/conftest.err >&5
   echo "$as_me:12434: \$? = $ac_status" >&5
   if (exit $ac_status) && test -s out/conftest2.$ac_objext
   then
     # The compiler can only warn and ignore the option if not recognized
     # So say no if there are warnings
     $echo "X$_lt_compiler_boilerplate" | $Xsed -e '/^$/d' > out/conftest.exp
     $SED '/^$/d; /^ *+/d' out/conftest.err >out/conftest.er2
     if test ! -s out/conftest.er2 || diff out/conftest.exp out/conftest.er2 >/dev/null; then
       lt_cv_prog_compiler_c_o_CXX=yes
     fi
   fi
   chmod u+w . 2>&5
   $rm conftest*
   # SGI C++ compiler will create directory out/ii_files/ for
   # template instantiation
   test -d out/ii_files && $rm out/ii_files/* && rmdir out/ii_files
   $rm out/* && rmdir out
   cd ..
   rmdir conftest
   $rm conftest*

fi
{ echo "$as_me:$LINENO: result: $lt_cv_prog_compiler_c_o_CXX" >&5
echo "${ECHO_T}$lt_cv_prog_compiler_c_o_CXX" >&6; }


hard_links="nottested"
if test "$lt_cv_prog_compiler_c_o_CXX" = no && test "$need_locks" != no; then
  # do not overwrite the value of need_locks provided by the user
  { echo "$as_me:$LINENO: checking if we can lock with hard links" >&5
echo $ECHO_N "checking if we can lock with hard links... $ECHO_C" >&6; }
  hard_links=yes
  $rm conftest*
  ln conftest.a conftest.b 2>/dev/null && hard_links=no
  touch conftest.a
  ln conftest.a conftest.b 2>&5 || hard_links=no
  ln conftest.a conftest.b 2>/dev/null && hard_links=no
  { echo "$as_me:$LINENO: result: $hard_links" >&5
echo "${ECHO_T}$hard_links" >&6; }
  if test "$hard_links" = no; then
    { echo "$as_me:$LINENO: WARNING: \`$CC' does not support \`-c -o', so \`make -j' may be unsafe" >&5
echo "$as_me: WARNING: \`$CC' does not support \`-c -o', so \`make -j' may be unsafe" >&2;}
    need_locks=warn
  fi
else
  need_locks=no
fi

{ echo "$as_me:$LINENO: checking whether the $compiler linker ($LD) supports shared libraries" >&5
echo $ECHO_N "checking whether the $compiler linker ($LD) supports shared libraries... $ECHO_C" >&6; }

  export_symbols_cmds_CXX='$NM $libobjs $convenience | $global_symbol_pipe | $SED '\''s/.* //'\'' | sort | uniq > $export_symbols'
  case $host_os in
  aix4* | aix5*)
    # If we're using GNU nm, then we don't want the "-C" option.
    # -C means demangle to AIX nm, but means don't demangle with GNU nm
    if $NM -V 2>&1 | grep 'GNU' > /dev/null; then
      export_symbols_cmds_CXX='$NM -Bpg $libobjs $convenience | awk '\''{ if (((\$2 == "T") || (\$2 == "D") || (\$2 == "B")) && (substr(\$3,1,1) != ".")) { print \$3 } }'\'' | sort -u > $export_symbols'
    else
      export_symbols_cmds_CXX='$NM -BCpg $libobjs $convenience | awk '\''{ if (((\$2 == "T") || (\$2 == "D") || (\$2 == "B")) && (substr(\$3,1,1) != ".")) { print \$3 } }'\'' | sort -u > $export_symbols'
    fi
    ;;
  pw32*)
    export_symbols_cmds_CXX="$ltdll_cmds"
  ;;
  cygwin* | mingw*)
    export_symbols_cmds_CXX='$NM $libobjs $convenience | $global_symbol_pipe | $SED -e '\''/^[BCDGRS][ ]/s/.*[ ]\([^ ]*\)/\1 DATA/;/^.*[ ]__nm__/s/^.*[ ]__nm__\([^ ]*\)[ ][^ ]*/\1 DATA/;/^I[ ]/d;/^[AITW][ ]/s/.*[ ]//'\'' | sort | uniq > $export_symbols'
  ;;
  *)
    export_symbols_cmds_CXX='$NM $libobjs $convenience | $global_symbol_pipe | $SED '\''s/.* //'\'' | sort | uniq > $export_symbols'
  ;;
  esac

{ echo "$as_me:$LINENO: result: $ld_shlibs_CXX" >&5
echo "${ECHO_T}$ld_shlibs_CXX" >&6; }
test "$ld_shlibs_CXX" = no && can_build_shared=no

#
# Do we need to explicitly link libc?
#
case "x$archive_cmds_need_lc_CXX" in
x|xyes)
  # Assume -lc should be added
  archive_cmds_need_lc_CXX=yes

  if test "$enable_shared" = yes && test "$GCC" = yes; then
    case $archive_cmds_CXX in
    *'~'*)
      # FIXME: we may have to deal with multi-command sequences.
      ;;
    '$CC '*)
      # Test whether the compiler implicitly links with -lc since on some
      # systems, -lgcc has to come before -lc. If gcc already passes -lc
      # to ld, don't add -lc before -lgcc.
      { echo "$as_me:$LINENO: checking whether -lc should be explicitly linked in" >&5
echo $ECHO_N "checking whether -lc should be explicitly linked in... $ECHO_C" >&6; }
      $rm conftest*
      echo "$lt_simple_compile_test_code" > conftest.$ac_ext

      if { (eval echo "$as_me:$LINENO: \"$ac_compile\"") >&5
  (eval $ac_compile) 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } 2>conftest.err; then
        soname=conftest
        lib=conftest
        libobjs=conftest.$ac_objext
        deplibs=
        wl=$lt_prog_compiler_wl_CXX
	pic_flag=$lt_prog_compiler_pic_CXX
        compiler_flags=-v
        linker_flags=-v
        verstring=
        output_objdir=.
        libname=conftest
        lt_save_allow_undefined_flag=$allow_undefined_flag_CXX
        allow_undefined_flag_CXX=
        if { (eval echo "$as_me:$LINENO: \"$archive_cmds_CXX 2\>\&1 \| grep \" -lc \" \>/dev/null 2\>\&1\"") >&5
  (eval $archive_cmds_CXX 2\>\&1 \| grep \" -lc \" \>/dev/null 2\>\&1) 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }
        then
	  archive_cmds_need_lc_CXX=no
        else
	  archive_cmds_need_lc_CXX=yes
        fi
        allow_undefined_flag_CXX=$lt_save_allow_undefined_flag
      else
        cat conftest.err 1>&5
      fi
      $rm conftest*
      { echo "$as_me:$LINENO: result: $archive_cmds_need_lc_CXX" >&5
echo "${ECHO_T}$archive_cmds_need_lc_CXX" >&6; }
      ;;
    esac
  fi
  ;;
esac

{ echo "$as_me:$LINENO: checking dynamic linker characteristics" >&5
echo $ECHO_N "checking dynamic linker characteristics... $ECHO_C" >&6; }
library_names_spec=
libname_spec='lib$name'
soname_spec=
shrext_cmds=".so"
postinstall_cmds=
postuninstall_cmds=
finish_cmds=
finish_eval=
shlibpath_var=
shlibpath_overrides_runpath=unknown
version_type=none
dynamic_linker="$host_os ld.so"
sys_lib_dlsearch_path_spec="/lib /usr/lib"

need_lib_prefix=unknown
hardcode_into_libs=no

# when you set need_version to no, make sure it does not cause -set_version
# flags to be left without arguments
need_version=unknown

case $host_os in
aix3*)
  version_type=linux
  library_names_spec='${libname}${release}${shared_ext}$versuffix $libname.a'
  shlibpath_var=LIBPATH

  # AIX 3 has no versioning support, so we append a major version to the name.
  soname_spec='${libname}${release}${shared_ext}$major'
  ;;

aix4* | aix5*)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  hardcode_into_libs=yes
  if test "$host_cpu" = ia64; then
    # AIX 5 supports IA64
    library_names_spec='${libname}${release}${shared_ext}$major ${libname}${release}${shared_ext}$versuffix $libname${shared_ext}'
    shlibpath_var=LD_LIBRARY_PATH
  else
    # With GCC up to 2.95.x, collect2 would create an import file
    # for dependence libraries.  The import file would start with
    # the line `#! .'.  This would cause the generated library to
    # depend on `.', always an invalid library.  This was fixed in
    # development snapshots of GCC prior to 3.0.
    case $host_os in
      aix4 | aix4.[01] | aix4.[01].*)
      if { echo '#if __GNUC__ > 2 || (__GNUC__ == 2 && __GNUC_MINOR__ >= 97)'
	   echo ' yes '
	   echo '#endif'; } | ${CC} -E - | grep yes > /dev/null; then
	:
      else
	can_build_shared=no
      fi
      ;;
    esac
    # AIX (on Power*) has no versioning support, so currently we can not hardcode correct
    # soname into executable. Probably we can add versioning support to
    # collect2, so additional links can be useful in future.
    if test "$aix_use_runtimelinking" = yes; then
      # If using run time linking (on AIX 4.2 or later) use lib<name>.so
      # instead of lib<name>.a to let people know that these are not
      # typical AIX shared libraries.
      library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
    else
      # We preserve .a as extension for shared libraries through AIX4.2
      # and later when we are not doing run time linking.
      library_names_spec='${libname}${release}.a $libname.a'
      soname_spec='${libname}${release}${shared_ext}$major'
    fi
    shlibpath_var=LIBPATH
  fi
  ;;

amigaos*)
  library_names_spec='$libname.ixlibrary $libname.a'
  # Create ${libname}_ixlibrary.a entries in /sys/libs.
  finish_eval='for lib in `ls $libdir/*.ixlibrary 2>/dev/null`; do libname=`$echo "X$lib" | $Xsed -e '\''s%^.*/\([^/]*\)\.ixlibrary$%\1%'\''`; test $rm /sys/libs/${libname}_ixlibrary.a; $show "cd /sys/libs && $LN_S $lib ${libname}_ixlibrary.a"; cd /sys/libs && $LN_S $lib ${libname}_ixlibrary.a || exit 1; done'
  ;;

beos*)
  library_names_spec='${libname}${shared_ext}'
  dynamic_linker="$host_os ld.so"
  shlibpath_var=LIBRARY_PATH
  ;;

bsdi[45]*)
  version_type=linux
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  finish_cmds='PATH="\$PATH:/sbin" ldconfig $libdir'
  shlibpath_var=LD_LIBRARY_PATH
  sys_lib_search_path_spec="/shlib /usr/lib /usr/X11/lib /usr/contrib/lib /lib /usr/local/lib"
  sys_lib_dlsearch_path_spec="/shlib /usr/lib /usr/local/lib"
  # the default ld.so.conf also contains /usr/contrib/lib and
  # /usr/X11R6/lib (/usr/X11 is a link to /usr/X11R6), but let us allow
  # libtool to hard-code these into programs
  ;;

cygwin* | mingw* | pw32*)
  version_type=windows
  shrext_cmds=".dll"
  need_version=no
  need_lib_prefix=no

  case $GCC,$host_os in
  yes,cygwin* | yes,mingw* | yes,pw32*)
    library_names_spec='$libname.dll.a'
    # DLL is installed to $(libdir)/../bin by postinstall_cmds
    postinstall_cmds='base_file=`basename \${file}`~
      dlpath=`$SHELL 2>&1 -c '\''. $dir/'\''\${base_file}'\''i;echo \$dlname'\''`~
      dldir=$destdir/`dirname \$dlpath`~
      test -d \$dldir || mkdir -p \$dldir~
      $install_prog $dir/$dlname \$dldir/$dlname~
      chmod a+x \$dldir/$dlname'
    postuninstall_cmds='dldll=`$SHELL 2>&1 -c '\''. $file; echo \$dlname'\''`~
      dlpath=$dir/\$dldll~
       $rm \$dlpath'
    shlibpath_overrides_runpath=yes

    case $host_os in
    cygwin*)
      # Cygwin DLLs use 'cyg' prefix rather than 'lib'
      soname_spec='`echo ${libname} | sed -e 's/^lib/cyg/'``echo ${release} | $SED -e 's/[.]/-/g'`${versuffix}${shared_ext}'
      sys_lib_search_path_spec="/usr/lib /lib/w32api /lib /usr/local/lib"
      ;;
    mingw*)
      # MinGW DLLs use traditional 'lib' prefix
      soname_spec='${libname}`echo ${release} | $SED -e 's/[.]/-/g'`${versuffix}${shared_ext}'
      sys_lib_search_path_spec=`$CC -print-search-dirs | grep "^libraries:" | $SED -e "s/^libraries://" -e "s,=/,/,g"`
      if echo "$sys_lib_search_path_spec" | grep ';[c-zC-Z]:/' >/dev/null; then
        # It is most probably a Windows format PATH printed by
        # mingw gcc, but we are running on Cygwin. Gcc prints its search
        # path with ; separators, and with drive letters. We can handle the
        # drive letters (cygwin fileutils understands them), so leave them,
        # especially as we might pass files found there to a mingw objdump,
        # which wouldn't understand a cygwinified path. Ahh.
        sys_lib_search_path_spec=`echo "$sys_lib_search_path_spec" | $SED -e 's/;/ /g'`
      else
        sys_lib_search_path_spec=`echo "$sys_lib_search_path_spec" | $SED  -e "s/$PATH_SEPARATOR/ /g"`
      fi
      ;;
    pw32*)
      # pw32 DLLs use 'pw' prefix rather than 'lib'
      library_names_spec='`echo ${libname} | sed -e 's/^lib/pw/'``echo ${release} | $SED -e 's/[.]/-/g'`${versuffix}${shared_ext}'
      ;;
    esac
    ;;

  *)
    library_names_spec='${libname}`echo ${release} | $SED -e 's/[.]/-/g'`${versuffix}${shared_ext} $libname.lib'
    ;;
  esac
  dynamic_linker='Win32 ld.exe'
  # FIXME: first we should search . and the directory the executable is in
  shlibpath_var=PATH
  ;;

darwin* | rhapsody*)
  dynamic_linker="$host_os dyld"
  version_type=darwin
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${versuffix}$shared_ext ${libname}${release}${major}$shared_ext ${libname}$shared_ext'
  soname_spec='${libname}${release}${major}$shared_ext'
  shlibpath_overrides_runpath=yes
  shlibpath_var=DYLD_LIBRARY_PATH
  shrext_cmds='`test .$module = .yes && echo .so || echo .dylib`'

  sys_lib_dlsearch_path_spec='/usr/local/lib /lib /usr/lib'
  ;;

dgux*)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname$shared_ext'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  ;;

freebsd1*)
  dynamic_linker=no
  ;;

freebsd* | dragonfly*)
  # DragonFly does not have aout.  When/if they implement a new
  # versioning mechanism, adjust this.
  if test -x /usr/bin/objformat; then
    objformat=`/usr/bin/objformat`
  else
    case $host_os in
    freebsd[123]*) objformat=aout ;;
    *) objformat=elf ;;
    esac
  fi
  version_type=freebsd-$objformat
  case $version_type in
    freebsd-elf*)
      library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext} $libname${shared_ext}'
      need_version=no
      need_lib_prefix=no
      ;;
    freebsd-*)
      library_names_spec='${libname}${release}${shared_ext}$versuffix $libname${shared_ext}$versuffix'
      need_version=yes
      ;;
  esac
  shlibpath_var=LD_LIBRARY_PATH
  case $host_os in
  freebsd2*)
    shlibpath_overrides_runpath=yes
    ;;
  freebsd3.[01]* | freebsdelf3.[01]*)
    shlibpath_overrides_runpath=yes
    hardcode_into_libs=yes
    ;;
  freebsd3.[2-9]* | freebsdelf3.[2-9]* | \
  freebsd4.[0-5] | freebsdelf4.[0-5] | freebsd4.1.1 | freebsdelf4.1.1)
    shlibpath_overrides_runpath=no
    hardcode_into_libs=yes
    ;;
  *) # from 4.6 on, and DragonFly
    shlibpath_overrides_runpath=yes
    hardcode_into_libs=yes
    ;;
  esac
  ;;

gnu*)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}${major} ${libname}${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  hardcode_into_libs=yes
  ;;

hpux9* | hpux10* | hpux11*)
  # Give a soname corresponding to the major version so that dld.sl refuses to
  # link against other versions.
  version_type=sunos
  need_lib_prefix=no
  need_version=no
  case $host_cpu in
  ia64*)
    shrext_cmds='.so'
    hardcode_into_libs=yes
    dynamic_linker="$host_os dld.so"
    shlibpath_var=LD_LIBRARY_PATH
    shlibpath_overrides_runpath=yes # Unless +noenvvar is specified.
    library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
    soname_spec='${libname}${release}${shared_ext}$major'
    if test "X$HPUX_IA64_MODE" = X32; then
      sys_lib_search_path_spec="/usr/lib/hpux32 /usr/local/lib/hpux32 /usr/local/lib"
    else
      sys_lib_search_path_spec="/usr/lib/hpux64 /usr/local/lib/hpux64"
    fi
    sys_lib_dlsearch_path_spec=$sys_lib_search_path_spec
    ;;
   hppa*64*)
     shrext_cmds='.sl'
     hardcode_into_libs=yes
     dynamic_linker="$host_os dld.sl"
     shlibpath_var=LD_LIBRARY_PATH # How should we handle SHLIB_PATH
     shlibpath_overrides_runpath=yes # Unless +noenvvar is specified.
     library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
     soname_spec='${libname}${release}${shared_ext}$major'
     sys_lib_search_path_spec="/usr/lib/pa20_64 /usr/ccs/lib/pa20_64"
     sys_lib_dlsearch_path_spec=$sys_lib_search_path_spec
     ;;
   *)
    shrext_cmds='.sl'
    dynamic_linker="$host_os dld.sl"
    shlibpath_var=SHLIB_PATH
    shlibpath_overrides_runpath=no # +s is required to enable SHLIB_PATH
    library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
    soname_spec='${libname}${release}${shared_ext}$major'
    ;;
  esac
  # HP-UX runs *really* slowly unless shared libraries are mode 555.
  postinstall_cmds='chmod 555 $lib'
  ;;

interix[3-9]*)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major ${libname}${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  dynamic_linker='Interix 3.x ld.so.1 (PE, like ELF)'
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=no
  hardcode_into_libs=yes
  ;;

irix5* | irix6* | nonstopux*)
  case $host_os in
    nonstopux*) version_type=nonstopux ;;
    *)
	if test "$lt_cv_prog_gnu_ld" = yes; then
		version_type=linux
	else
		version_type=irix
	fi ;;
  esac
  need_lib_prefix=no
  need_version=no
  soname_spec='${libname}${release}${shared_ext}$major'
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major ${libname}${release}${shared_ext} $libname${shared_ext}'
  case $host_os in
  irix5* | nonstopux*)
    libsuff= shlibsuff=
    ;;
  *)
    case $LD in # libtool.m4 will add one of these switches to LD
    *-32|*"-32 "|*-melf32bsmip|*"-melf32bsmip ")
      libsuff= shlibsuff= libmagic=32-bit;;
    *-n32|*"-n32 "|*-melf32bmipn32|*"-melf32bmipn32 ")
      libsuff=32 shlibsuff=N32 libmagic=N32;;
    *-64|*"-64 "|*-melf64bmip|*"-melf64bmip ")
      libsuff=64 shlibsuff=64 libmagic=64-bit;;
    *) libsuff= shlibsuff= libmagic=never-match;;
    esac
    ;;
  esac
  shlibpath_var=LD_LIBRARY${shlibsuff}_PATH
  shlibpath_overrides_runpath=no
  sys_lib_search_path_spec="/usr/lib${libsuff} /lib${libsuff} /usr/local/lib${libsuff}"
  sys_lib_dlsearch_path_spec="/usr/lib${libsuff} /lib${libsuff}"
  hardcode_into_libs=yes
  ;;

# No shared lib support for Linux oldld, aout, or coff.
linux*oldld* | linux*aout* | linux*coff*)
  dynamic_linker=no
  ;;

# This must be Linux ELF.
linux* | k*bsd*-gnu)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  finish_cmds='PATH="\$PATH:/sbin" ldconfig -n $libdir'
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=no
  # This implies no fast_install, which is unacceptable.
  # Some rework will be needed to allow for fast_install
  # before this can be enabled.
  hardcode_into_libs=yes

  # Append ld.so.conf contents to the search path
  if test -f /etc/ld.so.conf; then
    lt_ld_extra=`awk '/^include / { system(sprintf("cd /etc; cat %s 2>/dev/null", \$2)); skip = 1; } { if (!skip) print \$0; skip = 0; }' < /etc/ld.so.conf | $SED -e 's/#.*//;/^[ 	]*hwcap[ 	]/d;s/[:,	]/ /g;s/=[^=]*$//;s/=[^= ]* / /g;/^$/d' | tr '\n' ' '`
    sys_lib_dlsearch_path_spec="/lib /usr/lib $lt_ld_extra"
  fi

  # We used to test for /lib/ld.so.1 and disable shared libraries on
  # powerpc, because MkLinux only supported shared libraries with the
  # GNU dynamic linker.  Since this was broken with cross compilers,
  # most powerpc-linux boxes support dynamic linking these days and
  # people can always --disable-shared, the test was removed, and we
  # assume the GNU/Linux dynamic linker is in use.
  dynamic_linker='GNU/Linux ld.so'
  ;;

netbsd*)
  version_type=sunos
  need_lib_prefix=no
  need_version=no
  if echo __ELF__ | $CC -E - | grep __ELF__ >/dev/null; then
    library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${shared_ext}$versuffix'
    finish_cmds='PATH="\$PATH:/sbin" ldconfig -m $libdir'
    dynamic_linker='NetBSD (a.out) ld.so'
  else
    library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major ${libname}${shared_ext}'
    soname_spec='${libname}${release}${shared_ext}$major'
    dynamic_linker='NetBSD ld.elf_so'
  fi
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=yes
  hardcode_into_libs=yes
  ;;

newsos6)
  version_type=linux
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=yes
  ;;

nto-qnx*)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=yes
  ;;

openbsd*)
  version_type=sunos
  sys_lib_dlsearch_path_spec="/usr/lib"
  need_lib_prefix=no
  # Some older versions of OpenBSD (3.3 at least) *do* need versioned libs.
  case $host_os in
    openbsd3.3 | openbsd3.3.*) need_version=yes ;;
    *)                         need_version=no  ;;
  esac
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${shared_ext}$versuffix'
  finish_cmds='PATH="\$PATH:/sbin" ldconfig -m $libdir'
  shlibpath_var=LD_LIBRARY_PATH
  if test -z "`echo __ELF__ | $CC -E - | grep __ELF__`" || test "$host_os-$host_cpu" = "openbsd2.8-powerpc"; then
    case $host_os in
      openbsd2.[89] | openbsd2.[89].*)
	shlibpath_overrides_runpath=no
	;;
      *)
	shlibpath_overrides_runpath=yes
	;;
      esac
  else
    shlibpath_overrides_runpath=yes
  fi
  ;;

os2*)
  libname_spec='$name'
  shrext_cmds=".dll"
  need_lib_prefix=no
  library_names_spec='$libname${shared_ext} $libname.a'
  dynamic_linker='OS/2 ld.exe'
  shlibpath_var=LIBPATH
  ;;

osf3* | osf4* | osf5*)
  version_type=osf
  need_lib_prefix=no
  need_version=no
  soname_spec='${libname}${release}${shared_ext}$major'
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  shlibpath_var=LD_LIBRARY_PATH
  sys_lib_search_path_spec="/usr/shlib /usr/ccs/lib /usr/lib/cmplrs/cc /usr/lib /usr/local/lib /var/shlib"
  sys_lib_dlsearch_path_spec="$sys_lib_search_path_spec"
  ;;

rdos*)
  dynamic_linker=no
  ;;

solaris*)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=yes
  hardcode_into_libs=yes
  # ldd complains unless libraries are executable
  postinstall_cmds='chmod +x $lib'
  ;;

sunos4*)
  version_type=sunos
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${shared_ext}$versuffix'
  finish_cmds='PATH="\$PATH:/usr/etc" ldconfig $libdir'
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=yes
  if test "$with_gnu_ld" = yes; then
    need_lib_prefix=no
  fi
  need_version=yes
  ;;

sysv4 | sysv4.3*)
  version_type=linux
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  case $host_vendor in
    sni)
      shlibpath_overrides_runpath=no
      need_lib_prefix=no
      export_dynamic_flag_spec='${wl}-Blargedynsym'
      runpath_var=LD_RUN_PATH
      ;;
    siemens)
      need_lib_prefix=no
      ;;
    motorola)
      need_lib_prefix=no
      need_version=no
      shlibpath_overrides_runpath=no
      sys_lib_search_path_spec='/lib /usr/lib /usr/ccs/lib'
      ;;
  esac
  ;;

sysv4*MP*)
  if test -d /usr/nec ;then
    version_type=linux
    library_names_spec='$libname${shared_ext}.$versuffix $libname${shared_ext}.$major $libname${shared_ext}'
    soname_spec='$libname${shared_ext}.$major'
    shlibpath_var=LD_LIBRARY_PATH
  fi
  ;;

sysv5* | sco3.2v5* | sco5v6* | unixware* | OpenUNIX* | sysv4*uw2*)
  version_type=freebsd-elf
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext} $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  hardcode_into_libs=yes
  if test "$with_gnu_ld" = yes; then
    sys_lib_search_path_spec='/usr/local/lib /usr/gnu/lib /usr/ccs/lib /usr/lib /lib'
    shlibpath_overrides_runpath=no
  else
    sys_lib_search_path_spec='/usr/ccs/lib /usr/lib'
    shlibpath_overrides_runpath=yes
    case $host_os in
      sco3.2v5*)
        sys_lib_search_path_spec="$sys_lib_search_path_spec /lib"
	;;
    esac
  fi
  sys_lib_dlsearch_path_spec='/usr/lib'
  ;;

uts4*)
  version_type=linux
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  ;;

*)
  dynamic_linker=no
  ;;
esac
{ echo "$as_me:$LINENO: result: $dynamic_linker" >&5
echo "${ECHO_T}$dynamic_linker" >&6; }
test "$dynamic_linker" = no && can_build_shared=no

variables_saved_for_relink="PATH $shlibpath_var $runpath_var"
if test "$GCC" = yes; then
  variables_saved_for_relink="$variables_saved_for_relink GCC_EXEC_PREFIX COMPILER_PATH LIBRARY_PATH"
fi

{ echo "$as_me:$LINENO: checking how to hardcode library paths into programs" >&5
echo $ECHO_N "checking how to hardcode library paths into programs... $ECHO_C" >&6; }
hardcode_action_CXX=
if test -n "$hardcode_libdir_flag_spec_CXX" || \
   test -n "$runpath_var_CXX" || \
   test "X$hardcode_automatic_CXX" = "Xyes" ; then

  # We can hardcode non-existant directories.
  if test "$hardcode_direct_CXX" != no &&
     # If the only mechanism to avoid hardcoding is shlibpath_var, we
     # have to relink, otherwise we might link with an installed library
     # when we should be linking with a yet-to-be-installed one
     ## test "$_LT_AC_TAGVAR(hardcode_shlibpath_var, CXX)" != no &&
     test "$hardcode_minus_L_CXX" != no; then
    # Linking always hardcodes the temporary library directory.
    hardcode_action_CXX=relink
  else
    # We can link without hardcoding, and we can hardcode nonexisting dirs.
    hardcode_action_CXX=immediate
  fi
else
  # We cannot hardcode anything, or else we can only hardcode existing
  # directories.
  hardcode_action_CXX=unsupported
fi
{ echo "$as_me:$LINENO: result: $hardcode_action_CXX" >&5
echo "${ECHO_T}$hardcode_action_CXX" >&6; }

if test "$hardcode_action_CXX" = relink; then
  # Fast installation is not supported
  enable_fast_install=no
elif test "$shlibpath_overrides_runpath" = yes ||
     test "$enable_shared" = no; then
  # Fast installation is not necessary
  enable_fast_install=needless
fi


# The else clause should only fire when bootstrapping the
# libtool distribution, otherwise you forgot to ship ltmain.sh
# with your package, and you will get complaints that there are
# no rules to generate ltmain.sh.
if test -f "$ltmain"; then
  # See if we are running on zsh, and set the options which allow our commands through
  # without removal of \ escapes.
  if test -n "${ZSH_VERSION+set}" ; then
    setopt NO_GLOB_SUBST
  fi
  # Now quote all the things that may contain metacharacters while being
  # careful not to overquote the AC_SUBSTed values.  We take copies of the
  # variables and quote the copies for generation of the libtool script.
  for var in echo old_CC old_CFLAGS AR AR_FLAGS EGREP RANLIB LN_S LTCC LTCFLAGS NM \
    SED SHELL STRIP \
    libname_spec library_names_spec soname_spec extract_expsyms_cmds \
    old_striplib striplib file_magic_cmd finish_cmds finish_eval \
    deplibs_check_method reload_flag reload_cmds need_locks \
    lt_cv_sys_global_symbol_pipe lt_cv_sys_global_symbol_to_cdecl \
    lt_cv_sys_global_symbol_to_c_name_address \
    sys_lib_search_path_spec sys_lib_dlsearch_path_spec \
    old_postinstall_cmds old_postuninstall_cmds \
    compiler_CXX \
    CC_CXX \
    LD_CXX \
    lt_prog_compiler_wl_CXX \
    lt_prog_compiler_pic_CXX \
    lt_prog_compiler_static_CXX \
    lt_prog_compiler_no_builtin_flag_CXX \
    export_dynamic_flag_spec_CXX \
    thread_safe_flag_spec_CXX \
    whole_archive_flag_spec_CXX \
    enable_shared_with_static_runtimes_CXX \
    old_archive_cmds_CXX \
    old_archive_from_new_cmds_CXX \
    predep_objects_CXX \
    postdep_objects_CXX \
    predeps_CXX \
    postdeps_CXX \
    compiler_lib_search_path_CXX \
    archive_cmds_CXX \
    archive_expsym_cmds_CXX \
    postinstall_cmds_CXX \
    postuninstall_cmds_CXX \
    old_archive_from_expsyms_cmds_CXX \
    allow_undefined_flag_CXX \
    no_undefined_flag_CXX \
    export_symbols_cmds_CXX \
    hardcode_libdir_flag_spec_CXX \
    hardcode_libdir_flag_spec_ld_CXX \
    hardcode_libdir_separator_CXX \
    hardcode_automatic_CXX \
    module_cmds_CXX \
    module_expsym_cmds_CXX \
    lt_cv_prog_compiler_c_o_CXX \
    fix_srcfile_path_CXX \
    exclude_expsyms_CXX \
    include_expsyms_CXX; do

    case $var in
    old_archive_cmds_CXX | \
    old_archive_from_new_cmds_CXX | \
    archive_cmds_CXX | \
    archive_expsym_cmds_CXX | \
    module_cmds_CXX | \
    module_expsym_cmds_CXX | \
    old_archive_from_expsyms_cmds_CXX | \
    export_symbols_cmds_CXX | \
    extract_expsyms_cmds | reload_cmds | finish_cmds | \
    postinstall_cmds | postuninstall_cmds | \
    old_postinstall_cmds | old_postuninstall_cmds | \
    sys_lib_search_path_spec | sys_lib_dlsearch_path_spec)
      # Double-quote double-evaled strings.
      eval "lt_$var=\\\"\`\$echo \"X\$$var\" | \$Xsed -e \"\$double_quote_subst\" -e \"\$sed_quote_subst\" -e \"\$delay_variable_subst\"\`\\\""
      ;;
    *)
      eval "lt_$var=\\\"\`\$echo \"X\$$var\" | \$Xsed -e \"\$sed_quote_subst\"\`\\\""
      ;;
    esac
  done

  case $lt_echo in
  *'\$0 --fallback-echo"')
    lt_echo=`$echo "X$lt_echo" | $Xsed -e 's/\\\\\\\$0 --fallback-echo"$/$0 --fallback-echo"/'`
    ;;
  esac

cfgfile="$ofile"

  cat <<__EOF__ >> "$cfgfile"
# ### BEGIN LIBTOOL TAG CONFIG: $tagname

# Libtool was configured on host `(hostname || uname -n) 2>/dev/null | sed 1q`:

# Shell to use when invoking shell scripts.
SHELL=$lt_SHELL

# Whether or not to build shared libraries.
build_libtool_libs=$enable_shared

# Whether or not to build static libraries.
build_old_libs=$enable_static

# Whether or not to add -lc for building shared libraries.
build_libtool_need_lc=$archive_cmds_need_lc_CXX

# Whether or not to disallow shared libs when runtime libs are static
allow_libtool_libs_with_static_runtimes=$enable_shared_with_static_runtimes_CXX

# Whether or not to optimize for fast installation.
fast_install=$enable_fast_install

# The host system.
host_alias=$host_alias
host=$host
host_os=$host_os

# The build system.
build_alias=$build_alias
build=$build
build_os=$build_os

# An echo program that does not interpret backslashes.
echo=$lt_echo

# The archiver.
AR=$lt_AR
AR_FLAGS=$lt_AR_FLAGS

# A C compiler.
LTCC=$lt_LTCC

# LTCC compiler flags.
LTCFLAGS=$lt_LTCFLAGS

# A language-specific compiler.
CC=$lt_compiler_CXX

# Is the compiler the GNU C compiler?
with_gcc=$GCC_CXX

# An ERE matcher.
EGREP=$lt_EGREP

# The linker used to build libraries.
LD=$lt_LD_CXX

# Whether we need hard or soft links.
LN_S=$lt_LN_S

# A BSD-compatible nm program.
NM=$lt_NM

# A symbol stripping program
STRIP=$lt_STRIP

# Used to examine libraries when file_magic_cmd begins "file"
MAGIC_CMD=$MAGIC_CMD

# Used on cygwin: DLL creation program.
DLLTOOL="$DLLTOOL"

# Used on cygwin: object dumper.
OBJDUMP="$OBJDUMP"

# Used on cygwin: assembler.
AS="$AS"

# The name of the directory that contains temporary libtool files.
objdir=$objdir

# How to create reloadable object files.
reload_flag=$lt_reload_flag
reload_cmds=$lt_reload_cmds

# How to pass a linker flag through the compiler.
wl=$lt_lt_prog_compiler_wl_CXX

# Object file suffix (normally "o").
objext="$ac_objext"

# Old archive suffix (normally "a").
libext="$libext"

# Shared library suffix (normally ".so").
shrext_cmds='$shrext_cmds'

# Executable file suffix (normally "").
exeext="$exeext"

# Additional compiler flags for building library objects.
pic_flag=$lt_lt_prog_compiler_pic_CXX
pic_mode=$pic_mode

# What is the maximum length of a command?
max_cmd_len=$lt_cv_sys_max_cmd_len

# Does compiler simultaneously support -c and -o options?
compiler_c_o=$lt_lt_cv_prog_compiler_c_o_CXX

# Must we lock files when doing compilation?
need_locks=$lt_need_locks

# Do we need the lib prefix for modules?
need_lib_prefix=$need_lib_prefix

# Do we need a version for libraries?
need_version=$need_version

# Whether dlopen is supported.
dlopen_support=$enable_dlopen

# Whether dlopen of programs is supported.
dlopen_self=$enable_dlopen_self

# Whether dlopen of statically linked programs is supported.
dlopen_self_static=$enable_dlopen_self_static

# Compiler flag to prevent dynamic linking.
link_static_flag=$lt_lt_prog_compiler_static_CXX

# Compiler flag to turn off builtin functions.
no_builtin_flag=$lt_lt_prog_compiler_no_builtin_flag_CXX

# Compiler flag to allow reflexive dlopens.
export_dynamic_flag_spec=$lt_export_dynamic_flag_spec_CXX

# Compiler flag to generate shared objects directly from archives.
whole_archive_flag_spec=$lt_whole_archive_flag_spec_CXX

# Compiler flag to generate thread-safe objects.
thread_safe_flag_spec=$lt_thread_safe_flag_spec_CXX

# Library versioning type.
version_type=$version_type

# Format of library name prefix.
libname_spec=$lt_libname_spec

# List of archive names.  First name is the real one, the rest are links.
# The last name is the one that the linker finds with -lNAME.
library_names_spec=$lt_library_names_spec

# The coded name of the library, if different from the real name.
soname_spec=$lt_soname_spec

# Commands used to build and install an old-style archive.
RANLIB=$lt_RANLIB
old_archive_cmds=$lt_old_archive_cmds_CXX
old_postinstall_cmds=$lt_old_postinstall_cmds
old_postuninstall_cmds=$lt_old_postuninstall_cmds

# Create an old-style archive from a shared archive.
old_archive_from_new_cmds=$lt_old_archive_from_new_cmds_CXX

# Create a temporary old-style archive to link instead of a shared archive.
old_archive_from_expsyms_cmds=$lt_old_archive_from_expsyms_cmds_CXX

# Commands used to build and install a shared archive.
archive_cmds=$lt_archive_cmds_CXX
archive_expsym_cmds=$lt_archive_expsym_cmds_CXX
postinstall_cmds=$lt_postinstall_cmds
postuninstall_cmds=$lt_postuninstall_cmds

# Commands used to build a loadable module (assumed same as above if empty)
module_cmds=$lt_module_cmds_CXX
module_expsym_cmds=$lt_module_expsym_cmds_CXX

# Commands to strip libraries.
old_striplib=$lt_old_striplib
striplib=$lt_striplib

# Dependencies to place before the objects being linked to create a
# shared library.
predep_objects=$lt_predep_objects_CXX

# Dependencies to place after the objects being linked to create a
# shared library.
postdep_objects=$lt_postdep_objects_CXX

# Dependencies to place before the objects being linked to create a
# shared library.
predeps=$lt_predeps_CXX

# Dependencies to place after the objects being linked to create a
# shared library.
postdeps=$lt_postdeps_CXX

# The library search path used internally by the compiler when linking
# a shared library.
compiler_lib_search_path=$lt_compiler_lib_search_path_CXX

# Method to check whether dependent libraries are shared objects.
deplibs_check_method=$lt_deplibs_check_method

# Command to use when deplibs_check_method == file_magic.
file_magic_cmd=$lt_file_magic_cmd

# Flag that allows shared libraries with undefined symbols to be built.
allow_undefined_flag=$lt_allow_undefined_flag_CXX

# Flag that forces no undefined symbols.
no_undefined_flag=$lt_no_undefined_flag_CXX

# Commands used to finish a libtool library installation in a directory.
finish_cmds=$lt_finish_cmds

# Same as above, but a single script fragment to be evaled but not shown.
finish_eval=$lt_finish_eval

# Take the output of nm and produce a listing of raw symbols and C names.
global_symbol_pipe=$lt_lt_cv_sys_global_symbol_pipe

# Transform the output of nm in a proper C declaration
global_symbol_to_cdecl=$lt_lt_cv_sys_global_symbol_to_cdecl

# Transform the output of nm in a C name address pair
global_symbol_to_c_name_address=$lt_lt_cv_sys_global_symbol_to_c_name_address

# This is the shared library runtime path variable.
runpath_var=$runpath_var

# This is the shared library path variable.
shlibpath_var=$shlibpath_var

# Is shlibpath searched before the hard-coded library search path?
shlibpath_overrides_runpath=$shlibpath_overrides_runpath

# How to hardcode a shared library path into an executable.
hardcode_action=$hardcode_action_CXX

# Whether we should hardcode library paths into libraries.
hardcode_into_libs=$hardcode_into_libs

# Flag to hardcode \$libdir into a binary during linking.
# This must work even if \$libdir does not exist.
hardcode_libdir_flag_spec=$lt_hardcode_libdir_flag_spec_CXX

# If ld is used when linking, flag to hardcode \$libdir into
# a binary during linking. This must work even if \$libdir does
# not exist.
hardcode_libdir_flag_spec_ld=$lt_hardcode_libdir_flag_spec_ld_CXX

# Whether we need a single -rpath flag with a separated argument.
hardcode_libdir_separator=$lt_hardcode_libdir_separator_CXX

# Set to yes if using DIR/libNAME${shared_ext} during linking hardcodes DIR into the
# resulting binary.
hardcode_direct=$hardcode_direct_CXX

# Set to yes if using the -LDIR flag during linking hardcodes DIR into the
# resulting binary.
hardcode_minus_L=$hardcode_minus_L_CXX

# Set to yes if using SHLIBPATH_VAR=DIR during linking hardcodes DIR into
# the resulting binary.
hardcode_shlibpath_var=$hardcode_shlibpath_var_CXX

# Set to yes if building a shared library automatically hardcodes DIR into the library
# and all subsequent libraries and executables linked against it.
hardcode_automatic=$hardcode_automatic_CXX

# Variables whose values should be saved in libtool wrapper scripts and
# restored at relink time.
variables_saved_for_relink="$variables_saved_for_relink"

# Whether libtool must link a program against all its dependency libraries.
link_all_deplibs=$link_all_deplibs_CXX

# Compile-time system search path for libraries
sys_lib_search_path_spec=$lt_sys_lib_search_path_spec

# Run-time system search path for libraries
sys_lib_dlsearch_path_spec=$lt_sys_lib_dlsearch_path_spec

# Fix the shell variable \$srcfile for the compiler.
fix_srcfile_path=$lt_fix_srcfile_path

# Set to yes if exported symbols are required.
always_export_symbols=$always_export_symbols_CXX

# The commands to list exported symbols.
export_symbols_cmds=$lt_export_symbols_cmds_CXX

# The commands to extract the exported symbol list from a shared archive.
extract_expsyms_cmds=$lt_extract_expsyms_cmds

# Symbols that should not be listed in the preloaded symbols.
exclude_expsyms=$lt_exclude_expsyms_CXX

# Symbols that must always be exported.
include_expsyms=$lt_include_expsyms_CXX

# ### END LIBTOOL TAG CONFIG: $tagname

__EOF__


else
  # If there is no Makefile yet, we rely on a make rule to execute
  # `config.status --recheck' to rerun these tests and create the
  # libtool script then.
  ltmain_in=`echo $ltmain | sed -e 's/\.sh$/.in/'`
  if test -f "$ltmain_in"; then
    test -f Makefile && make "$ltmain"
  fi
fi


ac_ext=c
ac_cpp='$CPP $CPPFLAGS'
ac_compile='$CC -c $CFLAGS $CPPFLAGS conftest.$ac_ext >&5'
ac_link='$CC -o conftest$ac_exeext $CFLAGS $CPPFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_c_compiler_gnu

CC=$lt_save_CC
LDCXX=$LD
LD=$lt_save_LD
GCC=$lt_save_GCC
with_gnu_ldcxx=$with_gnu_ld
with_gnu_ld=$lt_save_with_gnu_ld
lt_cv_path_LDCXX=$lt_cv_path_LD
lt_cv_path_LD=$lt_save_path_LD
lt_cv_prog_gnu_ldcxx=$lt_cv_prog_gnu_ld
lt_cv_prog_gnu_ld=$lt_save_with_gnu_ld

	else
	  tagname=""
	fi
	;;

      F77)
	if test -n "$F77" && test "X$F77" != "Xno"; then

ac_ext=f
ac_compile='$F77 -c $FFLAGS conftest.$ac_ext >&5'
ac_link='$F77 -o conftest$ac_exeext $FFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_f77_compiler_gnu


archive_cmds_need_lc_F77=no
allow_undefined_flag_F77=
always_export_symbols_F77=no
archive_expsym_cmds_F77=
export_dynamic_flag_spec_F77=
hardcode_direct_F77=no
hardcode_libdir_flag_spec_F77=
hardcode_libdir_flag_spec_ld_F77=
hardcode_libdir_separator_F77=
hardcode_minus_L_F77=no
hardcode_automatic_F77=no
module_cmds_F77=
module_expsym_cmds_F77=
link_all_deplibs_F77=unknown
old_archive_cmds_F77=$old_archive_cmds
no_undefined_flag_F77=
whole_archive_flag_spec_F77=
enable_shared_with_static_runtimes_F77=no

# Source file extension for f77 test sources.
ac_ext=f

# Object file extension for compiled f77 test sources.
objext=o
objext_F77=$objext

# Code to be used in simple compile tests
lt_simple_compile_test_code="\
      subroutine t
      return
      end
"

# Code to be used in simple link tests
lt_simple_link_test_code="\
      program t
      end
"

# ltmain only uses $CC for tagged configurations so make sure $CC is set.

# If no C compiler was specified, use CC.
LTCC=${LTCC-"$CC"}

# If no C compiler flags were specified, use CFLAGS.
LTCFLAGS=${LTCFLAGS-"$CFLAGS"}

# Allow CC to be a program name with arguments.
compiler=$CC


# save warnings/boilerplate of simple test code
ac_outfile=conftest.$ac_objext
echo "$lt_simple_compile_test_code" >conftest.$ac_ext
eval "$ac_compile" 2>&1 >/dev/null | $SED '/^$/d; /^ *+/d' >conftest.err
_lt_compiler_boilerplate=`cat conftest.err`
$rm conftest*

ac_outfile=conftest.$ac_objext
echo "$lt_simple_link_test_code" >conftest.$ac_ext
eval "$ac_link" 2>&1 >/dev/null | $SED '/^$/d; /^ *+/d' >conftest.err
_lt_linker_boilerplate=`cat conftest.err`
$rm conftest*


# Allow CC to be a program name with arguments.
lt_save_CC="$CC"
CC=${F77-"f77"}
compiler=$CC
compiler_F77=$CC
for cc_temp in $compiler""; do
  case $cc_temp in
    compile | *[\\/]compile | ccache | *[\\/]ccache ) ;;
    distcc | *[\\/]distcc | purify | *[\\/]purify ) ;;
    \-*) ;;
    *) break;;
  esac
done
cc_basename=`$echo "X$cc_temp" | $Xsed -e 's%.*/%%' -e "s%^$host_alias-%%"`


{ echo "$as_me:$LINENO: checking if libtool supports shared libraries" >&5
echo $ECHO_N "checking if libtool supports shared libraries... $ECHO_C" >&6; }
{ echo "$as_me:$LINENO: result: $can_build_shared" >&5
echo "${ECHO_T}$can_build_shared" >&6; }

{ echo "$as_me:$LINENO: checking whether to build shared libraries" >&5
echo $ECHO_N "checking whether to build shared libraries... $ECHO_C" >&6; }
test "$can_build_shared" = "no" && enable_shared=no

# On AIX, shared libraries and static libraries use the same namespace, and
# are all built from PIC.
case $host_os in
aix3*)
  test "$enable_shared" = yes && enable_static=no
  if test -n "$RANLIB"; then
    archive_cmds="$archive_cmds~\$RANLIB \$lib"
    postinstall_cmds='$RANLIB $lib'
  fi
  ;;
aix4* | aix5*)
  if test "$host_cpu" != ia64 && test "$aix_use_runtimelinking" = no ; then
    test "$enable_shared" = yes && enable_static=no
  fi
  ;;
esac
{ echo "$as_me:$LINENO: result: $enable_shared" >&5
echo "${ECHO_T}$enable_shared" >&6; }

{ echo "$as_me:$LINENO: checking whether to build static libraries" >&5
echo $ECHO_N "checking whether to build static libraries... $ECHO_C" >&6; }
# Make sure either enable_shared or enable_static is yes.
test "$enable_shared" = yes || enable_static=yes
{ echo "$as_me:$LINENO: result: $enable_static" >&5
echo "${ECHO_T}$enable_static" >&6; }

GCC_F77="$G77"
LD_F77="$LD"

lt_prog_compiler_wl_F77=
lt_prog_compiler_pic_F77=
lt_prog_compiler_static_F77=

{ echo "$as_me:$LINENO: checking for $compiler option to produce PIC" >&5
echo $ECHO_N "checking for $compiler option to produce PIC... $ECHO_C" >&6; }

  if test "$GCC" = yes; then
    lt_prog_compiler_wl_F77='-Wl,'
    lt_prog_compiler_static_F77='-static'

    case $host_os in
      aix*)
      # All AIX code is PIC.
      if test "$host_cpu" = ia64; then
	# AIX 5 now supports IA64 processor
	lt_prog_compiler_static_F77='-Bstatic'
      fi
      ;;

    amigaos*)
      # FIXME: we need at least 68020 code to build shared libraries, but
      # adding the `-m68020' flag to GCC prevents building anything better,
      # like `-m68040'.
      lt_prog_compiler_pic_F77='-m68020 -resident32 -malways-restore-a4'
      ;;

    beos* | irix5* | irix6* | nonstopux* | osf3* | osf4* | osf5*)
      # PIC is the default for these OSes.
      ;;

    mingw* | cygwin* | pw32* | os2*)
      # This hack is so that the source file can tell whether it is being
      # built for inclusion in a dll (and should export symbols for example).
      # Although the cygwin gcc ignores -fPIC, still need this for old-style
      # (--disable-auto-import) libraries
      lt_prog_compiler_pic_F77='-DDLL_EXPORT'
      ;;

    darwin* | rhapsody*)
      # PIC is the default on this platform
      # Common symbols not allowed in MH_DYLIB files
      lt_prog_compiler_pic_F77='-fno-common'
      ;;

    interix[3-9]*)
      # Interix 3.x gcc -fpic/-fPIC options generate broken code.
      # Instead, we relocate shared libraries at runtime.
      ;;

    msdosdjgpp*)
      # Just because we use GCC doesn't mean we suddenly get shared libraries
      # on systems that don't support them.
      lt_prog_compiler_can_build_shared_F77=no
      enable_shared=no
      ;;

    sysv4*MP*)
      if test -d /usr/nec; then
	lt_prog_compiler_pic_F77=-Kconform_pic
      fi
      ;;

    hpux*)
      # PIC is the default for IA64 HP-UX and 64-bit HP-UX, but
      # not for PA HP-UX.
      case $host_cpu in
      hppa*64*|ia64*)
	# +Z the default
	;;
      *)
	lt_prog_compiler_pic_F77='-fPIC'
	;;
      esac
      ;;

    *)
      lt_prog_compiler_pic_F77='-fPIC'
      ;;
    esac
  else
    # PORTME Check for flag to pass linker flags through the system compiler.
    case $host_os in
    aix*)
      lt_prog_compiler_wl_F77='-Wl,'
      if test "$host_cpu" = ia64; then
	# AIX 5 now supports IA64 processor
	lt_prog_compiler_static_F77='-Bstatic'
      else
	lt_prog_compiler_static_F77='-bnso -bI:/lib/syscalls.exp'
      fi
      ;;
      darwin*)
        # PIC is the default on this platform
        # Common symbols not allowed in MH_DYLIB files
       case $cc_basename in
         xlc*)
         lt_prog_compiler_pic_F77='-qnocommon'
         lt_prog_compiler_wl_F77='-Wl,'
         ;;
       esac
       ;;

    mingw* | cygwin* | pw32* | os2*)
      # This hack is so that the source file can tell whether it is being
      # built for inclusion in a dll (and should export symbols for example).
      lt_prog_compiler_pic_F77='-DDLL_EXPORT'
      ;;

    hpux9* | hpux10* | hpux11*)
      lt_prog_compiler_wl_F77='-Wl,'
      # PIC is the default for IA64 HP-UX and 64-bit HP-UX, but
      # not for PA HP-UX.
      case $host_cpu in
      hppa*64*|ia64*)
	# +Z the default
	;;
      *)
	lt_prog_compiler_pic_F77='+Z'
	;;
      esac
      # Is there a better lt_prog_compiler_static that works with the bundled CC?
      lt_prog_compiler_static_F77='${wl}-a ${wl}archive'
      ;;

    irix5* | irix6* | nonstopux*)
      lt_prog_compiler_wl_F77='-Wl,'
      # PIC (with -KPIC) is the default.
      lt_prog_compiler_static_F77='-non_shared'
      ;;

    newsos6)
      lt_prog_compiler_pic_F77='-KPIC'
      lt_prog_compiler_static_F77='-Bstatic'
      ;;

    linux* | k*bsd*-gnu)
      case $cc_basename in
      icc* | ecc*)
	lt_prog_compiler_wl_F77='-Wl,'
	lt_prog_compiler_pic_F77='-KPIC'
	lt_prog_compiler_static_F77='-static'
        ;;
      pgcc* | pgf77* | pgf90* | pgf95*)
        # Portland Group compilers (*not* the Pentium gcc compiler,
	# which looks to be a dead project)
	lt_prog_compiler_wl_F77='-Wl,'
	lt_prog_compiler_pic_F77='-fpic'
	lt_prog_compiler_static_F77='-Bstatic'
        ;;
      ccc*)
        lt_prog_compiler_wl_F77='-Wl,'
        # All Alpha code is PIC.
        lt_prog_compiler_static_F77='-non_shared'
        ;;
      *)
        case `$CC -V 2>&1 | sed 5q` in
	*Sun\ C*)
	  # Sun C 5.9
	  lt_prog_compiler_pic_F77='-KPIC'
	  lt_prog_compiler_static_F77='-Bstatic'
	  lt_prog_compiler_wl_F77='-Wl,'
	  ;;
	*Sun\ F*)
	  # Sun Fortran 8.3 passes all unrecognized flags to the linker
	  lt_prog_compiler_pic_F77='-KPIC'
	  lt_prog_compiler_static_F77='-Bstatic'
	  lt_prog_compiler_wl_F77=''
	  ;;
	esac
	;;
      esac
      ;;

    osf3* | osf4* | osf5*)
      lt_prog_compiler_wl_F77='-Wl,'
      # All OSF/1 code is PIC.
      lt_prog_compiler_static_F77='-non_shared'
      ;;

    rdos*)
      lt_prog_compiler_static_F77='-non_shared'
      ;;

    solaris*)
      lt_prog_compiler_pic_F77='-KPIC'
      lt_prog_compiler_static_F77='-Bstatic'
      case $cc_basename in
      f77* | f90* | f95*)
	lt_prog_compiler_wl_F77='-Qoption ld ';;
      *)
	lt_prog_compiler_wl_F77='-Wl,';;
      esac
      ;;

    sunos4*)
      lt_prog_compiler_wl_F77='-Qoption ld '
      lt_prog_compiler_pic_F77='-PIC'
      lt_prog_compiler_static_F77='-Bstatic'
      ;;

    sysv4 | sysv4.2uw2* | sysv4.3*)
      lt_prog_compiler_wl_F77='-Wl,'
      lt_prog_compiler_pic_F77='-KPIC'
      lt_prog_compiler_static_F77='-Bstatic'
      ;;

    sysv4*MP*)
      if test -d /usr/nec ;then
	lt_prog_compiler_pic_F77='-Kconform_pic'
	lt_prog_compiler_static_F77='-Bstatic'
      fi
      ;;

    sysv5* | unixware* | sco3.2v5* | sco5v6* | OpenUNIX*)
      lt_prog_compiler_wl_F77='-Wl,'
      lt_prog_compiler_pic_F77='-KPIC'
      lt_prog_compiler_static_F77='-Bstatic'
      ;;

    unicos*)
      lt_prog_compiler_wl_F77='-Wl,'
      lt_prog_compiler_can_build_shared_F77=no
      ;;

    uts4*)
      lt_prog_compiler_pic_F77='-pic'
      lt_prog_compiler_static_F77='-Bstatic'
      ;;

    *)
      lt_prog_compiler_can_build_shared_F77=no
      ;;
    esac
  fi

{ echo "$as_me:$LINENO: result: $lt_prog_compiler_pic_F77" >&5
echo "${ECHO_T}$lt_prog_compiler_pic_F77" >&6; }

#
# Check to make sure the PIC flag actually works.
#
if test -n "$lt_prog_compiler_pic_F77"; then

{ echo "$as_me:$LINENO: checking if $compiler PIC flag $lt_prog_compiler_pic_F77 works" >&5
echo $ECHO_N "checking if $compiler PIC flag $lt_prog_compiler_pic_F77 works... $ECHO_C" >&6; }
if test "${lt_prog_compiler_pic_works_F77+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  lt_prog_compiler_pic_works_F77=no
  ac_outfile=conftest.$ac_objext
   echo "$lt_simple_compile_test_code" > conftest.$ac_ext
   lt_compiler_flag="$lt_prog_compiler_pic_F77"
   # Insert the option either (1) after the last *FLAGS variable, or
   # (2) before a word containing "conftest.", or (3) at the end.
   # Note that $ac_compile itself does not contain backslashes and begins
   # with a dollar sign (not a hyphen), so the echo should work correctly.
   # The option is referenced via a variable to avoid confusing sed.
   lt_compile=`echo "$ac_compile" | $SED \
   -e 's:.*FLAGS}\{0,1\} :&$lt_compiler_flag :; t' \
   -e 's: [^ ]*conftest\.: $lt_compiler_flag&:; t' \
   -e 's:$: $lt_compiler_flag:'`
   (eval echo "\"\$as_me:13992: $lt_compile\"" >&5)
   (eval "$lt_compile" 2>conftest.err)
   ac_status=$?
   cat conftest.err >&5
   echo "$as_me:13996: \$? = $ac_status" >&5
   if (exit $ac_status) && test -s "$ac_outfile"; then
     # The compiler can only warn and ignore the option if not recognized
     # So say no if there are warnings other than the usual output.
     $echo "X$_lt_compiler_boilerplate" | $Xsed -e '/^$/d' >conftest.exp
     $SED '/^$/d; /^ *+/d' conftest.err >conftest.er2
     if test ! -s conftest.er2 || diff conftest.exp conftest.er2 >/dev/null; then
       lt_prog_compiler_pic_works_F77=yes
     fi
   fi
   $rm conftest*

fi
{ echo "$as_me:$LINENO: result: $lt_prog_compiler_pic_works_F77" >&5
echo "${ECHO_T}$lt_prog_compiler_pic_works_F77" >&6; }

if test x"$lt_prog_compiler_pic_works_F77" = xyes; then
    case $lt_prog_compiler_pic_F77 in
     "" | " "*) ;;
     *) lt_prog_compiler_pic_F77=" $lt_prog_compiler_pic_F77" ;;
     esac
else
    lt_prog_compiler_pic_F77=
     lt_prog_compiler_can_build_shared_F77=no
fi

fi
case $host_os in
  # For platforms which do not support PIC, -DPIC is meaningless:
  *djgpp*)
    lt_prog_compiler_pic_F77=
    ;;
  *)
    lt_prog_compiler_pic_F77="$lt_prog_compiler_pic_F77"
    ;;
esac

#
# Check to make sure the static flag actually works.
#
wl=$lt_prog_compiler_wl_F77 eval lt_tmp_static_flag=\"$lt_prog_compiler_static_F77\"
{ echo "$as_me:$LINENO: checking if $compiler static flag $lt_tmp_static_flag works" >&5
echo $ECHO_N "checking if $compiler static flag $lt_tmp_static_flag works... $ECHO_C" >&6; }
if test "${lt_prog_compiler_static_works_F77+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  lt_prog_compiler_static_works_F77=no
   save_LDFLAGS="$LDFLAGS"
   LDFLAGS="$LDFLAGS $lt_tmp_static_flag"
   echo "$lt_simple_link_test_code" > conftest.$ac_ext
   if (eval $ac_link 2>conftest.err) && test -s conftest$ac_exeext; then
     # The linker can only warn and ignore the option if not recognized
     # So say no if there are warnings
     if test -s conftest.err; then
       # Append any errors to the config.log.
       cat conftest.err 1>&5
       $echo "X$_lt_linker_boilerplate" | $Xsed -e '/^$/d' > conftest.exp
       $SED '/^$/d; /^ *+/d' conftest.err >conftest.er2
       if diff conftest.exp conftest.er2 >/dev/null; then
         lt_prog_compiler_static_works_F77=yes
       fi
     else
       lt_prog_compiler_static_works_F77=yes
     fi
   fi
   $rm conftest*
   LDFLAGS="$save_LDFLAGS"

fi
{ echo "$as_me:$LINENO: result: $lt_prog_compiler_static_works_F77" >&5
echo "${ECHO_T}$lt_prog_compiler_static_works_F77" >&6; }

if test x"$lt_prog_compiler_static_works_F77" = xyes; then
    :
else
    lt_prog_compiler_static_F77=
fi


{ echo "$as_me:$LINENO: checking if $compiler supports -c -o file.$ac_objext" >&5
echo $ECHO_N "checking if $compiler supports -c -o file.$ac_objext... $ECHO_C" >&6; }
if test "${lt_cv_prog_compiler_c_o_F77+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  lt_cv_prog_compiler_c_o_F77=no
   $rm -r conftest 2>/dev/null
   mkdir conftest
   cd conftest
   mkdir out
   echo "$lt_simple_compile_test_code" > conftest.$ac_ext

   lt_compiler_flag="-o out/conftest2.$ac_objext"
   # Insert the option either (1) after the last *FLAGS variable, or
   # (2) before a word containing "conftest.", or (3) at the end.
   # Note that $ac_compile itself does not contain backslashes and begins
   # with a dollar sign (not a hyphen), so the echo should work correctly.
   lt_compile=`echo "$ac_compile" | $SED \
   -e 's:.*FLAGS}\{0,1\} :&$lt_compiler_flag :; t' \
   -e 's: [^ ]*conftest\.: $lt_compiler_flag&:; t' \
   -e 's:$: $lt_compiler_flag:'`
   (eval echo "\"\$as_me:14096: $lt_compile\"" >&5)
   (eval "$lt_compile" 2>out/conftest.err)
   ac_status=$?
   cat out/conftest.err >&5
   echo "$as_me:14100: \$? = $ac_status" >&5
   if (exit $ac_status) && test -s out/conftest2.$ac_objext
   then
     # The compiler can only warn and ignore the option if not recognized
     # So say no if there are warnings
     $echo "X$_lt_compiler_boilerplate" | $Xsed -e '/^$/d' > out/conftest.exp
     $SED '/^$/d; /^ *+/d' out/conftest.err >out/conftest.er2
     if test ! -s out/conftest.er2 || diff out/conftest.exp out/conftest.er2 >/dev/null; then
       lt_cv_prog_compiler_c_o_F77=yes
     fi
   fi
   chmod u+w . 2>&5
   $rm conftest*
   # SGI C++ compiler will create directory out/ii_files/ for
   # template instantiation
   test -d out/ii_files && $rm out/ii_files/* && rmdir out/ii_files
   $rm out/* && rmdir out
   cd ..
   rmdir conftest
   $rm conftest*

fi
{ echo "$as_me:$LINENO: result: $lt_cv_prog_compiler_c_o_F77" >&5
echo "${ECHO_T}$lt_cv_prog_compiler_c_o_F77" >&6; }


hard_links="nottested"
if test "$lt_cv_prog_compiler_c_o_F77" = no && test "$need_locks" != no; then
  # do not overwrite the value of need_locks provided by the user
  { echo "$as_me:$LINENO: checking if we can lock with hard links" >&5
echo $ECHO_N "checking if we can lock with hard links... $ECHO_C" >&6; }
  hard_links=yes
  $rm conftest*
  ln conftest.a conftest.b 2>/dev/null && hard_links=no
  touch conftest.a
  ln conftest.a conftest.b 2>&5 || hard_links=no
  ln conftest.a conftest.b 2>/dev/null && hard_links=no
  { echo "$as_me:$LINENO: result: $hard_links" >&5
echo "${ECHO_T}$hard_links" >&6; }
  if test "$hard_links" = no; then
    { echo "$as_me:$LINENO: WARNING: \`$CC' does not support \`-c -o', so \`make -j' may be unsafe" >&5
echo "$as_me: WARNING: \`$CC' does not support \`-c -o', so \`make -j' may be unsafe" >&2;}
    need_locks=warn
  fi
else
  need_locks=no
fi

{ echo "$as_me:$LINENO: checking whether the $compiler linker ($LD) supports shared libraries" >&5
echo $ECHO_N "checking whether the $compiler linker ($LD) supports shared libraries... $ECHO_C" >&6; }

  runpath_var=
  allow_undefined_flag_F77=
  enable_shared_with_static_runtimes_F77=no
  archive_cmds_F77=
  archive_expsym_cmds_F77=
  old_archive_From_new_cmds_F77=
  old_archive_from_expsyms_cmds_F77=
  export_dynamic_flag_spec_F77=
  whole_archive_flag_spec_F77=
  thread_safe_flag_spec_F77=
  hardcode_libdir_flag_spec_F77=
  hardcode_libdir_flag_spec_ld_F77=
  hardcode_libdir_separator_F77=
  hardcode_direct_F77=no
  hardcode_minus_L_F77=no
  hardcode_shlibpath_var_F77=unsupported
  link_all_deplibs_F77=unknown
  hardcode_automatic_F77=no
  module_cmds_F77=
  module_expsym_cmds_F77=
  always_export_symbols_F77=no
  export_symbols_cmds_F77='$NM $libobjs $convenience | $global_symbol_pipe | $SED '\''s/.* //'\'' | sort | uniq > $export_symbols'
  # include_expsyms should be a list of space-separated symbols to be *always*
  # included in the symbol list
  include_expsyms_F77=
  # exclude_expsyms can be an extended regexp of symbols to exclude
  # it will be wrapped by ` (' and `)$', so one must not match beginning or
  # end of line.  Example: `a|bc|.*d.*' will exclude the symbols `a' and `bc',
  # as well as any symbol that contains `d'.
  exclude_expsyms_F77="_GLOBAL_OFFSET_TABLE_"
  # Although _GLOBAL_OFFSET_TABLE_ is a valid symbol C name, most a.out
  # platforms (ab)use it in PIC code, but their linkers get confused if
  # the symbol is explicitly referenced.  Since portable code cannot
  # rely on this symbol name, it's probably fine to never include it in
  # preloaded symbol tables.
  extract_expsyms_cmds=
  # Just being paranoid about ensuring that cc_basename is set.
  for cc_temp in $compiler""; do
  case $cc_temp in
    compile | *[\\/]compile | ccache | *[\\/]ccache ) ;;
    distcc | *[\\/]distcc | purify | *[\\/]purify ) ;;
    \-*) ;;
    *) break;;
  esac
done
cc_basename=`$echo "X$cc_temp" | $Xsed -e 's%.*/%%' -e "s%^$host_alias-%%"`

  case $host_os in
  cygwin* | mingw* | pw32*)
    # FIXME: the MSVC++ port hasn't been tested in a loooong time
    # When not using gcc, we currently assume that we are using
    # Microsoft Visual C++.
    if test "$GCC" != yes; then
      with_gnu_ld=no
    fi
    ;;
  interix*)
    # we just hope/assume this is gcc and not c89 (= MSVC++)
    with_gnu_ld=yes
    ;;
  openbsd*)
    with_gnu_ld=no
    ;;
  esac

  ld_shlibs_F77=yes
  if test "$with_gnu_ld" = yes; then
    # If archive_cmds runs LD, not CC, wlarc should be empty
    wlarc='${wl}'

    # Set some defaults for GNU ld with shared library support. These
    # are reset later if shared libraries are not supported. Putting them
    # here allows them to be overridden if necessary.
    runpath_var=LD_RUN_PATH
    hardcode_libdir_flag_spec_F77='${wl}--rpath ${wl}$libdir'
    export_dynamic_flag_spec_F77='${wl}--export-dynamic'
    # ancient GNU ld didn't support --whole-archive et. al.
    if $LD --help 2>&1 | grep 'no-whole-archive' > /dev/null; then
	whole_archive_flag_spec_F77="$wlarc"'--whole-archive$convenience '"$wlarc"'--no-whole-archive'
      else
  	whole_archive_flag_spec_F77=
    fi
    supports_anon_versioning=no
    case `$LD -v 2>/dev/null` in
      *\ [01].* | *\ 2.[0-9].* | *\ 2.10.*) ;; # catch versions < 2.11
      *\ 2.11.93.0.2\ *) supports_anon_versioning=yes ;; # RH7.3 ...
      *\ 2.11.92.0.12\ *) supports_anon_versioning=yes ;; # Mandrake 8.2 ...
      *\ 2.11.*) ;; # other 2.11 versions
      *) supports_anon_versioning=yes ;;
    esac

    # See if GNU ld supports shared libraries.
    case $host_os in
    aix3* | aix4* | aix5*)
      # On AIX/PPC, the GNU linker is very broken
      if test "$host_cpu" != ia64; then
	ld_shlibs_F77=no
	cat <<EOF 1>&2

*** Warning: the GNU linker, at least up to release 2.9.1, is reported
*** to be unable to reliably create shared libraries on AIX.
*** Therefore, libtool is disabling shared libraries support.  If you
*** really care for shared libraries, you may want to modify your PATH
*** so that a non-GNU linker is found, and then restart.

EOF
      fi
      ;;

    amigaos*)
      archive_cmds_F77='$rm $output_objdir/a2ixlibrary.data~$echo "#define NAME $libname" > $output_objdir/a2ixlibrary.data~$echo "#define LIBRARY_ID 1" >> $output_objdir/a2ixlibrary.data~$echo "#define VERSION $major" >> $output_objdir/a2ixlibrary.data~$echo "#define REVISION $revision" >> $output_objdir/a2ixlibrary.data~$AR $AR_FLAGS $lib $libobjs~$RANLIB $lib~(cd $output_objdir && a2ixlibrary -32)'
      hardcode_libdir_flag_spec_F77='-L$libdir'
      hardcode_minus_L_F77=yes

      # Samuel A. Falvo II <kc5tja@dolphin.openprojects.net> reports
      # that the semantics of dynamic libraries on AmigaOS, at least up
      # to version 4, is to share data among multiple programs linked
      # with the same dynamic library.  Since this doesn't match the
      # behavior of shared libraries on other platforms, we can't use
      # them.
      ld_shlibs_F77=no
      ;;

    beos*)
      if $LD --help 2>&1 | grep ': supported targets:.* elf' > /dev/null; then
	allow_undefined_flag_F77=unsupported
	# Joseph Beckenbach <jrb3@best.com> says some releases of gcc
	# support --undefined.  This deserves some investigation.  FIXME
	archive_cmds_F77='$CC -nostart $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname -o $lib'
      else
	ld_shlibs_F77=no
      fi
      ;;

    cygwin* | mingw* | pw32*)
      # _LT_AC_TAGVAR(hardcode_libdir_flag_spec, F77) is actually meaningless,
      # as there is no search path for DLLs.
      hardcode_libdir_flag_spec_F77='-L$libdir'
      allow_undefined_flag_F77=unsupported
      always_export_symbols_F77=no
      enable_shared_with_static_runtimes_F77=yes
      export_symbols_cmds_F77='$NM $libobjs $convenience | $global_symbol_pipe | $SED -e '\''/^[BCDGRS][ ]/s/.*[ ]\([^ ]*\)/\1 DATA/'\'' -e '\''/^[AITW][ ]/s/.*[ ]//'\'' | sort | uniq > $export_symbols'

      if $LD --help 2>&1 | grep 'auto-import' > /dev/null; then
        archive_cmds_F77='$CC -shared $libobjs $deplibs $compiler_flags -o $output_objdir/$soname ${wl}--enable-auto-image-base -Xlinker --out-implib -Xlinker $lib'
	# If the export-symbols file already is a .def file (1st line
	# is EXPORTS), use it as is; otherwise, prepend...
	archive_expsym_cmds_F77='if test "x`$SED 1q $export_symbols`" = xEXPORTS; then
	  cp $export_symbols $output_objdir/$soname.def;
	else
	  echo EXPORTS > $output_objdir/$soname.def;
	  cat $export_symbols >> $output_objdir/$soname.def;
	fi~
	$CC -shared $output_objdir/$soname.def $libobjs $deplibs $compiler_flags -o $output_objdir/$soname ${wl}--enable-auto-image-base -Xlinker --out-implib -Xlinker $lib'
      else
	ld_shlibs_F77=no
      fi
      ;;

    interix[3-9]*)
      hardcode_direct_F77=no
      hardcode_shlibpath_var_F77=no
      hardcode_libdir_flag_spec_F77='${wl}-rpath,$libdir'
      export_dynamic_flag_spec_F77='${wl}-E'
      # Hack: On Interix 3.x, we cannot compile PIC because of a broken gcc.
      # Instead, shared libraries are loaded at an image base (0x10000000 by
      # default) and relocated if they conflict, which is a slow very memory
      # consuming and fragmenting process.  To avoid this, we pick a random,
      # 256 KiB-aligned image base between 0x50000000 and 0x6FFC0000 at link
      # time.  Moving up from 0x10000000 also allows more sbrk(2) space.
      archive_cmds_F77='$CC -shared $pic_flag $libobjs $deplibs $compiler_flags ${wl}-h,$soname ${wl}--image-base,`expr ${RANDOM-$$} % 4096 / 2 \* 262144 + 1342177280` -o $lib'
      archive_expsym_cmds_F77='sed "s,^,_," $export_symbols >$output_objdir/$soname.expsym~$CC -shared $pic_flag $libobjs $deplibs $compiler_flags ${wl}-h,$soname ${wl}--retain-symbols-file,$output_objdir/$soname.expsym ${wl}--image-base,`expr ${RANDOM-$$} % 4096 / 2 \* 262144 + 1342177280` -o $lib'
      ;;

    gnu* | linux* | k*bsd*-gnu)
      if $LD --help 2>&1 | grep ': supported targets:.* elf' > /dev/null; then
	tmp_addflag=
	case $cc_basename,$host_cpu in
	pgcc*)				# Portland Group C compiler
	  whole_archive_flag_spec_F77='${wl}--whole-archive`for conv in $convenience\"\"; do test  -n \"$conv\" && new_convenience=\"$new_convenience,$conv\"; done; $echo \"$new_convenience\"` ${wl}--no-whole-archive'
	  tmp_addflag=' $pic_flag'
	  ;;
	pgf77* | pgf90* | pgf95*)	# Portland Group f77 and f90 compilers
	  whole_archive_flag_spec_F77='${wl}--whole-archive`for conv in $convenience\"\"; do test  -n \"$conv\" && new_convenience=\"$new_convenience,$conv\"; done; $echo \"$new_convenience\"` ${wl}--no-whole-archive'
	  tmp_addflag=' $pic_flag -Mnomain' ;;
	ecc*,ia64* | icc*,ia64*)		# Intel C compiler on ia64
	  tmp_addflag=' -i_dynamic' ;;
	efc*,ia64* | ifort*,ia64*)	# Intel Fortran compiler on ia64
	  tmp_addflag=' -i_dynamic -nofor_main' ;;
	ifc* | ifort*)			# Intel Fortran compiler
	  tmp_addflag=' -nofor_main' ;;
	esac
	case `$CC -V 2>&1 | sed 5q` in
	*Sun\ C*)			# Sun C 5.9
	  whole_archive_flag_spec_F77='${wl}--whole-archive`new_convenience=; for conv in $convenience\"\"; do test -z \"$conv\" || new_convenience=\"$new_convenience,$conv\"; done; $echo \"$new_convenience\"` ${wl}--no-whole-archive'
	  tmp_sharedflag='-G' ;;
	*Sun\ F*)			# Sun Fortran 8.3
	  tmp_sharedflag='-G' ;;
	*)
	  tmp_sharedflag='-shared' ;;
	esac
	archive_cmds_F77='$CC '"$tmp_sharedflag""$tmp_addflag"' $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname -o $lib'

	if test $supports_anon_versioning = yes; then
	  archive_expsym_cmds_F77='$echo "{ global:" > $output_objdir/$libname.ver~
  cat $export_symbols | sed -e "s/\(.*\)/\1;/" >> $output_objdir/$libname.ver~
  $echo "local: *; };" >> $output_objdir/$libname.ver~
	  $CC '"$tmp_sharedflag""$tmp_addflag"' $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname ${wl}-version-script ${wl}$output_objdir/$libname.ver -o $lib'
	fi
      else
	ld_shlibs_F77=no
      fi
      ;;

    netbsd*)
      if echo __ELF__ | $CC -E - | grep __ELF__ >/dev/null; then
	archive_cmds_F77='$LD -Bshareable $libobjs $deplibs $linker_flags -o $lib'
	wlarc=
      else
	archive_cmds_F77='$CC -shared $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname -o $lib'
	archive_expsym_cmds_F77='$CC -shared $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname ${wl}-retain-symbols-file $wl$export_symbols -o $lib'
      fi
      ;;

    solaris*)
      if $LD -v 2>&1 | grep 'BFD 2\.8' > /dev/null; then
	ld_shlibs_F77=no
	cat <<EOF 1>&2

*** Warning: The releases 2.8.* of the GNU linker cannot reliably
*** create shared libraries on Solaris systems.  Therefore, libtool
*** is disabling shared libraries support.  We urge you to upgrade GNU
*** binutils to release 2.9.1 or newer.  Another option is to modify
*** your PATH or compiler configuration so that the native linker is
*** used, and then restart.

EOF
      elif $LD --help 2>&1 | grep ': supported targets:.* elf' > /dev/null; then
	archive_cmds_F77='$CC -shared $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname -o $lib'
	archive_expsym_cmds_F77='$CC -shared $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname ${wl}-retain-symbols-file $wl$export_symbols -o $lib'
      else
	ld_shlibs_F77=no
      fi
      ;;

    sysv5* | sco3.2v5* | sco5v6* | unixware* | OpenUNIX*)
      case `$LD -v 2>&1` in
        *\ [01].* | *\ 2.[0-9].* | *\ 2.1[0-5].*)
	ld_shlibs_F77=no
	cat <<_LT_EOF 1>&2

*** Warning: Releases of the GNU linker prior to 2.16.91.0.3 can not
*** reliably create shared libraries on SCO systems.  Therefore, libtool
*** is disabling shared libraries support.  We urge you to upgrade GNU
*** binutils to release 2.16.91.0.3 or newer.  Another option is to modify
*** your PATH or compiler configuration so that the native linker is
*** used, and then restart.

_LT_EOF
	;;
	*)
	  if $LD --help 2>&1 | grep ': supported targets:.* elf' > /dev/null; then
	    hardcode_libdir_flag_spec_F77='`test -z "$SCOABSPATH" && echo ${wl}-rpath,$libdir`'
	    archive_cmds_F77='$CC -shared $libobjs $deplibs $compiler_flags ${wl}-soname,\${SCOABSPATH:+${install_libdir}/}$soname -o $lib'
	    archive_expsym_cmds_F77='$CC -shared $libobjs $deplibs $compiler_flags ${wl}-soname,\${SCOABSPATH:+${install_libdir}/}$soname,-retain-symbols-file,$export_symbols -o $lib'
	  else
	    ld_shlibs_F77=no
	  fi
	;;
      esac
      ;;

    sunos4*)
      archive_cmds_F77='$LD -assert pure-text -Bshareable -o $lib $libobjs $deplibs $linker_flags'
      wlarc=
      hardcode_direct_F77=yes
      hardcode_shlibpath_var_F77=no
      ;;

    *)
      if $LD --help 2>&1 | grep ': supported targets:.* elf' > /dev/null; then
	archive_cmds_F77='$CC -shared $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname -o $lib'
	archive_expsym_cmds_F77='$CC -shared $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname ${wl}-retain-symbols-file $wl$export_symbols -o $lib'
      else
	ld_shlibs_F77=no
      fi
      ;;
    esac

    if test "$ld_shlibs_F77" = no; then
      runpath_var=
      hardcode_libdir_flag_spec_F77=
      export_dynamic_flag_spec_F77=
      whole_archive_flag_spec_F77=
    fi
  else
    # PORTME fill in a description of your system's linker (not GNU ld)
    case $host_os in
    aix3*)
      allow_undefined_flag_F77=unsupported
      always_export_symbols_F77=yes
      archive_expsym_cmds_F77='$LD -o $output_objdir/$soname $libobjs $deplibs $linker_flags -bE:$export_symbols -T512 -H512 -bM:SRE~$AR $AR_FLAGS $lib $output_objdir/$soname'
      # Note: this linker hardcodes the directories in LIBPATH if there
      # are no directories specified by -L.
      hardcode_minus_L_F77=yes
      if test "$GCC" = yes && test -z "$lt_prog_compiler_static"; then
	# Neither direct hardcoding nor static linking is supported with a
	# broken collect2.
	hardcode_direct_F77=unsupported
      fi
      ;;

    aix4* | aix5*)
      if test "$host_cpu" = ia64; then
	# On IA64, the linker does run time linking by default, so we don't
	# have to do anything special.
	aix_use_runtimelinking=no
	exp_sym_flag='-Bexport'
	no_entry_flag=""
      else
	# If we're using GNU nm, then we don't want the "-C" option.
	# -C means demangle to AIX nm, but means don't demangle with GNU nm
	if $NM -V 2>&1 | grep 'GNU' > /dev/null; then
	  export_symbols_cmds_F77='$NM -Bpg $libobjs $convenience | awk '\''{ if (((\$2 == "T") || (\$2 == "D") || (\$2 == "B")) && (substr(\$3,1,1) != ".")) { print \$3 } }'\'' | sort -u > $export_symbols'
	else
	  export_symbols_cmds_F77='$NM -BCpg $libobjs $convenience | awk '\''{ if (((\$2 == "T") || (\$2 == "D") || (\$2 == "B")) && (substr(\$3,1,1) != ".")) { print \$3 } }'\'' | sort -u > $export_symbols'
	fi
	aix_use_runtimelinking=no

	# Test if we are trying to use run time linking or normal
	# AIX style linking. If -brtl is somewhere in LDFLAGS, we
	# need to do runtime linking.
	case $host_os in aix4.[23]|aix4.[23].*|aix5*)
	  for ld_flag in $LDFLAGS; do
  	  if (test $ld_flag = "-brtl" || test $ld_flag = "-Wl,-brtl"); then
  	    aix_use_runtimelinking=yes
  	    break
  	  fi
	  done
	  ;;
	esac

	exp_sym_flag='-bexport'
	no_entry_flag='-bnoentry'
      fi

      # When large executables or shared objects are built, AIX ld can
      # have problems creating the table of contents.  If linking a library
      # or program results in "error TOC overflow" add -mminimal-toc to
      # CXXFLAGS/CFLAGS for g++/gcc.  In the cases where that is not
      # enough to fix the problem, add -Wl,-bbigtoc to LDFLAGS.

      archive_cmds_F77=''
      hardcode_direct_F77=yes
      hardcode_libdir_separator_F77=':'
      link_all_deplibs_F77=yes

      if test "$GCC" = yes; then
	case $host_os in aix4.[012]|aix4.[012].*)
	# We only want to do this on AIX 4.2 and lower, the check
	# below for broken collect2 doesn't work under 4.3+
	  collect2name=`${CC} -print-prog-name=collect2`
	  if test -f "$collect2name" && \
  	   strings "$collect2name" | grep resolve_lib_name >/dev/null
	  then
  	  # We have reworked collect2
  	  :
	  else
  	  # We have old collect2
  	  hardcode_direct_F77=unsupported
  	  # It fails to find uninstalled libraries when the uninstalled
  	  # path is not listed in the libpath.  Setting hardcode_minus_L
  	  # to unsupported forces relinking
  	  hardcode_minus_L_F77=yes
  	  hardcode_libdir_flag_spec_F77='-L$libdir'
  	  hardcode_libdir_separator_F77=
	  fi
	  ;;
	esac
	shared_flag='-shared'
	if test "$aix_use_runtimelinking" = yes; then
	  shared_flag="$shared_flag "'${wl}-G'
	fi
      else
	# not using gcc
	if test "$host_cpu" = ia64; then
  	# VisualAge C++, Version 5.5 for AIX 5L for IA-64, Beta 3 Release
  	# chokes on -Wl,-G. The following line is correct:
	  shared_flag='-G'
	else
	  if test "$aix_use_runtimelinking" = yes; then
	    shared_flag='${wl}-G'
	  else
	    shared_flag='${wl}-bM:SRE'
	  fi
	fi
      fi

      # It seems that -bexpall does not export symbols beginning with
      # underscore (_), so it is better to generate a list of symbols to export.
      always_export_symbols_F77=yes
      if test "$aix_use_runtimelinking" = yes; then
	# Warning - without using the other runtime loading flags (-brtl),
	# -berok will link without error, but may produce a broken library.
	allow_undefined_flag_F77='-berok'
       # Determine the default libpath from the value encoded in an empty executable.
       cat >conftest.$ac_ext <<_ACEOF
      program main

      end
_ACEOF
rm -f conftest.$ac_objext conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_f77_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest$ac_exeext &&
       $as_test_x conftest$ac_exeext; then

lt_aix_libpath_sed='
    /Import File Strings/,/^$/ {
	/^0/ {
	    s/^0  *\(.*\)$/\1/
	    p
	}
    }'
aix_libpath=`dump -H conftest$ac_exeext 2>/dev/null | $SED -n -e "$lt_aix_libpath_sed"`
# Check for a 64-bit object if we didn't find anything.
if test -z "$aix_libpath"; then
  aix_libpath=`dump -HX64 conftest$ac_exeext 2>/dev/null | $SED -n -e "$lt_aix_libpath_sed"`
fi
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5


fi

rm -f core conftest.err conftest.$ac_objext conftest_ipa8_conftest.oo \
      conftest$ac_exeext conftest.$ac_ext
if test -z "$aix_libpath"; then aix_libpath="/usr/lib:/lib"; fi

       hardcode_libdir_flag_spec_F77='${wl}-blibpath:$libdir:'"$aix_libpath"
	archive_expsym_cmds_F77="\$CC"' -o $output_objdir/$soname $libobjs $deplibs '"\${wl}$no_entry_flag"' $compiler_flags `if test "x${allow_undefined_flag}" != "x"; then echo "${wl}${allow_undefined_flag}"; else :; fi` '"\${wl}$exp_sym_flag:\$export_symbols $shared_flag"
       else
	if test "$host_cpu" = ia64; then
	  hardcode_libdir_flag_spec_F77='${wl}-R $libdir:/usr/lib:/lib'
	  allow_undefined_flag_F77="-z nodefs"
	  archive_expsym_cmds_F77="\$CC $shared_flag"' -o $output_objdir/$soname $libobjs $deplibs '"\${wl}$no_entry_flag"' $compiler_flags ${wl}${allow_undefined_flag} '"\${wl}$exp_sym_flag:\$export_symbols"
	else
	 # Determine the default libpath from the value encoded in an empty executable.
	 cat >conftest.$ac_ext <<_ACEOF
      program main

      end
_ACEOF
rm -f conftest.$ac_objext conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_f77_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest$ac_exeext &&
       $as_test_x conftest$ac_exeext; then

lt_aix_libpath_sed='
    /Import File Strings/,/^$/ {
	/^0/ {
	    s/^0  *\(.*\)$/\1/
	    p
	}
    }'
aix_libpath=`dump -H conftest$ac_exeext 2>/dev/null | $SED -n -e "$lt_aix_libpath_sed"`
# Check for a 64-bit object if we didn't find anything.
if test -z "$aix_libpath"; then
  aix_libpath=`dump -HX64 conftest$ac_exeext 2>/dev/null | $SED -n -e "$lt_aix_libpath_sed"`
fi
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5


fi

rm -f core conftest.err conftest.$ac_objext conftest_ipa8_conftest.oo \
      conftest$ac_exeext conftest.$ac_ext
if test -z "$aix_libpath"; then aix_libpath="/usr/lib:/lib"; fi

	 hardcode_libdir_flag_spec_F77='${wl}-blibpath:$libdir:'"$aix_libpath"
	  # Warning - without using the other run time loading flags,
	  # -berok will link without error, but may produce a broken library.
	  no_undefined_flag_F77=' ${wl}-bernotok'
	  allow_undefined_flag_F77=' ${wl}-berok'
	  # Exported symbols can be pulled into shared objects from archives
	  whole_archive_flag_spec_F77='$convenience'
	  archive_cmds_need_lc_F77=yes
	  # This is similar to how AIX traditionally builds its shared libraries.
	  archive_expsym_cmds_F77="\$CC $shared_flag"' -o $output_objdir/$soname $libobjs $deplibs ${wl}-bnoentry $compiler_flags ${wl}-bE:$export_symbols${allow_undefined_flag}~$AR $AR_FLAGS $output_objdir/$libname$release.a $output_objdir/$soname'
	fi
      fi
      ;;

    amigaos*)
      archive_cmds_F77='$rm $output_objdir/a2ixlibrary.data~$echo "#define NAME $libname" > $output_objdir/a2ixlibrary.data~$echo "#define LIBRARY_ID 1" >> $output_objdir/a2ixlibrary.data~$echo "#define VERSION $major" >> $output_objdir/a2ixlibrary.data~$echo "#define REVISION $revision" >> $output_objdir/a2ixlibrary.data~$AR $AR_FLAGS $lib $libobjs~$RANLIB $lib~(cd $output_objdir && a2ixlibrary -32)'
      hardcode_libdir_flag_spec_F77='-L$libdir'
      hardcode_minus_L_F77=yes
      # see comment about different semantics on the GNU ld section
      ld_shlibs_F77=no
      ;;

    bsdi[45]*)
      export_dynamic_flag_spec_F77=-rdynamic
      ;;

    cygwin* | mingw* | pw32*)
      # When not using gcc, we currently assume that we are using
      # Microsoft Visual C++.
      # hardcode_libdir_flag_spec is actually meaningless, as there is
      # no search path for DLLs.
      hardcode_libdir_flag_spec_F77=' '
      allow_undefined_flag_F77=unsupported
      # Tell ltmain to make .lib files, not .a files.
      libext=lib
      # Tell ltmain to make .dll files, not .so files.
      shrext_cmds=".dll"
      # FIXME: Setting linknames here is a bad hack.
      archive_cmds_F77='$CC -o $lib $libobjs $compiler_flags `echo "$deplibs" | $SED -e '\''s/ -lc$//'\''` -link -dll~linknames='
      # The linker will automatically build a .lib file if we build a DLL.
      old_archive_From_new_cmds_F77='true'
      # FIXME: Should let the user specify the lib program.
      old_archive_cmds_F77='lib -OUT:$oldlib$oldobjs$old_deplibs'
      fix_srcfile_path_F77='`cygpath -w "$srcfile"`'
      enable_shared_with_static_runtimes_F77=yes
      ;;

    darwin* | rhapsody*)
      case $host_os in
        rhapsody* | darwin1.[012])
         allow_undefined_flag_F77='${wl}-undefined ${wl}suppress'
         ;;
       *) # Darwin 1.3 on
         if test -z ${MACOSX_DEPLOYMENT_TARGET} ; then
           allow_undefined_flag_F77='${wl}-flat_namespace ${wl}-undefined ${wl}suppress'
         else
           case ${MACOSX_DEPLOYMENT_TARGET} in
             10.[012])
               allow_undefined_flag_F77='${wl}-flat_namespace ${wl}-undefined ${wl}suppress'
               ;;
             10.*)
               allow_undefined_flag_F77='${wl}-undefined ${wl}dynamic_lookup'
               ;;
           esac
         fi
         ;;
      esac
      archive_cmds_need_lc_F77=no
      hardcode_direct_F77=no
      hardcode_automatic_F77=yes
      hardcode_shlibpath_var_F77=unsupported
      whole_archive_flag_spec_F77=''
      link_all_deplibs_F77=yes
    if test "$GCC" = yes ; then
    	output_verbose_link_cmd='echo'
        archive_cmds_F77='$CC -dynamiclib $allow_undefined_flag -o $lib $libobjs $deplibs $compiler_flags -install_name $rpath/$soname $verstring'
      module_cmds_F77='$CC $allow_undefined_flag -o $lib -bundle $libobjs $deplibs$compiler_flags'
      # Don't fix this by using the ld -exported_symbols_list flag, it doesn't exist in older darwin lds
      archive_expsym_cmds_F77='sed -e "s,#.*,," -e "s,^[    ]*,," -e "s,^\(..*\),_&," < $export_symbols > $output_objdir/${libname}-symbols.expsym~$CC -dynamiclib $allow_undefined_flag -o $lib $libobjs $deplibs $compiler_flags -install_name $rpath/$soname $verstring~nmedit -s $output_objdir/${libname}-symbols.expsym ${lib}'
      module_expsym_cmds_F77='sed -e "s,#.*,," -e "s,^[    ]*,," -e "s,^\(..*\),_&," < $export_symbols > $output_objdir/${libname}-symbols.expsym~$CC $allow_undefined_flag  -o $lib -bundle $libobjs $deplibs$compiler_flags~nmedit -s $output_objdir/${libname}-symbols.expsym ${lib}'
    else
      case $cc_basename in
        xlc*)
         output_verbose_link_cmd='echo'
         archive_cmds_F77='$CC -qmkshrobj $allow_undefined_flag -o $lib $libobjs $deplibs $compiler_flags ${wl}-install_name ${wl}`echo $rpath/$soname` $xlcverstring'
         module_cmds_F77='$CC $allow_undefined_flag -o $lib -bundle $libobjs $deplibs$compiler_flags'
          # Don't fix this by using the ld -exported_symbols_list flag, it doesn't exist in older darwin lds
         archive_expsym_cmds_F77='sed -e "s,#.*,," -e "s,^[    ]*,," -e "s,^\(..*\),_&," < $export_symbols > $output_objdir/${libname}-symbols.expsym~$CC -qmkshrobj $allow_undefined_flag -o $lib $libobjs $deplibs $compiler_flags ${wl}-install_name ${wl}$rpath/$soname $xlcverstring~nmedit -s $output_objdir/${libname}-symbols.expsym ${lib}'
          module_expsym_cmds_F77='sed -e "s,#.*,," -e "s,^[    ]*,," -e "s,^\(..*\),_&," < $export_symbols > $output_objdir/${libname}-symbols.expsym~$CC $allow_undefined_flag  -o $lib -bundle $libobjs $deplibs$compiler_flags~nmedit -s $output_objdir/${libname}-symbols.expsym ${lib}'
          ;;
       *)
         ld_shlibs_F77=no
          ;;
      esac
    fi
      ;;

    dgux*)
      archive_cmds_F77='$LD -G -h $soname -o $lib $libobjs $deplibs $linker_flags'
      hardcode_libdir_flag_spec_F77='-L$libdir'
      hardcode_shlibpath_var_F77=no
      ;;

    freebsd1*)
      ld_shlibs_F77=no
      ;;

    # FreeBSD 2.2.[012] allows us to include c++rt0.o to get C++ constructor
    # support.  Future versions do this automatically, but an explicit c++rt0.o
    # does not break anything, and helps significantly (at the cost of a little
    # extra space).
    freebsd2.2*)
      archive_cmds_F77='$LD -Bshareable -o $lib $libobjs $deplibs $linker_flags /usr/lib/c++rt0.o'
      hardcode_libdir_flag_spec_F77='-R$libdir'
      hardcode_direct_F77=yes
      hardcode_shlibpath_var_F77=no
      ;;

    # Unfortunately, older versions of FreeBSD 2 do not have this feature.
    freebsd2*)
      archive_cmds_F77='$LD -Bshareable -o $lib $libobjs $deplibs $linker_flags'
      hardcode_direct_F77=yes
      hardcode_minus_L_F77=yes
      hardcode_shlibpath_var_F77=no
      ;;

    # FreeBSD 3 and greater uses gcc -shared to do shared libraries.
    freebsd* | dragonfly*)
      archive_cmds_F77='$CC -shared -o $lib $libobjs $deplibs $compiler_flags'
      hardcode_libdir_flag_spec_F77='-R$libdir'
      hardcode_direct_F77=yes
      hardcode_shlibpath_var_F77=no
      ;;

    hpux9*)
      if test "$GCC" = yes; then
	archive_cmds_F77='$rm $output_objdir/$soname~$CC -shared -fPIC ${wl}+b ${wl}$install_libdir -o $output_objdir/$soname $libobjs $deplibs $compiler_flags~test $output_objdir/$soname = $lib || mv $output_objdir/$soname $lib'
      else
	archive_cmds_F77='$rm $output_objdir/$soname~$LD -b +b $install_libdir -o $output_objdir/$soname $libobjs $deplibs $linker_flags~test $output_objdir/$soname = $lib || mv $output_objdir/$soname $lib'
      fi
      hardcode_libdir_flag_spec_F77='${wl}+b ${wl}$libdir'
      hardcode_libdir_separator_F77=:
      hardcode_direct_F77=yes

      # hardcode_minus_L: Not really in the search PATH,
      # but as the default location of the library.
      hardcode_minus_L_F77=yes
      export_dynamic_flag_spec_F77='${wl}-E'
      ;;

    hpux10*)
      if test "$GCC" = yes -a "$with_gnu_ld" = no; then
	archive_cmds_F77='$CC -shared -fPIC ${wl}+h ${wl}$soname ${wl}+b ${wl}$install_libdir -o $lib $libobjs $deplibs $compiler_flags'
      else
	archive_cmds_F77='$LD -b +h $soname +b $install_libdir -o $lib $libobjs $deplibs $linker_flags'
      fi
      if test "$with_gnu_ld" = no; then
	hardcode_libdir_flag_spec_F77='${wl}+b ${wl}$libdir'
	hardcode_libdir_separator_F77=:

	hardcode_direct_F77=yes
	export_dynamic_flag_spec_F77='${wl}-E'

	# hardcode_minus_L: Not really in the search PATH,
	# but as the default location of the library.
	hardcode_minus_L_F77=yes
      fi
      ;;

    hpux11*)
      if test "$GCC" = yes -a "$with_gnu_ld" = no; then
	case $host_cpu in
	hppa*64*)
	  archive_cmds_F77='$CC -shared ${wl}+h ${wl}$soname -o $lib $libobjs $deplibs $compiler_flags'
	  ;;
	ia64*)
	  archive_cmds_F77='$CC -shared ${wl}+h ${wl}$soname ${wl}+nodefaultrpath -o $lib $libobjs $deplibs $compiler_flags'
	  ;;
	*)
	  archive_cmds_F77='$CC -shared -fPIC ${wl}+h ${wl}$soname ${wl}+b ${wl}$install_libdir -o $lib $libobjs $deplibs $compiler_flags'
	  ;;
	esac
      else
	case $host_cpu in
	hppa*64*)
	  archive_cmds_F77='$CC -b ${wl}+h ${wl}$soname -o $lib $libobjs $deplibs $compiler_flags'
	  ;;
	ia64*)
	  archive_cmds_F77='$CC -b ${wl}+h ${wl}$soname ${wl}+nodefaultrpath -o $lib $libobjs $deplibs $compiler_flags'
	  ;;
	*)
	  archive_cmds_F77='$CC -b ${wl}+h ${wl}$soname ${wl}+b ${wl}$install_libdir -o $lib $libobjs $deplibs $compiler_flags'
	  ;;
	esac
      fi
      if test "$with_gnu_ld" = no; then
	hardcode_libdir_flag_spec_F77='${wl}+b ${wl}$libdir'
	hardcode_libdir_separator_F77=:

	case $host_cpu in
	hppa*64*|ia64*)
	  hardcode_libdir_flag_spec_ld_F77='+b $libdir'
	  hardcode_direct_F77=no
	  hardcode_shlibpath_var_F77=no
	  ;;
	*)
	  hardcode_direct_F77=yes
	  export_dynamic_flag_spec_F77='${wl}-E'

	  # hardcode_minus_L: Not really in the search PATH,
	  # but as the default location of the library.
	  hardcode_minus_L_F77=yes
	  ;;
	esac
      fi
      ;;

    irix5* | irix6* | nonstopux*)
      if test "$GCC" = yes; then
	archive_cmds_F77='$CC -shared $libobjs $deplibs $compiler_flags ${wl}-soname ${wl}$soname `test -n "$verstring" && echo ${wl}-set_version ${wl}$verstring` ${wl}-update_registry ${wl}${output_objdir}/so_locations -o $lib'
      else
	archive_cmds_F77='$LD -shared $libobjs $deplibs $linker_flags -soname $soname `test -n "$verstring" && echo -set_version $verstring` -update_registry ${output_objdir}/so_locations -o $lib'
	hardcode_libdir_flag_spec_ld_F77='-rpath $libdir'
      fi
      hardcode_libdir_flag_spec_F77='${wl}-rpath ${wl}$libdir'
      hardcode_libdir_separator_F77=:
      link_all_deplibs_F77=yes
      ;;

    netbsd*)
      if echo __ELF__ | $CC -E - | grep __ELF__ >/dev/null; then
	archive_cmds_F77='$LD -Bshareable -o $lib $libobjs $deplibs $linker_flags'  # a.out
      else
	archive_cmds_F77='$LD -shared -o $lib $libobjs $deplibs $linker_flags'      # ELF
      fi
      hardcode_libdir_flag_spec_F77='-R$libdir'
      hardcode_direct_F77=yes
      hardcode_shlibpath_var_F77=no
      ;;

    newsos6)
      archive_cmds_F77='$LD -G -h $soname -o $lib $libobjs $deplibs $linker_flags'
      hardcode_direct_F77=yes
      hardcode_libdir_flag_spec_F77='${wl}-rpath ${wl}$libdir'
      hardcode_libdir_separator_F77=:
      hardcode_shlibpath_var_F77=no
      ;;

    openbsd*)
      if test -f /usr/libexec/ld.so; then
	hardcode_direct_F77=yes
	hardcode_shlibpath_var_F77=no
	if test -z "`echo __ELF__ | $CC -E - | grep __ELF__`" || test "$host_os-$host_cpu" = "openbsd2.8-powerpc"; then
	  archive_cmds_F77='$CC -shared $pic_flag -o $lib $libobjs $deplibs $compiler_flags'
	  archive_expsym_cmds_F77='$CC -shared $pic_flag -o $lib $libobjs $deplibs $compiler_flags ${wl}-retain-symbols-file,$export_symbols'
	  hardcode_libdir_flag_spec_F77='${wl}-rpath,$libdir'
	  export_dynamic_flag_spec_F77='${wl}-E'
	else
	  case $host_os in
	   openbsd[01].* | openbsd2.[0-7] | openbsd2.[0-7].*)
	     archive_cmds_F77='$LD -Bshareable -o $lib $libobjs $deplibs $linker_flags'
	     hardcode_libdir_flag_spec_F77='-R$libdir'
	     ;;
	   *)
	     archive_cmds_F77='$CC -shared $pic_flag -o $lib $libobjs $deplibs $compiler_flags'
	     hardcode_libdir_flag_spec_F77='${wl}-rpath,$libdir'
	     ;;
	  esac
        fi
      else
	ld_shlibs_F77=no
      fi
      ;;

    os2*)
      hardcode_libdir_flag_spec_F77='-L$libdir'
      hardcode_minus_L_F77=yes
      allow_undefined_flag_F77=unsupported
      archive_cmds_F77='$echo "LIBRARY $libname INITINSTANCE" > $output_objdir/$libname.def~$echo "DESCRIPTION \"$libname\"" >> $output_objdir/$libname.def~$echo DATA >> $output_objdir/$libname.def~$echo " SINGLE NONSHARED" >> $output_objdir/$libname.def~$echo EXPORTS >> $output_objdir/$libname.def~emxexp $libobjs >> $output_objdir/$libname.def~$CC -Zdll -Zcrtdll -o $lib $libobjs $deplibs $compiler_flags $output_objdir/$libname.def'
      old_archive_From_new_cmds_F77='emximp -o $output_objdir/$libname.a $output_objdir/$libname.def'
      ;;

    osf3*)
      if test "$GCC" = yes; then
	allow_undefined_flag_F77=' ${wl}-expect_unresolved ${wl}\*'
	archive_cmds_F77='$CC -shared${allow_undefined_flag} $libobjs $deplibs $compiler_flags ${wl}-soname ${wl}$soname `test -n "$verstring" && echo ${wl}-set_version ${wl}$verstring` ${wl}-update_registry ${wl}${output_objdir}/so_locations -o $lib'
      else
	allow_undefined_flag_F77=' -expect_unresolved \*'
	archive_cmds_F77='$LD -shared${allow_undefined_flag} $libobjs $deplibs $linker_flags -soname $soname `test -n "$verstring" && echo -set_version $verstring` -update_registry ${output_objdir}/so_locations -o $lib'
      fi
      hardcode_libdir_flag_spec_F77='${wl}-rpath ${wl}$libdir'
      hardcode_libdir_separator_F77=:
      ;;

    osf4* | osf5*)	# as osf3* with the addition of -msym flag
      if test "$GCC" = yes; then
	allow_undefined_flag_F77=' ${wl}-expect_unresolved ${wl}\*'
	archive_cmds_F77='$CC -shared${allow_undefined_flag} $libobjs $deplibs $compiler_flags ${wl}-msym ${wl}-soname ${wl}$soname `test -n "$verstring" && echo ${wl}-set_version ${wl}$verstring` ${wl}-update_registry ${wl}${output_objdir}/so_locations -o $lib'
	hardcode_libdir_flag_spec_F77='${wl}-rpath ${wl}$libdir'
      else
	allow_undefined_flag_F77=' -expect_unresolved \*'
	archive_cmds_F77='$LD -shared${allow_undefined_flag} $libobjs $deplibs $linker_flags -msym -soname $soname `test -n "$verstring" && echo -set_version $verstring` -update_registry ${output_objdir}/so_locations -o $lib'
	archive_expsym_cmds_F77='for i in `cat $export_symbols`; do printf "%s %s\\n" -exported_symbol "\$i" >> $lib.exp; done; echo "-hidden">> $lib.exp~
	$LD -shared${allow_undefined_flag} -input $lib.exp $linker_flags $libobjs $deplibs -soname $soname `test -n "$verstring" && echo -set_version $verstring` -update_registry ${output_objdir}/so_locations -o $lib~$rm $lib.exp'

	# Both c and cxx compiler support -rpath directly
	hardcode_libdir_flag_spec_F77='-rpath $libdir'
      fi
      hardcode_libdir_separator_F77=:
      ;;

    solaris*)
      no_undefined_flag_F77=' -z text'
      if test "$GCC" = yes; then
	wlarc='${wl}'
	archive_cmds_F77='$CC -shared ${wl}-h ${wl}$soname -o $lib $libobjs $deplibs $compiler_flags'
	archive_expsym_cmds_F77='$echo "{ global:" > $lib.exp~cat $export_symbols | $SED -e "s/\(.*\)/\1;/" >> $lib.exp~$echo "local: *; };" >> $lib.exp~
	  $CC -shared ${wl}-M ${wl}$lib.exp ${wl}-h ${wl}$soname -o $lib $libobjs $deplibs $compiler_flags~$rm $lib.exp'
      else
	wlarc=''
	archive_cmds_F77='$LD -G${allow_undefined_flag} -h $soname -o $lib $libobjs $deplibs $linker_flags'
	archive_expsym_cmds_F77='$echo "{ global:" > $lib.exp~cat $export_symbols | $SED -e "s/\(.*\)/\1;/" >> $lib.exp~$echo "local: *; };" >> $lib.exp~
  	$LD -G${allow_undefined_flag} -M $lib.exp -h $soname -o $lib $libobjs $deplibs $linker_flags~$rm $lib.exp'
      fi
      hardcode_libdir_flag_spec_F77='-R$libdir'
      hardcode_shlibpath_var_F77=no
      case $host_os in
      solaris2.[0-5] | solaris2.[0-5].*) ;;
      *)
	# The compiler driver will combine and reorder linker options,
	# but understands `-z linker_flag'.  GCC discards it without `$wl',
	# but is careful enough not to reorder.
 	# Supported since Solaris 2.6 (maybe 2.5.1?)
	if test "$GCC" = yes; then
	  whole_archive_flag_spec_F77='${wl}-z ${wl}allextract$convenience ${wl}-z ${wl}defaultextract'
	else
	  whole_archive_flag_spec_F77='-z allextract$convenience -z defaultextract'
	fi
	;;
      esac
      link_all_deplibs_F77=yes
      ;;

    sunos4*)
      if test "x$host_vendor" = xsequent; then
	# Use $CC to link under sequent, because it throws in some extra .o
	# files that make .init and .fini sections work.
	archive_cmds_F77='$CC -G ${wl}-h $soname -o $lib $libobjs $deplibs $compiler_flags'
      else
	archive_cmds_F77='$LD -assert pure-text -Bstatic -o $lib $libobjs $deplibs $linker_flags'
      fi
      hardcode_libdir_flag_spec_F77='-L$libdir'
      hardcode_direct_F77=yes
      hardcode_minus_L_F77=yes
      hardcode_shlibpath_var_F77=no
      ;;

    sysv4)
      case $host_vendor in
	sni)
	  archive_cmds_F77='$LD -G -h $soname -o $lib $libobjs $deplibs $linker_flags'
	  hardcode_direct_F77=yes # is this really true???
	;;
	siemens)
	  ## LD is ld it makes a PLAMLIB
	  ## CC just makes a GrossModule.
	  archive_cmds_F77='$LD -G -o $lib $libobjs $deplibs $linker_flags'
	  reload_cmds_F77='$CC -r -o $output$reload_objs'
	  hardcode_direct_F77=no
        ;;
	motorola)
	  archive_cmds_F77='$LD -G -h $soname -o $lib $libobjs $deplibs $linker_flags'
	  hardcode_direct_F77=no #Motorola manual says yes, but my tests say they lie
	;;
      esac
      runpath_var='LD_RUN_PATH'
      hardcode_shlibpath_var_F77=no
      ;;

    sysv4.3*)
      archive_cmds_F77='$LD -G -h $soname -o $lib $libobjs $deplibs $linker_flags'
      hardcode_shlibpath_var_F77=no
      export_dynamic_flag_spec_F77='-Bexport'
      ;;

    sysv4*MP*)
      if test -d /usr/nec; then
	archive_cmds_F77='$LD -G -h $soname -o $lib $libobjs $deplibs $linker_flags'
	hardcode_shlibpath_var_F77=no
	runpath_var=LD_RUN_PATH
	hardcode_runpath_var=yes
	ld_shlibs_F77=yes
      fi
      ;;

    sysv4*uw2* | sysv5OpenUNIX* | sysv5UnixWare7.[01].[10]* | unixware7* | sco3.2v5.0.[024]*)
      no_undefined_flag_F77='${wl}-z,text'
      archive_cmds_need_lc_F77=no
      hardcode_shlibpath_var_F77=no
      runpath_var='LD_RUN_PATH'

      if test "$GCC" = yes; then
	archive_cmds_F77='$CC -shared ${wl}-h,$soname -o $lib $libobjs $deplibs $compiler_flags'
	archive_expsym_cmds_F77='$CC -shared ${wl}-Bexport:$export_symbols ${wl}-h,$soname -o $lib $libobjs $deplibs $compiler_flags'
      else
	archive_cmds_F77='$CC -G ${wl}-h,$soname -o $lib $libobjs $deplibs $compiler_flags'
	archive_expsym_cmds_F77='$CC -G ${wl}-Bexport:$export_symbols ${wl}-h,$soname -o $lib $libobjs $deplibs $compiler_flags'
      fi
      ;;

    sysv5* | sco3.2v5* | sco5v6*)
      # Note: We can NOT use -z defs as we might desire, because we do not
      # link with -lc, and that would cause any symbols used from libc to
      # always be unresolved, which means just about no library would
      # ever link correctly.  If we're not using GNU ld we use -z text
      # though, which does catch some bad symbols but isn't as heavy-handed
      # as -z defs.
      no_undefined_flag_F77='${wl}-z,text'
      allow_undefined_flag_F77='${wl}-z,nodefs'
      archive_cmds_need_lc_F77=no
      hardcode_shlibpath_var_F77=no
      hardcode_libdir_flag_spec_F77='`test -z "$SCOABSPATH" && echo ${wl}-R,$libdir`'
      hardcode_libdir_separator_F77=':'
      link_all_deplibs_F77=yes
      export_dynamic_flag_spec_F77='${wl}-Bexport'
      runpath_var='LD_RUN_PATH'

      if test "$GCC" = yes; then
	archive_cmds_F77='$CC -shared ${wl}-h,\${SCOABSPATH:+${install_libdir}/}$soname -o $lib $libobjs $deplibs $compiler_flags'
	archive_expsym_cmds_F77='$CC -shared ${wl}-Bexport:$export_symbols ${wl}-h,\${SCOABSPATH:+${install_libdir}/}$soname -o $lib $libobjs $deplibs $compiler_flags'
      else
	archive_cmds_F77='$CC -G ${wl}-h,\${SCOABSPATH:+${install_libdir}/}$soname -o $lib $libobjs $deplibs $compiler_flags'
	archive_expsym_cmds_F77='$CC -G ${wl}-Bexport:$export_symbols ${wl}-h,\${SCOABSPATH:+${install_libdir}/}$soname -o $lib $libobjs $deplibs $compiler_flags'
      fi
      ;;

    uts4*)
      archive_cmds_F77='$LD -G -h $soname -o $lib $libobjs $deplibs $linker_flags'
      hardcode_libdir_flag_spec_F77='-L$libdir'
      hardcode_shlibpath_var_F77=no
      ;;

    *)
      ld_shlibs_F77=no
      ;;
    esac
  fi

{ echo "$as_me:$LINENO: result: $ld_shlibs_F77" >&5
echo "${ECHO_T}$ld_shlibs_F77" >&6; }
test "$ld_shlibs_F77" = no && can_build_shared=no

#
# Do we need to explicitly link libc?
#
case "x$archive_cmds_need_lc_F77" in
x|xyes)
  # Assume -lc should be added
  archive_cmds_need_lc_F77=yes

  if test "$enable_shared" = yes && test "$GCC" = yes; then
    case $archive_cmds_F77 in
    *'~'*)
      # FIXME: we may have to deal with multi-command sequences.
      ;;
    '$CC '*)
      # Test whether the compiler implicitly links with -lc since on some
      # systems, -lgcc has to come before -lc. If gcc already passes -lc
      # to ld, don't add -lc before -lgcc.
      { echo "$as_me:$LINENO: checking whether -lc should be explicitly linked in" >&5
echo $ECHO_N "checking whether -lc should be explicitly linked in... $ECHO_C" >&6; }
      $rm conftest*
      echo "$lt_simple_compile_test_code" > conftest.$ac_ext

      if { (eval echo "$as_me:$LINENO: \"$ac_compile\"") >&5
  (eval $ac_compile) 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } 2>conftest.err; then
        soname=conftest
        lib=conftest
        libobjs=conftest.$ac_objext
        deplibs=
        wl=$lt_prog_compiler_wl_F77
	pic_flag=$lt_prog_compiler_pic_F77
        compiler_flags=-v
        linker_flags=-v
        verstring=
        output_objdir=.
        libname=conftest
        lt_save_allow_undefined_flag=$allow_undefined_flag_F77
        allow_undefined_flag_F77=
        if { (eval echo "$as_me:$LINENO: \"$archive_cmds_F77 2\>\&1 \| grep \" -lc \" \>/dev/null 2\>\&1\"") >&5
  (eval $archive_cmds_F77 2\>\&1 \| grep \" -lc \" \>/dev/null 2\>\&1) 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }
        then
	  archive_cmds_need_lc_F77=no
        else
	  archive_cmds_need_lc_F77=yes
        fi
        allow_undefined_flag_F77=$lt_save_allow_undefined_flag
      else
        cat conftest.err 1>&5
      fi
      $rm conftest*
      { echo "$as_me:$LINENO: result: $archive_cmds_need_lc_F77" >&5
echo "${ECHO_T}$archive_cmds_need_lc_F77" >&6; }
      ;;
    esac
  fi
  ;;
esac

{ echo "$as_me:$LINENO: checking dynamic linker characteristics" >&5
echo $ECHO_N "checking dynamic linker characteristics... $ECHO_C" >&6; }
library_names_spec=
libname_spec='lib$name'
soname_spec=
shrext_cmds=".so"
postinstall_cmds=
postuninstall_cmds=
finish_cmds=
finish_eval=
shlibpath_var=
shlibpath_overrides_runpath=unknown
version_type=none
dynamic_linker="$host_os ld.so"
sys_lib_dlsearch_path_spec="/lib /usr/lib"

need_lib_prefix=unknown
hardcode_into_libs=no

# when you set need_version to no, make sure it does not cause -set_version
# flags to be left without arguments
need_version=unknown

case $host_os in
aix3*)
  version_type=linux
  library_names_spec='${libname}${release}${shared_ext}$versuffix $libname.a'
  shlibpath_var=LIBPATH

  # AIX 3 has no versioning support, so we append a major version to the name.
  soname_spec='${libname}${release}${shared_ext}$major'
  ;;

aix4* | aix5*)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  hardcode_into_libs=yes
  if test "$host_cpu" = ia64; then
    # AIX 5 supports IA64
    library_names_spec='${libname}${release}${shared_ext}$major ${libname}${release}${shared_ext}$versuffix $libname${shared_ext}'
    shlibpath_var=LD_LIBRARY_PATH
  else
    # With GCC up to 2.95.x, collect2 would create an import file
    # for dependence libraries.  The import file would start with
    # the line `#! .'.  This would cause the generated library to
    # depend on `.', always an invalid library.  This was fixed in
    # development snapshots of GCC prior to 3.0.
    case $host_os in
      aix4 | aix4.[01] | aix4.[01].*)
      if { echo '#if __GNUC__ > 2 || (__GNUC__ == 2 && __GNUC_MINOR__ >= 97)'
	   echo ' yes '
	   echo '#endif'; } | ${CC} -E - | grep yes > /dev/null; then
	:
      else
	can_build_shared=no
      fi
      ;;
    esac
    # AIX (on Power*) has no versioning support, so currently we can not hardcode correct
    # soname into executable. Probably we can add versioning support to
    # collect2, so additional links can be useful in future.
    if test "$aix_use_runtimelinking" = yes; then
      # If using run time linking (on AIX 4.2 or later) use lib<name>.so
      # instead of lib<name>.a to let people know that these are not
      # typical AIX shared libraries.
      library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
    else
      # We preserve .a as extension for shared libraries through AIX4.2
      # and later when we are not doing run time linking.
      library_names_spec='${libname}${release}.a $libname.a'
      soname_spec='${libname}${release}${shared_ext}$major'
    fi
    shlibpath_var=LIBPATH
  fi
  ;;

amigaos*)
  library_names_spec='$libname.ixlibrary $libname.a'
  # Create ${libname}_ixlibrary.a entries in /sys/libs.
  finish_eval='for lib in `ls $libdir/*.ixlibrary 2>/dev/null`; do libname=`$echo "X$lib" | $Xsed -e '\''s%^.*/\([^/]*\)\.ixlibrary$%\1%'\''`; test $rm /sys/libs/${libname}_ixlibrary.a; $show "cd /sys/libs && $LN_S $lib ${libname}_ixlibrary.a"; cd /sys/libs && $LN_S $lib ${libname}_ixlibrary.a || exit 1; done'
  ;;

beos*)
  library_names_spec='${libname}${shared_ext}'
  dynamic_linker="$host_os ld.so"
  shlibpath_var=LIBRARY_PATH
  ;;

bsdi[45]*)
  version_type=linux
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  finish_cmds='PATH="\$PATH:/sbin" ldconfig $libdir'
  shlibpath_var=LD_LIBRARY_PATH
  sys_lib_search_path_spec="/shlib /usr/lib /usr/X11/lib /usr/contrib/lib /lib /usr/local/lib"
  sys_lib_dlsearch_path_spec="/shlib /usr/lib /usr/local/lib"
  # the default ld.so.conf also contains /usr/contrib/lib and
  # /usr/X11R6/lib (/usr/X11 is a link to /usr/X11R6), but let us allow
  # libtool to hard-code these into programs
  ;;

cygwin* | mingw* | pw32*)
  version_type=windows
  shrext_cmds=".dll"
  need_version=no
  need_lib_prefix=no

  case $GCC,$host_os in
  yes,cygwin* | yes,mingw* | yes,pw32*)
    library_names_spec='$libname.dll.a'
    # DLL is installed to $(libdir)/../bin by postinstall_cmds
    postinstall_cmds='base_file=`basename \${file}`~
      dlpath=`$SHELL 2>&1 -c '\''. $dir/'\''\${base_file}'\''i;echo \$dlname'\''`~
      dldir=$destdir/`dirname \$dlpath`~
      test -d \$dldir || mkdir -p \$dldir~
      $install_prog $dir/$dlname \$dldir/$dlname~
      chmod a+x \$dldir/$dlname'
    postuninstall_cmds='dldll=`$SHELL 2>&1 -c '\''. $file; echo \$dlname'\''`~
      dlpath=$dir/\$dldll~
       $rm \$dlpath'
    shlibpath_overrides_runpath=yes

    case $host_os in
    cygwin*)
      # Cygwin DLLs use 'cyg' prefix rather than 'lib'
      soname_spec='`echo ${libname} | sed -e 's/^lib/cyg/'``echo ${release} | $SED -e 's/[.]/-/g'`${versuffix}${shared_ext}'
      sys_lib_search_path_spec="/usr/lib /lib/w32api /lib /usr/local/lib"
      ;;
    mingw*)
      # MinGW DLLs use traditional 'lib' prefix
      soname_spec='${libname}`echo ${release} | $SED -e 's/[.]/-/g'`${versuffix}${shared_ext}'
      sys_lib_search_path_spec=`$CC -print-search-dirs | grep "^libraries:" | $SED -e "s/^libraries://" -e "s,=/,/,g"`
      if echo "$sys_lib_search_path_spec" | grep ';[c-zC-Z]:/' >/dev/null; then
        # It is most probably a Windows format PATH printed by
        # mingw gcc, but we are running on Cygwin. Gcc prints its search
        # path with ; separators, and with drive letters. We can handle the
        # drive letters (cygwin fileutils understands them), so leave them,
        # especially as we might pass files found there to a mingw objdump,
        # which wouldn't understand a cygwinified path. Ahh.
        sys_lib_search_path_spec=`echo "$sys_lib_search_path_spec" | $SED -e 's/;/ /g'`
      else
        sys_lib_search_path_spec=`echo "$sys_lib_search_path_spec" | $SED  -e "s/$PATH_SEPARATOR/ /g"`
      fi
      ;;
    pw32*)
      # pw32 DLLs use 'pw' prefix rather than 'lib'
      library_names_spec='`echo ${libname} | sed -e 's/^lib/pw/'``echo ${release} | $SED -e 's/[.]/-/g'`${versuffix}${shared_ext}'
      ;;
    esac
    ;;

  *)
    library_names_spec='${libname}`echo ${release} | $SED -e 's/[.]/-/g'`${versuffix}${shared_ext} $libname.lib'
    ;;
  esac
  dynamic_linker='Win32 ld.exe'
  # FIXME: first we should search . and the directory the executable is in
  shlibpath_var=PATH
  ;;

darwin* | rhapsody*)
  dynamic_linker="$host_os dyld"
  version_type=darwin
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${versuffix}$shared_ext ${libname}${release}${major}$shared_ext ${libname}$shared_ext'
  soname_spec='${libname}${release}${major}$shared_ext'
  shlibpath_overrides_runpath=yes
  shlibpath_var=DYLD_LIBRARY_PATH
  shrext_cmds='`test .$module = .yes && echo .so || echo .dylib`'

  sys_lib_dlsearch_path_spec='/usr/local/lib /lib /usr/lib'
  ;;

dgux*)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname$shared_ext'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  ;;

freebsd1*)
  dynamic_linker=no
  ;;

freebsd* | dragonfly*)
  # DragonFly does not have aout.  When/if they implement a new
  # versioning mechanism, adjust this.
  if test -x /usr/bin/objformat; then
    objformat=`/usr/bin/objformat`
  else
    case $host_os in
    freebsd[123]*) objformat=aout ;;
    *) objformat=elf ;;
    esac
  fi
  version_type=freebsd-$objformat
  case $version_type in
    freebsd-elf*)
      library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext} $libname${shared_ext}'
      need_version=no
      need_lib_prefix=no
      ;;
    freebsd-*)
      library_names_spec='${libname}${release}${shared_ext}$versuffix $libname${shared_ext}$versuffix'
      need_version=yes
      ;;
  esac
  shlibpath_var=LD_LIBRARY_PATH
  case $host_os in
  freebsd2*)
    shlibpath_overrides_runpath=yes
    ;;
  freebsd3.[01]* | freebsdelf3.[01]*)
    shlibpath_overrides_runpath=yes
    hardcode_into_libs=yes
    ;;
  freebsd3.[2-9]* | freebsdelf3.[2-9]* | \
  freebsd4.[0-5] | freebsdelf4.[0-5] | freebsd4.1.1 | freebsdelf4.1.1)
    shlibpath_overrides_runpath=no
    hardcode_into_libs=yes
    ;;
  *) # from 4.6 on, and DragonFly
    shlibpath_overrides_runpath=yes
    hardcode_into_libs=yes
    ;;
  esac
  ;;

gnu*)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}${major} ${libname}${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  hardcode_into_libs=yes
  ;;

hpux9* | hpux10* | hpux11*)
  # Give a soname corresponding to the major version so that dld.sl refuses to
  # link against other versions.
  version_type=sunos
  need_lib_prefix=no
  need_version=no
  case $host_cpu in
  ia64*)
    shrext_cmds='.so'
    hardcode_into_libs=yes
    dynamic_linker="$host_os dld.so"
    shlibpath_var=LD_LIBRARY_PATH
    shlibpath_overrides_runpath=yes # Unless +noenvvar is specified.
    library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
    soname_spec='${libname}${release}${shared_ext}$major'
    if test "X$HPUX_IA64_MODE" = X32; then
      sys_lib_search_path_spec="/usr/lib/hpux32 /usr/local/lib/hpux32 /usr/local/lib"
    else
      sys_lib_search_path_spec="/usr/lib/hpux64 /usr/local/lib/hpux64"
    fi
    sys_lib_dlsearch_path_spec=$sys_lib_search_path_spec
    ;;
   hppa*64*)
     shrext_cmds='.sl'
     hardcode_into_libs=yes
     dynamic_linker="$host_os dld.sl"
     shlibpath_var=LD_LIBRARY_PATH # How should we handle SHLIB_PATH
     shlibpath_overrides_runpath=yes # Unless +noenvvar is specified.
     library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
     soname_spec='${libname}${release}${shared_ext}$major'
     sys_lib_search_path_spec="/usr/lib/pa20_64 /usr/ccs/lib/pa20_64"
     sys_lib_dlsearch_path_spec=$sys_lib_search_path_spec
     ;;
   *)
    shrext_cmds='.sl'
    dynamic_linker="$host_os dld.sl"
    shlibpath_var=SHLIB_PATH
    shlibpath_overrides_runpath=no # +s is required to enable SHLIB_PATH
    library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
    soname_spec='${libname}${release}${shared_ext}$major'
    ;;
  esac
  # HP-UX runs *really* slowly unless shared libraries are mode 555.
  postinstall_cmds='chmod 555 $lib'
  ;;

interix[3-9]*)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major ${libname}${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  dynamic_linker='Interix 3.x ld.so.1 (PE, like ELF)'
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=no
  hardcode_into_libs=yes
  ;;

irix5* | irix6* | nonstopux*)
  case $host_os in
    nonstopux*) version_type=nonstopux ;;
    *)
	if test "$lt_cv_prog_gnu_ld" = yes; then
		version_type=linux
	else
		version_type=irix
	fi ;;
  esac
  need_lib_prefix=no
  need_version=no
  soname_spec='${libname}${release}${shared_ext}$major'
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major ${libname}${release}${shared_ext} $libname${shared_ext}'
  case $host_os in
  irix5* | nonstopux*)
    libsuff= shlibsuff=
    ;;
  *)
    case $LD in # libtool.m4 will add one of these switches to LD
    *-32|*"-32 "|*-melf32bsmip|*"-melf32bsmip ")
      libsuff= shlibsuff= libmagic=32-bit;;
    *-n32|*"-n32 "|*-melf32bmipn32|*"-melf32bmipn32 ")
      libsuff=32 shlibsuff=N32 libmagic=N32;;
    *-64|*"-64 "|*-melf64bmip|*"-melf64bmip ")
      libsuff=64 shlibsuff=64 libmagic=64-bit;;
    *) libsuff= shlibsuff= libmagic=never-match;;
    esac
    ;;
  esac
  shlibpath_var=LD_LIBRARY${shlibsuff}_PATH
  shlibpath_overrides_runpath=no
  sys_lib_search_path_spec="/usr/lib${libsuff} /lib${libsuff} /usr/local/lib${libsuff}"
  sys_lib_dlsearch_path_spec="/usr/lib${libsuff} /lib${libsuff}"
  hardcode_into_libs=yes
  ;;

# No shared lib support for Linux oldld, aout, or coff.
linux*oldld* | linux*aout* | linux*coff*)
  dynamic_linker=no
  ;;

# This must be Linux ELF.
linux* | k*bsd*-gnu)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  finish_cmds='PATH="\$PATH:/sbin" ldconfig -n $libdir'
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=no
  # This implies no fast_install, which is unacceptable.
  # Some rework will be needed to allow for fast_install
  # before this can be enabled.
  hardcode_into_libs=yes

  # Append ld.so.conf contents to the search path
  if test -f /etc/ld.so.conf; then
    lt_ld_extra=`awk '/^include / { system(sprintf("cd /etc; cat %s 2>/dev/null", \$2)); skip = 1; } { if (!skip) print \$0; skip = 0; }' < /etc/ld.so.conf | $SED -e 's/#.*//;/^[ 	]*hwcap[ 	]/d;s/[:,	]/ /g;s/=[^=]*$//;s/=[^= ]* / /g;/^$/d' | tr '\n' ' '`
    sys_lib_dlsearch_path_spec="/lib /usr/lib $lt_ld_extra"
  fi

  # We used to test for /lib/ld.so.1 and disable shared libraries on
  # powerpc, because MkLinux only supported shared libraries with the
  # GNU dynamic linker.  Since this was broken with cross compilers,
  # most powerpc-linux boxes support dynamic linking these days and
  # people can always --disable-shared, the test was removed, and we
  # assume the GNU/Linux dynamic linker is in use.
  dynamic_linker='GNU/Linux ld.so'
  ;;

netbsd*)
  version_type=sunos
  need_lib_prefix=no
  need_version=no
  if echo __ELF__ | $CC -E - | grep __ELF__ >/dev/null; then
    library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${shared_ext}$versuffix'
    finish_cmds='PATH="\$PATH:/sbin" ldconfig -m $libdir'
    dynamic_linker='NetBSD (a.out) ld.so'
  else
    library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major ${libname}${shared_ext}'
    soname_spec='${libname}${release}${shared_ext}$major'
    dynamic_linker='NetBSD ld.elf_so'
  fi
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=yes
  hardcode_into_libs=yes
  ;;

newsos6)
  version_type=linux
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=yes
  ;;

nto-qnx*)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=yes
  ;;

openbsd*)
  version_type=sunos
  sys_lib_dlsearch_path_spec="/usr/lib"
  need_lib_prefix=no
  # Some older versions of OpenBSD (3.3 at least) *do* need versioned libs.
  case $host_os in
    openbsd3.3 | openbsd3.3.*) need_version=yes ;;
    *)                         need_version=no  ;;
  esac
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${shared_ext}$versuffix'
  finish_cmds='PATH="\$PATH:/sbin" ldconfig -m $libdir'
  shlibpath_var=LD_LIBRARY_PATH
  if test -z "`echo __ELF__ | $CC -E - | grep __ELF__`" || test "$host_os-$host_cpu" = "openbsd2.8-powerpc"; then
    case $host_os in
      openbsd2.[89] | openbsd2.[89].*)
	shlibpath_overrides_runpath=no
	;;
      *)
	shlibpath_overrides_runpath=yes
	;;
      esac
  else
    shlibpath_overrides_runpath=yes
  fi
  ;;

os2*)
  libname_spec='$name'
  shrext_cmds=".dll"
  need_lib_prefix=no
  library_names_spec='$libname${shared_ext} $libname.a'
  dynamic_linker='OS/2 ld.exe'
  shlibpath_var=LIBPATH
  ;;

osf3* | osf4* | osf5*)
  version_type=osf
  need_lib_prefix=no
  need_version=no
  soname_spec='${libname}${release}${shared_ext}$major'
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  shlibpath_var=LD_LIBRARY_PATH
  sys_lib_search_path_spec="/usr/shlib /usr/ccs/lib /usr/lib/cmplrs/cc /usr/lib /usr/local/lib /var/shlib"
  sys_lib_dlsearch_path_spec="$sys_lib_search_path_spec"
  ;;

rdos*)
  dynamic_linker=no
  ;;

solaris*)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=yes
  hardcode_into_libs=yes
  # ldd complains unless libraries are executable
  postinstall_cmds='chmod +x $lib'
  ;;

sunos4*)
  version_type=sunos
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${shared_ext}$versuffix'
  finish_cmds='PATH="\$PATH:/usr/etc" ldconfig $libdir'
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=yes
  if test "$with_gnu_ld" = yes; then
    need_lib_prefix=no
  fi
  need_version=yes
  ;;

sysv4 | sysv4.3*)
  version_type=linux
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  case $host_vendor in
    sni)
      shlibpath_overrides_runpath=no
      need_lib_prefix=no
      export_dynamic_flag_spec='${wl}-Blargedynsym'
      runpath_var=LD_RUN_PATH
      ;;
    siemens)
      need_lib_prefix=no
      ;;
    motorola)
      need_lib_prefix=no
      need_version=no
      shlibpath_overrides_runpath=no
      sys_lib_search_path_spec='/lib /usr/lib /usr/ccs/lib'
      ;;
  esac
  ;;

sysv4*MP*)
  if test -d /usr/nec ;then
    version_type=linux
    library_names_spec='$libname${shared_ext}.$versuffix $libname${shared_ext}.$major $libname${shared_ext}'
    soname_spec='$libname${shared_ext}.$major'
    shlibpath_var=LD_LIBRARY_PATH
  fi
  ;;

sysv5* | sco3.2v5* | sco5v6* | unixware* | OpenUNIX* | sysv4*uw2*)
  version_type=freebsd-elf
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext} $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  hardcode_into_libs=yes
  if test "$with_gnu_ld" = yes; then
    sys_lib_search_path_spec='/usr/local/lib /usr/gnu/lib /usr/ccs/lib /usr/lib /lib'
    shlibpath_overrides_runpath=no
  else
    sys_lib_search_path_spec='/usr/ccs/lib /usr/lib'
    shlibpath_overrides_runpath=yes
    case $host_os in
      sco3.2v5*)
        sys_lib_search_path_spec="$sys_lib_search_path_spec /lib"
	;;
    esac
  fi
  sys_lib_dlsearch_path_spec='/usr/lib'
  ;;

uts4*)
  version_type=linux
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  ;;

*)
  dynamic_linker=no
  ;;
esac
{ echo "$as_me:$LINENO: result: $dynamic_linker" >&5
echo "${ECHO_T}$dynamic_linker" >&6; }
test "$dynamic_linker" = no && can_build_shared=no

variables_saved_for_relink="PATH $shlibpath_var $runpath_var"
if test "$GCC" = yes; then
  variables_saved_for_relink="$variables_saved_for_relink GCC_EXEC_PREFIX COMPILER_PATH LIBRARY_PATH"
fi

{ echo "$as_me:$LINENO: checking how to hardcode library paths into programs" >&5
echo $ECHO_N "checking how to hardcode library paths into programs... $ECHO_C" >&6; }
hardcode_action_F77=
if test -n "$hardcode_libdir_flag_spec_F77" || \
   test -n "$runpath_var_F77" || \
   test "X$hardcode_automatic_F77" = "Xyes" ; then

  # We can hardcode non-existant directories.
  if test "$hardcode_direct_F77" != no &&
     # If the only mechanism to avoid hardcoding is shlibpath_var, we
     # have to relink, otherwise we might link with an installed library
     # when we should be linking with a yet-to-be-installed one
     ## test "$_LT_AC_TAGVAR(hardcode_shlibpath_var, F77)" != no &&
     test "$hardcode_minus_L_F77" != no; then
    # Linking always hardcodes the temporary library directory.
    hardcode_action_F77=relink
  else
    # We can link without hardcoding, and we can hardcode nonexisting dirs.
    hardcode_action_F77=immediate
  fi
else
  # We cannot hardcode anything, or else we can only hardcode existing
  # directories.
  hardcode_action_F77=unsupported
fi
{ echo "$as_me:$LINENO: result: $hardcode_action_F77" >&5
echo "${ECHO_T}$hardcode_action_F77" >&6; }

if test "$hardcode_action_F77" = relink; then
  # Fast installation is not supported
  enable_fast_install=no
elif test "$shlibpath_overrides_runpath" = yes ||
     test "$enable_shared" = no; then
  # Fast installation is not necessary
  enable_fast_install=needless
fi


# The else clause should only fire when bootstrapping the
# libtool distribution, otherwise you forgot to ship ltmain.sh
# with your package, and you will get complaints that there are
# no rules to generate ltmain.sh.
if test -f "$ltmain"; then
  # See if we are running on zsh, and set the options which allow our commands through
  # without removal of \ escapes.
  if test -n "${ZSH_VERSION+set}" ; then
    setopt NO_GLOB_SUBST
  fi
  # Now quote all the things that may contain metacharacters while being
  # careful not to overquote the AC_SUBSTed values.  We take copies of the
  # variables and quote the copies for generation of the libtool script.
  for var in echo old_CC old_CFLAGS AR AR_FLAGS EGREP RANLIB LN_S LTCC LTCFLAGS NM \
    SED SHELL STRIP \
    libname_spec library_names_spec soname_spec extract_expsyms_cmds \
    old_striplib striplib file_magic_cmd finish_cmds finish_eval \
    deplibs_check_method reload_flag reload_cmds need_locks \
    lt_cv_sys_global_symbol_pipe lt_cv_sys_global_symbol_to_cdecl \
    lt_cv_sys_global_symbol_to_c_name_address \
    sys_lib_search_path_spec sys_lib_dlsearch_path_spec \
    old_postinstall_cmds old_postuninstall_cmds \
    compiler_F77 \
    CC_F77 \
    LD_F77 \
    lt_prog_compiler_wl_F77 \
    lt_prog_compiler_pic_F77 \
    lt_prog_compiler_static_F77 \
    lt_prog_compiler_no_builtin_flag_F77 \
    export_dynamic_flag_spec_F77 \
    thread_safe_flag_spec_F77 \
    whole_archive_flag_spec_F77 \
    enable_shared_with_static_runtimes_F77 \
    old_archive_cmds_F77 \
    old_archive_from_new_cmds_F77 \
    predep_objects_F77 \
    postdep_objects_F77 \
    predeps_F77 \
    postdeps_F77 \
    compiler_lib_search_path_F77 \
    archive_cmds_F77 \
    archive_expsym_cmds_F77 \
    postinstall_cmds_F77 \
    postuninstall_cmds_F77 \
    old_archive_from_expsyms_cmds_F77 \
    allow_undefined_flag_F77 \
    no_undefined_flag_F77 \
    export_symbols_cmds_F77 \
    hardcode_libdir_flag_spec_F77 \
    hardcode_libdir_flag_spec_ld_F77 \
    hardcode_libdir_separator_F77 \
    hardcode_automatic_F77 \
    module_cmds_F77 \
    module_expsym_cmds_F77 \
    lt_cv_prog_compiler_c_o_F77 \
    fix_srcfile_path_F77 \
    exclude_expsyms_F77 \
    include_expsyms_F77; do

    case $var in
    old_archive_cmds_F77 | \
    old_archive_from_new_cmds_F77 | \
    archive_cmds_F77 | \
    archive_expsym_cmds_F77 | \
    module_cmds_F77 | \
    module_expsym_cmds_F77 | \
    old_archive_from_expsyms_cmds_F77 | \
    export_symbols_cmds_F77 | \
    extract_expsyms_cmds | reload_cmds | finish_cmds | \
    postinstall_cmds | postuninstall_cmds | \
    old_postinstall_cmds | old_postuninstall_cmds | \
    sys_lib_search_path_spec | sys_lib_dlsearch_path_spec)
      # Double-quote double-evaled strings.
      eval "lt_$var=\\\"\`\$echo \"X\$$var\" | \$Xsed -e \"\$double_quote_subst\" -e \"\$sed_quote_subst\" -e \"\$delay_variable_subst\"\`\\\""
      ;;
    *)
      eval "lt_$var=\\\"\`\$echo \"X\$$var\" | \$Xsed -e \"\$sed_quote_subst\"\`\\\""
      ;;
    esac
  done

  case $lt_echo in
  *'\$0 --fallback-echo"')
    lt_echo=`$echo "X$lt_echo" | $Xsed -e 's/\\\\\\\$0 --fallback-echo"$/$0 --fallback-echo"/'`
    ;;
  esac

cfgfile="$ofile"

  cat <<__EOF__ >> "$cfgfile"
# ### BEGIN LIBTOOL TAG CONFIG: $tagname

# Libtool was configured on host `(hostname || uname -n) 2>/dev/null | sed 1q`:

# Shell to use when invoking shell scripts.
SHELL=$lt_SHELL

# Whether or not to build shared libraries.
build_libtool_libs=$enable_shared

# Whether or not to build static libraries.
build_old_libs=$enable_static

# Whether or not to add -lc for building shared libraries.
build_libtool_need_lc=$archive_cmds_need_lc_F77

# Whether or not to disallow shared libs when runtime libs are static
allow_libtool_libs_with_static_runtimes=$enable_shared_with_static_runtimes_F77

# Whether or not to optimize for fast installation.
fast_install=$enable_fast_install

# The host system.
host_alias=$host_alias
host=$host
host_os=$host_os

# The build system.
build_alias=$build_alias
build=$build
build_os=$build_os

# An echo program that does not interpret backslashes.
echo=$lt_echo

# The archiver.
AR=$lt_AR
AR_FLAGS=$lt_AR_FLAGS

# A C compiler.
LTCC=$lt_LTCC

# LTCC compiler flags.
LTCFLAGS=$lt_LTCFLAGS

# A language-specific compiler.
CC=$lt_compiler_F77

# Is the compiler the GNU C compiler?
with_gcc=$GCC_F77

# An ERE matcher.
EGREP=$lt_EGREP

# The linker used to build libraries.
LD=$lt_LD_F77

# Whether we need hard or soft links.
LN_S=$lt_LN_S

# A BSD-compatible nm program.
NM=$lt_NM

# A symbol stripping program
STRIP=$lt_STRIP

# Used to examine libraries when file_magic_cmd begins "file"
MAGIC_CMD=$MAGIC_CMD

# Used on cygwin: DLL creation program.
DLLTOOL="$DLLTOOL"

# Used on cygwin: object dumper.
OBJDUMP="$OBJDUMP"

# Used on cygwin: assembler.
AS="$AS"

# The name of the directory that contains temporary libtool files.
objdir=$objdir

# How to create reloadable object files.
reload_flag=$lt_reload_flag
reload_cmds=$lt_reload_cmds

# How to pass a linker flag through the compiler.
wl=$lt_lt_prog_compiler_wl_F77

# Object file suffix (normally "o").
objext="$ac_objext"

# Old archive suffix (normally "a").
libext="$libext"

# Shared library suffix (normally ".so").
shrext_cmds='$shrext_cmds'

# Executable file suffix (normally "").
exeext="$exeext"

# Additional compiler flags for building library objects.
pic_flag=$lt_lt_prog_compiler_pic_F77
pic_mode=$pic_mode

# What is the maximum length of a command?
max_cmd_len=$lt_cv_sys_max_cmd_len

# Does compiler simultaneously support -c and -o options?
compiler_c_o=$lt_lt_cv_prog_compiler_c_o_F77

# Must we lock files when doing compilation?
need_locks=$lt_need_locks

# Do we need the lib prefix for modules?
need_lib_prefix=$need_lib_prefix

# Do we need a version for libraries?
need_version=$need_version

# Whether dlopen is supported.
dlopen_support=$enable_dlopen

# Whether dlopen of programs is supported.
dlopen_self=$enable_dlopen_self

# Whether dlopen of statically linked programs is supported.
dlopen_self_static=$enable_dlopen_self_static

# Compiler flag to prevent dynamic linking.
link_static_flag=$lt_lt_prog_compiler_static_F77

# Compiler flag to turn off builtin functions.
no_builtin_flag=$lt_lt_prog_compiler_no_builtin_flag_F77

# Compiler flag to allow reflexive dlopens.
export_dynamic_flag_spec=$lt_export_dynamic_flag_spec_F77

# Compiler flag to generate shared objects directly from archives.
whole_archive_flag_spec=$lt_whole_archive_flag_spec_F77

# Compiler flag to generate thread-safe objects.
thread_safe_flag_spec=$lt_thread_safe_flag_spec_F77

# Library versioning type.
version_type=$version_type

# Format of library name prefix.
libname_spec=$lt_libname_spec

# List of archive names.  First name is the real one, the rest are links.
# The last name is the one that the linker finds with -lNAME.
library_names_spec=$lt_library_names_spec

# The coded name of the library, if different from the real name.
soname_spec=$lt_soname_spec

# Commands used to build and install an old-style archive.
RANLIB=$lt_RANLIB
old_archive_cmds=$lt_old_archive_cmds_F77
old_postinstall_cmds=$lt_old_postinstall_cmds
old_postuninstall_cmds=$lt_old_postuninstall_cmds

# Create an old-style archive from a shared archive.
old_archive_from_new_cmds=$lt_old_archive_from_new_cmds_F77

# Create a temporary old-style archive to link instead of a shared archive.
old_archive_from_expsyms_cmds=$lt_old_archive_from_expsyms_cmds_F77

# Commands used to build and install a shared archive.
archive_cmds=$lt_archive_cmds_F77
archive_expsym_cmds=$lt_archive_expsym_cmds_F77
postinstall_cmds=$lt_postinstall_cmds
postuninstall_cmds=$lt_postuninstall_cmds

# Commands used to build a loadable module (assumed same as above if empty)
module_cmds=$lt_module_cmds_F77
module_expsym_cmds=$lt_module_expsym_cmds_F77

# Commands to strip libraries.
old_striplib=$lt_old_striplib
striplib=$lt_striplib

# Dependencies to place before the objects being linked to create a
# shared library.
predep_objects=$lt_predep_objects_F77

# Dependencies to place after the objects being linked to create a
# shared library.
postdep_objects=$lt_postdep_objects_F77

# Dependencies to place before the objects being linked to create a
# shared library.
predeps=$lt_predeps_F77

# Dependencies to place after the objects being linked to create a
# shared library.
postdeps=$lt_postdeps_F77

# The library search path used internally by the compiler when linking
# a shared library.
compiler_lib_search_path=$lt_compiler_lib_search_path_F77

# Method to check whether dependent libraries are shared objects.
deplibs_check_method=$lt_deplibs_check_method

# Command to use when deplibs_check_method == file_magic.
file_magic_cmd=$lt_file_magic_cmd

# Flag that allows shared libraries with undefined symbols to be built.
allow_undefined_flag=$lt_allow_undefined_flag_F77

# Flag that forces no undefined symbols.
no_undefined_flag=$lt_no_undefined_flag_F77

# Commands used to finish a libtool library installation in a directory.
finish_cmds=$lt_finish_cmds

# Same as above, but a single script fragment to be evaled but not shown.
finish_eval=$lt_finish_eval

# Take the output of nm and produce a listing of raw symbols and C names.
global_symbol_pipe=$lt_lt_cv_sys_global_symbol_pipe

# Transform the output of nm in a proper C declaration
global_symbol_to_cdecl=$lt_lt_cv_sys_global_symbol_to_cdecl

# Transform the output of nm in a C name address pair
global_symbol_to_c_name_address=$lt_lt_cv_sys_global_symbol_to_c_name_address

# This is the shared library runtime path variable.
runpath_var=$runpath_var

# This is the shared library path variable.
shlibpath_var=$shlibpath_var

# Is shlibpath searched before the hard-coded library search path?
shlibpath_overrides_runpath=$shlibpath_overrides_runpath

# How to hardcode a shared library path into an executable.
hardcode_action=$hardcode_action_F77

# Whether we should hardcode library paths into libraries.
hardcode_into_libs=$hardcode_into_libs

# Flag to hardcode \$libdir into a binary during linking.
# This must work even if \$libdir does not exist.
hardcode_libdir_flag_spec=$lt_hardcode_libdir_flag_spec_F77

# If ld is used when linking, flag to hardcode \$libdir into
# a binary during linking. This must work even if \$libdir does
# not exist.
hardcode_libdir_flag_spec_ld=$lt_hardcode_libdir_flag_spec_ld_F77

# Whether we need a single -rpath flag with a separated argument.
hardcode_libdir_separator=$lt_hardcode_libdir_separator_F77

# Set to yes if using DIR/libNAME${shared_ext} during linking hardcodes DIR into the
# resulting binary.
hardcode_direct=$hardcode_direct_F77

# Set to yes if using the -LDIR flag during linking hardcodes DIR into the
# resulting binary.
hardcode_minus_L=$hardcode_minus_L_F77

# Set to yes if using SHLIBPATH_VAR=DIR during linking hardcodes DIR into
# the resulting binary.
hardcode_shlibpath_var=$hardcode_shlibpath_var_F77

# Set to yes if building a shared library automatically hardcodes DIR into the library
# and all subsequent libraries and executables linked against it.
hardcode_automatic=$hardcode_automatic_F77

# Variables whose values should be saved in libtool wrapper scripts and
# restored at relink time.
variables_saved_for_relink="$variables_saved_for_relink"

# Whether libtool must link a program against all its dependency libraries.
link_all_deplibs=$link_all_deplibs_F77

# Compile-time system search path for libraries
sys_lib_search_path_spec=$lt_sys_lib_search_path_spec

# Run-time system search path for libraries
sys_lib_dlsearch_path_spec=$lt_sys_lib_dlsearch_path_spec

# Fix the shell variable \$srcfile for the compiler.
fix_srcfile_path=$lt_fix_srcfile_path

# Set to yes if exported symbols are required.
always_export_symbols=$always_export_symbols_F77

# The commands to list exported symbols.
export_symbols_cmds=$lt_export_symbols_cmds_F77

# The commands to extract the exported symbol list from a shared archive.
extract_expsyms_cmds=$lt_extract_expsyms_cmds

# Symbols that should not be listed in the preloaded symbols.
exclude_expsyms=$lt_exclude_expsyms_F77

# Symbols that must always be exported.
include_expsyms=$lt_include_expsyms_F77

# ### END LIBTOOL TAG CONFIG: $tagname

__EOF__


else
  # If there is no Makefile yet, we rely on a make rule to execute
  # `config.status --recheck' to rerun these tests and create the
  # libtool script then.
  ltmain_in=`echo $ltmain | sed -e 's/\.sh$/.in/'`
  if test -f "$ltmain_in"; then
    test -f Makefile && make "$ltmain"
  fi
fi


ac_ext=c
ac_cpp='$CPP $CPPFLAGS'
ac_compile='$CC -c $CFLAGS $CPPFLAGS conftest.$ac_ext >&5'
ac_link='$CC -o conftest$ac_exeext $CFLAGS $CPPFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_c_compiler_gnu

CC="$lt_save_CC"

	else
	  tagname=""
	fi
	;;

      GCJ)
	if test -n "$GCJ" && test "X$GCJ" != "Xno"; then


# Source file extension for Java test sources.
ac_ext=java

# Object file extension for compiled Java test sources.
objext=o
objext_GCJ=$objext

# Code to be used in simple compile tests
lt_simple_compile_test_code="class foo {}"

# Code to be used in simple link tests
lt_simple_link_test_code='public class conftest { public static void main(String[] argv) {}; }'

# ltmain only uses $CC for tagged configurations so make sure $CC is set.

# If no C compiler was specified, use CC.
LTCC=${LTCC-"$CC"}

# If no C compiler flags were specified, use CFLAGS.
LTCFLAGS=${LTCFLAGS-"$CFLAGS"}

# Allow CC to be a program name with arguments.
compiler=$CC


# save warnings/boilerplate of simple test code
ac_outfile=conftest.$ac_objext
echo "$lt_simple_compile_test_code" >conftest.$ac_ext
eval "$ac_compile" 2>&1 >/dev/null | $SED '/^$/d; /^ *+/d' >conftest.err
_lt_compiler_boilerplate=`cat conftest.err`
$rm conftest*

ac_outfile=conftest.$ac_objext
echo "$lt_simple_link_test_code" >conftest.$ac_ext
eval "$ac_link" 2>&1 >/dev/null | $SED '/^$/d; /^ *+/d' >conftest.err
_lt_linker_boilerplate=`cat conftest.err`
$rm conftest*


# Allow CC to be a program name with arguments.
lt_save_CC="$CC"
CC=${GCJ-"gcj"}
compiler=$CC
compiler_GCJ=$CC
for cc_temp in $compiler""; do
  case $cc_temp in
    compile | *[\\/]compile | ccache | *[\\/]ccache ) ;;
    distcc | *[\\/]distcc | purify | *[\\/]purify ) ;;
    \-*) ;;
    *) break;;
  esac
done
cc_basename=`$echo "X$cc_temp" | $Xsed -e 's%.*/%%' -e "s%^$host_alias-%%"`


# GCJ did not exist at the time GCC didn't implicitly link libc in.
archive_cmds_need_lc_GCJ=no

old_archive_cmds_GCJ=$old_archive_cmds


lt_prog_compiler_no_builtin_flag_GCJ=

if test "$GCC" = yes; then
  lt_prog_compiler_no_builtin_flag_GCJ=' -fno-builtin'


{ echo "$as_me:$LINENO: checking if $compiler supports -fno-rtti -fno-exceptions" >&5
echo $ECHO_N "checking if $compiler supports -fno-rtti -fno-exceptions... $ECHO_C" >&6; }
if test "${lt_cv_prog_compiler_rtti_exceptions+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  lt_cv_prog_compiler_rtti_exceptions=no
  ac_outfile=conftest.$ac_objext
   echo "$lt_simple_compile_test_code" > conftest.$ac_ext
   lt_compiler_flag="-fno-rtti -fno-exceptions"
   # Insert the option either (1) after the last *FLAGS variable, or
   # (2) before a word containing "conftest.", or (3) at the end.
   # Note that $ac_compile itself does not contain backslashes and begins
   # with a dollar sign (not a hyphen), so the echo should work correctly.
   # The option is referenced via a variable to avoid confusing sed.
   lt_compile=`echo "$ac_compile" | $SED \
   -e 's:.*FLAGS}\{0,1\} :&$lt_compiler_flag :; t' \
   -e 's: [^ ]*conftest\.: $lt_compiler_flag&:; t' \
   -e 's:$: $lt_compiler_flag:'`
   (eval echo "\"\$as_me:16283: $lt_compile\"" >&5)
   (eval "$lt_compile" 2>conftest.err)
   ac_status=$?
   cat conftest.err >&5
   echo "$as_me:16287: \$? = $ac_status" >&5
   if (exit $ac_status) && test -s "$ac_outfile"; then
     # The compiler can only warn and ignore the option if not recognized
     # So say no if there are warnings other than the usual output.
     $echo "X$_lt_compiler_boilerplate" | $Xsed -e '/^$/d' >conftest.exp
     $SED '/^$/d; /^ *+/d' conftest.err >conftest.er2
     if test ! -s conftest.er2 || diff conftest.exp conftest.er2 >/dev/null; then
       lt_cv_prog_compiler_rtti_exceptions=yes
     fi
   fi
   $rm conftest*

fi
{ echo "$as_me:$LINENO: result: $lt_cv_prog_compiler_rtti_exceptions" >&5
echo "${ECHO_T}$lt_cv_prog_compiler_rtti_exceptions" >&6; }

if test x"$lt_cv_prog_compiler_rtti_exceptions" = xyes; then
    lt_prog_compiler_no_builtin_flag_GCJ="$lt_prog_compiler_no_builtin_flag_GCJ -fno-rtti -fno-exceptions"
else
    :
fi

fi

lt_prog_compiler_wl_GCJ=
lt_prog_compiler_pic_GCJ=
lt_prog_compiler_static_GCJ=

{ echo "$as_me:$LINENO: checking for $compiler option to produce PIC" >&5
echo $ECHO_N "checking for $compiler option to produce PIC... $ECHO_C" >&6; }

  if test "$GCC" = yes; then
    lt_prog_compiler_wl_GCJ='-Wl,'
    lt_prog_compiler_static_GCJ='-static'

    case $host_os in
      aix*)
      # All AIX code is PIC.
      if test "$host_cpu" = ia64; then
	# AIX 5 now supports IA64 processor
	lt_prog_compiler_static_GCJ='-Bstatic'
      fi
      ;;

    amigaos*)
      # FIXME: we need at least 68020 code to build shared libraries, but
      # adding the `-m68020' flag to GCC prevents building anything better,
      # like `-m68040'.
      lt_prog_compiler_pic_GCJ='-m68020 -resident32 -malways-restore-a4'
      ;;

    beos* | irix5* | irix6* | nonstopux* | osf3* | osf4* | osf5*)
      # PIC is the default for these OSes.
      ;;

    mingw* | cygwin* | pw32* | os2*)
      # This hack is so that the source file can tell whether it is being
      # built for inclusion in a dll (and should export symbols for example).
      # Although the cygwin gcc ignores -fPIC, still need this for old-style
      # (--disable-auto-import) libraries
      lt_prog_compiler_pic_GCJ='-DDLL_EXPORT'
      ;;

    darwin* | rhapsody*)
      # PIC is the default on this platform
      # Common symbols not allowed in MH_DYLIB files
      lt_prog_compiler_pic_GCJ='-fno-common'
      ;;

    interix[3-9]*)
      # Interix 3.x gcc -fpic/-fPIC options generate broken code.
      # Instead, we relocate shared libraries at runtime.
      ;;

    msdosdjgpp*)
      # Just because we use GCC doesn't mean we suddenly get shared libraries
      # on systems that don't support them.
      lt_prog_compiler_can_build_shared_GCJ=no
      enable_shared=no
      ;;

    sysv4*MP*)
      if test -d /usr/nec; then
	lt_prog_compiler_pic_GCJ=-Kconform_pic
      fi
      ;;

    hpux*)
      # PIC is the default for IA64 HP-UX and 64-bit HP-UX, but
      # not for PA HP-UX.
      case $host_cpu in
      hppa*64*|ia64*)
	# +Z the default
	;;
      *)
	lt_prog_compiler_pic_GCJ='-fPIC'
	;;
      esac
      ;;

    *)
      lt_prog_compiler_pic_GCJ='-fPIC'
      ;;
    esac
  else
    # PORTME Check for flag to pass linker flags through the system compiler.
    case $host_os in
    aix*)
      lt_prog_compiler_wl_GCJ='-Wl,'
      if test "$host_cpu" = ia64; then
	# AIX 5 now supports IA64 processor
	lt_prog_compiler_static_GCJ='-Bstatic'
      else
	lt_prog_compiler_static_GCJ='-bnso -bI:/lib/syscalls.exp'
      fi
      ;;
      darwin*)
        # PIC is the default on this platform
        # Common symbols not allowed in MH_DYLIB files
       case $cc_basename in
         xlc*)
         lt_prog_compiler_pic_GCJ='-qnocommon'
         lt_prog_compiler_wl_GCJ='-Wl,'
         ;;
       esac
       ;;

    mingw* | cygwin* | pw32* | os2*)
      # This hack is so that the source file can tell whether it is being
      # built for inclusion in a dll (and should export symbols for example).
      lt_prog_compiler_pic_GCJ='-DDLL_EXPORT'
      ;;

    hpux9* | hpux10* | hpux11*)
      lt_prog_compiler_wl_GCJ='-Wl,'
      # PIC is the default for IA64 HP-UX and 64-bit HP-UX, but
      # not for PA HP-UX.
      case $host_cpu in
      hppa*64*|ia64*)
	# +Z the default
	;;
      *)
	lt_prog_compiler_pic_GCJ='+Z'
	;;
      esac
      # Is there a better lt_prog_compiler_static that works with the bundled CC?
      lt_prog_compiler_static_GCJ='${wl}-a ${wl}archive'
      ;;

    irix5* | irix6* | nonstopux*)
      lt_prog_compiler_wl_GCJ='-Wl,'
      # PIC (with -KPIC) is the default.
      lt_prog_compiler_static_GCJ='-non_shared'
      ;;

    newsos6)
      lt_prog_compiler_pic_GCJ='-KPIC'
      lt_prog_compiler_static_GCJ='-Bstatic'
      ;;

    linux* | k*bsd*-gnu)
      case $cc_basename in
      icc* | ecc*)
	lt_prog_compiler_wl_GCJ='-Wl,'
	lt_prog_compiler_pic_GCJ='-KPIC'
	lt_prog_compiler_static_GCJ='-static'
        ;;
      pgcc* | pgf77* | pgf90* | pgf95*)
        # Portland Group compilers (*not* the Pentium gcc compiler,
	# which looks to be a dead project)
	lt_prog_compiler_wl_GCJ='-Wl,'
	lt_prog_compiler_pic_GCJ='-fpic'
	lt_prog_compiler_static_GCJ='-Bstatic'
        ;;
      ccc*)
        lt_prog_compiler_wl_GCJ='-Wl,'
        # All Alpha code is PIC.
        lt_prog_compiler_static_GCJ='-non_shared'
        ;;
      *)
        case `$CC -V 2>&1 | sed 5q` in
	*Sun\ C*)
	  # Sun C 5.9
	  lt_prog_compiler_pic_GCJ='-KPIC'
	  lt_prog_compiler_static_GCJ='-Bstatic'
	  lt_prog_compiler_wl_GCJ='-Wl,'
	  ;;
	*Sun\ F*)
	  # Sun Fortran 8.3 passes all unrecognized flags to the linker
	  lt_prog_compiler_pic_GCJ='-KPIC'
	  lt_prog_compiler_static_GCJ='-Bstatic'
	  lt_prog_compiler_wl_GCJ=''
	  ;;
	esac
	;;
      esac
      ;;

    osf3* | osf4* | osf5*)
      lt_prog_compiler_wl_GCJ='-Wl,'
      # All OSF/1 code is PIC.
      lt_prog_compiler_static_GCJ='-non_shared'
      ;;

    rdos*)
      lt_prog_compiler_static_GCJ='-non_shared'
      ;;

    solaris*)
      lt_prog_compiler_pic_GCJ='-KPIC'
      lt_prog_compiler_static_GCJ='-Bstatic'
      case $cc_basename in
      f77* | f90* | f95*)
	lt_prog_compiler_wl_GCJ='-Qoption ld ';;
      *)
	lt_prog_compiler_wl_GCJ='-Wl,';;
      esac
      ;;

    sunos4*)
      lt_prog_compiler_wl_GCJ='-Qoption ld '
      lt_prog_compiler_pic_GCJ='-PIC'
      lt_prog_compiler_static_GCJ='-Bstatic'
      ;;

    sysv4 | sysv4.2uw2* | sysv4.3*)
      lt_prog_compiler_wl_GCJ='-Wl,'
      lt_prog_compiler_pic_GCJ='-KPIC'
      lt_prog_compiler_static_GCJ='-Bstatic'
      ;;

    sysv4*MP*)
      if test -d /usr/nec ;then
	lt_prog_compiler_pic_GCJ='-Kconform_pic'
	lt_prog_compiler_static_GCJ='-Bstatic'
      fi
      ;;

    sysv5* | unixware* | sco3.2v5* | sco5v6* | OpenUNIX*)
      lt_prog_compiler_wl_GCJ='-Wl,'
      lt_prog_compiler_pic_GCJ='-KPIC'
      lt_prog_compiler_static_GCJ='-Bstatic'
      ;;

    unicos*)
      lt_prog_compiler_wl_GCJ='-Wl,'
      lt_prog_compiler_can_build_shared_GCJ=no
      ;;

    uts4*)
      lt_prog_compiler_pic_GCJ='-pic'
      lt_prog_compiler_static_GCJ='-Bstatic'
      ;;

    *)
      lt_prog_compiler_can_build_shared_GCJ=no
      ;;
    esac
  fi

{ echo "$as_me:$LINENO: result: $lt_prog_compiler_pic_GCJ" >&5
echo "${ECHO_T}$lt_prog_compiler_pic_GCJ" >&6; }

#
# Check to make sure the PIC flag actually works.
#
if test -n "$lt_prog_compiler_pic_GCJ"; then

{ echo "$as_me:$LINENO: checking if $compiler PIC flag $lt_prog_compiler_pic_GCJ works" >&5
echo $ECHO_N "checking if $compiler PIC flag $lt_prog_compiler_pic_GCJ works... $ECHO_C" >&6; }
if test "${lt_prog_compiler_pic_works_GCJ+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  lt_prog_compiler_pic_works_GCJ=no
  ac_outfile=conftest.$ac_objext
   echo "$lt_simple_compile_test_code" > conftest.$ac_ext
   lt_compiler_flag="$lt_prog_compiler_pic_GCJ"
   # Insert the option either (1) after the last *FLAGS variable, or
   # (2) before a word containing "conftest.", or (3) at the end.
   # Note that $ac_compile itself does not contain backslashes and begins
   # with a dollar sign (not a hyphen), so the echo should work correctly.
   # The option is referenced via a variable to avoid confusing sed.
   lt_compile=`echo "$ac_compile" | $SED \
   -e 's:.*FLAGS}\{0,1\} :&$lt_compiler_flag :; t' \
   -e 's: [^ ]*conftest\.: $lt_compiler_flag&:; t' \
   -e 's:$: $lt_compiler_flag:'`
   (eval echo "\"\$as_me:16573: $lt_compile\"" >&5)
   (eval "$lt_compile" 2>conftest.err)
   ac_status=$?
   cat conftest.err >&5
   echo "$as_me:16577: \$? = $ac_status" >&5
   if (exit $ac_status) && test -s "$ac_outfile"; then
     # The compiler can only warn and ignore the option if not recognized
     # So say no if there are warnings other than the usual output.
     $echo "X$_lt_compiler_boilerplate" | $Xsed -e '/^$/d' >conftest.exp
     $SED '/^$/d; /^ *+/d' conftest.err >conftest.er2
     if test ! -s conftest.er2 || diff conftest.exp conftest.er2 >/dev/null; then
       lt_prog_compiler_pic_works_GCJ=yes
     fi
   fi
   $rm conftest*

fi
{ echo "$as_me:$LINENO: result: $lt_prog_compiler_pic_works_GCJ" >&5
echo "${ECHO_T}$lt_prog_compiler_pic_works_GCJ" >&6; }

if test x"$lt_prog_compiler_pic_works_GCJ" = xyes; then
    case $lt_prog_compiler_pic_GCJ in
     "" | " "*) ;;
     *) lt_prog_compiler_pic_GCJ=" $lt_prog_compiler_pic_GCJ" ;;
     esac
else
    lt_prog_compiler_pic_GCJ=
     lt_prog_compiler_can_build_shared_GCJ=no
fi

fi
case $host_os in
  # For platforms which do not support PIC, -DPIC is meaningless:
  *djgpp*)
    lt_prog_compiler_pic_GCJ=
    ;;
  *)
    lt_prog_compiler_pic_GCJ="$lt_prog_compiler_pic_GCJ"
    ;;
esac

#
# Check to make sure the static flag actually works.
#
wl=$lt_prog_compiler_wl_GCJ eval lt_tmp_static_flag=\"$lt_prog_compiler_static_GCJ\"
{ echo "$as_me:$LINENO: checking if $compiler static flag $lt_tmp_static_flag works" >&5
echo $ECHO_N "checking if $compiler static flag $lt_tmp_static_flag works... $ECHO_C" >&6; }
if test "${lt_prog_compiler_static_works_GCJ+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  lt_prog_compiler_static_works_GCJ=no
   save_LDFLAGS="$LDFLAGS"
   LDFLAGS="$LDFLAGS $lt_tmp_static_flag"
   echo "$lt_simple_link_test_code" > conftest.$ac_ext
   if (eval $ac_link 2>conftest.err) && test -s conftest$ac_exeext; then
     # The linker can only warn and ignore the option if not recognized
     # So say no if there are warnings
     if test -s conftest.err; then
       # Append any errors to the config.log.
       cat conftest.err 1>&5
       $echo "X$_lt_linker_boilerplate" | $Xsed -e '/^$/d' > conftest.exp
       $SED '/^$/d; /^ *+/d' conftest.err >conftest.er2
       if diff conftest.exp conftest.er2 >/dev/null; then
         lt_prog_compiler_static_works_GCJ=yes
       fi
     else
       lt_prog_compiler_static_works_GCJ=yes
     fi
   fi
   $rm conftest*
   LDFLAGS="$save_LDFLAGS"

fi
{ echo "$as_me:$LINENO: result: $lt_prog_compiler_static_works_GCJ" >&5
echo "${ECHO_T}$lt_prog_compiler_static_works_GCJ" >&6; }

if test x"$lt_prog_compiler_static_works_GCJ" = xyes; then
    :
else
    lt_prog_compiler_static_GCJ=
fi


{ echo "$as_me:$LINENO: checking if $compiler supports -c -o file.$ac_objext" >&5
echo $ECHO_N "checking if $compiler supports -c -o file.$ac_objext... $ECHO_C" >&6; }
if test "${lt_cv_prog_compiler_c_o_GCJ+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  lt_cv_prog_compiler_c_o_GCJ=no
   $rm -r conftest 2>/dev/null
   mkdir conftest
   cd conftest
   mkdir out
   echo "$lt_simple_compile_test_code" > conftest.$ac_ext

   lt_compiler_flag="-o out/conftest2.$ac_objext"
   # Insert the option either (1) after the last *FLAGS variable, or
   # (2) before a word containing "conftest.", or (3) at the end.
   # Note that $ac_compile itself does not contain backslashes and begins
   # with a dollar sign (not a hyphen), so the echo should work correctly.
   lt_compile=`echo "$ac_compile" | $SED \
   -e 's:.*FLAGS}\{0,1\} :&$lt_compiler_flag :; t' \
   -e 's: [^ ]*conftest\.: $lt_compiler_flag&:; t' \
   -e 's:$: $lt_compiler_flag:'`
   (eval echo "\"\$as_me:16677: $lt_compile\"" >&5)
   (eval "$lt_compile" 2>out/conftest.err)
   ac_status=$?
   cat out/conftest.err >&5
   echo "$as_me:16681: \$? = $ac_status" >&5
   if (exit $ac_status) && test -s out/conftest2.$ac_objext
   then
     # The compiler can only warn and ignore the option if not recognized
     # So say no if there are warnings
     $echo "X$_lt_compiler_boilerplate" | $Xsed -e '/^$/d' > out/conftest.exp
     $SED '/^$/d; /^ *+/d' out/conftest.err >out/conftest.er2
     if test ! -s out/conftest.er2 || diff out/conftest.exp out/conftest.er2 >/dev/null; then
       lt_cv_prog_compiler_c_o_GCJ=yes
     fi
   fi
   chmod u+w . 2>&5
   $rm conftest*
   # SGI C++ compiler will create directory out/ii_files/ for
   # template instantiation
   test -d out/ii_files && $rm out/ii_files/* && rmdir out/ii_files
   $rm out/* && rmdir out
   cd ..
   rmdir conftest
   $rm conftest*

fi
{ echo "$as_me:$LINENO: result: $lt_cv_prog_compiler_c_o_GCJ" >&5
echo "${ECHO_T}$lt_cv_prog_compiler_c_o_GCJ" >&6; }


hard_links="nottested"
if test "$lt_cv_prog_compiler_c_o_GCJ" = no && test "$need_locks" != no; then
  # do not overwrite the value of need_locks provided by the user
  { echo "$as_me:$LINENO: checking if we can lock with hard links" >&5
echo $ECHO_N "checking if we can lock with hard links... $ECHO_C" >&6; }
  hard_links=yes
  $rm conftest*
  ln conftest.a conftest.b 2>/dev/null && hard_links=no
  touch conftest.a
  ln conftest.a conftest.b 2>&5 || hard_links=no
  ln conftest.a conftest.b 2>/dev/null && hard_links=no
  { echo "$as_me:$LINENO: result: $hard_links" >&5
echo "${ECHO_T}$hard_links" >&6; }
  if test "$hard_links" = no; then
    { echo "$as_me:$LINENO: WARNING: \`$CC' does not support \`-c -o', so \`make -j' may be unsafe" >&5
echo "$as_me: WARNING: \`$CC' does not support \`-c -o', so \`make -j' may be unsafe" >&2;}
    need_locks=warn
  fi
else
  need_locks=no
fi

{ echo "$as_me:$LINENO: checking whether the $compiler linker ($LD) supports shared libraries" >&5
echo $ECHO_N "checking whether the $compiler linker ($LD) supports shared libraries... $ECHO_C" >&6; }

  runpath_var=
  allow_undefined_flag_GCJ=
  enable_shared_with_static_runtimes_GCJ=no
  archive_cmds_GCJ=
  archive_expsym_cmds_GCJ=
  old_archive_From_new_cmds_GCJ=
  old_archive_from_expsyms_cmds_GCJ=
  export_dynamic_flag_spec_GCJ=
  whole_archive_flag_spec_GCJ=
  thread_safe_flag_spec_GCJ=
  hardcode_libdir_flag_spec_GCJ=
  hardcode_libdir_flag_spec_ld_GCJ=
  hardcode_libdir_separator_GCJ=
  hardcode_direct_GCJ=no
  hardcode_minus_L_GCJ=no
  hardcode_shlibpath_var_GCJ=unsupported
  link_all_deplibs_GCJ=unknown
  hardcode_automatic_GCJ=no
  module_cmds_GCJ=
  module_expsym_cmds_GCJ=
  always_export_symbols_GCJ=no
  export_symbols_cmds_GCJ='$NM $libobjs $convenience | $global_symbol_pipe | $SED '\''s/.* //'\'' | sort | uniq > $export_symbols'
  # include_expsyms should be a list of space-separated symbols to be *always*
  # included in the symbol list
  include_expsyms_GCJ=
  # exclude_expsyms can be an extended regexp of symbols to exclude
  # it will be wrapped by ` (' and `)$', so one must not match beginning or
  # end of line.  Example: `a|bc|.*d.*' will exclude the symbols `a' and `bc',
  # as well as any symbol that contains `d'.
  exclude_expsyms_GCJ="_GLOBAL_OFFSET_TABLE_"
  # Although _GLOBAL_OFFSET_TABLE_ is a valid symbol C name, most a.out
  # platforms (ab)use it in PIC code, but their linkers get confused if
  # the symbol is explicitly referenced.  Since portable code cannot
  # rely on this symbol name, it's probably fine to never include it in
  # preloaded symbol tables.
  extract_expsyms_cmds=
  # Just being paranoid about ensuring that cc_basename is set.
  for cc_temp in $compiler""; do
  case $cc_temp in
    compile | *[\\/]compile | ccache | *[\\/]ccache ) ;;
    distcc | *[\\/]distcc | purify | *[\\/]purify ) ;;
    \-*) ;;
    *) break;;
  esac
done
cc_basename=`$echo "X$cc_temp" | $Xsed -e 's%.*/%%' -e "s%^$host_alias-%%"`

  case $host_os in
  cygwin* | mingw* | pw32*)
    # FIXME: the MSVC++ port hasn't been tested in a loooong time
    # When not using gcc, we currently assume that we are using
    # Microsoft Visual C++.
    if test "$GCC" != yes; then
      with_gnu_ld=no
    fi
    ;;
  interix*)
    # we just hope/assume this is gcc and not c89 (= MSVC++)
    with_gnu_ld=yes
    ;;
  openbsd*)
    with_gnu_ld=no
    ;;
  esac

  ld_shlibs_GCJ=yes
  if test "$with_gnu_ld" = yes; then
    # If archive_cmds runs LD, not CC, wlarc should be empty
    wlarc='${wl}'

    # Set some defaults for GNU ld with shared library support. These
    # are reset later if shared libraries are not supported. Putting them
    # here allows them to be overridden if necessary.
    runpath_var=LD_RUN_PATH
    hardcode_libdir_flag_spec_GCJ='${wl}--rpath ${wl}$libdir'
    export_dynamic_flag_spec_GCJ='${wl}--export-dynamic'
    # ancient GNU ld didn't support --whole-archive et. al.
    if $LD --help 2>&1 | grep 'no-whole-archive' > /dev/null; then
	whole_archive_flag_spec_GCJ="$wlarc"'--whole-archive$convenience '"$wlarc"'--no-whole-archive'
      else
  	whole_archive_flag_spec_GCJ=
    fi
    supports_anon_versioning=no
    case `$LD -v 2>/dev/null` in
      *\ [01].* | *\ 2.[0-9].* | *\ 2.10.*) ;; # catch versions < 2.11
      *\ 2.11.93.0.2\ *) supports_anon_versioning=yes ;; # RH7.3 ...
      *\ 2.11.92.0.12\ *) supports_anon_versioning=yes ;; # Mandrake 8.2 ...
      *\ 2.11.*) ;; # other 2.11 versions
      *) supports_anon_versioning=yes ;;
    esac

    # See if GNU ld supports shared libraries.
    case $host_os in
    aix3* | aix4* | aix5*)
      # On AIX/PPC, the GNU linker is very broken
      if test "$host_cpu" != ia64; then
	ld_shlibs_GCJ=no
	cat <<EOF 1>&2

*** Warning: the GNU linker, at least up to release 2.9.1, is reported
*** to be unable to reliably create shared libraries on AIX.
*** Therefore, libtool is disabling shared libraries support.  If you
*** really care for shared libraries, you may want to modify your PATH
*** so that a non-GNU linker is found, and then restart.

EOF
      fi
      ;;

    amigaos*)
      archive_cmds_GCJ='$rm $output_objdir/a2ixlibrary.data~$echo "#define NAME $libname" > $output_objdir/a2ixlibrary.data~$echo "#define LIBRARY_ID 1" >> $output_objdir/a2ixlibrary.data~$echo "#define VERSION $major" >> $output_objdir/a2ixlibrary.data~$echo "#define REVISION $revision" >> $output_objdir/a2ixlibrary.data~$AR $AR_FLAGS $lib $libobjs~$RANLIB $lib~(cd $output_objdir && a2ixlibrary -32)'
      hardcode_libdir_flag_spec_GCJ='-L$libdir'
      hardcode_minus_L_GCJ=yes

      # Samuel A. Falvo II <kc5tja@dolphin.openprojects.net> reports
      # that the semantics of dynamic libraries on AmigaOS, at least up
      # to version 4, is to share data among multiple programs linked
      # with the same dynamic library.  Since this doesn't match the
      # behavior of shared libraries on other platforms, we can't use
      # them.
      ld_shlibs_GCJ=no
      ;;

    beos*)
      if $LD --help 2>&1 | grep ': supported targets:.* elf' > /dev/null; then
	allow_undefined_flag_GCJ=unsupported
	# Joseph Beckenbach <jrb3@best.com> says some releases of gcc
	# support --undefined.  This deserves some investigation.  FIXME
	archive_cmds_GCJ='$CC -nostart $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname -o $lib'
      else
	ld_shlibs_GCJ=no
      fi
      ;;

    cygwin* | mingw* | pw32*)
      # _LT_AC_TAGVAR(hardcode_libdir_flag_spec, GCJ) is actually meaningless,
      # as there is no search path for DLLs.
      hardcode_libdir_flag_spec_GCJ='-L$libdir'
      allow_undefined_flag_GCJ=unsupported
      always_export_symbols_GCJ=no
      enable_shared_with_static_runtimes_GCJ=yes
      export_symbols_cmds_GCJ='$NM $libobjs $convenience | $global_symbol_pipe | $SED -e '\''/^[BCDGRS][ ]/s/.*[ ]\([^ ]*\)/\1 DATA/'\'' -e '\''/^[AITW][ ]/s/.*[ ]//'\'' | sort | uniq > $export_symbols'

      if $LD --help 2>&1 | grep 'auto-import' > /dev/null; then
        archive_cmds_GCJ='$CC -shared $libobjs $deplibs $compiler_flags -o $output_objdir/$soname ${wl}--enable-auto-image-base -Xlinker --out-implib -Xlinker $lib'
	# If the export-symbols file already is a .def file (1st line
	# is EXPORTS), use it as is; otherwise, prepend...
	archive_expsym_cmds_GCJ='if test "x`$SED 1q $export_symbols`" = xEXPORTS; then
	  cp $export_symbols $output_objdir/$soname.def;
	else
	  echo EXPORTS > $output_objdir/$soname.def;
	  cat $export_symbols >> $output_objdir/$soname.def;
	fi~
	$CC -shared $output_objdir/$soname.def $libobjs $deplibs $compiler_flags -o $output_objdir/$soname ${wl}--enable-auto-image-base -Xlinker --out-implib -Xlinker $lib'
      else
	ld_shlibs_GCJ=no
      fi
      ;;

    interix[3-9]*)
      hardcode_direct_GCJ=no
      hardcode_shlibpath_var_GCJ=no
      hardcode_libdir_flag_spec_GCJ='${wl}-rpath,$libdir'
      export_dynamic_flag_spec_GCJ='${wl}-E'
      # Hack: On Interix 3.x, we cannot compile PIC because of a broken gcc.
      # Instead, shared libraries are loaded at an image base (0x10000000 by
      # default) and relocated if they conflict, which is a slow very memory
      # consuming and fragmenting process.  To avoid this, we pick a random,
      # 256 KiB-aligned image base between 0x50000000 and 0x6FFC0000 at link
      # time.  Moving up from 0x10000000 also allows more sbrk(2) space.
      archive_cmds_GCJ='$CC -shared $pic_flag $libobjs $deplibs $compiler_flags ${wl}-h,$soname ${wl}--image-base,`expr ${RANDOM-$$} % 4096 / 2 \* 262144 + 1342177280` -o $lib'
      archive_expsym_cmds_GCJ='sed "s,^,_," $export_symbols >$output_objdir/$soname.expsym~$CC -shared $pic_flag $libobjs $deplibs $compiler_flags ${wl}-h,$soname ${wl}--retain-symbols-file,$output_objdir/$soname.expsym ${wl}--image-base,`expr ${RANDOM-$$} % 4096 / 2 \* 262144 + 1342177280` -o $lib'
      ;;

    gnu* | linux* | k*bsd*-gnu)
      if $LD --help 2>&1 | grep ': supported targets:.* elf' > /dev/null; then
	tmp_addflag=
	case $cc_basename,$host_cpu in
	pgcc*)				# Portland Group C compiler
	  whole_archive_flag_spec_GCJ='${wl}--whole-archive`for conv in $convenience\"\"; do test  -n \"$conv\" && new_convenience=\"$new_convenience,$conv\"; done; $echo \"$new_convenience\"` ${wl}--no-whole-archive'
	  tmp_addflag=' $pic_flag'
	  ;;
	pgf77* | pgf90* | pgf95*)	# Portland Group f77 and f90 compilers
	  whole_archive_flag_spec_GCJ='${wl}--whole-archive`for conv in $convenience\"\"; do test  -n \"$conv\" && new_convenience=\"$new_convenience,$conv\"; done; $echo \"$new_convenience\"` ${wl}--no-whole-archive'
	  tmp_addflag=' $pic_flag -Mnomain' ;;
	ecc*,ia64* | icc*,ia64*)		# Intel C compiler on ia64
	  tmp_addflag=' -i_dynamic' ;;
	efc*,ia64* | ifort*,ia64*)	# Intel Fortran compiler on ia64
	  tmp_addflag=' -i_dynamic -nofor_main' ;;
	ifc* | ifort*)			# Intel Fortran compiler
	  tmp_addflag=' -nofor_main' ;;
	esac
	case `$CC -V 2>&1 | sed 5q` in
	*Sun\ C*)			# Sun C 5.9
	  whole_archive_flag_spec_GCJ='${wl}--whole-archive`new_convenience=; for conv in $convenience\"\"; do test -z \"$conv\" || new_convenience=\"$new_convenience,$conv\"; done; $echo \"$new_convenience\"` ${wl}--no-whole-archive'
	  tmp_sharedflag='-G' ;;
	*Sun\ F*)			# Sun Fortran 8.3
	  tmp_sharedflag='-G' ;;
	*)
	  tmp_sharedflag='-shared' ;;
	esac
	archive_cmds_GCJ='$CC '"$tmp_sharedflag""$tmp_addflag"' $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname -o $lib'

	if test $supports_anon_versioning = yes; then
	  archive_expsym_cmds_GCJ='$echo "{ global:" > $output_objdir/$libname.ver~
  cat $export_symbols | sed -e "s/\(.*\)/\1;/" >> $output_objdir/$libname.ver~
  $echo "local: *; };" >> $output_objdir/$libname.ver~
	  $CC '"$tmp_sharedflag""$tmp_addflag"' $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname ${wl}-version-script ${wl}$output_objdir/$libname.ver -o $lib'
	fi
      else
	ld_shlibs_GCJ=no
      fi
      ;;

    netbsd*)
      if echo __ELF__ | $CC -E - | grep __ELF__ >/dev/null; then
	archive_cmds_GCJ='$LD -Bshareable $libobjs $deplibs $linker_flags -o $lib'
	wlarc=
      else
	archive_cmds_GCJ='$CC -shared $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname -o $lib'
	archive_expsym_cmds_GCJ='$CC -shared $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname ${wl}-retain-symbols-file $wl$export_symbols -o $lib'
      fi
      ;;

    solaris*)
      if $LD -v 2>&1 | grep 'BFD 2\.8' > /dev/null; then
	ld_shlibs_GCJ=no
	cat <<EOF 1>&2

*** Warning: The releases 2.8.* of the GNU linker cannot reliably
*** create shared libraries on Solaris systems.  Therefore, libtool
*** is disabling shared libraries support.  We urge you to upgrade GNU
*** binutils to release 2.9.1 or newer.  Another option is to modify
*** your PATH or compiler configuration so that the native linker is
*** used, and then restart.

EOF
      elif $LD --help 2>&1 | grep ': supported targets:.* elf' > /dev/null; then
	archive_cmds_GCJ='$CC -shared $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname -o $lib'
	archive_expsym_cmds_GCJ='$CC -shared $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname ${wl}-retain-symbols-file $wl$export_symbols -o $lib'
      else
	ld_shlibs_GCJ=no
      fi
      ;;

    sysv5* | sco3.2v5* | sco5v6* | unixware* | OpenUNIX*)
      case `$LD -v 2>&1` in
        *\ [01].* | *\ 2.[0-9].* | *\ 2.1[0-5].*)
	ld_shlibs_GCJ=no
	cat <<_LT_EOF 1>&2

*** Warning: Releases of the GNU linker prior to 2.16.91.0.3 can not
*** reliably create shared libraries on SCO systems.  Therefore, libtool
*** is disabling shared libraries support.  We urge you to upgrade GNU
*** binutils to release 2.16.91.0.3 or newer.  Another option is to modify
*** your PATH or compiler configuration so that the native linker is
*** used, and then restart.

_LT_EOF
	;;
	*)
	  if $LD --help 2>&1 | grep ': supported targets:.* elf' > /dev/null; then
	    hardcode_libdir_flag_spec_GCJ='`test -z "$SCOABSPATH" && echo ${wl}-rpath,$libdir`'
	    archive_cmds_GCJ='$CC -shared $libobjs $deplibs $compiler_flags ${wl}-soname,\${SCOABSPATH:+${install_libdir}/}$soname -o $lib'
	    archive_expsym_cmds_GCJ='$CC -shared $libobjs $deplibs $compiler_flags ${wl}-soname,\${SCOABSPATH:+${install_libdir}/}$soname,-retain-symbols-file,$export_symbols -o $lib'
	  else
	    ld_shlibs_GCJ=no
	  fi
	;;
      esac
      ;;

    sunos4*)
      archive_cmds_GCJ='$LD -assert pure-text -Bshareable -o $lib $libobjs $deplibs $linker_flags'
      wlarc=
      hardcode_direct_GCJ=yes
      hardcode_shlibpath_var_GCJ=no
      ;;

    *)
      if $LD --help 2>&1 | grep ': supported targets:.* elf' > /dev/null; then
	archive_cmds_GCJ='$CC -shared $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname -o $lib'
	archive_expsym_cmds_GCJ='$CC -shared $libobjs $deplibs $compiler_flags ${wl}-soname $wl$soname ${wl}-retain-symbols-file $wl$export_symbols -o $lib'
      else
	ld_shlibs_GCJ=no
      fi
      ;;
    esac

    if test "$ld_shlibs_GCJ" = no; then
      runpath_var=
      hardcode_libdir_flag_spec_GCJ=
      export_dynamic_flag_spec_GCJ=
      whole_archive_flag_spec_GCJ=
    fi
  else
    # PORTME fill in a description of your system's linker (not GNU ld)
    case $host_os in
    aix3*)
      allow_undefined_flag_GCJ=unsupported
      always_export_symbols_GCJ=yes
      archive_expsym_cmds_GCJ='$LD -o $output_objdir/$soname $libobjs $deplibs $linker_flags -bE:$export_symbols -T512 -H512 -bM:SRE~$AR $AR_FLAGS $lib $output_objdir/$soname'
      # Note: this linker hardcodes the directories in LIBPATH if there
      # are no directories specified by -L.
      hardcode_minus_L_GCJ=yes
      if test "$GCC" = yes && test -z "$lt_prog_compiler_static"; then
	# Neither direct hardcoding nor static linking is supported with a
	# broken collect2.
	hardcode_direct_GCJ=unsupported
      fi
      ;;

    aix4* | aix5*)
      if test "$host_cpu" = ia64; then
	# On IA64, the linker does run time linking by default, so we don't
	# have to do anything special.
	aix_use_runtimelinking=no
	exp_sym_flag='-Bexport'
	no_entry_flag=""
      else
	# If we're using GNU nm, then we don't want the "-C" option.
	# -C means demangle to AIX nm, but means don't demangle with GNU nm
	if $NM -V 2>&1 | grep 'GNU' > /dev/null; then
	  export_symbols_cmds_GCJ='$NM -Bpg $libobjs $convenience | awk '\''{ if (((\$2 == "T") || (\$2 == "D") || (\$2 == "B")) && (substr(\$3,1,1) != ".")) { print \$3 } }'\'' | sort -u > $export_symbols'
	else
	  export_symbols_cmds_GCJ='$NM -BCpg $libobjs $convenience | awk '\''{ if (((\$2 == "T") || (\$2 == "D") || (\$2 == "B")) && (substr(\$3,1,1) != ".")) { print \$3 } }'\'' | sort -u > $export_symbols'
	fi
	aix_use_runtimelinking=no

	# Test if we are trying to use run time linking or normal
	# AIX style linking. If -brtl is somewhere in LDFLAGS, we
	# need to do runtime linking.
	case $host_os in aix4.[23]|aix4.[23].*|aix5*)
	  for ld_flag in $LDFLAGS; do
  	  if (test $ld_flag = "-brtl" || test $ld_flag = "-Wl,-brtl"); then
  	    aix_use_runtimelinking=yes
  	    break
  	  fi
	  done
	  ;;
	esac

	exp_sym_flag='-bexport'
	no_entry_flag='-bnoentry'
      fi

      # When large executables or shared objects are built, AIX ld can
      # have problems creating the table of contents.  If linking a library
      # or program results in "error TOC overflow" add -mminimal-toc to
      # CXXFLAGS/CFLAGS for g++/gcc.  In the cases where that is not
      # enough to fix the problem, add -Wl,-bbigtoc to LDFLAGS.

      archive_cmds_GCJ=''
      hardcode_direct_GCJ=yes
      hardcode_libdir_separator_GCJ=':'
      link_all_deplibs_GCJ=yes

      if test "$GCC" = yes; then
	case $host_os in aix4.[012]|aix4.[012].*)
	# We only want to do this on AIX 4.2 and lower, the check
	# below for broken collect2 doesn't work under 4.3+
	  collect2name=`${CC} -print-prog-name=collect2`
	  if test -f "$collect2name" && \
  	   strings "$collect2name" | grep resolve_lib_name >/dev/null
	  then
  	  # We have reworked collect2
  	  :
	  else
  	  # We have old collect2
  	  hardcode_direct_GCJ=unsupported
  	  # It fails to find uninstalled libraries when the uninstalled
  	  # path is not listed in the libpath.  Setting hardcode_minus_L
  	  # to unsupported forces relinking
  	  hardcode_minus_L_GCJ=yes
  	  hardcode_libdir_flag_spec_GCJ='-L$libdir'
  	  hardcode_libdir_separator_GCJ=
	  fi
	  ;;
	esac
	shared_flag='-shared'
	if test "$aix_use_runtimelinking" = yes; then
	  shared_flag="$shared_flag "'${wl}-G'
	fi
      else
	# not using gcc
	if test "$host_cpu" = ia64; then
  	# VisualAge C++, Version 5.5 for AIX 5L for IA-64, Beta 3 Release
  	# chokes on -Wl,-G. The following line is correct:
	  shared_flag='-G'
	else
	  if test "$aix_use_runtimelinking" = yes; then
	    shared_flag='${wl}-G'
	  else
	    shared_flag='${wl}-bM:SRE'
	  fi
	fi
      fi

      # It seems that -bexpall does not export symbols beginning with
      # underscore (_), so it is better to generate a list of symbols to export.
      always_export_symbols_GCJ=yes
      if test "$aix_use_runtimelinking" = yes; then
	# Warning - without using the other runtime loading flags (-brtl),
	# -berok will link without error, but may produce a broken library.
	allow_undefined_flag_GCJ='-berok'
       # Determine the default libpath from the value encoded in an empty executable.
       cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

int
main ()
{

  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_c_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest$ac_exeext &&
       $as_test_x conftest$ac_exeext; then

lt_aix_libpath_sed='
    /Import File Strings/,/^$/ {
	/^0/ {
	    s/^0  *\(.*\)$/\1/
	    p
	}
    }'
aix_libpath=`dump -H conftest$ac_exeext 2>/dev/null | $SED -n -e "$lt_aix_libpath_sed"`
# Check for a 64-bit object if we didn't find anything.
if test -z "$aix_libpath"; then
  aix_libpath=`dump -HX64 conftest$ac_exeext 2>/dev/null | $SED -n -e "$lt_aix_libpath_sed"`
fi
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5


fi

rm -f core conftest.err conftest.$ac_objext conftest_ipa8_conftest.oo \
      conftest$ac_exeext conftest.$ac_ext
if test -z "$aix_libpath"; then aix_libpath="/usr/lib:/lib"; fi

       hardcode_libdir_flag_spec_GCJ='${wl}-blibpath:$libdir:'"$aix_libpath"
	archive_expsym_cmds_GCJ="\$CC"' -o $output_objdir/$soname $libobjs $deplibs '"\${wl}$no_entry_flag"' $compiler_flags `if test "x${allow_undefined_flag}" != "x"; then echo "${wl}${allow_undefined_flag}"; else :; fi` '"\${wl}$exp_sym_flag:\$export_symbols $shared_flag"
       else
	if test "$host_cpu" = ia64; then
	  hardcode_libdir_flag_spec_GCJ='${wl}-R $libdir:/usr/lib:/lib'
	  allow_undefined_flag_GCJ="-z nodefs"
	  archive_expsym_cmds_GCJ="\$CC $shared_flag"' -o $output_objdir/$soname $libobjs $deplibs '"\${wl}$no_entry_flag"' $compiler_flags ${wl}${allow_undefined_flag} '"\${wl}$exp_sym_flag:\$export_symbols"
	else
	 # Determine the default libpath from the value encoded in an empty executable.
	 cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

int
main ()
{

  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && {
	 test -z "$ac_c_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest$ac_exeext &&
       $as_test_x conftest$ac_exeext; then

lt_aix_libpath_sed='
    /Import File Strings/,/^$/ {
	/^0/ {
	    s/^0  *\(.*\)$/\1/
	    p
	}
    }'
aix_libpath=`dump -H conftest$ac_exeext 2>/dev/null | $SED -n -e "$lt_aix_libpath_sed"`
# Check for a 64-bit object if we didn't find anything.
if test -z "$aix_libpath"; then
  aix_libpath=`dump -HX64 conftest$ac_exeext 2>/dev/null | $SED -n -e "$lt_aix_libpath_sed"`
fi
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5


fi

rm -f core conftest.err conftest.$ac_objext conftest_ipa8_conftest.oo \
      conftest$ac_exeext conftest.$ac_ext
if test -z "$aix_libpath"; then aix_libpath="/usr/lib:/lib"; fi

	 hardcode_libdir_flag_spec_GCJ='${wl}-blibpath:$libdir:'"$aix_libpath"
	  # Warning - without using the other run time loading flags,
	  # -berok will link without error, but may produce a broken library.
	  no_undefined_flag_GCJ=' ${wl}-bernotok'
	  allow_undefined_flag_GCJ=' ${wl}-berok'
	  # Exported symbols can be pulled into shared objects from archives
	  whole_archive_flag_spec_GCJ='$convenience'
	  archive_cmds_need_lc_GCJ=yes
	  # This is similar to how AIX traditionally builds its shared libraries.
	  archive_expsym_cmds_GCJ="\$CC $shared_flag"' -o $output_objdir/$soname $libobjs $deplibs ${wl}-bnoentry $compiler_flags ${wl}-bE:$export_symbols${allow_undefined_flag}~$AR $AR_FLAGS $output_objdir/$libname$release.a $output_objdir/$soname'
	fi
      fi
      ;;

    amigaos*)
      archive_cmds_GCJ='$rm $output_objdir/a2ixlibrary.data~$echo "#define NAME $libname" > $output_objdir/a2ixlibrary.data~$echo "#define LIBRARY_ID 1" >> $output_objdir/a2ixlibrary.data~$echo "#define VERSION $major" >> $output_objdir/a2ixlibrary.data~$echo "#define REVISION $revision" >> $output_objdir/a2ixlibrary.data~$AR $AR_FLAGS $lib $libobjs~$RANLIB $lib~(cd $output_objdir && a2ixlibrary -32)'
      hardcode_libdir_flag_spec_GCJ='-L$libdir'
      hardcode_minus_L_GCJ=yes
      # see comment about different semantics on the GNU ld section
      ld_shlibs_GCJ=no
      ;;

    bsdi[45]*)
      export_dynamic_flag_spec_GCJ=-rdynamic
      ;;

    cygwin* | mingw* | pw32*)
      # When not using gcc, we currently assume that we are using
      # Microsoft Visual C++.
      # hardcode_libdir_flag_spec is actually meaningless, as there is
      # no search path for DLLs.
      hardcode_libdir_flag_spec_GCJ=' '
      allow_undefined_flag_GCJ=unsupported
      # Tell ltmain to make .lib files, not .a files.
      libext=lib
      # Tell ltmain to make .dll files, not .so files.
      shrext_cmds=".dll"
      # FIXME: Setting linknames here is a bad hack.
      archive_cmds_GCJ='$CC -o $lib $libobjs $compiler_flags `echo "$deplibs" | $SED -e '\''s/ -lc$//'\''` -link -dll~linknames='
      # The linker will automatically build a .lib file if we build a DLL.
      old_archive_From_new_cmds_GCJ='true'
      # FIXME: Should let the user specify the lib program.
      old_archive_cmds_GCJ='lib -OUT:$oldlib$oldobjs$old_deplibs'
      fix_srcfile_path_GCJ='`cygpath -w "$srcfile"`'
      enable_shared_with_static_runtimes_GCJ=yes
      ;;

    darwin* | rhapsody*)
      case $host_os in
        rhapsody* | darwin1.[012])
         allow_undefined_flag_GCJ='${wl}-undefined ${wl}suppress'
         ;;
       *) # Darwin 1.3 on
         if test -z ${MACOSX_DEPLOYMENT_TARGET} ; then
           allow_undefined_flag_GCJ='${wl}-flat_namespace ${wl}-undefined ${wl}suppress'
         else
           case ${MACOSX_DEPLOYMENT_TARGET} in
             10.[012])
               allow_undefined_flag_GCJ='${wl}-flat_namespace ${wl}-undefined ${wl}suppress'
               ;;
             10.*)
               allow_undefined_flag_GCJ='${wl}-undefined ${wl}dynamic_lookup'
               ;;
           esac
         fi
         ;;
      esac
      archive_cmds_need_lc_GCJ=no
      hardcode_direct_GCJ=no
      hardcode_automatic_GCJ=yes
      hardcode_shlibpath_var_GCJ=unsupported
      whole_archive_flag_spec_GCJ=''
      link_all_deplibs_GCJ=yes
    if test "$GCC" = yes ; then
    	output_verbose_link_cmd='echo'
        archive_cmds_GCJ='$CC -dynamiclib $allow_undefined_flag -o $lib $libobjs $deplibs $compiler_flags -install_name $rpath/$soname $verstring'
      module_cmds_GCJ='$CC $allow_undefined_flag -o $lib -bundle $libobjs $deplibs$compiler_flags'
      # Don't fix this by using the ld -exported_symbols_list flag, it doesn't exist in older darwin lds
      archive_expsym_cmds_GCJ='sed -e "s,#.*,," -e "s,^[    ]*,," -e "s,^\(..*\),_&," < $export_symbols > $output_objdir/${libname}-symbols.expsym~$CC -dynamiclib $allow_undefined_flag -o $lib $libobjs $deplibs $compiler_flags -install_name $rpath/$soname $verstring~nmedit -s $output_objdir/${libname}-symbols.expsym ${lib}'
      module_expsym_cmds_GCJ='sed -e "s,#.*,," -e "s,^[    ]*,," -e "s,^\(..*\),_&," < $export_symbols > $output_objdir/${libname}-symbols.expsym~$CC $allow_undefined_flag  -o $lib -bundle $libobjs $deplibs$compiler_flags~nmedit -s $output_objdir/${libname}-symbols.expsym ${lib}'
    else
      case $cc_basename in
        xlc*)
         output_verbose_link_cmd='echo'
         archive_cmds_GCJ='$CC -qmkshrobj $allow_undefined_flag -o $lib $libobjs $deplibs $compiler_flags ${wl}-install_name ${wl}`echo $rpath/$soname` $xlcverstring'
         module_cmds_GCJ='$CC $allow_undefined_flag -o $lib -bundle $libobjs $deplibs$compiler_flags'
          # Don't fix this by using the ld -exported_symbols_list flag, it doesn't exist in older darwin lds
         archive_expsym_cmds_GCJ='sed -e "s,#.*,," -e "s,^[    ]*,," -e "s,^\(..*\),_&," < $export_symbols > $output_objdir/${libname}-symbols.expsym~$CC -qmkshrobj $allow_undefined_flag -o $lib $libobjs $deplibs $compiler_flags ${wl}-install_name ${wl}$rpath/$soname $xlcverstring~nmedit -s $output_objdir/${libname}-symbols.expsym ${lib}'
          module_expsym_cmds_GCJ='sed -e "s,#.*,," -e "s,^[    ]*,," -e "s,^\(..*\),_&," < $export_symbols > $output_objdir/${libname}-symbols.expsym~$CC $allow_undefined_flag  -o $lib -bundle $libobjs $deplibs$compiler_flags~nmedit -s $output_objdir/${libname}-symbols.expsym ${lib}'
          ;;
       *)
         ld_shlibs_GCJ=no
          ;;
      esac
    fi
      ;;

    dgux*)
      archive_cmds_GCJ='$LD -G -h $soname -o $lib $libobjs $deplibs $linker_flags'
      hardcode_libdir_flag_spec_GCJ='-L$libdir'
      hardcode_shlibpath_var_GCJ=no
      ;;

    freebsd1*)
      ld_shlibs_GCJ=no
      ;;

    # FreeBSD 2.2.[012] allows us to include c++rt0.o to get C++ constructor
    # support.  Future versions do this automatically, but an explicit c++rt0.o
    # does not break anything, and helps significantly (at the cost of a little
    # extra space).
    freebsd2.2*)
      archive_cmds_GCJ='$LD -Bshareable -o $lib $libobjs $deplibs $linker_flags /usr/lib/c++rt0.o'
      hardcode_libdir_flag_spec_GCJ='-R$libdir'
      hardcode_direct_GCJ=yes
      hardcode_shlibpath_var_GCJ=no
      ;;

    # Unfortunately, older versions of FreeBSD 2 do not have this feature.
    freebsd2*)
      archive_cmds_GCJ='$LD -Bshareable -o $lib $libobjs $deplibs $linker_flags'
      hardcode_direct_GCJ=yes
      hardcode_minus_L_GCJ=yes
      hardcode_shlibpath_var_GCJ=no
      ;;

    # FreeBSD 3 and greater uses gcc -shared to do shared libraries.
    freebsd* | dragonfly*)
      archive_cmds_GCJ='$CC -shared -o $lib $libobjs $deplibs $compiler_flags'
      hardcode_libdir_flag_spec_GCJ='-R$libdir'
      hardcode_direct_GCJ=yes
      hardcode_shlibpath_var_GCJ=no
      ;;

    hpux9*)
      if test "$GCC" = yes; then
	archive_cmds_GCJ='$rm $output_objdir/$soname~$CC -shared -fPIC ${wl}+b ${wl}$install_libdir -o $output_objdir/$soname $libobjs $deplibs $compiler_flags~test $output_objdir/$soname = $lib || mv $output_objdir/$soname $lib'
      else
	archive_cmds_GCJ='$rm $output_objdir/$soname~$LD -b +b $install_libdir -o $output_objdir/$soname $libobjs $deplibs $linker_flags~test $output_objdir/$soname = $lib || mv $output_objdir/$soname $lib'
      fi
      hardcode_libdir_flag_spec_GCJ='${wl}+b ${wl}$libdir'
      hardcode_libdir_separator_GCJ=:
      hardcode_direct_GCJ=yes

      # hardcode_minus_L: Not really in the search PATH,
      # but as the default location of the library.
      hardcode_minus_L_GCJ=yes
      export_dynamic_flag_spec_GCJ='${wl}-E'
      ;;

    hpux10*)
      if test "$GCC" = yes -a "$with_gnu_ld" = no; then
	archive_cmds_GCJ='$CC -shared -fPIC ${wl}+h ${wl}$soname ${wl}+b ${wl}$install_libdir -o $lib $libobjs $deplibs $compiler_flags'
      else
	archive_cmds_GCJ='$LD -b +h $soname +b $install_libdir -o $lib $libobjs $deplibs $linker_flags'
      fi
      if test "$with_gnu_ld" = no; then
	hardcode_libdir_flag_spec_GCJ='${wl}+b ${wl}$libdir'
	hardcode_libdir_separator_GCJ=:

	hardcode_direct_GCJ=yes
	export_dynamic_flag_spec_GCJ='${wl}-E'

	# hardcode_minus_L: Not really in the search PATH,
	# but as the default location of the library.
	hardcode_minus_L_GCJ=yes
      fi
      ;;

    hpux11*)
      if test "$GCC" = yes -a "$with_gnu_ld" = no; then
	case $host_cpu in
	hppa*64*)
	  archive_cmds_GCJ='$CC -shared ${wl}+h ${wl}$soname -o $lib $libobjs $deplibs $compiler_flags'
	  ;;
	ia64*)
	  archive_cmds_GCJ='$CC -shared ${wl}+h ${wl}$soname ${wl}+nodefaultrpath -o $lib $libobjs $deplibs $compiler_flags'
	  ;;
	*)
	  archive_cmds_GCJ='$CC -shared -fPIC ${wl}+h ${wl}$soname ${wl}+b ${wl}$install_libdir -o $lib $libobjs $deplibs $compiler_flags'
	  ;;
	esac
      else
	case $host_cpu in
	hppa*64*)
	  archive_cmds_GCJ='$CC -b ${wl}+h ${wl}$soname -o $lib $libobjs $deplibs $compiler_flags'
	  ;;
	ia64*)
	  archive_cmds_GCJ='$CC -b ${wl}+h ${wl}$soname ${wl}+nodefaultrpath -o $lib $libobjs $deplibs $compiler_flags'
	  ;;
	*)
	  archive_cmds_GCJ='$CC -b ${wl}+h ${wl}$soname ${wl}+b ${wl}$install_libdir -o $lib $libobjs $deplibs $compiler_flags'
	  ;;
	esac
      fi
      if test "$with_gnu_ld" = no; then
	hardcode_libdir_flag_spec_GCJ='${wl}+b ${wl}$libdir'
	hardcode_libdir_separator_GCJ=:

	case $host_cpu in
	hppa*64*|ia64*)
	  hardcode_libdir_flag_spec_ld_GCJ='+b $libdir'
	  hardcode_direct_GCJ=no
	  hardcode_shlibpath_var_GCJ=no
	  ;;
	*)
	  hardcode_direct_GCJ=yes
	  export_dynamic_flag_spec_GCJ='${wl}-E'

	  # hardcode_minus_L: Not really in the search PATH,
	  # but as the default location of the library.
	  hardcode_minus_L_GCJ=yes
	  ;;
	esac
      fi
      ;;

    irix5* | irix6* | nonstopux*)
      if test "$GCC" = yes; then
	archive_cmds_GCJ='$CC -shared $libobjs $deplibs $compiler_flags ${wl}-soname ${wl}$soname `test -n "$verstring" && echo ${wl}-set_version ${wl}$verstring` ${wl}-update_registry ${wl}${output_objdir}/so_locations -o $lib'
      else
	archive_cmds_GCJ='$LD -shared $libobjs $deplibs $linker_flags -soname $soname `test -n "$verstring" && echo -set_version $verstring` -update_registry ${output_objdir}/so_locations -o $lib'
	hardcode_libdir_flag_spec_ld_GCJ='-rpath $libdir'
      fi
      hardcode_libdir_flag_spec_GCJ='${wl}-rpath ${wl}$libdir'
      hardcode_libdir_separator_GCJ=:
      link_all_deplibs_GCJ=yes
      ;;

    netbsd*)
      if echo __ELF__ | $CC -E - | grep __ELF__ >/dev/null; then
	archive_cmds_GCJ='$LD -Bshareable -o $lib $libobjs $deplibs $linker_flags'  # a.out
      else
	archive_cmds_GCJ='$LD -shared -o $lib $libobjs $deplibs $linker_flags'      # ELF
      fi
      hardcode_libdir_flag_spec_GCJ='-R$libdir'
      hardcode_direct_GCJ=yes
      hardcode_shlibpath_var_GCJ=no
      ;;

    newsos6)
      archive_cmds_GCJ='$LD -G -h $soname -o $lib $libobjs $deplibs $linker_flags'
      hardcode_direct_GCJ=yes
      hardcode_libdir_flag_spec_GCJ='${wl}-rpath ${wl}$libdir'
      hardcode_libdir_separator_GCJ=:
      hardcode_shlibpath_var_GCJ=no
      ;;

    openbsd*)
      if test -f /usr/libexec/ld.so; then
	hardcode_direct_GCJ=yes
	hardcode_shlibpath_var_GCJ=no
	if test -z "`echo __ELF__ | $CC -E - | grep __ELF__`" || test "$host_os-$host_cpu" = "openbsd2.8-powerpc"; then
	  archive_cmds_GCJ='$CC -shared $pic_flag -o $lib $libobjs $deplibs $compiler_flags'
	  archive_expsym_cmds_GCJ='$CC -shared $pic_flag -o $lib $libobjs $deplibs $compiler_flags ${wl}-retain-symbols-file,$export_symbols'
	  hardcode_libdir_flag_spec_GCJ='${wl}-rpath,$libdir'
	  export_dynamic_flag_spec_GCJ='${wl}-E'
	else
	  case $host_os in
	   openbsd[01].* | openbsd2.[0-7] | openbsd2.[0-7].*)
	     archive_cmds_GCJ='$LD -Bshareable -o $lib $libobjs $deplibs $linker_flags'
	     hardcode_libdir_flag_spec_GCJ='-R$libdir'
	     ;;
	   *)
	     archive_cmds_GCJ='$CC -shared $pic_flag -o $lib $libobjs $deplibs $compiler_flags'
	     hardcode_libdir_flag_spec_GCJ='${wl}-rpath,$libdir'
	     ;;
	  esac
        fi
      else
	ld_shlibs_GCJ=no
      fi
      ;;

    os2*)
      hardcode_libdir_flag_spec_GCJ='-L$libdir'
      hardcode_minus_L_GCJ=yes
      allow_undefined_flag_GCJ=unsupported
      archive_cmds_GCJ='$echo "LIBRARY $libname INITINSTANCE" > $output_objdir/$libname.def~$echo "DESCRIPTION \"$libname\"" >> $output_objdir/$libname.def~$echo DATA >> $output_objdir/$libname.def~$echo " SINGLE NONSHARED" >> $output_objdir/$libname.def~$echo EXPORTS >> $output_objdir/$libname.def~emxexp $libobjs >> $output_objdir/$libname.def~$CC -Zdll -Zcrtdll -o $lib $libobjs $deplibs $compiler_flags $output_objdir/$libname.def'
      old_archive_From_new_cmds_GCJ='emximp -o $output_objdir/$libname.a $output_objdir/$libname.def'
      ;;

    osf3*)
      if test "$GCC" = yes; then
	allow_undefined_flag_GCJ=' ${wl}-expect_unresolved ${wl}\*'
	archive_cmds_GCJ='$CC -shared${allow_undefined_flag} $libobjs $deplibs $compiler_flags ${wl}-soname ${wl}$soname `test -n "$verstring" && echo ${wl}-set_version ${wl}$verstring` ${wl}-update_registry ${wl}${output_objdir}/so_locations -o $lib'
      else
	allow_undefined_flag_GCJ=' -expect_unresolved \*'
	archive_cmds_GCJ='$LD -shared${allow_undefined_flag} $libobjs $deplibs $linker_flags -soname $soname `test -n "$verstring" && echo -set_version $verstring` -update_registry ${output_objdir}/so_locations -o $lib'
      fi
      hardcode_libdir_flag_spec_GCJ='${wl}-rpath ${wl}$libdir'
      hardcode_libdir_separator_GCJ=:
      ;;

    osf4* | osf5*)	# as osf3* with the addition of -msym flag
      if test "$GCC" = yes; then
	allow_undefined_flag_GCJ=' ${wl}-expect_unresolved ${wl}\*'
	archive_cmds_GCJ='$CC -shared${allow_undefined_flag} $libobjs $deplibs $compiler_flags ${wl}-msym ${wl}-soname ${wl}$soname `test -n "$verstring" && echo ${wl}-set_version ${wl}$verstring` ${wl}-update_registry ${wl}${output_objdir}/so_locations -o $lib'
	hardcode_libdir_flag_spec_GCJ='${wl}-rpath ${wl}$libdir'
      else
	allow_undefined_flag_GCJ=' -expect_unresolved \*'
	archive_cmds_GCJ='$LD -shared${allow_undefined_flag} $libobjs $deplibs $linker_flags -msym -soname $soname `test -n "$verstring" && echo -set_version $verstring` -update_registry ${output_objdir}/so_locations -o $lib'
	archive_expsym_cmds_GCJ='for i in `cat $export_symbols`; do printf "%s %s\\n" -exported_symbol "\$i" >> $lib.exp; done; echo "-hidden">> $lib.exp~
	$LD -shared${allow_undefined_flag} -input $lib.exp $linker_flags $libobjs $deplibs -soname $soname `test -n "$verstring" && echo -set_version $verstring` -update_registry ${output_objdir}/so_locations -o $lib~$rm $lib.exp'

	# Both c and cxx compiler support -rpath directly
	hardcode_libdir_flag_spec_GCJ='-rpath $libdir'
      fi
      hardcode_libdir_separator_GCJ=:
      ;;

    solaris*)
      no_undefined_flag_GCJ=' -z text'
      if test "$GCC" = yes; then
	wlarc='${wl}'
	archive_cmds_GCJ='$CC -shared ${wl}-h ${wl}$soname -o $lib $libobjs $deplibs $compiler_flags'
	archive_expsym_cmds_GCJ='$echo "{ global:" > $lib.exp~cat $export_symbols | $SED -e "s/\(.*\)/\1;/" >> $lib.exp~$echo "local: *; };" >> $lib.exp~
	  $CC -shared ${wl}-M ${wl}$lib.exp ${wl}-h ${wl}$soname -o $lib $libobjs $deplibs $compiler_flags~$rm $lib.exp'
      else
	wlarc=''
	archive_cmds_GCJ='$LD -G${allow_undefined_flag} -h $soname -o $lib $libobjs $deplibs $linker_flags'
	archive_expsym_cmds_GCJ='$echo "{ global:" > $lib.exp~cat $export_symbols | $SED -e "s/\(.*\)/\1;/" >> $lib.exp~$echo "local: *; };" >> $lib.exp~
  	$LD -G${allow_undefined_flag} -M $lib.exp -h $soname -o $lib $libobjs $deplibs $linker_flags~$rm $lib.exp'
      fi
      hardcode_libdir_flag_spec_GCJ='-R$libdir'
      hardcode_shlibpath_var_GCJ=no
      case $host_os in
      solaris2.[0-5] | solaris2.[0-5].*) ;;
      *)
	# The compiler driver will combine and reorder linker options,
	# but understands `-z linker_flag'.  GCC discards it without `$wl',
	# but is careful enough not to reorder.
 	# Supported since Solaris 2.6 (maybe 2.5.1?)
	if test "$GCC" = yes; then
	  whole_archive_flag_spec_GCJ='${wl}-z ${wl}allextract$convenience ${wl}-z ${wl}defaultextract'
	else
	  whole_archive_flag_spec_GCJ='-z allextract$convenience -z defaultextract'
	fi
	;;
      esac
      link_all_deplibs_GCJ=yes
      ;;

    sunos4*)
      if test "x$host_vendor" = xsequent; then
	# Use $CC to link under sequent, because it throws in some extra .o
	# files that make .init and .fini sections work.
	archive_cmds_GCJ='$CC -G ${wl}-h $soname -o $lib $libobjs $deplibs $compiler_flags'
      else
	archive_cmds_GCJ='$LD -assert pure-text -Bstatic -o $lib $libobjs $deplibs $linker_flags'
      fi
      hardcode_libdir_flag_spec_GCJ='-L$libdir'
      hardcode_direct_GCJ=yes
      hardcode_minus_L_GCJ=yes
      hardcode_shlibpath_var_GCJ=no
      ;;

    sysv4)
      case $host_vendor in
	sni)
	  archive_cmds_GCJ='$LD -G -h $soname -o $lib $libobjs $deplibs $linker_flags'
	  hardcode_direct_GCJ=yes # is this really true???
	;;
	siemens)
	  ## LD is ld it makes a PLAMLIB
	  ## CC just makes a GrossModule.
	  archive_cmds_GCJ='$LD -G -o $lib $libobjs $deplibs $linker_flags'
	  reload_cmds_GCJ='$CC -r -o $output$reload_objs'
	  hardcode_direct_GCJ=no
        ;;
	motorola)
	  archive_cmds_GCJ='$LD -G -h $soname -o $lib $libobjs $deplibs $linker_flags'
	  hardcode_direct_GCJ=no #Motorola manual says yes, but my tests say they lie
	;;
      esac
      runpath_var='LD_RUN_PATH'
      hardcode_shlibpath_var_GCJ=no
      ;;

    sysv4.3*)
      archive_cmds_GCJ='$LD -G -h $soname -o $lib $libobjs $deplibs $linker_flags'
      hardcode_shlibpath_var_GCJ=no
      export_dynamic_flag_spec_GCJ='-Bexport'
      ;;

    sysv4*MP*)
      if test -d /usr/nec; then
	archive_cmds_GCJ='$LD -G -h $soname -o $lib $libobjs $deplibs $linker_flags'
	hardcode_shlibpath_var_GCJ=no
	runpath_var=LD_RUN_PATH
	hardcode_runpath_var=yes
	ld_shlibs_GCJ=yes
      fi
      ;;

    sysv4*uw2* | sysv5OpenUNIX* | sysv5UnixWare7.[01].[10]* | unixware7* | sco3.2v5.0.[024]*)
      no_undefined_flag_GCJ='${wl}-z,text'
      archive_cmds_need_lc_GCJ=no
      hardcode_shlibpath_var_GCJ=no
      runpath_var='LD_RUN_PATH'

      if test "$GCC" = yes; then
	archive_cmds_GCJ='$CC -shared ${wl}-h,$soname -o $lib $libobjs $deplibs $compiler_flags'
	archive_expsym_cmds_GCJ='$CC -shared ${wl}-Bexport:$export_symbols ${wl}-h,$soname -o $lib $libobjs $deplibs $compiler_flags'
      else
	archive_cmds_GCJ='$CC -G ${wl}-h,$soname -o $lib $libobjs $deplibs $compiler_flags'
	archive_expsym_cmds_GCJ='$CC -G ${wl}-Bexport:$export_symbols ${wl}-h,$soname -o $lib $libobjs $deplibs $compiler_flags'
      fi
      ;;

    sysv5* | sco3.2v5* | sco5v6*)
      # Note: We can NOT use -z defs as we might desire, because we do not
      # link with -lc, and that would cause any symbols used from libc to
      # always be unresolved, which means just about no library would
      # ever link correctly.  If we're not using GNU ld we use -z text
      # though, which does catch some bad symbols but isn't as heavy-handed
      # as -z defs.
      no_undefined_flag_GCJ='${wl}-z,text'
      allow_undefined_flag_GCJ='${wl}-z,nodefs'
      archive_cmds_need_lc_GCJ=no
      hardcode_shlibpath_var_GCJ=no
      hardcode_libdir_flag_spec_GCJ='`test -z "$SCOABSPATH" && echo ${wl}-R,$libdir`'
      hardcode_libdir_separator_GCJ=':'
      link_all_deplibs_GCJ=yes
      export_dynamic_flag_spec_GCJ='${wl}-Bexport'
      runpath_var='LD_RUN_PATH'

      if test "$GCC" = yes; then
	archive_cmds_GCJ='$CC -shared ${wl}-h,\${SCOABSPATH:+${install_libdir}/}$soname -o $lib $libobjs $deplibs $compiler_flags'
	archive_expsym_cmds_GCJ='$CC -shared ${wl}-Bexport:$export_symbols ${wl}-h,\${SCOABSPATH:+${install_libdir}/}$soname -o $lib $libobjs $deplibs $compiler_flags'
      else
	archive_cmds_GCJ='$CC -G ${wl}-h,\${SCOABSPATH:+${install_libdir}/}$soname -o $lib $libobjs $deplibs $compiler_flags'
	archive_expsym_cmds_GCJ='$CC -G ${wl}-Bexport:$export_symbols ${wl}-h,\${SCOABSPATH:+${install_libdir}/}$soname -o $lib $libobjs $deplibs $compiler_flags'
      fi
      ;;

    uts4*)
      archive_cmds_GCJ='$LD -G -h $soname -o $lib $libobjs $deplibs $linker_flags'
      hardcode_libdir_flag_spec_GCJ='-L$libdir'
      hardcode_shlibpath_var_GCJ=no
      ;;

    *)
      ld_shlibs_GCJ=no
      ;;
    esac
  fi

{ echo "$as_me:$LINENO: result: $ld_shlibs_GCJ" >&5
echo "${ECHO_T}$ld_shlibs_GCJ" >&6; }
test "$ld_shlibs_GCJ" = no && can_build_shared=no

#
# Do we need to explicitly link libc?
#
case "x$archive_cmds_need_lc_GCJ" in
x|xyes)
  # Assume -lc should be added
  archive_cmds_need_lc_GCJ=yes

  if test "$enable_shared" = yes && test "$GCC" = yes; then
    case $archive_cmds_GCJ in
    *'~'*)
      # FIXME: we may have to deal with multi-command sequences.
      ;;
    '$CC '*)
      # Test whether the compiler implicitly links with -lc since on some
      # systems, -lgcc has to come before -lc. If gcc already passes -lc
      # to ld, don't add -lc before -lgcc.
      { echo "$as_me:$LINENO: checking whether -lc should be explicitly linked in" >&5
echo $ECHO_N "checking whether -lc should be explicitly linked in... $ECHO_C" >&6; }
      $rm conftest*
      echo "$lt_simple_compile_test_code" > conftest.$ac_ext

      if { (eval echo "$as_me:$LINENO: \"$ac_compile\"") >&5
  (eval $ac_compile) 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } 2>conftest.err; then
        soname=conftest
        lib=conftest
        libobjs=conftest.$ac_objext
        deplibs=
        wl=$lt_prog_compiler_wl_GCJ
	pic_flag=$lt_prog_compiler_pic_GCJ
        compiler_flags=-v
        linker_flags=-v
        verstring=
        output_objdir=.
        libname=conftest
        lt_save_allow_undefined_flag=$allow_undefined_flag_GCJ
        allow_undefined_flag_GCJ=
        if { (eval echo "$as_me:$LINENO: \"$archive_cmds_GCJ 2\>\&1 \| grep \" -lc \" \>/dev/null 2\>\&1\"") >&5
  (eval $archive_cmds_GCJ 2\>\&1 \| grep \" -lc \" \>/dev/null 2\>\&1) 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }
        then
	  archive_cmds_need_lc_GCJ=no
        else
	  archive_cmds_need_lc_GCJ=yes
        fi
        allow_undefined_flag_GCJ=$lt_save_allow_undefined_flag
      else
        cat conftest.err 1>&5
      fi
      $rm conftest*
      { echo "$as_me:$LINENO: result: $archive_cmds_need_lc_GCJ" >&5
echo "${ECHO_T}$archive_cmds_need_lc_GCJ" >&6; }
      ;;
    esac
  fi
  ;;
esac

{ echo "$as_me:$LINENO: checking dynamic linker characteristics" >&5
echo $ECHO_N "checking dynamic linker characteristics... $ECHO_C" >&6; }
library_names_spec=
libname_spec='lib$name'
soname_spec=
shrext_cmds=".so"
postinstall_cmds=
postuninstall_cmds=
finish_cmds=
finish_eval=
shlibpath_var=
shlibpath_overrides_runpath=unknown
version_type=none
dynamic_linker="$host_os ld.so"
sys_lib_dlsearch_path_spec="/lib /usr/lib"

need_lib_prefix=unknown
hardcode_into_libs=no

# when you set need_version to no, make sure it does not cause -set_version
# flags to be left without arguments
need_version=unknown

case $host_os in
aix3*)
  version_type=linux
  library_names_spec='${libname}${release}${shared_ext}$versuffix $libname.a'
  shlibpath_var=LIBPATH

  # AIX 3 has no versioning support, so we append a major version to the name.
  soname_spec='${libname}${release}${shared_ext}$major'
  ;;

aix4* | aix5*)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  hardcode_into_libs=yes
  if test "$host_cpu" = ia64; then
    # AIX 5 supports IA64
    library_names_spec='${libname}${release}${shared_ext}$major ${libname}${release}${shared_ext}$versuffix $libname${shared_ext}'
    shlibpath_var=LD_LIBRARY_PATH
  else
    # With GCC up to 2.95.x, collect2 would create an import file
    # for dependence libraries.  The import file would start with
    # the line `#! .'.  This would cause the generated library to
    # depend on `.', always an invalid library.  This was fixed in
    # development snapshots of GCC prior to 3.0.
    case $host_os in
      aix4 | aix4.[01] | aix4.[01].*)
      if { echo '#if __GNUC__ > 2 || (__GNUC__ == 2 && __GNUC_MINOR__ >= 97)'
	   echo ' yes '
	   echo '#endif'; } | ${CC} -E - | grep yes > /dev/null; then
	:
      else
	can_build_shared=no
      fi
      ;;
    esac
    # AIX (on Power*) has no versioning support, so currently we can not hardcode correct
    # soname into executable. Probably we can add versioning support to
    # collect2, so additional links can be useful in future.
    if test "$aix_use_runtimelinking" = yes; then
      # If using run time linking (on AIX 4.2 or later) use lib<name>.so
      # instead of lib<name>.a to let people know that these are not
      # typical AIX shared libraries.
      library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
    else
      # We preserve .a as extension for shared libraries through AIX4.2
      # and later when we are not doing run time linking.
      library_names_spec='${libname}${release}.a $libname.a'
      soname_spec='${libname}${release}${shared_ext}$major'
    fi
    shlibpath_var=LIBPATH
  fi
  ;;

amigaos*)
  library_names_spec='$libname.ixlibrary $libname.a'
  # Create ${libname}_ixlibrary.a entries in /sys/libs.
  finish_eval='for lib in `ls $libdir/*.ixlibrary 2>/dev/null`; do libname=`$echo "X$lib" | $Xsed -e '\''s%^.*/\([^/]*\)\.ixlibrary$%\1%'\''`; test $rm /sys/libs/${libname}_ixlibrary.a; $show "cd /sys/libs && $LN_S $lib ${libname}_ixlibrary.a"; cd /sys/libs && $LN_S $lib ${libname}_ixlibrary.a || exit 1; done'
  ;;

beos*)
  library_names_spec='${libname}${shared_ext}'
  dynamic_linker="$host_os ld.so"
  shlibpath_var=LIBRARY_PATH
  ;;

bsdi[45]*)
  version_type=linux
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  finish_cmds='PATH="\$PATH:/sbin" ldconfig $libdir'
  shlibpath_var=LD_LIBRARY_PATH
  sys_lib_search_path_spec="/shlib /usr/lib /usr/X11/lib /usr/contrib/lib /lib /usr/local/lib"
  sys_lib_dlsearch_path_spec="/shlib /usr/lib /usr/local/lib"
  # the default ld.so.conf also contains /usr/contrib/lib and
  # /usr/X11R6/lib (/usr/X11 is a link to /usr/X11R6), but let us allow
  # libtool to hard-code these into programs
  ;;

cygwin* | mingw* | pw32*)
  version_type=windows
  shrext_cmds=".dll"
  need_version=no
  need_lib_prefix=no

  case $GCC,$host_os in
  yes,cygwin* | yes,mingw* | yes,pw32*)
    library_names_spec='$libname.dll.a'
    # DLL is installed to $(libdir)/../bin by postinstall_cmds
    postinstall_cmds='base_file=`basename \${file}`~
      dlpath=`$SHELL 2>&1 -c '\''. $dir/'\''\${base_file}'\''i;echo \$dlname'\''`~
      dldir=$destdir/`dirname \$dlpath`~
      test -d \$dldir || mkdir -p \$dldir~
      $install_prog $dir/$dlname \$dldir/$dlname~
      chmod a+x \$dldir/$dlname'
    postuninstall_cmds='dldll=`$SHELL 2>&1 -c '\''. $file; echo \$dlname'\''`~
      dlpath=$dir/\$dldll~
       $rm \$dlpath'
    shlibpath_overrides_runpath=yes

    case $host_os in
    cygwin*)
      # Cygwin DLLs use 'cyg' prefix rather than 'lib'
      soname_spec='`echo ${libname} | sed -e 's/^lib/cyg/'``echo ${release} | $SED -e 's/[.]/-/g'`${versuffix}${shared_ext}'
      sys_lib_search_path_spec="/usr/lib /lib/w32api /lib /usr/local/lib"
      ;;
    mingw*)
      # MinGW DLLs use traditional 'lib' prefix
      soname_spec='${libname}`echo ${release} | $SED -e 's/[.]/-/g'`${versuffix}${shared_ext}'
      sys_lib_search_path_spec=`$CC -print-search-dirs | grep "^libraries:" | $SED -e "s/^libraries://" -e "s,=/,/,g"`
      if echo "$sys_lib_search_path_spec" | grep ';[c-zC-Z]:/' >/dev/null; then
        # It is most probably a Windows format PATH printed by
        # mingw gcc, but we are running on Cygwin. Gcc prints its search
        # path with ; separators, and with drive letters. We can handle the
        # drive letters (cygwin fileutils understands them), so leave them,
        # especially as we might pass files found there to a mingw objdump,
        # which wouldn't understand a cygwinified path. Ahh.
        sys_lib_search_path_spec=`echo "$sys_lib_search_path_spec" | $SED -e 's/;/ /g'`
      else
        sys_lib_search_path_spec=`echo "$sys_lib_search_path_spec" | $SED  -e "s/$PATH_SEPARATOR/ /g"`
      fi
      ;;
    pw32*)
      # pw32 DLLs use 'pw' prefix rather than 'lib'
      library_names_spec='`echo ${libname} | sed -e 's/^lib/pw/'``echo ${release} | $SED -e 's/[.]/-/g'`${versuffix}${shared_ext}'
      ;;
    esac
    ;;

  *)
    library_names_spec='${libname}`echo ${release} | $SED -e 's/[.]/-/g'`${versuffix}${shared_ext} $libname.lib'
    ;;
  esac
  dynamic_linker='Win32 ld.exe'
  # FIXME: first we should search . and the directory the executable is in
  shlibpath_var=PATH
  ;;

darwin* | rhapsody*)
  dynamic_linker="$host_os dyld"
  version_type=darwin
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${versuffix}$shared_ext ${libname}${release}${major}$shared_ext ${libname}$shared_ext'
  soname_spec='${libname}${release}${major}$shared_ext'
  shlibpath_overrides_runpath=yes
  shlibpath_var=DYLD_LIBRARY_PATH
  shrext_cmds='`test .$module = .yes && echo .so || echo .dylib`'

  sys_lib_dlsearch_path_spec='/usr/local/lib /lib /usr/lib'
  ;;

dgux*)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname$shared_ext'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  ;;

freebsd1*)
  dynamic_linker=no
  ;;

freebsd* | dragonfly*)
  # DragonFly does not have aout.  When/if they implement a new
  # versioning mechanism, adjust this.
  if test -x /usr/bin/objformat; then
    objformat=`/usr/bin/objformat`
  else
    case $host_os in
    freebsd[123]*) objformat=aout ;;
    *) objformat=elf ;;
    esac
  fi
  version_type=freebsd-$objformat
  case $version_type in
    freebsd-elf*)
      library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext} $libname${shared_ext}'
      need_version=no
      need_lib_prefix=no
      ;;
    freebsd-*)
      library_names_spec='${libname}${release}${shared_ext}$versuffix $libname${shared_ext}$versuffix'
      need_version=yes
      ;;
  esac
  shlibpath_var=LD_LIBRARY_PATH
  case $host_os in
  freebsd2*)
    shlibpath_overrides_runpath=yes
    ;;
  freebsd3.[01]* | freebsdelf3.[01]*)
    shlibpath_overrides_runpath=yes
    hardcode_into_libs=yes
    ;;
  freebsd3.[2-9]* | freebsdelf3.[2-9]* | \
  freebsd4.[0-5] | freebsdelf4.[0-5] | freebsd4.1.1 | freebsdelf4.1.1)
    shlibpath_overrides_runpath=no
    hardcode_into_libs=yes
    ;;
  *) # from 4.6 on, and DragonFly
    shlibpath_overrides_runpath=yes
    hardcode_into_libs=yes
    ;;
  esac
  ;;

gnu*)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}${major} ${libname}${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  hardcode_into_libs=yes
  ;;

hpux9* | hpux10* | hpux11*)
  # Give a soname corresponding to the major version so that dld.sl refuses to
  # link against other versions.
  version_type=sunos
  need_lib_prefix=no
  need_version=no
  case $host_cpu in
  ia64*)
    shrext_cmds='.so'
    hardcode_into_libs=yes
    dynamic_linker="$host_os dld.so"
    shlibpath_var=LD_LIBRARY_PATH
    shlibpath_overrides_runpath=yes # Unless +noenvvar is specified.
    library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
    soname_spec='${libname}${release}${shared_ext}$major'
    if test "X$HPUX_IA64_MODE" = X32; then
      sys_lib_search_path_spec="/usr/lib/hpux32 /usr/local/lib/hpux32 /usr/local/lib"
    else
      sys_lib_search_path_spec="/usr/lib/hpux64 /usr/local/lib/hpux64"
    fi
    sys_lib_dlsearch_path_spec=$sys_lib_search_path_spec
    ;;
   hppa*64*)
     shrext_cmds='.sl'
     hardcode_into_libs=yes
     dynamic_linker="$host_os dld.sl"
     shlibpath_var=LD_LIBRARY_PATH # How should we handle SHLIB_PATH
     shlibpath_overrides_runpath=yes # Unless +noenvvar is specified.
     library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
     soname_spec='${libname}${release}${shared_ext}$major'
     sys_lib_search_path_spec="/usr/lib/pa20_64 /usr/ccs/lib/pa20_64"
     sys_lib_dlsearch_path_spec=$sys_lib_search_path_spec
     ;;
   *)
    shrext_cmds='.sl'
    dynamic_linker="$host_os dld.sl"
    shlibpath_var=SHLIB_PATH
    shlibpath_overrides_runpath=no # +s is required to enable SHLIB_PATH
    library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
    soname_spec='${libname}${release}${shared_ext}$major'
    ;;
  esac
  # HP-UX runs *really* slowly unless shared libraries are mode 555.
  postinstall_cmds='chmod 555 $lib'
  ;;

interix[3-9]*)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major ${libname}${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  dynamic_linker='Interix 3.x ld.so.1 (PE, like ELF)'
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=no
  hardcode_into_libs=yes
  ;;

irix5* | irix6* | nonstopux*)
  case $host_os in
    nonstopux*) version_type=nonstopux ;;
    *)
	if test "$lt_cv_prog_gnu_ld" = yes; then
		version_type=linux
	else
		version_type=irix
	fi ;;
  esac
  need_lib_prefix=no
  need_version=no
  soname_spec='${libname}${release}${shared_ext}$major'
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major ${libname}${release}${shared_ext} $libname${shared_ext}'
  case $host_os in
  irix5* | nonstopux*)
    libsuff= shlibsuff=
    ;;
  *)
    case $LD in # libtool.m4 will add one of these switches to LD
    *-32|*"-32 "|*-melf32bsmip|*"-melf32bsmip ")
      libsuff= shlibsuff= libmagic=32-bit;;
    *-n32|*"-n32 "|*-melf32bmipn32|*"-melf32bmipn32 ")
      libsuff=32 shlibsuff=N32 libmagic=N32;;
    *-64|*"-64 "|*-melf64bmip|*"-melf64bmip ")
      libsuff=64 shlibsuff=64 libmagic=64-bit;;
    *) libsuff= shlibsuff= libmagic=never-match;;
    esac
    ;;
  esac
  shlibpath_var=LD_LIBRARY${shlibsuff}_PATH
  shlibpath_overrides_runpath=no
  sys_lib_search_path_spec="/usr/lib${libsuff} /lib${libsuff} /usr/local/lib${libsuff}"
  sys_lib_dlsearch_path_spec="/usr/lib${libsuff} /lib${libsuff}"
  hardcode_into_libs=yes
  ;;

# No shared lib support for Linux oldld, aout, or coff.
linux*oldld* | linux*aout* | linux*coff*)
  dynamic_linker=no
  ;;

# This must be Linux ELF.
linux* | k*bsd*-gnu)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  finish_cmds='PATH="\$PATH:/sbin" ldconfig -n $libdir'
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=no
  # This implies no fast_install, which is unacceptable.
  # Some rework will be needed to allow for fast_install
  # before this can be enabled.
  hardcode_into_libs=yes

  # Append ld.so.conf contents to the search path
  if test -f /etc/ld.so.conf; then
    lt_ld_extra=`awk '/^include / { system(sprintf("cd /etc; cat %s 2>/dev/null", \$2)); skip = 1; } { if (!skip) print \$0; skip = 0; }' < /etc/ld.so.conf | $SED -e 's/#.*//;/^[ 	]*hwcap[ 	]/d;s/[:,	]/ /g;s/=[^=]*$//;s/=[^= ]* / /g;/^$/d' | tr '\n' ' '`
    sys_lib_dlsearch_path_spec="/lib /usr/lib $lt_ld_extra"
  fi

  # We used to test for /lib/ld.so.1 and disable shared libraries on
  # powerpc, because MkLinux only supported shared libraries with the
  # GNU dynamic linker.  Since this was broken with cross compilers,
  # most powerpc-linux boxes support dynamic linking these days and
  # people can always --disable-shared, the test was removed, and we
  # assume the GNU/Linux dynamic linker is in use.
  dynamic_linker='GNU/Linux ld.so'
  ;;

netbsd*)
  version_type=sunos
  need_lib_prefix=no
  need_version=no
  if echo __ELF__ | $CC -E - | grep __ELF__ >/dev/null; then
    library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${shared_ext}$versuffix'
    finish_cmds='PATH="\$PATH:/sbin" ldconfig -m $libdir'
    dynamic_linker='NetBSD (a.out) ld.so'
  else
    library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major ${libname}${shared_ext}'
    soname_spec='${libname}${release}${shared_ext}$major'
    dynamic_linker='NetBSD ld.elf_so'
  fi
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=yes
  hardcode_into_libs=yes
  ;;

newsos6)
  version_type=linux
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=yes
  ;;

nto-qnx*)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=yes
  ;;

openbsd*)
  version_type=sunos
  sys_lib_dlsearch_path_spec="/usr/lib"
  need_lib_prefix=no
  # Some older versions of OpenBSD (3.3 at least) *do* need versioned libs.
  case $host_os in
    openbsd3.3 | openbsd3.3.*) need_version=yes ;;
    *)                         need_version=no  ;;
  esac
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${shared_ext}$versuffix'
  finish_cmds='PATH="\$PATH:/sbin" ldconfig -m $libdir'
  shlibpath_var=LD_LIBRARY_PATH
  if test -z "`echo __ELF__ | $CC -E - | grep __ELF__`" || test "$host_os-$host_cpu" = "openbsd2.8-powerpc"; then
    case $host_os in
      openbsd2.[89] | openbsd2.[89].*)
	shlibpath_overrides_runpath=no
	;;
      *)
	shlibpath_overrides_runpath=yes
	;;
      esac
  else
    shlibpath_overrides_runpath=yes
  fi
  ;;

os2*)
  libname_spec='$name'
  shrext_cmds=".dll"
  need_lib_prefix=no
  library_names_spec='$libname${shared_ext} $libname.a'
  dynamic_linker='OS/2 ld.exe'
  shlibpath_var=LIBPATH
  ;;

osf3* | osf4* | osf5*)
  version_type=osf
  need_lib_prefix=no
  need_version=no
  soname_spec='${libname}${release}${shared_ext}$major'
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  shlibpath_var=LD_LIBRARY_PATH
  sys_lib_search_path_spec="/usr/shlib /usr/ccs/lib /usr/lib/cmplrs/cc /usr/lib /usr/local/lib /var/shlib"
  sys_lib_dlsearch_path_spec="$sys_lib_search_path_spec"
  ;;

rdos*)
  dynamic_linker=no
  ;;

solaris*)
  version_type=linux
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=yes
  hardcode_into_libs=yes
  # ldd complains unless libraries are executable
  postinstall_cmds='chmod +x $lib'
  ;;

sunos4*)
  version_type=sunos
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${shared_ext}$versuffix'
  finish_cmds='PATH="\$PATH:/usr/etc" ldconfig $libdir'
  shlibpath_var=LD_LIBRARY_PATH
  shlibpath_overrides_runpath=yes
  if test "$with_gnu_ld" = yes; then
    need_lib_prefix=no
  fi
  need_version=yes
  ;;

sysv4 | sysv4.3*)
  version_type=linux
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  case $host_vendor in
    sni)
      shlibpath_overrides_runpath=no
      need_lib_prefix=no
      export_dynamic_flag_spec='${wl}-Blargedynsym'
      runpath_var=LD_RUN_PATH
      ;;
    siemens)
      need_lib_prefix=no
      ;;
    motorola)
      need_lib_prefix=no
      need_version=no
      shlibpath_overrides_runpath=no
      sys_lib_search_path_spec='/lib /usr/lib /usr/ccs/lib'
      ;;
  esac
  ;;

sysv4*MP*)
  if test -d /usr/nec ;then
    version_type=linux
    library_names_spec='$libname${shared_ext}.$versuffix $libname${shared_ext}.$major $libname${shared_ext}'
    soname_spec='$libname${shared_ext}.$major'
    shlibpath_var=LD_LIBRARY_PATH
  fi
  ;;

sysv5* | sco3.2v5* | sco5v6* | unixware* | OpenUNIX* | sysv4*uw2*)
  version_type=freebsd-elf
  need_lib_prefix=no
  need_version=no
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext} $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  hardcode_into_libs=yes
  if test "$with_gnu_ld" = yes; then
    sys_lib_search_path_spec='/usr/local/lib /usr/gnu/lib /usr/ccs/lib /usr/lib /lib'
    shlibpath_overrides_runpath=no
  else
    sys_lib_search_path_spec='/usr/ccs/lib /usr/lib'
    shlibpath_overrides_runpath=yes
    case $host_os in
      sco3.2v5*)
        sys_lib_search_path_spec="$sys_lib_search_path_spec /lib"
	;;
    esac
  fi
  sys_lib_dlsearch_path_spec='/usr/lib'
  ;;

uts4*)
  version_type=linux
  library_names_spec='${libname}${release}${shared_ext}$versuffix ${libname}${release}${shared_ext}$major $libname${shared_ext}'
  soname_spec='${libname}${release}${shared_ext}$major'
  shlibpath_var=LD_LIBRARY_PATH
  ;;

*)
  dynamic_linker=no
  ;;
esac
{ echo "$as_me:$LINENO: result: $dynamic_linker" >&5
echo "${ECHO_T}$dynamic_linker" >&6; }
test "$dynamic_linker" = no && can_build_shared=no

variables_saved_for_relink="PATH $shlibpath_var $runpath_var"
if test "$GCC" = yes; then
  variables_saved_for_relink="$variables_saved_for_relink GCC_EXEC_PREFIX COMPILER_PATH LIBRARY_PATH"
fi

{ echo "$as_me:$LINENO: checking how to hardcode library paths into programs" >&5
echo $ECHO_N "checking how to hardcode library paths into programs... $ECHO_C" >&6; }
hardcode_action_GCJ=
if test -n "$hardcode_libdir_flag_spec_GCJ" || \
   test -n "$runpath_var_GCJ" || \
   test "X$hardcode_automatic_GCJ" = "Xyes" ; then

  # We can hardcode non-existant directories.
  if test "$hardcode_direct_GCJ" != no &&
     # If the only mechanism to avoid hardcoding is shlibpath_var, we
     # have to relink, otherwise we might link with an installed library
     # when we should be linking with a yet-to-be-installed one
     ## test "$_LT_AC_TAGVAR(hardcode_shlibpath_var, GCJ)" != no &&
     test "$hardcode_minus_L_GCJ" != no; then
    # Linking always hardcodes the temporary library directory.
    hardcode_action_GCJ=relink
  else
    # We can link without hardcoding, and we can hardcode nonexisting dirs.
    hardcode_action_GCJ=immediate
  fi
else
  # We cannot hardcode anything, or else we can only hardcode existing
  # directories.
  hardcode_action_GCJ=unsupported
fi
{ echo "$as_me:$LINENO: result: $hardcode_action_GCJ" >&5
echo "${ECHO_T}$hardcode_action_GCJ" >&6; }

if test "$hardcode_action_GCJ" = relink; then
  # Fast installation is not supported
  enable_fast_install=no
elif test "$shlibpath_overrides_runpath" = yes ||
     test "$enable_shared" = no; then
  # Fast installation is not necessary
  enable_fast_install=needless
fi


# The else clause should only fire when bootstrapping the
# libtool distribution, otherwise you forgot to ship ltmain.sh
# with your package, and you will get complaints that there are
# no rules to generate ltmain.sh.
if test -f "$ltmain"; then
  # See if we are running on zsh, and set the options which allow our commands through
  # without removal of \ escapes.
  if test -n "${ZSH_VERSION+set}" ; then
    setopt NO_GLOB_SUBST
  fi
  # Now quote all the things that may contain metacharacters while being
  # careful not to overquote the AC_SUBSTed values.  We take copies of the
  # variables and quote the copies for generation of the libtool script.
  for var in echo old_CC old_CFLAGS AR AR_FLAGS EGREP RANLIB LN_S LTCC LTCFLAGS NM \
    SED SHELL STRIP \
    libname_spec library_names_spec soname_spec extract_expsyms_cmds \
    old_striplib striplib file_magic_cmd finish_cmds finish_eval \
    deplibs_check_method reload_flag reload_cmds need_locks \
    lt_cv_sys_global_symbol_pipe lt_cv_sys_global_symbol_to_cdecl \
    lt_cv_sys_global_symbol_to_c_name_address \
    sys_lib_search_path_spec sys_lib_dlsearch_path_spec \
    old_postinstall_cmds old_postuninstall_cmds \
    compiler_GCJ \
    CC_GCJ \
    LD_GCJ \
    lt_prog_compiler_wl_GCJ \
    lt_prog_compiler_pic_GCJ \
    lt_prog_compiler_static_GCJ \
    lt_prog_compiler_no_builtin_flag_GCJ \
    export_dynamic_flag_spec_GCJ \
    thread_safe_flag_spec_GCJ \
    whole_archive_flag_spec_GCJ \
    enable_shared_with_static_runtimes_GCJ \
    old_archive_cmds_GCJ \
    old_archive_from_new_cmds_GCJ \
    predep_objects_GCJ \
    postdep_objects_GCJ \
    predeps_GCJ \
    postdeps_GCJ \
    compiler_lib_search_path_GCJ \
    archive_cmds_GCJ \
    archive_expsym_cmds_GCJ \
    postinstall_cmds_GCJ \
    postuninstall_cmds_GCJ \
    old_archive_from_expsyms_cmds_GCJ \
    allow_undefined_flag_GCJ \
    no_undefined_flag_GCJ \
    export_symbols_cmds_GCJ \
    hardcode_libdir_flag_spec_GCJ \
    hardcode_libdir_flag_spec_ld_GCJ \
    hardcode_libdir_separator_GCJ \
    hardcode_automatic_GCJ \
    module_cmds_GCJ \
    module_expsym_cmds_GCJ \
    lt_cv_prog_compiler_c_o_GCJ \
    fix_srcfile_path_GCJ \
    exclude_expsyms_GCJ \
    include_expsyms_GCJ; do

    case $var in
    old_archive_cmds_GCJ | \
    old_archive_from_new_cmds_GCJ | \
    archive_cmds_GCJ | \
    archive_expsym_cmds_GCJ | \
    module_cmds_GCJ | \
    module_expsym_cmds_GCJ | \
    old_archive_from_expsyms_cmds_GCJ | \
    export_symbols_cmds_GCJ | \
    extract_expsyms_cmds | reload_cmds | finish_cmds | \
    postinstall_cmds | postuninstall_cmds | \
    old_postinstall_cmds | old_postuninstall_cmds | \
    sys_lib_search_path_spec | sys_lib_dlsearch_path_spec)
      # Double-quote double-evaled strings.
      eval "lt_$var=\\\"\`\$echo \"X\$$var\" | \$Xsed -e \"\$double_quote_subst\" -e \"\$sed_quote_subst\" -e \"\$delay_variable_subst\"\`\\\""
      ;;
    *)
      eval "lt_$var=\\\"\`\$echo \"X\$$var\" | \$Xsed -e \"\$sed_quote_subst\"\`\\\""
      ;;
    esac
  done

  case $lt_echo in
  *'\$0 --fallback-echo"')
    lt_echo=`$echo "X$lt_echo" | $Xsed -e 's/\\\\\\\$0 --fallback-echo"$/$0 --fallback-echo"/'`
    ;;
  esac

cfgfile="$ofile"

  cat <<__EOF__ >> "$cfgfile"
# ### BEGIN LIBTOOL TAG CONFIG: $tagname

# Libtool was configured on host `(hostname || uname -n) 2>/dev/null | sed 1q`:

# Shell to use when invoking shell scripts.
SHELL=$lt_SHELL

# Whether or not to build shared libraries.
build_libtool_libs=$enable_shared

# Whether or not to build static libraries.
build_old_libs=$enable_static

# Whether or not to add -lc for building shared libraries.
build_libtool_need_lc=$archive_cmds_need_lc_GCJ

# Whether or not to disallow shared libs when runtime libs are static
allow_libtool_libs_with_static_runtimes=$enable_shared_with_static_runtimes_GCJ

# Whether or not to optimize for fast installation.
fast_install=$enable_fast_install

# The host system.
host_alias=$host_alias
host=$host
host_os=$host_os

# The build system.
build_alias=$build_alias
build=$build
build_os=$build_os

# An echo program that does not interpret backslashes.
echo=$lt_echo

# The archiver.
AR=$lt_AR
AR_FLAGS=$lt_AR_FLAGS

# A C compiler.
LTCC=$lt_LTCC

# LTCC compiler flags.
LTCFLAGS=$lt_LTCFLAGS

# A language-specific compiler.
CC=$lt_compiler_GCJ

# Is the compiler the GNU C compiler?
with_gcc=$GCC_GCJ

# An ERE matcher.
EGREP=$lt_EGREP

# The linker used to build libraries.
LD=$lt_LD_GCJ

# Whether we need hard or soft links.
LN_S=$lt_LN_S

# A BSD-compatible nm program.
NM=$lt_NM

# A symbol stripping program
STRIP=$lt_STRIP

# Used to examine libraries when file_magic_cmd begins "file"
MAGIC_CMD=$MAGIC_CMD

# Used on cygwin: DLL creation program.
DLLTOOL="$DLLTOOL"

# Used on cygwin: object dumper.
OBJDUMP="$OBJDUMP"

# Used on cygwin: assembler.
AS="$AS"

# The name of the directory that contains temporary libtool files.
objdir=$objdir

# How to create reloadable object files.
reload_flag=$lt_reload_flag
reload_cmds=$lt_reload_cmds

# How to pass a linker flag through the compiler.
wl=$lt_lt_prog_compiler_wl_GCJ

# Object file suffix (normally "o").
objext="$ac_objext"

# Old archive suffix (normally "a").
libext="$libext"

# Shared library suffix (normally ".so").
shrext_cmds='$shrext_cmds'

# Executable file suffix (normally "").
exeext="$exeext"

# Additional compiler flags for building library objects.
pic_flag=$lt_lt_prog_compiler_pic_GCJ
pic_mode=$pic_mode

# What is the maximum length of a command?
max_cmd_len=$lt_cv_sys_max_cmd_len

# Does compiler simultaneously support -c and -o options?
compiler_c_o=$lt_lt_cv_prog_compiler_c_o_GCJ

# Must we lock files when doing compilation?
need_locks=$lt_need_locks

# Do we need the lib prefix for modules?
need_lib_prefix=$need_lib_prefix

# Do we need a version for libraries?
need_version=$need_version

# Whether dlopen is supported.
dlopen_support=$enable_dlopen

# Whether dlopen of programs is supported.
dlopen_self=$enable_dlopen_self

# Whether dlopen of statically linked programs is supported.
dlopen_self_static=$enable_dlopen_self_static

# Compiler flag to prevent dynamic linking.
link_static_flag=$lt_lt_prog_compiler_static_GCJ

# Compiler flag to turn off builtin functions.
no_builtin_flag=$lt_lt_prog_compiler_no_builtin_flag_GCJ

# Compiler flag to allow reflexive dlopens.
export_dynamic_flag_spec=$lt_export_dynamic_flag_spec_GCJ

# Compiler flag to generate shared objects directly from archives.
whole_archive_flag_spec=$lt_whole_archive_flag_spec_GCJ

# Compiler flag to generate thread-safe objects.
thread_safe_flag_spec=$lt_thread_safe_flag_spec_GCJ

# Library versioning type.
version_type=$version_type

# Format of library name prefix.
libname_spec=$lt_libname_spec

# List of archive names.  First name is the real one, the rest are links.
# The last name is the one that the linker finds with -lNAME.
library_names_spec=$lt_library_names_spec

# The coded name of the library, if different from the real name.
soname_spec=$lt_soname_spec

# Commands used to build and install an old-style archive.
RANLIB=$lt_RANLIB
old_archive_cmds=$lt_old_archive_cmds_GCJ
old_postinstall_cmds=$lt_old_postinstall_cmds
old_postuninstall_cmds=$lt_old_postuninstall_cmds

# Create an old-style archive from a shared archive.
old_archive_from_new_cmds=$lt_old_archive_from_new_cmds_GCJ

# Create a temporary old-style archive to link instead of a shared archive.
old_archive_from_expsyms_cmds=$lt_old_archive_from_expsyms_cmds_GCJ

# Commands used to build and install a shared archive.
archive_cmds=$lt_archive_cmds_GCJ
archive_expsym_cmds=$lt_archive_expsym_cmds_GCJ
postinstall_cmds=$lt_postinstall_cmds
postuninstall_cmds=$lt_postuninstall_cmds

# Commands used to build a loadable module (assumed same as above if empty)
module_cmds=$lt_module_cmds_GCJ
module_expsym_cmds=$lt_module_expsym_cmds_GCJ

# Commands to strip libraries.
old_striplib=$lt_old_striplib
striplib=$lt_striplib

# Dependencies to place before the objects being linked to create a
# shared library.
predep_objects=$lt_predep_objects_GCJ

# Dependencies to place after the objects being linked to create a
# shared library.
postdep_objects=$lt_postdep_objects_GCJ

# Dependencies to place before the objects being linked to create a
# shared library.
predeps=$lt_predeps_GCJ

# Dependencies to place after the objects being linked to create a
# shared library.
postdeps=$lt_postdeps_GCJ

# The library search path used internally by the compiler when linking
# a shared library.
compiler_lib_search_path=$lt_compiler_lib_search_path_GCJ

# Method to check whether dependent libraries are shared objects.
deplibs_check_method=$lt_deplibs_check_method

# Command to use when deplibs_check_method == file_magic.
file_magic_cmd=$lt_file_magic_cmd

# Flag that allows shared libraries with undefined symbols to be built.
allow_undefined_flag=$lt_allow_undefined_flag_GCJ

# Flag that forces no undefined symbols.
no_undefined_flag=$lt_no_undefined_flag_GCJ

# Commands used to finish a libtool library installation in a directory.
finish_cmds=$lt_finish_cmds

# Same as above, but a single script fragment to be evaled but not shown.
finish_eval=$lt_finish_eval

# Take the output of nm and produce a listing of raw symbols and C names.
global_symbol_pipe=$lt_lt_cv_sys_global_symbol_pipe

# Transform the output of nm in a proper C declaration
global_symbol_to_cdecl=$lt_lt_cv_sys_global_symbol_to_cdecl

# Transform the output of nm in a C name address pair
global_symbol_to_c_name_address=$lt_lt_cv_sys_global_symbol_to_c_name_address

# This is the shared library runtime path variable.
runpath_var=$runpath_var

# This is the shared library path variable.
shlibpath_var=$shlibpath_var

# Is shlibpath searched before the hard-coded library search path?
shlibpath_overrides_runpath=$shlibpath_overrides_runpath

# How to hardcode a shared library path into an executable.
hardcode_action=$hardcode_action_GCJ

# Whether we should hardcode library paths into libraries.
hardcode_into_libs=$hardcode_into_libs

# Flag to hardcode \$libdir into a binary during linking.
# This must work even if \$libdir does not exist.
hardcode_libdir_flag_spec=$lt_hardcode_libdir_flag_spec_GCJ

# If ld is used when linking, flag to hardcode \$libdir into
# a binary during linking. This must work even if \$libdir does
# not exist.
hardcode_libdir_flag_spec_ld=$lt_hardcode_libdir_flag_spec_ld_GCJ

# Whether we need a single -rpath flag with a separated argument.
hardcode_libdir_separator=$lt_hardcode_libdir_separator_GCJ

# Set to yes if using DIR/libNAME${shared_ext} during linking hardcodes DIR into the
# resulting binary.
hardcode_direct=$hardcode_direct_GCJ

# Set to yes if using the -LDIR flag during linking hardcodes DIR into the
# resulting binary.
hardcode_minus_L=$hardcode_minus_L_GCJ

# Set to yes if using SHLIBPATH_VAR=DIR during linking hardcodes DIR into
# the resulting binary.
hardcode_shlibpath_var=$hardcode_shlibpath_var_GCJ

# Set to yes if building a shared library automatically hardcodes DIR into the library
# and all subsequent libraries and executables linked against it.
hardcode_automatic=$hardcode_automatic_GCJ

# Variables whose values should be saved in libtool wrapper scripts and
# restored at relink time.
variables_saved_for_relink="$variables_saved_for_relink"

# Whether libtool must link a program against all its dependency libraries.
link_all_deplibs=$link_all_deplibs_GCJ

# Compile-time system search path for libraries
sys_lib_search_path_spec=$lt_sys_lib_search_path_spec

# Run-time system search path for libraries
sys_lib_dlsearch_path_spec=$lt_sys_lib_dlsearch_path_spec

# Fix the shell variable \$srcfile for the compiler.
fix_srcfile_path=$lt_fix_srcfile_path

# Set to yes if exported symbols are required.
always_export_symbols=$always_export_symbols_GCJ

# The commands to list exported symbols.
export_symbols_cmds=$lt_export_symbols_cmds_GCJ

# The commands to extract the exported symbol list from a shared archive.
extract_expsyms_cmds=$lt_extract_expsyms_cmds

# Symbols that should not be listed in the preloaded symbols.
exclude_expsyms=$lt_exclude_expsyms_GCJ

# Symbols that must always be exported.
include_expsyms=$lt_include_expsyms_GCJ

# ### END LIBTOOL TAG CONFIG: $tagname

__EOF__


else
  # If there is no Makefile yet, we rely on a make rule to execute
  # `config.status --recheck' to rerun these tests and create the
  # libtool script then.
  ltmain_in=`echo $ltmain | sed -e 's/\.sh$/.in/'`
  if test -f "$ltmain_in"; then
    test -f Makefile && make "$ltmain"
  fi
fi


ac_ext=c
ac_cpp='$CPP $CPPFLAGS'
ac_compile='$CC -c $CFLAGS $CPPFLAGS conftest.$ac_ext >&5'
ac_link='$CC -o conftest$ac_exeext $CFLAGS $CPPFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_c_compiler_gnu

CC="$lt_save_CC"

	else
	  tagname=""
	fi
	;;

      RC)


# Source file extension for RC test sources.
ac_ext=rc

# Object file extension for compiled RC test sources.
objext=o
objext_RC=$objext

# Code to be used in simple compile tests
lt_simple_compile_test_code='sample MENU { MENUITEM "&Soup", 100, CHECKED }'

# Code to be used in simple link tests
lt_simple_link_test_code="$lt_simple_compile_test_code"

# ltmain only uses $CC for tagged configurations so make sure $CC is set.

# If no C compiler was specified, use CC.
LTCC=${LTCC-"$CC"}

# If no C compiler flags were specified, use CFLAGS.
LTCFLAGS=${LTCFLAGS-"$CFLAGS"}

# Allow CC to be a program name with arguments.
compiler=$CC


# save warnings/boilerplate of simple test code
ac_outfile=conftest.$ac_objext
echo "$lt_simple_compile_test_code" >conftest.$ac_ext
eval "$ac_compile" 2>&1 >/dev/null | $SED '/^$/d; /^ *+/d' >conftest.err
_lt_compiler_boilerplate=`cat conftest.err`
$rm conftest*

ac_outfile=conftest.$ac_objext
echo "$lt_simple_link_test_code" >conftest.$ac_ext
eval "$ac_link" 2>&1 >/dev/null | $SED '/^$/d; /^ *+/d' >conftest.err
_lt_linker_boilerplate=`cat conftest.err`
$rm conftest*


# Allow CC to be a program name with arguments.
lt_save_CC="$CC"
CC=${RC-"windres"}
compiler=$CC
compiler_RC=$CC
for cc_temp in $compiler""; do
  case $cc_temp in
    compile | *[\\/]compile | ccache | *[\\/]ccache ) ;;
    distcc | *[\\/]distcc | purify | *[\\/]purify ) ;;
    \-*) ;;
    *) break;;
  esac
done
cc_basename=`$echo "X$cc_temp" | $Xsed -e 's%.*/%%' -e "s%^$host_alias-%%"`

lt_cv_prog_compiler_c_o_RC=yes

# The else clause should only fire when bootstrapping the
# libtool distribution, otherwise you forgot to ship ltmain.sh
# with your package, and you will get complaints that there are
# no rules to generate ltmain.sh.
if test -f "$ltmain"; then
  # See if we are running on zsh, and set the options which allow our commands through
  # without removal of \ escapes.
  if test -n "${ZSH_VERSION+set}" ; then
    setopt NO_GLOB_SUBST
  fi
  # Now quote all the things that may contain metacharacters while being
  # careful not to overquote the AC_SUBSTed values.  We take copies of the
  # variables and quote the copies for generation of the libtool script.
  for var in echo old_CC old_CFLAGS AR AR_FLAGS EGREP RANLIB LN_S LTCC LTCFLAGS NM \
    SED SHELL STRIP \
    libname_spec library_names_spec soname_spec extract_expsyms_cmds \
    old_striplib striplib file_magic_cmd finish_cmds finish_eval \
    deplibs_check_method reload_flag reload_cmds need_locks \
    lt_cv_sys_global_symbol_pipe lt_cv_sys_global_symbol_to_cdecl \
    lt_cv_sys_global_symbol_to_c_name_address \
    sys_lib_search_path_spec sys_lib_dlsearch_path_spec \
    old_postinstall_cmds old_postuninstall_cmds \
    compiler_RC \
    CC_RC \
    LD_RC \
    lt_prog_compiler_wl_RC \
    lt_prog_compiler_pic_RC \
    lt_prog_compiler_static_RC \
    lt_prog_compiler_no_builtin_flag_RC \
    export_dynamic_flag_spec_RC \
    thread_safe_flag_spec_RC \
    whole_archive_flag_spec_RC \
    enable_shared_with_static_runtimes_RC \
    old_archive_cmds_RC \
    old_archive_from_new_cmds_RC \
    predep_objects_RC \
    postdep_objects_RC \
    predeps_RC \
    postdeps_RC \
    compiler_lib_search_path_RC \
    archive_cmds_RC \
    archive_expsym_cmds_RC \
    postinstall_cmds_RC \
    postuninstall_cmds_RC \
    old_archive_from_expsyms_cmds_RC \
    allow_undefined_flag_RC \
    no_undefined_flag_RC \
    export_symbols_cmds_RC \
    hardcode_libdir_flag_spec_RC \
    hardcode_libdir_flag_spec_ld_RC \
    hardcode_libdir_separator_RC \
    hardcode_automatic_RC \
    module_cmds_RC \
    module_expsym_cmds_RC \
    lt_cv_prog_compiler_c_o_RC \
    fix_srcfile_path_RC \
    exclude_expsyms_RC \
    include_expsyms_RC; do

    case $var in
    old_archive_cmds_RC | \
    old_archive_from_new_cmds_RC | \
    archive_cmds_RC | \
    archive_expsym_cmds_RC | \
    module_cmds_RC | \
    module_expsym_cmds_RC | \
    old_archive_from_expsyms_cmds_RC | \
    export_symbols_cmds_RC | \
    extract_expsyms_cmds | reload_cmds | finish_cmds | \
    postinstall_cmds | postuninstall_cmds | \
    old_postinstall_cmds | old_postuninstall_cmds | \
    sys_lib_search_path_spec | sys_lib_dlsearch_path_spec)
      # Double-quote double-evaled strings.
      eval "lt_$var=\\\"\`\$echo \"X\$$var\" | \$Xsed -e \"\$double_quote_subst\" -e \"\$sed_quote_subst\" -e \"\$delay_variable_subst\"\`\\\""
      ;;
    *)
      eval "lt_$var=\\\"\`\$echo \"X\$$var\" | \$Xsed -e \"\$sed_quote_subst\"\`\\\""
      ;;
    esac
  done

  case $lt_echo in
  *'\$0 --fallback-echo"')
    lt_echo=`$echo "X$lt_echo" | $Xsed -e 's/\\\\\\\$0 --fallback-echo"$/$0 --fallback-echo"/'`
    ;;
  esac

cfgfile="$ofile"

  cat <<__EOF__ >> "$cfgfile"
# ### BEGIN LIBTOOL TAG CONFIG: $tagname

# Libtool was configured on host `(hostname || uname -n) 2>/dev/null | sed 1q`:

# Shell to use when invoking shell scripts.
SHELL=$lt_SHELL

# Whether or not to build shared libraries.
build_libtool_libs=$enable_shared

# Whether or not to build static libraries.
build_old_libs=$enable_static

# Whether or not to add -lc for building shared libraries.
build_libtool_need_lc=$archive_cmds_need_lc_RC

# Whether or not to disallow shared libs when runtime libs are static
allow_libtool_libs_with_static_runtimes=$enable_shared_with_static_runtimes_RC

# Whether or not to optimize for fast installation.
fast_install=$enable_fast_install

# The host system.
host_alias=$host_alias
host=$host
host_os=$host_os

# The build system.
build_alias=$build_alias
build=$build
build_os=$build_os

# An echo program that does not interpret backslashes.
echo=$lt_echo

# The archiver.
AR=$lt_AR
AR_FLAGS=$lt_AR_FLAGS

# A C compiler.
LTCC=$lt_LTCC

# LTCC compiler flags.
LTCFLAGS=$lt_LTCFLAGS

# A language-specific compiler.
CC=$lt_compiler_RC

# Is the compiler the GNU C compiler?
with_gcc=$GCC_RC

# An ERE matcher.
EGREP=$lt_EGREP

# The linker used to build libraries.
LD=$lt_LD_RC

# Whether we need hard or soft links.
LN_S=$lt_LN_S

# A BSD-compatible nm program.
NM=$lt_NM

# A symbol stripping program
STRIP=$lt_STRIP

# Used to examine libraries when file_magic_cmd begins "file"
MAGIC_CMD=$MAGIC_CMD

# Used on cygwin: DLL creation program.
DLLTOOL="$DLLTOOL"

# Used on cygwin: object dumper.
OBJDUMP="$OBJDUMP"

# Used on cygwin: assembler.
AS="$AS"

# The name of the directory that contains temporary libtool files.
objdir=$objdir

# How to create reloadable object files.
reload_flag=$lt_reload_flag
reload_cmds=$lt_reload_cmds

# How to pass a linker flag through the compiler.
wl=$lt_lt_prog_compiler_wl_RC

# Object file suffix (normally "o").
objext="$ac_objext"

# Old archive suffix (normally "a").
libext="$libext"

# Shared library suffix (normally ".so").
shrext_cmds='$shrext_cmds'

# Executable file suffix (normally "").
exeext="$exeext"

# Additional compiler flags for building library objects.
pic_flag=$lt_lt_prog_compiler_pic_RC
pic_mode=$pic_mode

# What is the maximum length of a command?
max_cmd_len=$lt_cv_sys_max_cmd_len

# Does compiler simultaneously support -c and -o options?
compiler_c_o=$lt_lt_cv_prog_compiler_c_o_RC

# Must we lock files when doing compilation?
need_locks=$lt_need_locks

# Do we need the lib prefix for modules?
need_lib_prefix=$need_lib_prefix

# Do we need a version for libraries?
need_version=$need_version

# Whether dlopen is supported.
dlopen_support=$enable_dlopen

# Whether dlopen of programs is supported.
dlopen_self=$enable_dlopen_self

# Whether dlopen of statically linked programs is supported.
dlopen_self_static=$enable_dlopen_self_static

# Compiler flag to prevent dynamic linking.
link_static_flag=$lt_lt_prog_compiler_static_RC

# Compiler flag to turn off builtin functions.
no_builtin_flag=$lt_lt_prog_compiler_no_builtin_flag_RC

# Compiler flag to allow reflexive dlopens.
export_dynamic_flag_spec=$lt_export_dynamic_flag_spec_RC

# Compiler flag to generate shared objects directly from archives.
whole_archive_flag_spec=$lt_whole_archive_flag_spec_RC

# Compiler flag to generate thread-safe objects.
thread_safe_flag_spec=$lt_thread_safe_flag_spec_RC

# Library versioning type.
version_type=$version_type

# Format of library name prefix.
libname_spec=$lt_libname_spec

# List of archive names.  First name is the real one, the rest are links.
# The last name is the one that the linker finds with -lNAME.
library_names_spec=$lt_library_names_spec

# The coded name of the library, if different from the real name.
soname_spec=$lt_soname_spec

# Commands used to build and install an old-style archive.
RANLIB=$lt_RANLIB
old_archive_cmds=$lt_old_archive_cmds_RC
old_postinstall_cmds=$lt_old_postinstall_cmds
old_postuninstall_cmds=$lt_old_postuninstall_cmds

# Create an old-style archive from a shared archive.
old_archive_from_new_cmds=$lt_old_archive_from_new_cmds_RC

# Create a temporary old-style archive to link instead of a shared archive.
old_archive_from_expsyms_cmds=$lt_old_archive_from_expsyms_cmds_RC

# Commands used to build and install a shared archive.
archive_cmds=$lt_archive_cmds_RC
archive_expsym_cmds=$lt_archive_expsym_cmds_RC
postinstall_cmds=$lt_postinstall_cmds
postuninstall_cmds=$lt_postuninstall_cmds

# Commands used to build a loadable module (assumed same as above if empty)
module_cmds=$lt_module_cmds_RC
module_expsym_cmds=$lt_module_expsym_cmds_RC

# Commands to strip libraries.
old_striplib=$lt_old_striplib
striplib=$lt_striplib

# Dependencies to place before the objects being linked to create a
# shared library.
predep_objects=$lt_predep_objects_RC

# Dependencies to place after the objects being linked to create a
# shared library.
postdep_objects=$lt_postdep_objects_RC

# Dependencies to place before the objects being linked to create a
# shared library.
predeps=$lt_predeps_RC

# Dependencies to place after the objects being linked to create a
# shared library.
postdeps=$lt_postdeps_RC

# The library search path used internally by the compiler when linking
# a shared library.
compiler_lib_search_path=$lt_compiler_lib_search_path_RC

# Method to check whether dependent libraries are shared objects.
deplibs_check_method=$lt_deplibs_check_method

# Command to use when deplibs_check_method == file_magic.
file_magic_cmd=$lt_file_magic_cmd

# Flag that allows shared libraries with undefined symbols to be built.
allow_undefined_flag=$lt_allow_undefined_flag_RC

# Flag that forces no undefined symbols.
no_undefined_flag=$lt_no_undefined_flag_RC

# Commands used to finish a libtool library installation in a directory.
finish_cmds=$lt_finish_cmds

# Same as above, but a single script fragment to be evaled but not shown.
finish_eval=$lt_finish_eval

# Take the output of nm and produce a listing of raw symbols and C names.
global_symbol_pipe=$lt_lt_cv_sys_global_symbol_pipe

# Transform the output of nm in a proper C declaration
global_symbol_to_cdecl=$lt_lt_cv_sys_global_symbol_to_cdecl

# Transform the output of nm in a C name address pair
global_symbol_to_c_name_address=$lt_lt_cv_sys_global_symbol_to_c_name_address

# This is the shared library runtime path variable.
runpath_var=$runpath_var

# This is the shared library path variable.
shlibpath_var=$shlibpath_var

# Is shlibpath searched before the hard-coded library search path?
shlibpath_overrides_runpath=$shlibpath_overrides_runpath

# How to hardcode a shared library path into an executable.
hardcode_action=$hardcode_action_RC

# Whether we should hardcode library paths into libraries.
hardcode_into_libs=$hardcode_into_libs

# Flag to hardcode \$libdir into a binary during linking.
# This must work even if \$libdir does not exist.
hardcode_libdir_flag_spec=$lt_hardcode_libdir_flag_spec_RC

# If ld is used when linking, flag to hardcode \$libdir into
# a binary during linking. This must work even if \$libdir does
# not exist.
hardcode_libdir_flag_spec_ld=$lt_hardcode_libdir_flag_spec_ld_RC

# Whether we need a single -rpath flag with a separated argument.
hardcode_libdir_separator=$lt_hardcode_libdir_separator_RC

# Set to yes if using DIR/libNAME${shared_ext} during linking hardcodes DIR into the
# resulting binary.
hardcode_direct=$hardcode_direct_RC

# Set to yes if using the -LDIR flag during linking hardcodes DIR into the
# resulting binary.
hardcode_minus_L=$hardcode_minus_L_RC

# Set to yes if using SHLIBPATH_VAR=DIR during linking hardcodes DIR into
# the resulting binary.
hardcode_shlibpath_var=$hardcode_shlibpath_var_RC

# Set to yes if building a shared library automatically hardcodes DIR into the library
# and all subsequent libraries and executables linked against it.
hardcode_automatic=$hardcode_automatic_RC

# Variables whose values should be saved in libtool wrapper scripts and
# restored at relink time.
variables_saved_for_relink="$variables_saved_for_relink"

# Whether libtool must link a program against all its dependency libraries.
link_all_deplibs=$link_all_deplibs_RC

# Compile-time system search path for libraries
sys_lib_search_path_spec=$lt_sys_lib_search_path_spec

# Run-time system search path for libraries
sys_lib_dlsearch_path_spec=$lt_sys_lib_dlsearch_path_spec

# Fix the shell variable \$srcfile for the compiler.
fix_srcfile_path=$lt_fix_srcfile_path

# Set to yes if exported symbols are required.
always_export_symbols=$always_export_symbols_RC

# The commands to list exported symbols.
export_symbols_cmds=$lt_export_symbols_cmds_RC

# The commands to extract the exported symbol list from a shared archive.
extract_expsyms_cmds=$lt_extract_expsyms_cmds

# Symbols that should not be listed in the preloaded symbols.
exclude_expsyms=$lt_exclude_expsyms_RC

# Symbols that must always be exported.
include_expsyms=$lt_include_expsyms_RC

# ### END LIBTOOL TAG CONFIG: $tagname

__EOF__


else
  # If there is no Makefile yet, we rely on a make rule to execute
  # `config.status --recheck' to rerun these tests and create the
  # libtool script then.
  ltmain_in=`echo $ltmain | sed -e 's/\.sh$/.in/'`
  if test -f "$ltmain_in"; then
    test -f Makefile && make "$ltmain"
  fi
fi


ac_ext=c
ac_cpp='$CPP $CPPFLAGS'
ac_compile='$CC -c $CFLAGS $CPPFLAGS conftest.$ac_ext >&5'
ac_link='$CC -o conftest$ac_exeext $CFLAGS $CPPFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_c_compiler_gnu

CC="$lt_save_CC"

	;;

      *)
	{ { echo "$as_me:$LINENO: error: Unsupported tag name: $tagname" >&5
echo "$as_me: error: Unsupported tag name: $tagname" >&2;}
   { (exit 1); exit 1; }; }
	;;
      esac

      # Append the new tag name to the list of available tags.
      if test -n "$tagname" ; then
      available_tags="$available_tags $tagname"
    fi
    fi
  done
  IFS="$lt_save_ifs"

  # Now substitute the updated list of available tags.
  if eval "sed -e 's/^available_tags=.*\$/available_tags=\"$available_tags\"/' \"$ofile\" > \"${ofile}T\""; then
    mv "${ofile}T" "$ofile"
    chmod +x "$ofile"
  else
    rm -f "${ofile}T"
    { { echo "$as_me:$LINENO: error: unable to update list of available tagged configurations." >&5
echo "$as_me: error: unable to update list of available tagged configurations." >&2;}
   { (exit 1); exit 1; }; }
  fi
fi



# This can be used to rebuild libtool when needed
LIBTOOL_DEPS="$ac_aux_dir/ltmain.sh"

# Always use our own libtool.
LIBTOOL='$(SHELL) $(top_builddir)/libtool'

# Prevent multiple expansion





















# Extract the first word of "latex", so it can be a program name with args.
set dummy latex; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_LATEX+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$LATEX"; then
  ac_cv_prog_LATEX="$LATEX" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_test_x "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_LATEX="latex"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
LATEX=$ac_cv_prog_LATEX
if test -n "$LATEX"; then
  { echo "$as_me:$LINENO: result: $LATEX" >&5
echo "${ECHO_T}$LATEX" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi


# Extract the first word of "pdflatex", so it can be a program name with args.
set dummy pdflatex; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_PDFLATEX+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$PDFLATEX"; then
  ac_cv_prog_PDFLATEX="$PDFLATEX" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_test_x "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_PDFLATEX="pdflatex"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
PDFLATEX=$ac_cv_prog_PDFLATEX
if test -n "$PDFLATEX"; then
  { echo "$as_me:$LINENO: result: $PDFLATEX" >&5
echo "${ECHO_T}$PDFLATEX" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi


# Extract the first word of "bibtex", so it can be a program name with args.
set dummy bibtex; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_BIBTEX+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$BIBTEX"; then
  ac_cv_prog_BIBTEX="$BIBTEX" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_test_x "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_BIBTEX="bibtex"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
BIBTEX=$ac_cv_prog_BIBTEX
if test -n "$BIBTEX"; then
  { echo "$as_me:$LINENO: result: $BIBTEX" >&5
echo "${ECHO_T}$BIBTEX" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi


# Extract the first word of "dvips", so it can be a program name with args.
set dummy dvips; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_DVIPS+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$DVIPS"; then
  ac_cv_prog_DVIPS="$DVIPS" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_test_x "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_DVIPS="dvips"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
DVIPS=$ac_cv_prog_DVIPS
if test -n "$DVIPS"; then
  { echo "$as_me:$LINENO: result: $DVIPS" >&5
echo "${ECHO_T}$DVIPS" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi


# Extract the first word of "ps2pdf", so it can be a program name with args.
set dummy ps2pdf; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_PS2PDF+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$PS2PDF"; then
  ac_cv_prog_PS2PDF="$PS2PDF" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_test_x "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_PS2PDF="ps2pdf"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
PS2PDF=$ac_cv_prog_PS2PDF
if test -n "$PS2PDF"; then
  { echo "$as_me:$LINENO: result: $PS2PDF" >&5
echo "${ECHO_T}$PS2PDF" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi



# Checks for libraries.

# Checks for header files.

# Checks for typedefs, structures, and compiler characteristics.

# Checks for library functions.

ac_config_files="$ac_config_files Makefile"

cat >confcache <<\_ACEOF
# This file is a shell script that caches the results of configure
# tests run on this system so they can be shared between configure
# scripts and configure runs, see configure's option --config-cache.
# It is not useful on other systems.  If it contains results you don't
# want to keep, you may remove or edit it.
#
# config.status only pays attention to the cache file if you give it
# the --recheck option to rerun configure.
#
# `ac_cv_env_foo' variables (set or unset) will be overridden when
# loading this file, other *unset* `ac_cv_foo' will be assigned the
# following values.

_ACEOF

# The following way of writing the cache mishandles newlines in values,
# but we know of no workaround that is simple, portable, and efficient.
# So, we kill variables containing newlines.
# Ultrix sh set writes to stderr and can't be redirected directly,
# and sets the high bit in the cache file unless we assign to the vars.
(
  for ac_var in `(set) 2>&1 | sed -n 's/^\([a-zA-Z_][a-zA-Z0-9_]*\)=.*/\1/p'`; do
    eval ac_val=\$$ac_var
    case $ac_val in #(
    *${as_nl}*)
      case $ac_var in #(
      *_cv_*) { echo "$as_me:$LINENO: WARNING: Cache variable $ac_var contains a newline." >&5
echo "$as_me: WARNING: Cache variable $ac_var contains a newline." >&2;} ;;
      esac
      case $ac_var in #(
      _ | IFS | as_nl) ;; #(
      *) $as_unset $ac_var ;;
      esac ;;
    esac
  done

  (set) 2>&1 |
    case $as_nl`(ac_space=' '; set) 2>&1` in #(
    *${as_nl}ac_space=\ *)
      # `set' does not quote correctly, so add quotes (double-quote
      # substitution turns \\\\ into \\, and sed turns \\ into \).
      sed -n \
	"s/'/'\\\\''/g;
	  s/^\\([_$as_cr_alnum]*_cv_[_$as_cr_alnum]*\\)=\\(.*\\)/\\1='\\2'/p"
      ;; #(
    *)
      # `set' quotes correctly as required by POSIX, so do not add quotes.
      sed -n "/^[_$as_cr_alnum]*_cv_[_$as_cr_alnum]*=/p"
      ;;
    esac |
    sort
) |
  sed '
     /^ac_cv_env_/b end
     t clear
     :clear
     s/^\([^=]*\)=\(.*[{}].*\)$/test "${\1+set}" = set || &/
     t end
     s/^\([^=]*\)=\(.*\)$/\1=${\1=\2}/
     :end' >>confcache
if diff "$cache_file" confcache >/dev/null 2>&1; then :; else
  if test -w "$cache_file"; then
    test "x$cache_file" != "x/dev/null" &&
      { echo "$as_me:$LINENO: updating cache $cache_file" >&5
echo "$as_me: updating cache $cache_file" >&6;}
    cat confcache >$cache_file
  else
    { echo "$as_me:$LINENO: not updating unwritable cache $cache_file" >&5
echo "$as_me: not updating unwritable cache $cache_file" >&6;}
  fi
fi
rm -f confcache

test "x$prefix" = xNONE && prefix=$ac_default_prefix
# Let make expand exec_prefix.
test "x$exec_prefix" = xNONE && exec_prefix='${prefix}'

# Transform confdefs.h into DEFS.
# Protect against shell expansion while executing Makefile rules.
# Protect against Makefile macro expansion.
#
# If the first sed substitution is executed (which looks for macros that
# take arguments), then branch to the quote section.  Otherwise,
# look for a macro that doesn't take arguments.
ac_script='
t clear
:clear
s/^[	 ]*#[	 ]*define[	 ][	 ]*\([^	 (][^	 (]*([^)]*)\)[	 ]*\(.*\)/-D\1=\2/g
t quote
s/^[	 ]*#[	 ]*define[	 ][	 ]*\([^	 ][^	 ]*\)[	 ]*\(.*\)/-D\1=\2/g
t quote
b any
:quote
s/[	 `~#$^&*(){}\\|;'\''"<>?]/\\&/g
s/\[/\\&/g
s/\]/\\&/g
s/\$/$$/g
H
:any
${
	g
	s/^\n//
	s/\n/ /g
	p
}
'
DEFS=`sed -n "$ac_script" confdefs.h`


ac_libobjs=
ac_ltlibobjs=
for ac_i in : $LIBOBJS; do test "x$ac_i" = x: && continue
  # 1. Remove the extension, and $U if already installed.
  ac_script='s/\$U\././;s/\.o$//;s/\.obj$//'
  ac_i=`echo "$ac_i" | sed "$ac_script"`
  # 2. Prepend LIBOBJDIR.  When used with automake>=1.10 LIBOBJDIR
  #    will be set to the directory where LIBOBJS objects are built.
  ac_libobjs="$ac_libobjs \${LIBOBJDIR}$ac_i\$U.$ac_objext"
  ac_ltlibobjs="$ac_ltlibobjs \${LIBOBJDIR}$ac_i"'$U.lo'
done
LIBOBJS=$ac_libobjs

LTLIBOBJS=$ac_ltlibobjs


if test -z "${AMDEP_TRUE}" && test -z "${AMDEP_FALSE}"; then
  { { echo "$as_me:$LINENO: error: conditional \"AMDEP\" was never defined.
Usually this means the macro was only invoked conditionally." >&5
echo "$as_me: error: conditional \"AMDEP\" was never defined.
Usually this means the macro was only invoked conditionally." >&2;}
   { (exit 1); exit 1; }; }
fi
if test -z "${am__fastdepCC_TRUE}" && test -z "${am__fastdepCC_FALSE}"; then
  { { echo "$as_me:$LINENO: error: conditional \"am__fastdepCC\" was never defined.
Usually this means the macro was only invoked conditionally." >&5
echo "$as_me: error: conditional \"am__fastdepCC\" was never defined.
Usually this means the macro was only invoked conditionally." >&2;}
   { (exit 1); exit 1; }; }
fi
if test -z "${am__fastdepCXX_TRUE}" && test -z "${am__fastdepCXX_FALSE}"; then
  { { echo "$as_me:$LINENO: error: conditional \"am__fastdepCXX\" was never defined.
Usually this means the macro was only invoked conditionally." >&5
echo "$as_me: error: conditional \"am__fastdepCXX\" was never defined.
Usually this means the macro was only invoked conditionally." >&2;}
   { (exit 1); exit 1; }; }
fi

: ${CONFIG_STATUS=./config.status}
ac_clean_files_save=$ac_clean_files
ac_clean_files="$ac_clean_files $CONFIG_STATUS"
{ echo "$as_me:$LINENO: creating $CONFIG_STATUS" >&5
echo "$as_me: creating $CONFIG_STATUS" >&6;}
cat >$CONFIG_STATUS <<_ACEOF
#! $SHELL
# Generated by $as_me.
# Run this file to recreate the current configuration.
# Compiler output produced by configure, useful for debugging
# configure, is in config.log if it exists.

debug=false
ac_cs_recheck=false
ac_cs_silent=false
SHELL=\${CONFIG_SHELL-$SHELL}
_ACEOF

cat >>$CONFIG_STATUS <<\_ACEOF
## --------------------- ##
## M4sh Initialization.  ##
## --------------------- ##

# Be more Bourne compatible
DUALCASE=1; export DUALCASE # for MKS sh
if test -n "${ZSH_VERSION+set}" && (emulate sh) >/dev/null 2>&1; then
  emulate sh
  NULLCMD=:
  # Zsh 3.x and 4.x performs word splitting on ${1+"$@"}, which
  # is contrary to our usage.  Disable this feature.
  alias -g '${1+"$@"}'='"$@"'
  setopt NO_GLOB_SUBST
else
  case `(set -o) 2>/dev/null` in
  *posix*) set -o posix ;;
esac

fi




# PATH needs CR
# Avoid depending upon Character Ranges.
as_cr_letters='abcdefghijklmnopqrstuvwxyz'
as_cr_LETTERS='ABCDEFGHIJKLMNOPQRSTUVWXYZ'
as_cr_Letters=$as_cr_letters$as_cr_LETTERS
as_cr_digits='0123456789'
as_cr_alnum=$as_cr_Letters$as_cr_digits

# The user is always right.
if test "${PATH_SEPARATOR+set}" != set; then
  echo "#! /bin/sh" >conf$$.sh
  echo  "exit 0"   >>conf$$.sh
  chmod +x conf$$.sh
  if (PATH="/nonexistent;."; conf$$.sh) >/dev/null 2>&1; then
    PATH_SEPARATOR=';'
  else
    PATH_SEPARATOR=:
  fi
  rm -f conf$$.sh
fi

# Support unset when possible.
if ( (MAIL=60; unset MAIL) || exit) >/dev/null 2>&1; then
  as_unset=unset
else
  as_unset=false
fi


# IFS
# We need space, tab and new line, in precisely that order.  Quoting is
# there to prevent editors from complaining about space-tab.
# (If _AS_PATH_WALK were called with IFS unset, it would disable word
# splitting by setting IFS to empty value.)
as_nl='
'
IFS=" ""	$as_nl"

# Find who we are.  Look in the path if we contain no directory separator.
case $0 in
  *[\\/]* ) as_myself=$0 ;;
  *) as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  test -r "$as_dir/$0" && as_myself=$as_dir/$0 && break
done
IFS=$as_save_IFS

     ;;
esac
# We did not find ourselves, most probably we were run as `sh COMMAND'
# in which case we are not to be found in the path.
if test "x$as_myself" = x; then
  as_myself=$0
fi
if test ! -f "$as_myself"; then
  echo "$as_myself: error: cannot find myself; rerun with an absolute file name" >&2
  { (exit 1); exit 1; }
fi

# Work around bugs in pre-3.0 UWIN ksh.
for as_var in ENV MAIL MAILPATH
do ($as_unset $as_var) >/dev/null 2>&1 && $as_unset $as_var
done
PS1='$ '
PS2='> '
PS4='+ '

# NLS nuisances.
for as_var in \
  LANG LANGUAGE LC_ADDRESS LC_ALL LC_COLLATE LC_CTYPE LC_IDENTIFICATION \
  LC_MEASUREMENT LC_MESSAGES LC_MONETARY LC_NAME LC_NUMERIC LC_PAPER \
  LC_TELEPHONE LC_TIME
do
  if (set +x; test -z "`(eval $as_var=C; export $as_var) 2>&1`"); then
    eval $as_var=C; export $as_var
  else
    ($as_unset $as_var) >/dev/null 2>&1 && $as_unset $as_var
  fi
done

# Required to use basename.
if expr a : '\(a\)' >/dev/null 2>&1 &&
   test "X`expr 00001 : '.*\(...\)'`" = X001; then
  as_expr=expr
else
  as_expr=false
fi

if (basename -- /) >/dev/null 2>&1 && test "X`basename -- / 2>&1`" = "X/"; then
  as_basename=basename
else
  as_basename=false
fi


# Name of the executable.
as_me=`$as_basename -- "$0" ||
$as_expr X/"$0" : '.*/\([^/][^/]*\)/*$' \| \
	 X"$0" : 'X\(//\)$' \| \
	 X"$0" : 'X\(/\)' \| . 2>/dev/null ||
echo X/"$0" |
    sed '/^.*\/\([^/][^/]*\)\/*$/{
	    s//\1/
	    q
	  }
	  /^X\/\(\/\/\)$/{
	    s//\1/
	    q
	  }
	  /^X\/\(\/\).*/{
	    s//\1/
	    q
	  }
	  s/.*/./; q'`

# CDPATH.
$as_unset CDPATH



  as_lineno_1=$LINENO
  as_lineno_2=$LINENO
  test "x$as_lineno_1" != "x$as_lineno_2" &&
  test "x`expr $as_lineno_1 + 1`" = "x$as_lineno_2" || {

  # Create $as_me.lineno as a copy of $as_myself, but with $LINENO
  # uniformly replaced by the line number.  The first 'sed' inserts a
  # line-number line after each line using $LINENO; the second 'sed'
  # does the real work.  The second script uses 'N' to pair each
  # line-number line with the line containing $LINENO, and appends
  # trailing '-' during substitution so that $LINENO is not a special
  # case at line end.
  # (Raja R Harinath suggested sed '=', and Paul Eggert wrote the
  # scripts with optimization help from Paolo Bonzini.  Blame Lee
  # E. McMahon (1931-1989) for sed's syntax.  :-)
  sed -n '
    p
    /[$]LINENO/=
  ' <$as_myself |
    sed '
      s/[$]LINENO.*/&-/
      t lineno
      b
      :lineno
      N
      :loop
      s/[$]LINENO\([^'$as_cr_alnum'_].*\n\)\(.*\)/\2\1\2/
      t loop
      s/-\n.*//
    ' >$as_me.lineno &&
  chmod +x "$as_me.lineno" ||
    { echo "$as_me: error: cannot create $as_me.lineno; rerun with a POSIX shell" >&2
   { (exit 1); exit 1; }; }

  # Don't try to exec as it changes $[0], causing all sort of problems
  # (the dirname of $[0] is not the place where we might find the
  # original and so on.  Autoconf is especially sensitive to this).
  . "./$as_me.lineno"
  # Exit status is that of the last command.
  exit
}


if (as_dir=`dirname -- /` && test "X$as_dir" = X/) >/dev/null 2>&1; then
  as_dirname=dirname
else
  as_dirname=false
fi

ECHO_C= ECHO_N= ECHO_T=
case `echo -n x` in
-n*)
  case `echo 'x\c'` in
  *c*) ECHO_T='	';;	# ECHO_T is single tab character.
  *)   ECHO_C='\c';;
  esac;;
*)
  ECHO_N='-n';;
esac

if expr a : '\(a\)' >/dev/null 2>&1 &&
   test "X`expr 00001 : '.*\(...\)'`" = X001; then
  as_expr=expr
else
  as_expr=false
fi

rm -f conf$$ conf$$.exe conf$$.file
if test -d conf$$.dir; then
  rm -f conf$$.dir/conf$$.file
else
  rm -f conf$$.dir
  mkdir conf$$.dir
fi
echo >conf$$.file
if ln -s conf$$.file conf$$ 2>/dev/null; then
  as_ln_s='ln -s'
  # ... but there are two gotchas:
  # 1) On MSYS, both `ln -s file dir' and `ln file dir' fail.
  # 2) DJGPP < 2.04 has no symlinks; `ln -s' creates a wrapper executable.
  # In both cases, we have to default to `cp -p'.
  ln -s conf$$.file conf$$.dir 2>/dev/null && test ! -f conf$$.exe ||
    as_ln_s='cp -p'
elif ln conf$$.file conf$$ 2>/dev/null; then
  as_ln_s=ln
else
  as_ln_s='cp -p'
fi
rm -f conf$$ conf$$.exe conf$$.dir/conf$$.file conf$$.file
rmdir conf$$.dir 2>/dev/null

if mkdir -p . 2>/dev/null; then
  as_mkdir_p=:
else
  test -d ./-p && rmdir ./-p
  as_mkdir_p=false
fi

if test -x / >/dev/null 2>&1; then
  as_test_x='test -x'
else
  if ls -dL / >/dev/null 2>&1; then
    as_ls_L_option=L
  else
    as_ls_L_option=
  fi
  as_test_x='
    eval sh -c '\''
      if test -d "$1"; then
        test -d "$1/.";
      else
	case $1 in
        -*)set "./$1";;
	esac;
	case `ls -ld'$as_ls_L_option' "$1" 2>/dev/null` in
	???[sx]*):;;*)false;;esac;fi
    '\'' sh
  '
fi
as_executable_p=$as_test_x

# Sed expression to map a string onto a valid CPP name.
as_tr_cpp="eval sed 'y%*$as_cr_letters%P$as_cr_LETTERS%;s%[^_$as_cr_alnum]%_%g'"

# Sed expression to map a string onto a valid variable name.
as_tr_sh="eval sed 'y%*+%pp%;s%[^_$as_cr_alnum]%_%g'"


exec 6>&1

# Save the log message, to keep $[0] and so on meaningful, and to
# report actual input values of CONFIG_FILES etc. instead of their
# values after options handling.
ac_log="
This file was extended by WWND2008_Winter $as_me 1.0, which was
generated by GNU Autoconf 2.61.  Invocation command line was

  CONFIG_FILES    = $CONFIG_FILES
  CONFIG_HEADERS  = $CONFIG_HEADERS
  CONFIG_LINKS    = $CONFIG_LINKS
  CONFIG_COMMANDS = $CONFIG_COMMANDS
  $ $0 $@

on `(hostname || uname -n) 2>/dev/null | sed 1q`
"

_ACEOF

cat >>$CONFIG_STATUS <<_ACEOF
# Files that config.status was made for.
config_files="$ac_config_files"
config_commands="$ac_config_commands"

_ACEOF

cat >>$CONFIG_STATUS <<\_ACEOF
ac_cs_usage="\
\`$as_me' instantiates files from templates according to the
current configuration.

Usage: $0 [OPTIONS] [FILE]...

  -h, --help       print this help, then exit
  -V, --version    print version number and configuration settings, then exit
  -q, --quiet      do not print progress messages
  -d, --debug      don't remove temporary files
      --recheck    update $as_me by reconfiguring in the same conditions
  --file=FILE[:TEMPLATE]
		   instantiate the configuration file FILE

Configuration files:
$config_files

Configuration commands:
$config_commands

Report bugs to <bug-autoconf@gnu.org>."

_ACEOF
cat >>$CONFIG_STATUS <<_ACEOF
ac_cs_version="\\
WWND2008_Winter config.status 1.0
configured by $0, generated by GNU Autoconf 2.61,
  with options \\"`echo "$ac_configure_args" | sed 's/^ //; s/[\\""\`\$]/\\\\&/g'`\\"

Copyright (C) 2006 Free Software Foundation, Inc.
This config.status script is free software; the Free Software Foundation
gives unlimited permission to copy, distribute and modify it."

ac_pwd='$ac_pwd'
srcdir='$srcdir'
INSTALL='$INSTALL'
MKDIR_P='$MKDIR_P'
_ACEOF

cat >>$CONFIG_STATUS <<\_ACEOF
# If no file are specified by the user, then we need to provide default
# value.  By we need to know if files were specified by the user.
ac_need_defaults=:
while test $# != 0
do
  case $1 in
  --*=*)
    ac_option=`expr "X$1" : 'X\([^=]*\)='`
    ac_optarg=`expr "X$1" : 'X[^=]*=\(.*\)'`
    ac_shift=:
    ;;
  *)
    ac_option=$1
    ac_optarg=$2
    ac_shift=shift
    ;;
  esac

  case $ac_option in
  # Handling of the options.
  -recheck | --recheck | --rechec | --reche | --rech | --rec | --re | --r)
    ac_cs_recheck=: ;;
  --version | --versio | --versi | --vers | --ver | --ve | --v | -V )
    echo "$ac_cs_version"; exit ;;
  --debug | --debu | --deb | --de | --d | -d )
    debug=: ;;
  --file | --fil | --fi | --f )
    $ac_shift
    CONFIG_FILES="$CONFIG_FILES $ac_optarg"
    ac_need_defaults=false;;
  --he | --h |  --help | --hel | -h )
    echo "$ac_cs_usage"; exit ;;
  -q | -quiet | --quiet | --quie | --qui | --qu | --q \
  | -silent | --silent | --silen | --sile | --sil | --si | --s)
    ac_cs_silent=: ;;

  # This is an error.
  -*) { echo "$as_me: error: unrecognized option: $1
Try \`$0 --help' for more information." >&2
   { (exit 1); exit 1; }; } ;;

  *) ac_config_targets="$ac_config_targets $1"
     ac_need_defaults=false ;;

  esac
  shift
done

ac_configure_extra_args=

if $ac_cs_silent; then
  exec 6>/dev/null
  ac_configure_extra_args="$ac_configure_extra_args --silent"
fi

_ACEOF
cat >>$CONFIG_STATUS <<_ACEOF
if \$ac_cs_recheck; then
  echo "running CONFIG_SHELL=$SHELL $SHELL $0 "$ac_configure_args \$ac_configure_extra_args " --no-create --no-recursion" >&6
  CONFIG_SHELL=$SHELL
  export CONFIG_SHELL
  exec $SHELL "$0"$ac_configure_args \$ac_configure_extra_args --no-create --no-recursion
fi

_ACEOF
cat >>$CONFIG_STATUS <<\_ACEOF
exec 5>>config.log
{
  echo
  sed 'h;s/./-/g;s/^.../## /;s/...$/ ##/;p;x;p;x' <<_ASBOX
## Running $as_me. ##
_ASBOX
  echo "$ac_log"
} >&5

_ACEOF
cat >>$CONFIG_STATUS <<_ACEOF
#
# INIT-COMMANDS
#
AMDEP_TRUE="$AMDEP_TRUE" ac_aux_dir="$ac_aux_dir"

_ACEOF

cat >>$CONFIG_STATUS <<\_ACEOF

# Handling of arguments.
for ac_config_target in $ac_config_targets
do
  case $ac_config_target in
    "depfiles") CONFIG_COMMANDS="$CONFIG_COMMANDS depfiles" ;;
    "Makefile") CONFIG_FILES="$CONFIG_FILES Makefile" ;;

  *) { { echo "$as_me:$LINENO: error: invalid argument: $ac_config_target" >&5
echo "$as_me: error: invalid argument: $ac_config_target" >&2;}
   { (exit 1); exit 1; }; };;
  esac
done


# If the user did not use the arguments to specify the items to instantiate,
# then the envvar interface is used.  Set only those that are not.
# We use the long form for the default assignment because of an extremely
# bizarre bug on SunOS 4.1.3.
if $ac_need_defaults; then
  test "${CONFIG_FILES+set}" = set || CONFIG_FILES=$config_files
  test "${CONFIG_COMMANDS+set}" = set || CONFIG_COMMANDS=$config_commands
fi

# Have a temporary directory for convenience.  Make it in the build tree
# simply because there is no reason against having it here, and in addition,
# creating and moving files from /tmp can sometimes cause problems.
# Hook for its removal unless debugging.
# Note that there is a small window in which the directory will not be cleaned:
# after its creation but before its name has been assigned to `$tmp'.
$debug ||
{
  tmp=
  trap 'exit_status=$?
  { test -z "$tmp" || test ! -d "$tmp" || rm -fr "$tmp"; } && exit $exit_status
' 0
  trap '{ (exit 1); exit 1; }' 1 2 13 15
}
# Create a (secure) tmp directory for tmp files.

{
  tmp=`(umask 077 && mktemp -d "./confXXXXXX") 2>/dev/null` &&
  test -n "$tmp" && test -d "$tmp"
}  ||
{
  tmp=./conf$$-$RANDOM
  (umask 077 && mkdir "$tmp")
} ||
{
   echo "$me: cannot create a temporary directory in ." >&2
   { (exit 1); exit 1; }
}

#
# Set up the sed scripts for CONFIG_FILES section.
#

# No need to generate the scripts if there are no CONFIG_FILES.
# This happens for instance when ./config.status config.h
if test -n "$CONFIG_FILES"; then

_ACEOF



ac_delim='%!_!# '
for ac_last_try in false false false false false :; do
  cat >conf$$subs.sed <<_ACEOF
SHELL!$SHELL$ac_delim
PATH_SEPARATOR!$PATH_SEPARATOR$ac_delim
PACKAGE_NAME!$PACKAGE_NAME$ac_delim
PACKAGE_TARNAME!$PACKAGE_TARNAME$ac_delim
PACKAGE_VERSION!$PACKAGE_VERSION$ac_delim
PACKAGE_STRING!$PACKAGE_STRING$ac_delim
PACKAGE_BUGREPORT!$PACKAGE_BUGREPORT$ac_delim
exec_prefix!$exec_prefix$ac_delim
prefix!$prefix$ac_delim
program_transform_name!$program_transform_name$ac_delim
bindir!$bindir$ac_delim
sbindir!$sbindir$ac_delim
libexecdir!$libexecdir$ac_delim
datarootdir!$datarootdir$ac_delim
datadir!$datadir$ac_delim
sysconfdir!$sysconfdir$ac_delim
sharedstatedir!$sharedstatedir$ac_delim
localstatedir!$localstatedir$ac_delim
includedir!$includedir$ac_delim
oldincludedir!$oldincludedir$ac_delim
docdir!$docdir$ac_delim
infodir!$infodir$ac_delim
htmldir!$htmldir$ac_delim
dvidir!$dvidir$ac_delim
pdfdir!$pdfdir$ac_delim
psdir!$psdir$ac_delim
libdir!$libdir$ac_delim
localedir!$localedir$ac_delim
mandir!$mandir$ac_delim
DEFS!$DEFS$ac_delim
ECHO_C!$ECHO_C$ac_delim
ECHO_N!$ECHO_N$ac_delim
ECHO_T!$ECHO_T$ac_delim
LIBS!$LIBS$ac_delim
build_alias!$build_alias$ac_delim
host_alias!$host_alias$ac_delim
target_alias!$target_alias$ac_delim
INSTALL_PROGRAM!$INSTALL_PROGRAM$ac_delim
INSTALL_SCRIPT!$INSTALL_SCRIPT$ac_delim
INSTALL_DATA!$INSTALL_DATA$ac_delim
am__isrc!$am__isrc$ac_delim
CYGPATH_W!$CYGPATH_W$ac_delim
PACKAGE!$PACKAGE$ac_delim
VERSION!$VERSION$ac_delim
ACLOCAL!$ACLOCAL$ac_delim
AUTOCONF!$AUTOCONF$ac_delim
AUTOMAKE!$AUTOMAKE$ac_delim
AUTOHEADER!$AUTOHEADER$ac_delim
MAKEINFO!$MAKEINFO$ac_delim
install_sh!$install_sh$ac_delim
STRIP!$STRIP$ac_delim
INSTALL_STRIP_PROGRAM!$INSTALL_STRIP_PROGRAM$ac_delim
mkdir_p!$mkdir_p$ac_delim
AWK!$AWK$ac_delim
SET_MAKE!$SET_MAKE$ac_delim
am__leading_dot!$am__leading_dot$ac_delim
AMTAR!$AMTAR$ac_delim
am__tar!$am__tar$ac_delim
am__untar!$am__untar$ac_delim
CC!$CC$ac_delim
CFLAGS!$CFLAGS$ac_delim
LDFLAGS!$LDFLAGS$ac_delim
CPPFLAGS!$CPPFLAGS$ac_delim
ac_ct_CC!$ac_ct_CC$ac_delim
EXEEXT!$EXEEXT$ac_delim
OBJEXT!$OBJEXT$ac_delim
DEPDIR!$DEPDIR$ac_delim
am__include!$am__include$ac_delim
am__quote!$am__quote$ac_delim
AMDEP_TRUE!$AMDEP_TRUE$ac_delim
AMDEP_FALSE!$AMDEP_FALSE$ac_delim
AMDEPBACKSLASH!$AMDEPBACKSLASH$ac_delim
CCDEPMODE!$CCDEPMODE$ac_delim
am__fastdepCC_TRUE!$am__fastdepCC_TRUE$ac_delim
am__fastdepCC_FALSE!$am__fastdepCC_FALSE$ac_delim
CXX!$CXX$ac_delim
CXXFLAGS!$CXXFLAGS$ac_delim
ac_ct_CXX!$ac_ct_CXX$ac_delim
CXXDEPMODE!$CXXDEPMODE$ac_delim
am__fastdepCXX_TRUE!$am__fastdepCXX_TRUE$ac_delim
am__fastdepCXX_FALSE!$am__fastdepCXX_FALSE$ac_delim
build!$build$ac_delim
build_cpu!$build_cpu$ac_delim
build_vendor!$build_vendor$ac_delim
build_os!$build_os$ac_delim
host!$host$ac_delim
host_cpu!$host_cpu$ac_delim
host_vendor!$host_vendor$ac_delim
host_os!$host_os$ac_delim
SED!$SED$ac_delim
GREP!$GREP$ac_delim
EGREP!$EGREP$ac_delim
LN_S!$LN_S$ac_delim
ECHO!$ECHO$ac_delim
AR!$AR$ac_delim
RANLIB!$RANLIB$ac_delim
CPP!$CPP$ac_delim
_ACEOF

  if test `sed -n "s/.*$ac_delim\$/X/p" conf$$subs.sed | grep -c X` = 97; then
    break
  elif $ac_last_try; then
    { { echo "$as_me:$LINENO: error: could not make $CONFIG_STATUS" >&5
echo "$as_me: error: could not make $CONFIG_STATUS" >&2;}
   { (exit 1); exit 1; }; }
  else
    ac_delim="$ac_delim!$ac_delim _$ac_delim!! "
  fi
done

ac_eof=`sed -n '/^CEOF[0-9]*$/s/CEOF/0/p' conf$$subs.sed`
if test -n "$ac_eof"; then
  ac_eof=`echo "$ac_eof" | sort -nru | sed 1q`
  ac_eof=`expr $ac_eof + 1`
fi

cat >>$CONFIG_STATUS <<_ACEOF
cat >"\$tmp/subs-1.sed" <<\CEOF$ac_eof
/@[a-zA-Z_][a-zA-Z_0-9]*@/!b
_ACEOF
sed '
s/[,\\&]/\\&/g; s/@/@|#_!!_#|/g
s/^/s,@/; s/!/@,|#_!!_#|/
:n
t n
s/'"$ac_delim"'$/,g/; t
s/$/\\/; p
N; s/^.*\n//; s/[,\\&]/\\&/g; s/@/@|#_!!_#|/g; b n
' >>$CONFIG_STATUS <conf$$subs.sed
rm -f conf$$subs.sed
cat >>$CONFIG_STATUS <<_ACEOF
CEOF$ac_eof
_ACEOF


ac_delim='%!_!# '
for ac_last_try in false false false false false :; do
  cat >conf$$subs.sed <<_ACEOF
CXXCPP!$CXXCPP$ac_delim
F77!$F77$ac_delim
FFLAGS!$FFLAGS$ac_delim
ac_ct_F77!$ac_ct_F77$ac_delim
LIBTOOL!$LIBTOOL$ac_delim
LATEX!$LATEX$ac_delim
PDFLATEX!$PDFLATEX$ac_delim
BIBTEX!$BIBTEX$ac_delim
DVIPS!$DVIPS$ac_delim
PS2PDF!$PS2PDF$ac_delim
LIBOBJS!$LIBOBJS$ac_delim
LTLIBOBJS!$LTLIBOBJS$ac_delim
_ACEOF

  if test `sed -n "s/.*$ac_delim\$/X/p" conf$$subs.sed | grep -c X` = 12; then
    break
  elif $ac_last_try; then
    { { echo "$as_me:$LINENO: error: could not make $CONFIG_STATUS" >&5
echo "$as_me: error: could not make $CONFIG_STATUS" >&2;}
   { (exit 1); exit 1; }; }
  else
    ac_delim="$ac_delim!$ac_delim _$ac_delim!! "
  fi
done

ac_eof=`sed -n '/^CEOF[0-9]*$/s/CEOF/0/p' conf$$subs.sed`
if test -n "$ac_eof"; then
  ac_eof=`echo "$ac_eof" | sort -nru | sed 1q`
  ac_eof=`expr $ac_eof + 1`
fi

cat >>$CONFIG_STATUS <<_ACEOF
cat >"\$tmp/subs-2.sed" <<\CEOF$ac_eof
/@[a-zA-Z_][a-zA-Z_0-9]*@/!b end
_ACEOF
sed '
s/[,\\&]/\\&/g; s/@/@|#_!!_#|/g
s/^/s,@/; s/!/@,|#_!!_#|/
:n
t n
s/'"$ac_delim"'$/,g/; t
s/$/\\/; p
N; s/^.*\n//; s/[,\\&]/\\&/g; s/@/@|#_!!_#|/g; b n
' >>$CONFIG_STATUS <conf$$subs.sed
rm -f conf$$subs.sed
cat >>$CONFIG_STATUS <<_ACEOF
:end
s/|#_!!_#|//g
CEOF$ac_eof
_ACEOF


# VPATH may cause trouble with some makes, so we remove $(srcdir),
# ${srcdir} and @srcdir@ from VPATH if srcdir is ".", strip leading and
# trailing colons and then remove the whole line if VPATH becomes empty
# (actually we leave an empty line to preserve line numbers).
if test "x$srcdir" = x.; then
  ac_vpsub='/^[	 ]*VPATH[	 ]*=/{
s/:*\$(srcdir):*/:/
s/:*\${srcdir}:*/:/
s/:*@srcdir@:*/:/
s/^\([^=]*=[	 ]*\):*/\1/
s/:*$//
s/^[^=]*=[	 ]*$//
}'
fi

cat >>$CONFIG_STATUS <<\_ACEOF
fi # test -n "$CONFIG_FILES"


for ac_tag in  :F $CONFIG_FILES      :C $CONFIG_COMMANDS
do
  case $ac_tag in
  :[FHLC]) ac_mode=$ac_tag; continue;;
  esac
  case $ac_mode$ac_tag in
  :[FHL]*:*);;
  :L* | :C*:*) { { echo "$as_me:$LINENO: error: Invalid tag $ac_tag." >&5
echo "$as_me: error: Invalid tag $ac_tag." >&2;}
   { (exit 1); exit 1; }; };;
  :[FH]-) ac_tag=-:-;;
  :[FH]*) ac_tag=$ac_tag:$ac_tag.in;;
  esac
  ac_save_IFS=$IFS
  IFS=:
  set x $ac_tag
  IFS=$ac_save_IFS
  shift
  ac_file=$1
  shift

  case $ac_mode in
  :L) ac_source=$1;;
  :[FH])
    ac_file_inputs=
    for ac_f
    do
      case $ac_f in
      -) ac_f="$tmp/stdin";;
      *) # Look for the file first in the build tree, then in the source tree
	 # (if the path is not absolute).  The absolute path cannot be DOS-style,
	 # because $ac_f cannot contain `:'.
	 test -f "$ac_f" ||
	   case $ac_f in
	   [\\/$]*) false;;
	   *) test -f "$srcdir/$ac_f" && ac_f="$srcdir/$ac_f";;
	   esac ||
	   { { echo "$as_me:$LINENO: error: cannot find input file: $ac_f" >&5
echo "$as_me: error: cannot find input file: $ac_f" >&2;}
   { (exit 1); exit 1; }; };;
      esac
      ac_file_inputs="$ac_file_inputs $ac_f"
    done

    # Let's still pretend it is `configure' which instantiates (i.e., don't
    # use $as_me), people would be surprised to read:
    #    /* config.h.  Generated by config.status.  */
    configure_input="Generated from "`IFS=:
	  echo $* | sed 's|^[^:]*/||;s|:[^:]*/|, |g'`" by configure."
    if test x"$ac_file" != x-; then
      configure_input="$ac_file.  $configure_input"
      { echo "$as_me:$LINENO: creating $ac_file" >&5
echo "$as_me: creating $ac_file" >&6;}
    fi

    case $ac_tag in
    *:-:* | *:-) cat >"$tmp/stdin";;
    esac
    ;;
  esac

  ac_dir=`$as_dirname -- "$ac_file" ||
$as_expr X"$ac_file" : 'X\(.*[^/]\)//*[^/][^/]*/*$' \| \
	 X"$ac_file" : 'X\(//\)[^/]' \| \
	 X"$ac_file" : 'X\(//\)$' \| \
	 X"$ac_file" : 'X\(/\)' \| . 2>/dev/null ||
echo X"$ac_file" |
    sed '/^X\(.*[^/]\)\/\/*[^/][^/]*\/*$/{
	    s//\1/
	    q
	  }
	  /^X\(\/\/\)[^/].*/{
	    s//\1/
	    q
	  }
	  /^X\(\/\/\)$/{
	    s//\1/
	    q
	  }
	  /^X\(\/\).*/{
	    s//\1/
	    q
	  }
	  s/.*/./; q'`
  { as_dir="$ac_dir"
  case $as_dir in #(
  -*) as_dir=./$as_dir;;
  esac
  test -d "$as_dir" || { $as_mkdir_p && mkdir -p "$as_dir"; } || {
    as_dirs=
    while :; do
      case $as_dir in #(
      *\'*) as_qdir=`echo "$as_dir" | sed "s/'/'\\\\\\\\''/g"`;; #(
      *) as_qdir=$as_dir;;
      esac
      as_dirs="'$as_qdir' $as_dirs"
      as_dir=`$as_dirname -- "$as_dir" ||
$as_expr X"$as_dir" : 'X\(.*[^/]\)//*[^/][^/]*/*$' \| \
	 X"$as_dir" : 'X\(//\)[^/]' \| \
	 X"$as_dir" : 'X\(//\)$' \| \
	 X"$as_dir" : 'X\(/\)' \| . 2>/dev/null ||
echo X"$as_dir" |
    sed '/^X\(.*[^/]\)\/\/*[^/][^/]*\/*$/{
	    s//\1/
	    q
	  }
	  /^X\(\/\/\)[^/].*/{
	    s//\1/
	    q
	  }
	  /^X\(\/\/\)$/{
	    s//\1/
	    q
	  }
	  /^X\(\/\).*/{
	    s//\1/
	    q
	  }
	  s/.*/./; q'`
      test -d "$as_dir" && break
    done
    test -z "$as_dirs" || eval "mkdir $as_dirs"
  } || test -d "$as_dir" || { { echo "$as_me:$LINENO: error: cannot create directory $as_dir" >&5
echo "$as_me: error: cannot create directory $as_dir" >&2;}
   { (exit 1); exit 1; }; }; }
  ac_builddir=.

case "$ac_dir" in
.) ac_dir_suffix= ac_top_builddir_sub=. ac_top_build_prefix= ;;
*)
  ac_dir_suffix=/`echo "$ac_dir" | sed 's,^\.[\\/],,'`
  # A ".." for each directory in $ac_dir_suffix.
  ac_top_builddir_sub=`echo "$ac_dir_suffix" | sed 's,/[^\\/]*,/..,g;s,/,,'`
  case $ac_top_builddir_sub in
  "") ac_top_builddir_sub=. ac_top_build_prefix= ;;
  *)  ac_top_build_prefix=$ac_top_builddir_sub/ ;;
  esac ;;
esac
ac_abs_top_builddir=$ac_pwd
ac_abs_builddir=$ac_pwd$ac_dir_suffix
# for backward compatibility:
ac_top_builddir=$ac_top_build_prefix

case $srcdir in
  .)  # We are building in place.
    ac_srcdir=.
    ac_top_srcdir=$ac_top_builddir_sub
    ac_abs_top_srcdir=$ac_pwd ;;
  [\\/]* | ?:[\\/]* )  # Absolute name.
    ac_srcdir=$srcdir$ac_dir_suffix;
    ac_top_srcdir=$srcdir
    ac_abs_top_srcdir=$srcdir ;;
  *) # Relative name.
    ac_srcdir=$ac_top_build_prefix$srcdir$ac_dir_suffix
    ac_top_srcdir=$ac_top_build_prefix$srcdir
    ac_abs_top_srcdir=$ac_pwd/$srcdir ;;
esac
ac_abs_srcdir=$ac_abs_top_srcdir$ac_dir_suffix


  case $ac_mode in
  :F)
  #
  # CONFIG_FILE
  #

  case $INSTALL in
  [\\/$]* | ?:[\\/]* ) ac_INSTALL=$INSTALL ;;
  *) ac_INSTALL=$ac_top_build_prefix$INSTALL ;;
  esac
  ac_MKDIR_P=$MKDIR_P
  case $MKDIR_P in
  [\\/$]* | ?:[\\/]* ) ;;
  */*) ac_MKDIR_P=$ac_top_build_prefix$MKDIR_P ;;
  esac
_ACEOF

cat >>$CONFIG_STATUS <<\_ACEOF
# If the template does not know about datarootdir, expand it.
# FIXME: This hack should be removed a few years after 2.60.
ac_datarootdir_hack=; ac_datarootdir_seen=

case `sed -n '/datarootdir/ {
  p
  q
}
/@datadir@/p
/@docdir@/p
/@infodir@/p
/@localedir@/p
/@mandir@/p
' $ac_file_inputs` in
*datarootdir*) ac_datarootdir_seen=yes;;
*@datadir@*|*@docdir@*|*@infodir@*|*@localedir@*|*@mandir@*)
  { echo "$as_me:$LINENO: WARNING: $ac_file_inputs seems to ignore the --datarootdir setting" >&5
echo "$as_me: WARNING: $ac_file_inputs seems to ignore the --datarootdir setting" >&2;}
_ACEOF
cat >>$CONFIG_STATUS <<_ACEOF
  ac_datarootdir_hack='
  s&@datadir@&$datadir&g
  s&@docdir@&$docdir&g
  s&@infodir@&$infodir&g
  s&@localedir@&$localedir&g
  s&@mandir@&$mandir&g
    s&\\\${datarootdir}&$datarootdir&g' ;;
esac
_ACEOF

# Neutralize VPATH when `$srcdir' = `.'.
# Shell code in configure.ac might set extrasub.
# FIXME: do we really want to maintain this feature?
cat >>$CONFIG_STATUS <<_ACEOF
  sed "$ac_vpsub
$extrasub
_ACEOF
cat >>$CONFIG_STATUS <<\_ACEOF
:t
/@[a-zA-Z_][a-zA-Z_0-9]*@/!b
s&@configure_input@&$configure_input&;t t
s&@top_builddir@&$ac_top_builddir_sub&;t t
s&@srcdir@&$ac_srcdir&;t t
s&@abs_srcdir@&$ac_abs_srcdir&;t t
s&@top_srcdir@&$ac_top_srcdir&;t t
s&@abs_top_srcdir@&$ac_abs_top_srcdir&;t t
s&@builddir@&$ac_builddir&;t t
s&@abs_builddir@&$ac_abs_builddir&;t t
s&@abs_top_builddir@&$ac_abs_top_builddir&;t t
s&@INSTALL@&$ac_INSTALL&;t t
s&@MKDIR_P@&$ac_MKDIR_P&;t t
$ac_datarootdir_hack
" $ac_file_inputs | sed -f "$tmp/subs-1.sed" | sed -f "$tmp/subs-2.sed" >$tmp/out

test -z "$ac_datarootdir_hack$ac_datarootdir_seen" &&
  { ac_out=`sed -n '/\${datarootdir}/p' "$tmp/out"`; test -n "$ac_out"; } &&
  { ac_out=`sed -n '/^[	 ]*datarootdir[	 ]*:*=/p' "$tmp/out"`; test -z "$ac_out"; } &&
  { echo "$as_me:$LINENO: WARNING: $ac_file contains a reference to the variable \`datarootdir'
which seems to be undefined.  Please make sure it is defined." >&5
echo "$as_me: WARNING: $ac_file contains a reference to the variable \`datarootdir'
which seems to be undefined.  Please make sure it is defined." >&2;}

  rm -f "$tmp/stdin"
  case $ac_file in
  -) cat "$tmp/out"; rm -f "$tmp/out";;
  *) rm -f "$ac_file"; mv "$tmp/out" $ac_file;;
  esac
 ;;


  :C)  { echo "$as_me:$LINENO: executing $ac_file commands" >&5
echo "$as_me: executing $ac_file commands" >&6;}
 ;;
  esac


  case $ac_file$ac_mode in
    "depfiles":C) test x"$AMDEP_TRUE" != x"" || for mf in $CONFIG_FILES; do
  # Strip MF so we end up with the name of the file.
  mf=`echo "$mf" | sed -e 's/:.*$//'`
  # Check whether this is an Automake generated Makefile or not.
  # We used to match only the files named `Makefile.in', but
  # some people rename them; so instead we look at the file content.
  # Grep'ing the first line is not enough: some people post-process
  # each Makefile.in and add a new line on top of each file to say so.
  # Grep'ing the whole file is not good either: AIX grep has a line
  # limit of 2048, but all sed's we know have understand at least 4000.
  if sed -n 's,^#.*generated by automake.*,X,p' "$mf" | grep X >/dev/null 2>&1; then
    dirpart=`$as_dirname -- "$mf" ||
$as_expr X"$mf" : 'X\(.*[^/]\)//*[^/][^/]*/*$' \| \
	 X"$mf" : 'X\(//\)[^/]' \| \
	 X"$mf" : 'X\(//\)$' \| \
	 X"$mf" : 'X\(/\)' \| . 2>/dev/null ||
echo X"$mf" |
    sed '/^X\(.*[^/]\)\/\/*[^/][^/]*\/*$/{
	    s//\1/
	    q
	  }
	  /^X\(\/\/\)[^/].*/{
	    s//\1/
	    q
	  }
	  /^X\(\/\/\)$/{
	    s//\1/
	    q
	  }
	  /^X\(\/\).*/{
	    s//\1/
	    q
	  }
	  s/.*/./; q'`
  else
    continue
  fi
  # Extract the definition of DEPDIR, am__include, and am__quote
  # from the Makefile without running `make'.
  DEPDIR=`sed -n 's/^DEPDIR = //p' < "$mf"`
  test -z "$DEPDIR" && continue
  am__include=`sed -n 's/^am__include = //p' < "$mf"`
  test -z "am__include" && continue
  am__quote=`sed -n 's/^am__quote = //p' < "$mf"`
  # When using ansi2knr, U may be empty or an underscore; expand it
  U=`sed -n 's/^U = //p' < "$mf"`
  # Find all dependency output files, they are included files with
  # $(DEPDIR) in their names.  We invoke sed twice because it is the
  # simplest approach to changing $(DEPDIR) to its actual value in the
  # expansion.
  for file in `sed -n "
    s/^$am__include $am__quote\(.*(DEPDIR).*\)$am__quote"'$/\1/p' <"$mf" | \
       sed -e 's/\$(DEPDIR)/'"$DEPDIR"'/g' -e 's/\$U/'"$U"'/g'`; do
    # Make sure the directory exists.
    test -f "$dirpart/$file" && continue
    fdir=`$as_dirname -- "$file" ||
$as_expr X"$file" : 'X\(.*[^/]\)//*[^/][^/]*/*$' \| \
	 X"$file" : 'X\(//\)[^/]' \| \
	 X"$file" : 'X\(//\)$' \| \
	 X"$file" : 'X\(/\)' \| . 2>/dev/null ||
echo X"$file" |
    sed '/^X\(.*[^/]\)\/\/*[^/][^/]*\/*$/{
	    s//\1/
	    q
	  }
	  /^X\(\/\/\)[^/].*/{
	    s//\1/
	    q
	  }
	  /^X\(\/\/\)$/{
	    s//\1/
	    q
	  }
	  /^X\(\/\).*/{
	    s//\1/
	    q
	  }
	  s/.*/./; q'`
    { as_dir=$dirpart/$fdir
  case $as_dir in #(
  -*) as_dir=./$as_dir;;
  esac
  test -d "$as_dir" || { $as_mkdir_p && mkdir -p "$as_dir"; } || {
    as_dirs=
    while :; do
      case $as_dir in #(
      *\'*) as_qdir=`echo "$as_dir" | sed "s/'/'\\\\\\\\''/g"`;; #(
      *) as_qdir=$as_dir;;
      esac
      as_dirs="'$as_qdir' $as_dirs"
      as_dir=`$as_dirname -- "$as_dir" ||
$as_expr X"$as_dir" : 'X\(.*[^/]\)//*[^/][^/]*/*$' \| \
	 X"$as_dir" : 'X\(//\)[^/]' \| \
	 X"$as_dir" : 'X\(//\)$' \| \
	 X"$as_dir" : 'X\(/\)' \| . 2>/dev/null ||
echo X"$as_dir" |
    sed '/^X\(.*[^/]\)\/\/*[^/][^/]*\/*$/{
	    s//\1/
	    q
	  }
	  /^X\(\/\/\)[^/].*/{
	    s//\1/
	    q
	  }
	  /^X\(\/\/\)$/{
	    s//\1/
	    q
	  }
	  /^X\(\/\).*/{
	    s//\1/
	    q
	  }
	  s/.*/./; q'`
      test -d "$as_dir" && break
    done
    test -z "$as_dirs" || eval "mkdir $as_dirs"
  } || test -d "$as_dir" || { { echo "$as_me:$LINENO: error: cannot create directory $as_dir" >&5
echo "$as_me: error: cannot create directory $as_dir" >&2;}
   { (exit 1); exit 1; }; }; }
    # echo "creating $dirpart/$file"
    echo '# dummy' > "$dirpart/$file"
  done
done
 ;;

  esac
done # for ac_tag


{ (exit 0); exit 0; }
_ACEOF
chmod +x $CONFIG_STATUS
ac_clean_files=$ac_clean_files_save


# configure is writing to config.log, and then calls config.status.
# config.status does its own redirection, appending to config.log.
# Unfortunately, on DOS this fails, as config.log is still kept open
# by configure, so config.status won't be able to write to it; its
# output is simply discarded.  So we exec the FD to /dev/null,
# effectively closing config.log, so it can be properly (re)opened and
# appended to by config.status.  When coming back to configure, we
# need to make the FD available again.
if test "$no_create" != yes; then
  ac_cs_success=:
  ac_config_status_args=
  test "$silent" = yes &&
    ac_config_status_args="$ac_config_status_args --quiet"
  exec 5>/dev/null
  $SHELL $CONFIG_STATUS $ac_config_status_args || ac_cs_success=false
  exec 5>>config.log
  # Use ||, not &&, to avoid exiting from the if with $? = 1, which
  # would make configure fail if this is the last instruction.
  $ac_cs_success || { (exit 1); exit 1; }
fi



==> install-sh <==
#!/bin/sh
# install - install a program, script, or datafile

scriptversion=2006-12-25.00

# This originates from X11R5 (mit/util/scripts/install.sh), which was
# later released in X11R6 (xc/config/util/install.sh) with the
# following copyright and license.
#
# Copyright (C) 1994 X Consortium
#
# Permission is hereby granted, free of charge, to any person obtaining a copy
# of this software and associated documentation files (the "Software"), to
# deal in the Software without restriction, including without limitation the
# rights to use, copy, modify, merge, publish, distribute, sublicense, and/or
# sell copies of the Software, and to permit persons to whom the Software is
# furnished to do so, subject to the following conditions:
#
# The above copyright notice and this permission notice shall be included in
# all copies or substantial portions of the Software.
#
# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND, EXPRESS OR
# IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF MERCHANTABILITY,
# FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT.  IN NO EVENT SHALL THE
# X CONSORTIUM BE LIABLE FOR ANY CLAIM, DAMAGES OR OTHER LIABILITY, WHETHER IN
# AN ACTION OF CONTRACT, TORT OR OTHERWISE, ARISING FROM, OUT OF OR IN CONNEC-
# TION WITH THE SOFTWARE OR THE USE OR OTHER DEALINGS IN THE SOFTWARE.
#
# Except as contained in this notice, the name of the X Consortium shall not
# be used in advertising or otherwise to promote the sale, use or other deal-
# ings in this Software without prior written authorization from the X Consor-
# tium.
#
#
# FSF changes to this file are in the public domain.
#
# Calling this script install-sh is preferred over install.sh, to prevent
# `make' implicit rules from creating a file called install from it
# when there is no Makefile.
#
# This script is compatible with the BSD install script, but was written
# from scratch.

nl='
'
IFS=" ""	$nl"

# set DOITPROG to echo to test this script

# Don't use :- since 4.3BSD and earlier shells don't like it.
doit=${DOITPROG-}
if test -z "$doit"; then
  doit_exec=exec
else
  doit_exec=$doit
fi

# Put in absolute file names if you don't have them in your path;
# or use environment vars.

chgrpprog=${CHGRPPROG-chgrp}
chmodprog=${CHMODPROG-chmod}
chownprog=${CHOWNPROG-chown}
cmpprog=${CMPPROG-cmp}
cpprog=${CPPROG-cp}
mkdirprog=${MKDIRPROG-mkdir}
mvprog=${MVPROG-mv}
rmprog=${RMPROG-rm}
stripprog=${STRIPPROG-strip}

posix_glob='?'
initialize_posix_glob='
  test "$posix_glob" != "?" || {
    if (set -f) 2>/dev/null; then
      posix_glob=
    else
      posix_glob=:
    fi
  }
'

posix_mkdir=

# Desired mode of installed file.
mode=0755

chgrpcmd=
chmodcmd=$chmodprog
chowncmd=
mvcmd=$mvprog
rmcmd="$rmprog -f"
stripcmd=

src=
dst=
dir_arg=
dst_arg=

copy_on_change=false
no_target_directory=

usage="\
Usage: $0 [OPTION]... [-T] SRCFILE DSTFILE
   or: $0 [OPTION]... SRCFILES... DIRECTORY
   or: $0 [OPTION]... -t DIRECTORY SRCFILES...
   or: $0 [OPTION]... -d DIRECTORIES...

In the 1st form, copy SRCFILE to DSTFILE.
In the 2nd and 3rd, copy all SRCFILES to DIRECTORY.
In the 4th, create DIRECTORIES.

Options:
     --help     display this help and exit.
     --version  display version info and exit.

  -c            (ignored)
  -C            install only if different (preserve the last data modification time)
  -d            create directories instead of installing files.
  -g GROUP      $chgrpprog installed files to GROUP.
  -m MODE       $chmodprog installed files to MODE.
  -o USER       $chownprog installed files to USER.
  -s            $stripprog installed files.
  -t DIRECTORY  install into DIRECTORY.
  -T            report an error if DSTFILE is a directory.

Environment variables override the default commands:
  CHGRPPROG CHMODPROG CHOWNPROG CMPPROG CPPROG MKDIRPROG MVPROG
  RMPROG STRIPPROG
"

while test $# -ne 0; do
  case $1 in
    -c) ;;

    -C) copy_on_change=true;;

    -d) dir_arg=true;;

    -g) chgrpcmd="$chgrpprog $2"
	shift;;

    --help) echo "$usage"; exit $?;;

    -m) mode=$2
	case $mode in
	  *' '* | *'	'* | *'
'*	  | *'*'* | *'?'* | *'['*)
	    echo "$0: invalid mode: $mode" >&2
	    exit 1;;
	esac
	shift;;

    -o) chowncmd="$chownprog $2"
	shift;;

    -s) stripcmd=$stripprog;;

    -t) dst_arg=$2
	shift;;

    -T) no_target_directory=true;;

    --version) echo "$0 $scriptversion"; exit $?;;

    --)	shift
	break;;

    -*)	echo "$0: invalid option: $1" >&2
	exit 1;;

    *)  break;;
  esac
  shift
done

if test $# -ne 0 && test -z "$dir_arg$dst_arg"; then
  # When -d is used, all remaining arguments are directories to create.
  # When -t is used, the destination is already specified.
  # Otherwise, the last argument is the destination.  Remove it from $@.
  for arg
  do
    if test -n "$dst_arg"; then
      # $@ is not empty: it contains at least $arg.
      set fnord "$@" "$dst_arg"
      shift # fnord
    fi
    shift # arg
    dst_arg=$arg
  done
fi

if test $# -eq 0; then
  if test -z "$dir_arg"; then
    echo "$0: no input file specified." >&2
    exit 1
  fi
  # It's OK to call `install-sh -d' without argument.
  # This can happen when creating conditional directories.
  exit 0
fi

if test -z "$dir_arg"; then
  trap '(exit $?); exit' 1 2 13 15

  # Set umask so as not to create temps with too-generous modes.
  # However, 'strip' requires both read and write access to temps.
  case $mode in
    # Optimize common cases.
    *644) cp_umask=133;;
    *755) cp_umask=22;;

    *[0-7])
      if test -z "$stripcmd"; then
	u_plus_rw=
      else
	u_plus_rw='% 200'
      fi
      cp_umask=`expr '(' 777 - $mode % 1000 ')' $u_plus_rw`;;
    *)
      if test -z "$stripcmd"; then
	u_plus_rw=
      else
	u_plus_rw=,u+rw
      fi
      cp_umask=$mode$u_plus_rw;;
  esac
fi

for src
do
  # Protect names starting with `-'.
  case $src in
    -*) src=./$src;;
  esac

  if test -n "$dir_arg"; then
    dst=$src
    dstdir=$dst
    test -d "$dstdir"
    dstdir_status=$?
  else

    # Waiting for this to be detected by the "$cpprog $src $dsttmp" command
    # might cause directories to be created, which would be especially bad
    # if $src (and thus $dsttmp) contains '*'.
    if test ! -f "$src" && test ! -d "$src"; then
      echo "$0: $src does not exist." >&2
      exit 1
    fi

    if test -z "$dst_arg"; then
      echo "$0: no destination specified." >&2
      exit 1
    fi

    dst=$dst_arg
    # Protect names starting with `-'.
    case $dst in
      -*) dst=./$dst;;
    esac

    # If destination is a directory, append the input filename; won't work
    # if double slashes aren't ignored.
    if test -d "$dst"; then
      if test -n "$no_target_directory"; then
	echo "$0: $dst_arg: Is a directory" >&2
	exit 1
      fi
      dstdir=$dst
      dst=$dstdir/`basename "$src"`
      dstdir_status=0
    else
      # Prefer dirname, but fall back on a substitute if dirname fails.
      dstdir=`
	(dirname "$dst") 2>/dev/null ||
	expr X"$dst" : 'X\(.*[^/]\)//*[^/][^/]*/*$' \| \
	     X"$dst" : 'X\(//\)[^/]' \| \
	     X"$dst" : 'X\(//\)$' \| \
	     X"$dst" : 'X\(/\)' \| . 2>/dev/null ||
	echo X"$dst" |
	    sed '/^X\(.*[^/]\)\/\/*[^/][^/]*\/*$/{
		   s//\1/
		   q
		 }
		 /^X\(\/\/\)[^/].*/{
		   s//\1/
		   q
		 }
		 /^X\(\/\/\)$/{
		   s//\1/
		   q
		 }
		 /^X\(\/\).*/{
		   s//\1/
		   q
		 }
		 s/.*/./; q'
      `

      test -d "$dstdir"
      dstdir_status=$?
    fi
  fi

  obsolete_mkdir_used=false

  if test $dstdir_status != 0; then
    case $posix_mkdir in
      '')
	# Create intermediate dirs using mode 755 as modified by the umask.
	# This is like FreeBSD 'install' as of 1997-10-28.
	umask=`umask`
	case $stripcmd.$umask in
	  # Optimize common cases.
	  *[2367][2367]) mkdir_umask=$umask;;
	  .*0[02][02] | .[02][02] | .[02]) mkdir_umask=22;;

	  *[0-7])
	    mkdir_umask=`expr $umask + 22 \
	      - $umask % 100 % 40 + $umask % 20 \
	      - $umask % 10 % 4 + $umask % 2
	    `;;
	  *) mkdir_umask=$umask,go-w;;
	esac

	# With -d, create the new directory with the user-specified mode.
	# Otherwise, rely on $mkdir_umask.
	if test -n "$dir_arg"; then
	  mkdir_mode=-m$mode
	else
	  mkdir_mode=
	fi

	posix_mkdir=false
	case $umask in
	  *[123567][0-7][0-7])
	    # POSIX mkdir -p sets u+wx bits regardless of umask, which
	    # is incompatible with FreeBSD 'install' when (umask & 300) != 0.
	    ;;
	  *)
	    tmpdir=${TMPDIR-/tmp}/ins$RANDOM-$$
	    trap 'ret=$?; rmdir "$tmpdir/d" "$tmpdir" 2>/dev/null; exit $ret' 0

	    if (umask $mkdir_umask &&
		exec $mkdirprog $mkdir_mode -p -- "$tmpdir/d") >/dev/null 2>&1
	    then
	      if test -z "$dir_arg" || {
		   # Check for POSIX incompatibilities with -m.
		   # HP-UX 11.23 and IRIX 6.5 mkdir -m -p sets group- or
		   # other-writeable bit of parent directory when it shouldn't.
		   # FreeBSD 6.1 mkdir -m -p sets mode of existing directory.
		   ls_ld_tmpdir=`ls -ld "$tmpdir"`
		   case $ls_ld_tmpdir in
		     d????-?r-*) different_mode=700;;
		     d????-?--*) different_mode=755;;
		     *) false;;
		   esac &&
		   $mkdirprog -m$different_mode -p -- "$tmpdir" && {
		     ls_ld_tmpdir_1=`ls -ld "$tmpdir"`
		     test "$ls_ld_tmpdir" = "$ls_ld_tmpdir_1"
		   }
		 }
	      then posix_mkdir=:
	      fi
	      rmdir "$tmpdir/d" "$tmpdir"
	    else
	      # Remove any dirs left behind by ancient mkdir implementations.
	      rmdir ./$mkdir_mode ./-p ./-- 2>/dev/null
	    fi
	    trap '' 0;;
	esac;;
    esac

    if
      $posix_mkdir && (
	umask $mkdir_umask &&
	$doit_exec $mkdirprog $mkdir_mode -p -- "$dstdir"
      )
    then :
    else

      # The umask is ridiculous, or mkdir does not conform to POSIX,
      # or it failed possibly due to a race condition.  Create the
      # directory the slow way, step by step, checking for races as we go.

      case $dstdir in
	/*) prefix='/';;
	-*) prefix='./';;
	*)  prefix='';;
      esac

      eval "$initialize_posix_glob"

      oIFS=$IFS
      IFS=/
      $posix_glob set -f
      set fnord $dstdir
      shift
      $posix_glob set +f
      IFS=$oIFS

      prefixes=

      for d
      do
	test -z "$d" && continue

	prefix=$prefix$d
	if test -d "$prefix"; then
	  prefixes=
	else
	  if $posix_mkdir; then
	    (umask=$mkdir_umask &&
	     $doit_exec $mkdirprog $mkdir_mode -p -- "$dstdir") && break
	    # Don't fail if two instances are running concurrently.
	    test -d "$prefix" || exit 1
	  else
	    case $prefix in
	      *\'*) qprefix=`echo "$prefix" | sed "s/'/'\\\\\\\\''/g"`;;
	      *) qprefix=$prefix;;
	    esac
	    prefixes="$prefixes '$qprefix'"
	  fi
	fi
	prefix=$prefix/
      done

      if test -n "$prefixes"; then
	# Don't fail if two instances are running concurrently.
	(umask $mkdir_umask &&
	 eval "\$doit_exec \$mkdirprog $prefixes") ||
	  test -d "$dstdir" || exit 1
	obsolete_mkdir_used=true
      fi
    fi
  fi

  if test -n "$dir_arg"; then
    { test -z "$chowncmd" || $doit $chowncmd "$dst"; } &&
    { test -z "$chgrpcmd" || $doit $chgrpcmd "$dst"; } &&
    { test "$obsolete_mkdir_used$chowncmd$chgrpcmd" = false ||
      test -z "$chmodcmd" || $doit $chmodcmd $mode "$dst"; } || exit 1
  else

    # Make a couple of temp file names in the proper directory.
    dsttmp=$dstdir/_inst.$$_
    rmtmp=$dstdir/_rm.$$_

    # Trap to clean up those temp files at exit.
    trap 'ret=$?; rm -f "$dsttmp" "$rmtmp" && exit $ret' 0

    # Copy the file name to the temp name.
    (umask $cp_umask && $doit_exec $cpprog "$src" "$dsttmp") &&

    # and set any options; do chmod last to preserve setuid bits.
    #
    # If any of these fail, we abort the whole thing.  If we want to
    # ignore errors from any of these, just make sure not to ignore
    # errors from the above "$doit $cpprog $src $dsttmp" command.
    #
    { test -z "$chowncmd" || $doit $chowncmd "$dsttmp"; } &&
    { test -z "$chgrpcmd" || $doit $chgrpcmd "$dsttmp"; } &&
    { test -z "$stripcmd" || $doit $stripcmd "$dsttmp"; } &&
    { test -z "$chmodcmd" || $doit $chmodcmd $mode "$dsttmp"; } &&

    # If -C, don't bother to copy if it wouldn't change the file.
    if $copy_on_change &&
       old=`LC_ALL=C ls -dlL "$dst"	2>/dev/null` &&
       new=`LC_ALL=C ls -dlL "$dsttmp"	2>/dev/null` &&

       eval "$initialize_posix_glob" &&
       $posix_glob set -f &&
       set X $old && old=:$2:$4:$5:$6 &&
       set X $new && new=:$2:$4:$5:$6 &&
       $posix_glob set +f &&

       test "$old" = "$new" &&
       $cmpprog "$dst" "$dsttmp" >/dev/null 2>&1
    then
      rm -f "$dsttmp"
    else
      # Rename the file to the real destination.
      $doit $mvcmd -f "$dsttmp" "$dst" 2>/dev/null ||

      # The rename failed, perhaps because mv can't rename something else
      # to itself, or perhaps because mv is so ancient that it does not
      # support -f.
      {
	# Now remove or move aside any old file at destination location.
	# We try this two ways since rm can't unlink itself on some
	# systems and the destination file might be busy for other
	# reasons.  In this case, the final cleanup might fail but the new
	# file should still install successfully.
	{
	  test ! -f "$dst" ||
	  $doit $rmcmd -f "$dst" 2>/dev/null ||
	  { $doit $mvcmd -f "$dst" "$rmtmp" 2>/dev/null &&
	    { $doit $rmcmd -f "$rmtmp" 2>/dev/null; :; }
	  } ||
	  { echo "$0: cannot unlink or rename $dst" >&2
	    (exit 1); exit 1
	  }
	} &&

	# Now rename the file to the real destination.
	$doit $mvcmd "$dsttmp" "$dst"
      }
    fi || exit 1

    trap '' 0
  fi
done

# Local variables:
# eval: (add-hook 'write-file-hooks 'time-stamp)
# time-stamp-start: "scriptversion="
# time-stamp-format: "%:y-%02m-%02d.%02H"
# time-stamp-end: "$"
# End:


==> missing <==
#! /bin/sh
# Common stub for a few missing GNU programs while installing.

scriptversion=2006-05-10.23

# Copyright (C) 1996, 1997, 1999, 2000, 2002, 2003, 2004, 2005, 2006
#   Free Software Foundation, Inc.
# Originally by Fran,cois Pinard <pinard@iro.umontreal.ca>, 1996.

# This program is free software; you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation; either version 2, or (at your option)
# any later version.

# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.

# You should have received a copy of the GNU General Public License
# along with this program; if not, write to the Free Software
# Foundation, Inc., 51 Franklin Street, Fifth Floor, Boston, MA
# 02110-1301, USA.

# As a special exception to the GNU General Public License, if you
# distribute this file as part of a program that contains a
# configuration script generated by Autoconf, you may include it under
# the same distribution terms that you use for the rest of that program.

if test $# -eq 0; then
  echo 1>&2 "Try \`$0 --help' for more information"
  exit 1
fi

run=:
sed_output='s/.* --output[ =]\([^ ]*\).*/\1/p'
sed_minuso='s/.* -o \([^ ]*\).*/\1/p'

# In the cases where this matters, `missing' is being run in the
# srcdir already.
if test -f configure.ac; then
  configure_ac=configure.ac
else
  configure_ac=configure.in
fi

msg="missing on your system"

case $1 in
--run)
  # Try to run requested program, and just exit if it succeeds.
  run=
  shift
  "$@" && exit 0
  # Exit code 63 means version mismatch.  This often happens
  # when the user try to use an ancient version of a tool on
  # a file that requires a minimum version.  In this case we
  # we should proceed has if the program had been absent, or
  # if --run hadn't been passed.
  if test $? = 63; then
    run=:
    msg="probably too old"
  fi
  ;;

  -h|--h|--he|--hel|--help)
    echo "\
$0 [OPTION]... PROGRAM [ARGUMENT]...

Handle \`PROGRAM [ARGUMENT]...' for when PROGRAM is missing, or return an
error status if there is no known handling for PROGRAM.

Options:
  -h, --help      display this help and exit
  -v, --version   output version information and exit
  --run           try to run the given command, and emulate it if it fails

Supported PROGRAM values:
  aclocal      touch file \`aclocal.m4'
  autoconf     touch file \`configure'
  autoheader   touch file \`config.h.in'
  autom4te     touch the output file, or create a stub one
  automake     touch all \`Makefile.in' files
  bison        create \`y.tab.[ch]', if possible, from existing .[ch]
  flex         create \`lex.yy.c', if possible, from existing .c
  help2man     touch the output file
  lex          create \`lex.yy.c', if possible, from existing .c
  makeinfo     touch the output file
  tar          try tar, gnutar, gtar, then tar without non-portable flags
  yacc         create \`y.tab.[ch]', if possible, from existing .[ch]

Send bug reports to <bug-automake@gnu.org>."
    exit $?
    ;;

  -v|--v|--ve|--ver|--vers|--versi|--versio|--version)
    echo "missing $scriptversion (GNU Automake)"
    exit $?
    ;;

  -*)
    echo 1>&2 "$0: Unknown \`$1' option"
    echo 1>&2 "Try \`$0 --help' for more information"
    exit 1
    ;;

esac

# Now exit if we have it, but it failed.  Also exit now if we
# don't have it and --version was passed (most likely to detect
# the program).
case $1 in
  lex|yacc)
    # Not GNU programs, they don't have --version.
    ;;

  tar)
    if test -n "$run"; then
       echo 1>&2 "ERROR: \`tar' requires --run"
       exit 1
    elif test "x$2" = "x--version" || test "x$2" = "x--help"; then
       exit 1
    fi
    ;;

  *)
    if test -z "$run" && ($1 --version) > /dev/null 2>&1; then
       # We have it, but it failed.
       exit 1
    elif test "x$2" = "x--version" || test "x$2" = "x--help"; then
       # Could not run --version or --help.  This is probably someone
       # running `$TOOL --version' or `$TOOL --help' to check whether
       # $TOOL exists and not knowing $TOOL uses missing.
       exit 1
    fi
    ;;
esac

# If it does not exist, or fails to run (possibly an outdated version),
# try to emulate it.
case $1 in
  aclocal*)
    echo 1>&2 "\
WARNING: \`$1' is $msg.  You should only need it if
         you modified \`acinclude.m4' or \`${configure_ac}'.  You might want
         to install the \`Automake' and \`Perl' packages.  Grab them from
         any GNU archive site."
    touch aclocal.m4
    ;;

  autoconf)
    echo 1>&2 "\
WARNING: \`$1' is $msg.  You should only need it if
         you modified \`${configure_ac}'.  You might want to install the
         \`Autoconf' and \`GNU m4' packages.  Grab them from any GNU
         archive site."
    touch configure
    ;;

  autoheader)
    echo 1>&2 "\
WARNING: \`$1' is $msg.  You should only need it if
         you modified \`acconfig.h' or \`${configure_ac}'.  You might want
         to install the \`Autoconf' and \`GNU m4' packages.  Grab them
         from any GNU archive site."
    files=`sed -n 's/^[ ]*A[CM]_CONFIG_HEADER(\([^)]*\)).*/\1/p' ${configure_ac}`
    test -z "$files" && files="config.h"
    touch_files=
    for f in $files; do
      case $f in
      *:*) touch_files="$touch_files "`echo "$f" |
				       sed -e 's/^[^:]*://' -e 's/:.*//'`;;
      *) touch_files="$touch_files $f.in";;
      esac
    done
    touch $touch_files
    ;;

  automake*)
    echo 1>&2 "\
WARNING: \`$1' is $msg.  You should only need it if
         you modified \`Makefile.am', \`acinclude.m4' or \`${configure_ac}'.
         You might want to install the \`Automake' and \`Perl' packages.
         Grab them from any GNU archive site."
    find . -type f -name Makefile.am -print |
	   sed 's/\.am$/.in/' |
	   while read f; do touch "$f"; done
    ;;

  autom4te)
    echo 1>&2 "\
WARNING: \`$1' is needed, but is $msg.
         You might have modified some files without having the
         proper tools for further handling them.
         You can get \`$1' as part of \`Autoconf' from any GNU
         archive site."

    file=`echo "$*" | sed -n "$sed_output"`
    test -z "$file" && file=`echo "$*" | sed -n "$sed_minuso"`
    if test -f "$file"; then
	touch $file
    else
	test -z "$file" || exec >$file
	echo "#! /bin/sh"
	echo "# Created by GNU Automake missing as a replacement of"
	echo "#  $ $@"
	echo "exit 0"
	chmod +x $file
	exit 1
    fi
    ;;

  bison|yacc)
    echo 1>&2 "\
WARNING: \`$1' $msg.  You should only need it if
         you modified a \`.y' file.  You may need the \`Bison' package
         in order for those modifications to take effect.  You can get
         \`Bison' from any GNU archive site."
    rm -f y.tab.c y.tab.h
    if test $# -ne 1; then
        eval LASTARG="\${$#}"
	case $LASTARG in
	*.y)
	    SRCFILE=`echo "$LASTARG" | sed 's/y$/c/'`
	    if test -f "$SRCFILE"; then
	         cp "$SRCFILE" y.tab.c
	    fi
	    SRCFILE=`echo "$LASTARG" | sed 's/y$/h/'`
	    if test -f "$SRCFILE"; then
	         cp "$SRCFILE" y.tab.h
	    fi
	  ;;
	esac
    fi
    if test ! -f y.tab.h; then
	echo >y.tab.h
    fi
    if test ! -f y.tab.c; then
	echo 'main() { return 0; }' >y.tab.c
    fi
    ;;

  lex|flex)
    echo 1>&2 "\
WARNING: \`$1' is $msg.  You should only need it if
         you modified a \`.l' file.  You may need the \`Flex' package
         in order for those modifications to take effect.  You can get
         \`Flex' from any GNU archive site."
    rm -f lex.yy.c
    if test $# -ne 1; then
        eval LASTARG="\${$#}"
	case $LASTARG in
	*.l)
	    SRCFILE=`echo "$LASTARG" | sed 's/l$/c/'`
	    if test -f "$SRCFILE"; then
	         cp "$SRCFILE" lex.yy.c
	    fi
	  ;;
	esac
    fi
    if test ! -f lex.yy.c; then
	echo 'main() { return 0; }' >lex.yy.c
    fi
    ;;

  help2man)
    echo 1>&2 "\
WARNING: \`$1' is $msg.  You should only need it if
	 you modified a dependency of a manual page.  You may need the
	 \`Help2man' package in order for those modifications to take
	 effect.  You can get \`Help2man' from any GNU archive site."

    file=`echo "$*" | sed -n "$sed_output"`
    test -z "$file" && file=`echo "$*" | sed -n "$sed_minuso"`
    if test -f "$file"; then
	touch $file
    else
	test -z "$file" || exec >$file
	echo ".ab help2man is required to generate this page"
	exit 1
    fi
    ;;

  makeinfo)
    echo 1>&2 "\
WARNING: \`$1' is $msg.  You should only need it if
         you modified a \`.texi' or \`.texinfo' file, or any other file
         indirectly affecting the aspect of the manual.  The spurious
         call might also be the consequence of using a buggy \`make' (AIX,
         DU, IRIX).  You might want to install the \`Texinfo' package or
         the \`GNU make' package.  Grab either from any GNU archive site."
    # The file to touch is that specified with -o ...
    file=`echo "$*" | sed -n "$sed_output"`
    test -z "$file" && file=`echo "$*" | sed -n "$sed_minuso"`
    if test -z "$file"; then
      # ... or it is the one specified with @setfilename ...
      infile=`echo "$*" | sed 's/.* \([^ ]*\) *$/\1/'`
      file=`sed -n '
	/^@setfilename/{
	  s/.* \([^ ]*\) *$/\1/
	  p
	  q
	}' $infile`
      # ... or it is derived from the source name (dir/f.texi becomes f.info)
      test -z "$file" && file=`echo "$infile" | sed 's,.*/,,;s,.[^.]*$,,'`.info
    fi
    # If the file does not exist, the user really needs makeinfo;
    # let's fail without touching anything.
    test -f $file || exit 1
    touch $file
    ;;

  tar)
    shift

    # We have already tried tar in the generic part.
    # Look for gnutar/gtar before invocation to avoid ugly error
    # messages.
    if (gnutar --version > /dev/null 2>&1); then
       gnutar "$@" && exit 0
    fi
    if (gtar --version > /dev/null 2>&1); then
       gtar "$@" && exit 0
    fi
    firstarg="$1"
    if shift; then
	case $firstarg in
	*o*)
	    firstarg=`echo "$firstarg" | sed s/o//`
	    tar "$firstarg" "$@" && exit 0
	    ;;
	esac
	case $firstarg in
	*h*)
	    firstarg=`echo "$firstarg" | sed s/h//`
	    tar "$firstarg" "$@" && exit 0
	    ;;
	esac
    fi

    echo 1>&2 "\
WARNING: I can't seem to be able to run \`tar' with the given arguments.
         You may want to install GNU tar or Free paxutils, or check the
         command line arguments."
    exit 1
    ;;

  *)
    echo 1>&2 "\
WARNING: \`$1' is needed, and is $msg.
         You might have modified some files without having the
         proper tools for further handling them.  Check the \`README' file,
         it often tells you about the needed prerequisites for installing
         this package.  You may also peek at any GNU archive site, in case
         some other package would contain this missing \`$1' program."
    exit 1
    ;;
esac

exit 0

# Local variables:
# eval: (add-hook 'write-file-hooks 'time-stamp)
# time-stamp-start: "scriptversion="
# time-stamp-format: "%:y-%02m-%02d.%02H"
# time-stamp-end: "$"
# End:

